Learning Visuo-Motor Behaviours for Robot Locomotion Over Difficult Terrain

As mobile robots become useful performing everyday tasks in complex real-world environments, they must be able to traverse a range of difficult terrain types such as stairs, stepping stones, gaps, jumps and narrow passages. This work investigated traversing these types of environments with a bipedal robot (simulation experiments), and a tracked robot (real world). Developing a traditional monolithic controller for traversing all terrain types is challenging, and for large physical robots realistic test facilities are required and safety must be ensured. An alternative is a suite of simple behaviour controllers that can be composed to achieve complex tasks. This work efficiently trained complex behaviours to enable mobile robots to traverse difficult terrain. By minimising retraining as new behaviours became available, robots were able to traverse increasingly complex terrain sets, leading toward the development of scalable behaviour libraries.

==> alternative/notation.tex <==
% Insert custom \newcommand{}s here


==> examples/maths.tex <==
% Ch3.tex

\chapter[Math Equations]{Math Equations}
\label{cha:cha3}

This chapter shows you how to typeset math equations. We are not going to give a comprehensive description on this topic; but merely demonstrate this through some examples. 

Several sections of this chapter are directly taken from our paper \citep{TianPLA07}. We are not going to cite this paper everywhere in this chapter. However, keep in mind that the majority of the materials shown below come from this paper. 



%===========================
\section{Theoretical Background of Time Series Analysis}
\label{sec:theory}
%---------------
\subsection{R/S Analysis}

Denote the dynamics of the network traffic shown in Figure
\ref{fig:DelayS} as $x=\{x_k\}_{k=1}^N$, where $N$ is the length
of the sequence. This sequence can be treated as fractal records
in time. Hurst invented the $R/S$ analysis method to study such
sequences. Later, Mandelbrot and
Feder further developed this method in fractal
theory.

\begin{figure}[htb!]
\begin{center}
	\includegraphics[scale=0.48]{./DelayS.eps}
%	\includegraphics[scale=0.39]{./Part3NCS/ComplexNet/images/DelayDist.eps}
\end{center}
	\caption[Sensor-to-controller delay]{Sensor-to-controller delay.}
	\label{fig:DelayS}
\end{figure}


For any fractal records in time $x=\{x_k\}_{k=1}^N$ and any $2\le n\le N$,
define
%
\begin{equation} <x>_{n}=\frac{1}{n}\sum_{i=1}^{n}x_i \end{equation}
%
\begin{equation} X(i,n)=\sum_{u=1}^i[x_u-<x>_{n}] \end{equation}
%
\begin{equation} R(n)=\max_{1\le i\le n}X(i,n)-\min_{1\le i\le n}X(i,n) \end{equation}
%
\begin{equation} S(n)=[\frac{1}{n}\sum_{i=1}^{n}(x_i-<x>_{n})^2]^{1/2} \end{equation}

Hurst found that
%
\begin{equation} R(n)/S(n) \ \sim\ (\frac{n}{2})^H \end{equation}
where $H$ is called the {\it Hurst exponent}.

As $n$ changes from $m$ to $N$, we obtain $N-m+1$ points
in $\ln(n)$ v.s. $\displaystyle{\ln(R(n) \over S(n))}$
 plane. Then, we can calculate the Hurst exponent for the time series
using the least-square linear fit.

The Hurst exponent is usually used as a measure of complexity.
The trajectory
of the record is a curve with a fractal dimension $D=2-H$. Hence
a smaller $H$ means a more complex system.
When applied to fractional Brownian motion, if $H > \displaystyle{1 \over 2}$,
the system is said to be {\em  persistent}, which means that if
for a given time period $t$ the motion is along one direction,
then in the time succeeding $t$ it is more likely that the motion
will follow the same direction. For a system with $H < \displaystyle{1 \over 2}$,
the opposite holds, that is, the system is 
{\em antipersistent}. But when $H=\displaystyle{1 \over 2}$
the system produces Brownian motion, which is random.

==> examples/tables.tex <==
% Ch4.tex

\chapter[Demonstration of Tables]{Demonstration of Tables}
\label{cha:cha4}

This is Chapter \ref{cha:cha4}. We will demonstrate how to present results in tables. It is not difficult but need to practice. 

The materials shown below is taken from my own PhD thesis. For simplicity, I do not cite any reference here. 


%-------------------------
\section[Task Decomposition with Fixed Periods]{Task Decomposition with Fixed Control Periods}

To employ the hierarchical feedback scheduling proposed in this work, we first develop a new task model in which each of the original six control tasks is decomposed into two subtasks: data acquisition and QoC evaluation, and control computation and output. Without loss of the generality, the settings of the decomposed tasks and their priorities are shown in Table \ref{tab:taskmodel}. 

\begin{table}[htb!]
\setlength{\abovecaptionskip}{0.10\baselineskip plus 0.01\baselineskip minus 0.01\baselineskip}
\begin{center}
\caption[Task model in the case studies]{Task model in the case studies. Top level scheduler task T$_0$. Sampling and control task set T$_i = T_{i1}\bigcup T_{i2}$, $i = 1, 2, \cdots, 6$. Control periods are the same as those in Table ...(omitted...). Priority levels are valid only for FP scheduling.}
\label{tab:taskmodel}
\begin{tabular}{lcccccc}
\hline
Settings & {$G_1(s)$} & {$G_2(s)$} & {$G_3(s)$} & {$G_4(s)$} & {$G_5(s)$} & {$G_6(s)$}\\
 & T$_{11}$, T$_{12}$ & T$_{21}$, T$_{22}$ & T$_{31}$, T$_{32}$ & T$_{41}$, T$_{42}$ & T$_{51}$, T$_{52}$ & T$_{61}$, T$_{62}$\\
 \hline
 Priority & 2, 8 & 3, 9 & 4, 10 & 5, 11 & 6, 12 & 7, 13\\
 Period (ms) & {0.8 - 2.0} & {1.0 - 2.5} & {1.0 - 2.5} & {1.2 - 3.0} & {1.2 - 3.0} & {1.5 - 3.8}\\
 \hline
\multicolumn{7}{l}{Top level scheduler task T$_0$ with the highest priority of 1.}\\
\multicolumn{7}{l}{Execution times c$_{0} = 10\mu$s; c$_{i1} = 50\mu$s and c$_{i2}=250\mu$s, $i = 1, 2, \cdots, 6$.}\\
\multicolumn{7}{l}{Deadlines $d_{0} = 1$ms; $d_{i1}$ and $d_{i2}$, $i = 1, 2, \cdots, 6$, are calculated using Eqn. (...omitted...).}\\
\multicolumn{7}{l}{Other Settings: $\Delta_H = 0.05; \Delta_L = 0.01, \epsilon = 0.9, U_{sp} = 0.92, N_{rqsp}=5$.}\\
\hline
\end{tabular}
\end{center}
\end{table}

We have tested the new task model, in which the original six tasks are decomposed into twelve subtasks, under fixed task periods and FP.

%======================
\section{More Results}

More results are omitted here......

==> nomenclature.tex <==
% nomenclature

%\newenvironment{nomenc}{\prefacesection{Nomenclature}}{}

%\chapter*{Nomenclature}
%\addcontentsline{toc}{chapter}{Nomenclature}
% Acronyms
%\begin{nomenc}
{
\renewcommand{\arraystretch}{1.2} 
\begin{longtable}{llr}
\multicolumn{3}{l}{\textbf{Abbreviations}\hspace{0.4\textwidth}~~}\\
ACRA & Australasian Conference on Robotics and Automation \\
APF & Artificial Potential Fields \\
AsDDPG & Assisted Deep Deterministic Policy Gradient \\
ATR & All Terrain Robot \\
AWR & Advantage Weighted Regression \\
CL & Curriculum Learning\\
CNN & Convolutional Neural Network \\
CNP & Critical Navigation Point \\
CoM & Centre of Mass\\
CP & Capture Point \\
CSIRO & Commonwealth Scientific and Industrial Research Organisation \\
DARPA & Defense Advanced Research Projects Agency \\
DCM & Divergent Component of Motion \\
DMP & Dynamic Movement Primitive \\
DNN & Deep Neural Network \\
DoA & Domain of Attraction \\
DoF & Degree of Freedom \\
DQN & Deep Q Network \\
DRL & Deep Reinforcement Learning \\
GAE & General Advantage Estimation \\
GCL & Guided Curriculum Learning\\
HMMs & Hidden Markov Models \\
HRL & Hierarchical Reinforcement Learning \\
IROS & IEEE International Conference on Intelligent Robots and Systems \\
MCP & Multiplicative Compositional Policies \\
MDP & Markov Decision Process \\
PD & Proportional Derivative \\
PPO & Proximal Policy Optimisation \\
PRM & Probabilistic Roadmap \\
RA-L & IEEE Robotics and Automation Letters \\
RoA & Region of Attraction \\
RRT & Rapidly-exploring Random Tree \\
SAC & Soft Actor-Critic \\
SLAM & Simultaneous Localisation and Mapping \\
TD & Temporal Difference \\
TRPO & Trust Region Policy Optimisation \\
V-MPO & Value Maximum a Posteriori Policy Optimization \\
VFH & Vector Field Histogram \\
ZMP & Zero Moment Point\\
\end{longtable}
}

%\end{nomenc}


==> old/Ch2LiteratureReview_old.tex <==

% A behaviour was developed for An efficient method for guiding the robot towards a target behaviour with an intermediate controller was developed for behaviours without a reliable overlap

%  Behaviour-based control allows the extensibility of robot capabilities, new behaviours can be included as they become available. 

% The sources of sim-to-real disparity were discussed for improvement in future work.

% the states that exist on the transition border between sequential behaviours are not easily determined.

% switching or transitioning between sequential behaviours is challenging. 
% 
% resulting in policies that are incorporated into a larger behaviour library. 


% Finally, behaviours and behaviours switching trained in simulation were transferred to a real tracked robot required to pass through narrow gaps. The tracked robot uses several pre-existing hand designed behaviours, and the learned behaviour was integrated into this control stack, achieving a 40\% success rate with autonomous traversal compared to 0\% with the existing method. The sources of sim-to-real disparity were discussed for improvement in future work. This work allows mobile agents to operate over an increasing set of complex obstacles.


% curriculum learning method a for learning behaviours, 


% where a simpler form of the problem is considered initially, and the difficulty increased as the robot achieves success. 

% Several aspects of behaviour switching were investigated, . including the importance of a state overlap between controllers, considering when the robot is in a suitable state to switch, and learning Setup Policies for safe transition to a target behaviour. Using a large tracked platform, a goal conditioned Behaviour Selection policy was trained that activates a Gap Behaviour when a goal is presented. The effect of training these behaviours in simulation for use in a real world scenario was also explored.


% Behaviours for a dynamic biped were developed in simulation using an efficient three stage curriculum learning method. The robot is required to traverse complex obstacles such as stairs, gaps, hurdles, and steps. It was demonstrated that without a particular stage, the  performance of the system was degraded. The importance of overlapping policies was investigated, and by learning when to switch between these behaviours the agent was able to successfully traverse a randomised sequence of terrain types in 71.4\% of cases, compared to a 0.7\% success rate when policies do not overlap. For sequential behaviours where there are no overlapping states, an efficient method for learning how to guide the robot towards the target behaviour was developed, achieving an 82\% success rate on a difficult jump task (from 51.3\% with the best existing method). Finally, behaviours and behaviours switching trained in simulation were transferred to a real tracked robot required to pass through narrow gaps. The tracked robot uses several pre-existing hand designed behaviours, and the learned behaviour was integrated into this control stack, achieving a 40\% success rate with autonomous traversal compared to 0\% with the existing method. The sources of sim-to-real disparity were discussed for improvement in future work. This work will allow mobile agents to operate over an increasing set of complex obstacles.

% Abstract?
% The challenges of traversing complex terrains with a simulated biped were investigated. For learning single behaviours, the paradigm of curriculum learning (CL) was developed, where a simpler form of the problem is considered initially, and the difficulty was increased as the robot achieves success. Several aspects of behaviour switching were explored, including the importance of a state overlap between controllers, considering when the robot is in a suitable state to switch, and learning Setup Policies for safe transition to a target behaviour. Using a large tracked platform, a goal conditioned Behaviour Selection policy was trained that activates a Gap Behaviour when a goal is presented. The effect of training these behaviours in simulation for use in a real world scenario was also explored.




% The introduction should contain succinct statements encompassing:
% • description of the research problem investigated;
% • overall outcomes of the study;
% • evidence of significance of the study to the discipline;
% • account of key research and/or methods that have informed the study;
% • articulation of the linkages between the research papers and the author’s contribution within
% those works in realising a significant and original contribution to knowledge

% Why is modular control design important, what is the scope of this work?
% Single point per paragraph, should know what that point is from the first sentence

%  where multiple behaviours may be required, however it may be implausible to interact with multiple obstacle types at the same time

% This work experiments with a dynamic biped in simulation, and a large tracked platform in a real world scenario. Bipedal robots offer the capability of covering a similar range of scenarios compared with a human delivery driver. However, these robots are extremely complex, and switching between behaviours must occur with care to prevent damage to the robot or the environment. For mobile platforms with less complexity, such as tracked robots, significant challenges exist when traversing obstacles such as narrow doorways. Robots that rely on coarse occupancy maps have a reduced ability to plan through gaps that are marginally wider than the robot. The complexity is increased in these scenarios when the robot may be required to make contact with the environment to jump over an obstacle, or wiggle through a small gap. Real world scenarios, such as those presented in the DARPA Subterranean challenge, requires behaviour diversity, and highlights the difficulty of developing a single controller for all obstacles a robot may encounter.

% Real world scenarios
% The complexity increases
% Robots that rely on coarse perception
% Biped robots offer
% However these robots are
% But even simpler mobile platforms
% Therefore this work looks at bipeds and tracks.

% Introducing experimental platforms. 

% , and highlighting the difficulty of developing a single controller for all obstacles a robot may encounter. The complexity is increased in scenarios when the robot is required to make contact with the environment (for example to jump over an obstacle, or wiggle through a doorway).

% For simpler mobile platforms with less complexity, such as tracked robots, significant challenges exist when traversing obstacles such as narrow doorways, where traditional path planning algorithms fail.
% The tasks in the SubT provide significant challenges even for mobile platforms with less complexity, such as tracked robots
% Moreover, most of
% real applications utilize wheeled mobile robots with stable
% motion properties

% even for.

% , and when low resolution occupancy maps inhibit planning through gaps marginally wider than the robot.

% wiggle through a small gap


% in an underground environment. 

% The DARPA Subterranean challenge highlights the importance of behaviour diversity.

% Papers: deep mimic, really good biped one (cassie?)?, sequential composition for bipeds? Anymal one? Maybe after lit review

% What is it we have done


% Ch2LiteratureReview.tex


% This will be key to developing general robotic solutions of large behaviour libraries.

% , and setting up a robot for an upcoming behaviour where switching may not be possible.
% for traversing complex obstacles. The common theme is efficiently learning  visuo-motor behaviours,
% and the integration of multiple individual behaviours to create a scalable libraries.. 

% Abstract?
% The challenges of traversing complex terrains with a simulated biped were investigated. For learning single behaviours, the paradigm of curriculum learning (CL) was developed, where a simpler form of the problem is considered initially, and the difficulty was increased as the robot achieves success. Several aspects of behaviour switching were explored, including the importance of a state overlap between controllers, considering when the robot is in a suitable state to switch, and learning Setup Policies for safe transition to a target behaviour. Using a large tracked platform, a goal conditioned Behaviour Selection policy was trained that activates a Gap Behaviour when a goal is presented. The effect of training these behaviours in simulation for use in a real world scenario was also explored.

% Closing remarks to seal the deal




\chapter[Literature Review]{Literature Review}
\label{cha:LiteratureReview}
% TODO:
% - Trim DRL section
% - Trim classical biped section
% - Adding in setup papers - Depending on what Juxi says
% - Add in stragglers better
% - Proof read and send to Juxi.

% Juxi's comments on summary

% ==================================================================
% ------------------------------------------------------------------
% ==================================================================

% In this chapter the relevant literature is discussed within the scope of traversing difficult obstacles with mobile platforms. Methods for developing behaviours for a dynamic bipedal robot is discussed, looking into classical approaches for dynamic control before considering deep reinforcement learning (DRL) methods and curriculum learning (CL). Then the literature is reviewed for behaviour switching, considering the traditional and learning methods for combining controllers. In the final section we discuss the navigation methods that have been used for negotiating small gaps with a mobile robot. We consider the classical and learning methods, as well as relevant simulation to real world techniques found the literature. 

% \cite{zhao_reactive_2021} - Fit this somewhere

% to solve broader problems

% Learning methods have been used for complex tasks such as walking, and for pa complex high degree of freedom (DoF) robots such as bipeds, and for navigation tasks where perception .  Curriculum learning (CL) has improved the efficiency of deep reinforcement learning (DRL) methods, improving learning outcomes in many settings including learning complex locomotion behaviours. In the classical control community, behaviour composition is a mature research area, however, requires the region of attraction (RoA) for each controller to be defined. For controllers where the RoA is not explicitly understood, for example for learned visuo-motor policies, combining behaviours remains challenging. This chapter summarises the existing solutions for robot locomotion and identifies areas of interest for further investigation.

% \section{Designing Behaviours}


% In this section, the literature is reviewed for bipedal walking methods from both a classical and a deep reinforcement learning perspective. Also presented is a summary of curriculum learning methods, with a particular focus on recent implementations for legged platforms traversing complex terrains. 

% \subsubsection{Classical Methods for Designing Walking Behaviours}


% further adding to the complexity of classical systems. 

% [\cite{ching-long_shih_ascending_1999, gong_feedback_2019, xiong_bipedal_2018}]
% There must be many more examples!
% \subsubsection{Learning Methods for Designing Walking Behaviours}
% \subsection{Deep Reinforcement Learning for Bipedal Robots}


% the gradient of the loss becomes zero for values that result from large changes to the policy prediction (i.e. if the actions of the current policy are very different from the old policy we do not want to update too much), the gradient becomes zero (as shown in Fig. \ref{fig:ch2_ppo}).  In the special case where the advantage is negative, and the action from the new policy is more likely than the with the old policy, we are allowed to reverse the update that lead to the bad behaviour. This is shown in the right diagram of \ref{fig:ch2_ppo}. Therefore policy updates remain close to the policy that generated the data.


% There must be many more examples!




% Skills are combined by normalising the value function of each policy, and a new composite policy is trained that is able to perform a set of goal conditioned behaviours. 

% The reward function encourages matching the expert trajectory:

% \begin{equation}
%     r_t^I = w^pr^p_t + w^vr^v_t + w^er^e_t + w^cr^c_t
% \end{equation}

% where $w$ is a tuned weighting for each element, and each element $r_t^{**}$ is defined by:

% \begin{equation}
%     r_t^{**} = \text{exp}[-w^{**}(\sum_{j}||\hat{q}^{**}_t - q^{**}_t||^2)]
% \end{equation}

% where $**$ is one of ${p,v,e,c}$ corresponding to joint position, velocity, end effector position, and CoM position. $j$ refers to each element of $**$ (for example each joint or end effector), $w$ is a tuned weighting, and $\hat{q}$ refers to the reference motion collected using motion capture. 

% In their work, \cite{peng_deepmimic_2018}  first train the agent on flat terrain, then the policy is augmented to include a heightmap to allow the agent to walk up stairs. While learning from motion capture allows for complex behaviours, it requires having demonstrations of the desired behaviour. 

% Should this go in the behaviour composition section? This is a big write up for deep mimic. 

% While learning from motion capture allows for complex behaviours, it requires having demonstrations of the desired behaviour, and requires all behaviours be available during training, which may not be possible as the number of skills are increased and expensive retraining is required as new skills are included. Furthermore, this method relies on a phase variable supplied as additional information to the policy, meaning skills must complete their full action before transitioning to the next skill.

% \cite{merel_hierarchical_2019} train a humanoid to navigate and walk over gaps using an RGB camera. Policies are trained from snippets of motion capture trajectories, and are then stitched together with a high level selection policy. 



% On-policy learning benefits from curriculum learning [\cite{yu_learning_2018, rudin_learning_2021}]


% Other algoritms:  
% Reinforce / DDPG? Anything more recent?
% TRPO: [\cite{hwangbo_learning_2019, lee_robust_2019, lee_learning_quad_2020}]
% On-line is preferable to offline learning when.. 
% Is more simple that soft actor-critic (SAC) [\cite{haarnoja_soft_2018}], twin delayed DDPG (TD3) [\cite{fujimoto_td3_2018}], and value maximum posteriori optimisation (V-MPO) [\cite{Song2020V-MPO}]. 


% DRL has recently demonstrated impressive locomotion policies for robots in simulation [\cite{schulman_proximal_2017, xie_allsteps_2020}] and in real-world tasks [\cite{tan_sim--real_2018, hwangbo_learning_2019}]. DRL behaviours have been developed for highly complex robots for walking over complex terrain [\cite{heess_emergence_2017, xie_allsteps_2020}], performing complex maneuvers replicating motion capture [\cite{peng_deepmimic_2018}], and sim-to-real transfer [\cite{tan_sim--real_2018, rudin_learning_2021}]. DRL has been used with increasing popularity for locomotion through cluttered indoor spaces [\cite{rana_multiplicative_2020}], navigation tasks [\cite{bruce_learning_2018}], and field deployment [\cite{kahn_badgr_2020}]. 


% \noindent\textbf{Deep Reinforcement Learning (DRL):}
% \\

% is given the observed reward and the value estimate of the next state. 

% \begin{equation}
%     A^\pi(s_t, a_t) = Q^\pi(s_t, a_t) - V^\pi(s_t)
% \end{equation}

% where $Q^\pi(s_t) = \mathbb{E}_{\tau \sim \pi}[R(\tau) | s_0 = s_t, a_0 = a_t]$. In practice, PPO uses general advantage estimation (GAE) [\cite{schulman_gae_2016}], to provide a low variance estimate of the advantage $\hat{A}_t$. 

% The bootstrapped estimate of the advantage is given by:

z
% quadruped robot is free to learn an initial walking behaviour, then reward evolution guides the robot towards a more desirable gait throughout training [\cite{hwangbo_learning_2019}]. 



% This work also includes a penalty that encourages symmetrical motions. 

% \begin{equation} 
%     \pi_\theta(s) = \Psi_a(\pi_\theta(\Psi_o(s)))
% \end{equation}

% \begin{equation}
%     L_{sym}(\theta) = \sum^B_{i=0}||\pi_\theta(\mathbf{s_i}) - \Psi(\pi_\theta(\Psi_o(\mathbf{s_i})))||^2
% \end{equation}

% \begin{equation}
%     % \pi_\theta* = \underset{\theta}{\text{argmin}} L_{\text{PPO}(\theta) + w L_{sym}(\theta)}
%     \pi_\theta* = \underset{\theta}{\text{argmin}} L_{\text{PPO}}(\theta) + wL_{sym}(\theta)
% \end{equation}




% Our method combines ideas from \cite{yu_learning_2018}, and \cite{rana_multiplicative_2020}, where we stabilise the robot CoM by applying external forces, and also guide exploration using a simple prior controller applying forces to each joint. We apply these ideas, and increase the difficulty of the terrain, resulting in the traversal of complex terrain artifacts.



% Notes: Visual and mapless navigation are huge fields, and I'm not sure they make sense to add these papers. They are not specific to the gaps problem

% Mapless navigation? Visual navigation, point goal navigation, prm-rl. Navigation in cluttered environments. Imitation learning for autonomous navigation.



% T. Lei, G. Paolo, and M. Liu, “Virtual-to-real deep reinforcement
% learning: Continuous control of mobile robots for mapless navigation,”
% IEEE/RSJ International Conference on Intelligent Robots and Systems
% (IROS), 2017.

% M. Enrico, and A. Farinelli, “Discrete deep reinforcement learning for
% mapless navigation,” IEEE International Conference on Robotics and
% Automation (ICRA), 2020.
% [4] J. Jin, N. Nguyen, N. Sakib, et al., “Mapless navigation among dynam-
% ics with social-safety-awareness: a reinforcement learning approach
% from 2D laser scans,” IEEE IcRa

% ] S. Gupta, J. Davidson, S. Levine, R. Sukthankar, and J. Malik, “Cog-
% nitive mapping and planning for visual navigation,” in Proceedings of
% the IEEE Conference on Computer Vision and Pattern Recognition,
% 2017, pp. 2616–2625.
% [8] K. Fang, A. Toshev, L. Fei-Fei, and S. Savarese, “Scene memory
% transformer for embodied agents in long-horizon tasks,” in Proceed-
% ings of the IEEE/CVF Conference on Computer Vision and Pattern
% Recognition, 2019, pp. 538–547.
% [9] E. Wijmans, A. Kadian, A. Morcos, S. Lee, I. Essa, D. Parikh,
% M. Savva, and D. Batra, “Dd-ppo: Learning near-perfect pointgoal
% navigators from 2.5 billion frames,” arXiv, pp. arXiv–1911, 2019.
% D. S. Chaplot, D. Gandhi, S. Gupta, A. Gupta, and R. Salakhutdi-
% nov, “Learning to explore using active neural slam,” arXiv preprint
% arXiv:2004.05155, 2020.
% [11] A. Francis, A. Faust, H.-T. L. Chiang, J. Hsu, J. C. Kew, M. Fiser,
% and T.-W. E. Lee, “Long-range indoor navigation with prm-rl,” IEEE
% Transactions on Robotics, vol. 36, no. 4, pp. 1115–1134, 2020.
% [12] A. Petrenko, Z. Huang, T. Kumar, G. Sukhatme, and V. Koltun,
% “Sample factory: Egocentric 3d control from pixels at 100000 fps with
% asynchronous reinforcement learning,” in International Conference on
% Machine Learning. PMLR, 2020, pp. 7652–7662.
% [13] D. Hoeller, L. Wellhausen, F. Farshidian, and M. Hutter, “Learning a
% state representation and navigation in cluttered and dynamic environ-
% ments,” IEEE Robotics and Automation Letters, 2021.
% [14] H. Karnan, G. Warnell, X. Xiao, and P. Stone, “Voila: Visual-
% observation-only imitation learning for autonomous navigation,” arXiv
% preprint arXiv:2105.09371, 2021.

% Designing an autonomous navigation system to handle difficult terrain scenarios is challenging. Often a set of behaviours is required, where each behaviour has been tuned to handle a unique situation. 



% \subsubsection{Classical Methods for Robot Navigation}

% Krishan's paper for other methods (Vectore Field Histograms?)
% Vector Field Histograms (VHF) [4] is a real time mo-
% tion planning algorithm that generates a polar histogram to
% represent the polar density of surrounding obstacles. The
% robot’s steering angle is then chosen based on the direction
% exhibiting the least density and cl
% approach, the polar histogram has to be computed at everyoseness to goal. For this
% time step, making it suitable for dynamic obstacle avoidance


% Perception limitations require the robot to make contact with the surface to make progress through tightprevent each of these methods.

% In each of these approaches, the robot does not make contact with the environment.

% , limiting ability to make contact assisted progress through a small gap.

% Manual tuning is a limitation of complex behaviours. Furthermore, in each of these approaches, the robot does not make contact with the environment, limiting its ability to make contact assisted progress through a small gap.
% Next, we review some of the learning methods for autonomous navigation.


% By integrating both methods, the trained policy reduces oscillations caused by the classical controller, and for states not seen in the training data the classical method has priority.
% This limits the use of pre-existing behaviour stacks with learned behaviours that can traverse difficult obstacles.

% In our previous work we introduce the idea of developing behaviours separately [\cite{tidd_guided_2020}], then learning when they should be used, either with a supervised approach [\cite{tidd_learning_2021}], or through reinforcement learning [\cite{tidd_learning_2021-1}]. For our problem we require a behaviour that can learn to perform complex maneuvers (such as make contact with a door), and can be integrated into an existing behaviour stack. 



%  When the learned behaviour exhibits high uncertainty in a given state, the system switches to rely completely on the prior controller. % (for example a skid steer robot over more challenging terrain)
%  Statically stable mobile robots suffer with less sim-to-real disparity than dynamic platforms, whereas actuator latency is a considerable factor in dynamic robots [\cite{tan_sim--real_2018, hwangbo_learning_2019}].

% \textbf{Not sure if we want more literature about the sim-to-real for legs, or is this out of scope} e.g. [\cite{tan_sim--real_2018}], sim-to-real modelling [\cite{hwangbo_learning_2019, peng_learning_2020, rudin_learning_2021}], and heavy dynamics randomisation [\cite{peng_learning_2020}]. \cite{peng_learning_2020} retargets motion capture data from animal reference motions to a robot coordinate frame, and trains a reinforcement learning policy for a quadruped robot to imitate the behaviour. This work applies domain adaption using advantage weighted regression (AWR) [\cite{AWRPeng19}] to showcase the behaviours trained in simulation on the real robot.


% 
% Quadruped and biped sim2real?



% Additionally, with the exception of \cite{xie_learning_2018, rana_residual_2020}, learning methods are not typically integrated with classical methods. 




% Behaviour-based robotics utilises a hierarchy of behaviours, with low-level controllers and a mechanism to determine which behaviour to employ.
% Instead of monolithic controllers, its often common to combine behaviours. 

% Progressive nets and distillation, need to mention these % refine, combine, and compress policies \cite{xie_learning_2020}




% For dynamic controllers, it is not only important to know what behaviour to activate, it is vital that behaviours are selected in such a way that the robot always remains in a stable. We are interested in the latter problem, where sequential behaviours that have little or no overlapping states can be safely integrated to allow the robot to perform tasks that are more complex than any single behaviour. 

% Designing a single policy that can display multiple behaviours is challenging, and often results in the degraded performance of individual behaviours [\cite{lee_robust_2019}]

% \subsection{Classical Methods for Behaviour Selection}

% Need to look at these and slot them in:
% \cite{manchester_2011_regions, matallana_2010_estimation}
% \cite{matallana_2010_estimation} estimate the RoA of 

% The method used involves decomposition of the dynamics about the target cycle into tangential and transverse components, and a search for a Lyapunov function in the transverse dynamics using sum-of-squares analysis (semidefinite programming).


% you need to write more about the current shortcomings as to link it to your work in the papers.

% To ensure stability, it is important to understand when it safe to switch between behaviours.



% n the context of a high dimensional biped traversing complex obstacles using vision.


% Improving the efficiency of training a biped to traverse complex obstacles will be investigated in Chapter \ref{cha:ch3a}. A gap in the literature was found for the specific task of traversing narrow gaps with a mobile robot in the case that doorways are perceived as smaller than the robot in low resolution costmaps. A solution to this problem was investigated in Chapter \ref{cha:ch3b}.

%  may require contact with the environment to squeeze through. Planning methods are often used for navigation, however. A gap in the literature was discovered for small spaces that are marginally wider than the robot, where complex behaviours, such as making contact with the doorway, may be required for traversal.

% No examples in the literature were found where these conditions were present. 

% smaller than the robot footprint in low resolution costmaps


% Sim-to-real



% however examples are required for every behaviour,  the desired behaviour. Furthermore all behaviours need to be available during training, which may not be possible as the number of skills are increased and expensive retraining is required as new skills are included. 

% Furthermore, this method relies on a phase variable supplied as additional information to the policy, meaning skills must complete their full action before transitioning to the next skill.



% While the literature has examples of navigation algorithms used to pass through small gaps, no cases were found for getting through gaps with path planning methods where the gap is marginally wider than the robot (to the degree that perception resolution appears smaller). Learning approaches have shown examples when sensor data can be used directly, for example using a camera or depth sensor. However, for course occupancy maps, where the gap that is larger than the robot may appear smaller in the occupancy map, the robot must make contact with the environment to determine if it can in fact make it through. Chapter \ref{cha:ch5} investigates the challenges of developing a behaviour where the robot is able to make contact with the environment in order to wiggle through. We also consider the challenges that are present in sim-to-real transfer of locomotion policies, and discuss the sources of disparity between the simulation results and those of the robot in the real world.


% In all examples presented, no work considered gaps that are small enough to fall within a margin of error for the perception. The gaps explored are wide enough to be distinguished by the perception system, and no examples describe the requirement of the robot to make contact with a surface in order to get through a small gap. This presents a gap in the literature for small spaces that are marginally wider than the robot, where complex behaviours, such as making contact with the doorway, may be required for traversal. 

% Furthermore, developing a single policy to perform multiple behaviours can degrade the performance of each behaviour [\cite{lee_robust_2019}].


% In many examples from the literature, separate behaviours were combined to create a 

% to increase the capabilities of a robot beyond a single controller. Several works address behaviour composition, where controllers must be switched in a compatible state for the target controller. It is important to understand when it safe to switch between behaviours to improve reliability. Classical methods determine the set of safe states explicitly, however for learned policies it is often difficult to determine these states. 

% For high DoF robots and black box behaviours like neural network policies, it is difficult to know what states are suitable to activate a particular behaviour. While there are examples of learning transition policies when there is little or no overlap between behaviours [\cite{najafi_learning_2016,lee_composing_2019}], for high DoF robots executing complex behaviours there exists a gap in the literature. Chapter \ref{cha:ch4} considers the Chapter \ref{cha:ch5}

% Learned policies usually solve a single task, whereas real-world scenarios may require an agent to perform several tasks.

% , and for new terrains to be added as the behaviours become available. DRL methods optimise a single scalar reward function, and require costly retraining if new tasks are introduced. In a real setting it may be not be possible to train on all scenarios.

% Chapter \ref{cha:ch4} will investigate learning when to switch between policies, and transitioning between behaviours. 

% Chapter \ref{cha:ch5} will show an example of switching that includes a pre-existing library of manually tuned behaviours.

%  where controllers with several levels of abstraction are trained concurrently, and cases where it is beneficial to design separate behaviours and then determine where to activate the appropriate behaviour.

% Locomotion behaviours for traversing difficult obstacles were developed with both classical and learned methods. As the task complexity increases, behaviours become difficult to model with classical methods and learning approaches thrive. Learning methods are notoriously sample inefficient, requiring extensive interaction with the environment, with local minima often preventing the learning of complex behaviours

% Improving the efficiency of learning complex behaviours is investigated in this thesis.
% y, where switching is possible from the RoA of the receiving controller


% Learning methods are particular suited when perception is linked to action in a complex way, however, large numbers of samples are required for training. For complex behaviours it is also challenging to train policies with na\"ive exploration or sparse rewards. Often these policies succumb to local minima or result in overfitting the simulation in unrealistic ways.



% Other work with DRL has shown that expanding the RoA of each primitive with transition policies improves switching [\cite{lee_composing_2019}]. RoA estimation to combine DRL policies is a promising approach to scale the capabilities of legged robots, and is an area of research that requires more investigation.

% Behaviour switching must occur within the RoA of the receiving controller, however when there is no reliable overlap, Separate controllers that occupy different subsets of the state, may not result in stable behaviour if there is no RoA overlap between controllers.

% 
% DeepMimic by \cite{peng_deepmimic_2018} combines pre-trained behaviours learned from motion capture, with reliance on a phase variable to determine when one behaviour has been completed.

% In our previous work [\cite{tidd_learning_2021}], we learn when to switch between low level primitives for a simulated biped by randomly sampling from a collection of behaviours.


% Work by \cite{peng_mcp_2019} combines pre-trained policies using a gating function that learns a multiplicative combination of actsions.
% Our setup policies are also use an intermediate controller, however we show that our method performs more reliably with complex locomotion behaviours.

% Using pre-trained policies requires a suitable handling of transitions between behaviours. \cite{faloutsos_composable_2001} learns pre and post-conditions for each controller, such that switching only occurs when these conditions have been satisfied.  



% where $s=[rs, I]$, and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is the set of states policy $\pi_i$ was designed to operate within (Goal Set or Invariant Set), and $\mathcal{R}(\pi_i)$ is the set of states that will converge to a state in $\mathcal{G}(\pi_i)$. 

Notes:

Acceleration limits of the robot in simulation

Moreover, most of
real applications utilize wheeled mobile robots with stable
motion properties

T. Lei, G. Paolo, and M. Liu, “Virtual-to-real deep reinforcement
learning: Continuous control of mobile robots for mapless navigation,”
IEEE/RSJ International Conference on Intelligent Robots and Systems
(IROS), 2017.

M. Enrico, and A. Farinelli, “Discrete deep reinforcement learning for
mapless navigation,” IEEE International Conference on Robotics and
Automation (ICRA), 2020.
[4] J. Jin, N. Nguyen, N. Sakib, et al., “Mapless navigation among dynam-
ics with social-safety-awareness: a reinforcement learning approach
from 2D laser scans,” IEEE IcRa

] S. Gupta, J. Davidson, S. Levine, R. Sukthankar, and J. Malik, “Cog-
nitive mapping and planning for visual navigation,” in Proceedings of
the IEEE Conference on Computer Vision and Pattern Recognition,
2017, pp. 2616–2625.
[8] K. Fang, A. Toshev, L. Fei-Fei, and S. Savarese, “Scene memory
transformer for embodied agents in long-horizon tasks,” in Proceed-
ings of the IEEE/CVF Conference on Computer Vision and Pattern
Recognition, 2019, pp. 538–547.
[9] E. Wijmans, A. Kadian, A. Morcos, S. Lee, I. Essa, D. Parikh,
M. Savva, and D. Batra, “Dd-ppo: Learning near-perfect pointgoal
navigators from 2.5 billion frames,” arXiv, pp. arXiv–1911, 2019.
D. S. Chaplot, D. Gandhi, S. Gupta, A. Gupta, and R. Salakhutdi-
nov, “Learning to explore using active neural slam,” arXiv preprint
arXiv:2004.05155, 2020.
[11] A. Francis, A. Faust, H.-T. L. Chiang, J. Hsu, J. C. Kew, M. Fiser,
and T.-W. E. Lee, “Long-range indoor navigation with prm-rl,” IEEE
Transactions on Robotics, vol. 36, no. 4, pp. 1115–1134, 2020.
[12] A. Petrenko, Z. Huang, T. Kumar, G. Sukhatme, and V. Koltun,
“Sample factory: Egocentric 3d control from pixels at 100000 fps with
asynchronous reinforcement learning,” in International Conference on
Machine Learning. PMLR, 2020, pp. 7652–7662.
[13] D. Hoeller, L. Wellhausen, F. Farshidian, and M. Hutter, “Learning a
state representation and navigation in cluttered and dynamic environ-
ments,” IEEE Robotics and Automation Letters, 2021.
[14] H. Karnan, G. Warnell, X. Xiao, and P. Stone, “Voila: Visual-
observation-only imitation learning for autonomous navigation,” arXiv
preprint arXiv:2105.09371, 2021.


composing controllers for manipulation:
https://www.youtube.com/watch?v=pC8RbComKP0&t=2s
Jie Tan's work?
RA-L reviews

Go through we's
Juxi's comments on summary

Layout:
- Behaviour design wrt efficiency and visuo-motor policies
    - DRL - PPO
    - Biped - classical and DRL
    - Curriculum
    - Navigation
- Switching behaviours
    - Sequential composition
    - HRL?
- Setup Policies
% ==================================================================
% ------------------------------------------------------------------
% ==================================================================

% In this chapter the relevant literature is discussed within the scope of traversing difficult obstacles with mobile platforms. Methods for developing behaviours for a dynamic bipedal robot is discussed, looking into classical approaches for dynamic control before considering deep reinforcement learning (DRL) methods and curriculum learning (CL). Then the literature is reviewed for behaviour switching, considering the traditional and learning methods for combining controllers. In the final section we discuss the navigation methods that have been used for negotiating small gaps with a mobile robot. We consider the classical and learning methods, as well as relevant simulation to real world techniques found the literature. 

In this chapter, a survey of related literature is presented. For decades classical methods have been used to enable robots to move over complex terrains. In recent years, learning methods have been used with increasing popularity for controlling robots in difficult locomotion tasks requiring visuo-motor policies. Curriculum learning has been shown to improve learning outcomes in many settings, and has been applied to learning for locomotion. In the classical community, combining a set of known behaviours is a well researched area. For controllers that are less well know, hierarchical methods is a relative under explored field of reinforcement learning. This chapter summarises the existing solutions, and identifies areas of interest for further investigation.

\section{Designing Behaviours}

In this section, literature is presented from classical and deep reinforcement learning methods for bipedal walking. 
Walking is a challenging control problem. Once stable walking is achieved, the average infant falls 17 times per hour [\cite{adolph_how_2012}]. In this section, we review the literature on bipedal walking methods from both a classical and a deep reinforcement learning perspective. We also provide a review of curriculum learning, with a particular focus on recent implementations for legged platforms traversing complex terrains. 

\subsection{Classical Behaviour Design for Bipedal Robots}

Designing controllers for dynamic bipedal walking robots is difficult, particularly when operating over complex terrain [\cite{atkeson_what_2016}]. Classical control methods for walking that use Zero Moment Point (ZMP) [\cite{kajita_biped_2003}] or Capture Point (CP) [\cite{pratt_capture_2006}] control, rely on simplified dynamical models such as the spring loaded inverted pendulum (SLIP) [\cite{geyer_compliant_2006}]. ZMP is a widely used idea for bipedal walking and refers to the point on the ground where the horizontal moments sum to zero. This location is the same as the centre of pressure if both feet are on the same plane (centre of pressure is linked to contact forces, ZMP to inertial and gravity forces). While this point is contained within the support polygon created by the stance feet, the robot will remain stable. Fig. \ref{fig:zmp} shows the ZMP idea with a simple cart-table model, along with the inverted pendulum model used by \cite{kajita_biped_2003} to plan walking trajectories. Capture point (CP, also referred to as Divergent Component of Motion (DCM)) refers to a point that can bring the robot to a complete stop if that point is located within the support polygon created by the stance feet. If we consider the inverted pendulum with flywheel model (Fig. \ref{fig:capture_point}.b)) the CP is not a unique point. A capture region defines a collection of CP's that exist within reach of the swing foot (Fig. \ref{fig:capture_point}.a)). Using the CP idea, it is not necessary to have perfect foot placement, but good foot placement within a capture region is important [\cite{pratt_capture_2006}].


\begin{figure}[h!tb]
% \vspace{2mm}
\centering
\subfloat[A cart-table model]{\includegraphics[width=0.4\columnwidth]{images/ch2/zmp.png}}
\subfloat[A pendulum under constraint]{\includegraphics[width=0.4\columnwidth]{images/ch2/zmp2.png}}

% \hfill
\caption{Zero moment point (ZMP) model using a inverted pendulum under constraint[\cite{kajita_biped_2003}].}
\label{fig:zmp}
% \vspace{-3mm}
\end{figure}

\begin{figure}[h!tb]
% \vspace{2mm}
\centering
\subfloat[The capture point (CP) is located within the capture region, and defines a point the robot can step to come to a complete stop.]%{\includegraphics[height=12cm]{images/ch2/capture_point2.png}}
{\includegraphics[width=0.5\columnwidth]{images/ch2/capture_point3.png}}
% \hfill
\hspace{0.5cm}
\subfloat[The flywheel inverted pendulum considers the inertia of the center of mass (CoM).]
% {\includegraphics[height=6cm]{images/ch2/capture_point1.png}}
{\includegraphics[width=0.4\columnwidth]{images/ch2/capture_point1.png}}
% \hfill
\caption{Capture point (CP) controller using a flywheel inverted pendulum model[\cite{pratt_capture_2006}].}
\label{fig:capture_point}
% \vspace{-3mm}
\end{figure}

Classical methods for controller design have allowed bipedal robots to perform complex behaviours such as ascending and descending stairs [\cite{ching-long_shih_ascending_1999}], balancing on a Segway [\cite{gong_feedback_2019}], and executing a jump [\cite{xiong_bipedal_2018}]. Humanoid robots often employ a set of control primitives, each individually developed and tuned, such as Dynamic Movement Primitives (DMP) which uses discrete and rhythmic controllers that have been used to allow a humanoid robot to play the drums and swing a tennis racket [\cite{schaal_dynamic_2006}]. \cite{siciliano_using_2008} uses primitives to place and remove a foot from contact, enabling a robot to walk on uneven terrain, up a step, and climb a ladder. Primitives developed from motion capture can be stitched together with Hidden Markov Models (HMMs) to create sequences of motions [\cite{kulic_incremental_2012}]. While classical methods can achieve complex behaviours, they typically require extensive expert tuning. Furthermore, behaviours that rely on perception, for example walking up and down stairs, require footstep locations to be resolved explicitly from high dimensional sensors, further adding to the complexity of classical systems. For these reasons, classical methods are limited in their extension to more challenging obstacles.

% [\cite{ching-long_shih_ascending_1999, gong_feedback_2019, xiong_bipedal_2018}]
% There must be many more examples!

\subsection{Deep Reinforcement Learning for Bipedal Robots}

Deep reinforcement learning (DRL) offers an alternative to classical control methods, policies learn behaviours by interacting with the environment. DRL has recently demonstrated impressive feats for bipeds in simulation, demonstrated bipedal walking over complex terrain [\cite{schulman_proximal_2017, heess_emergence_2017, peng_deeploco_2017, xie_allsteps_2020}], and performing complex maneuvers replicating motion capture [\cite{peng_deepmimic_2018}]. Recently, DRL has been used for an increasing number of real world applications with legged robots [\cite{tan_sim--real_2018, xie_learning_2020, hwangbo_learning_2019, lee_robust_2019, peng_learning_2020, siekmann_sim--real_2021,  rudin_learning_2021}]. 

An agent acting in an environment is considered a Markov Decision Process $\text{MDP}$, defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and $\gamma \in [0,1)$ is a discount factor. The goal of reinforcement learning is to maximise the sum of future rewards:

\begin{equation}
R(\tau) = \sum_{t=0}^{\infty}\gamma^tr_t
\end{equation}

where $r_t$ is a scalar reward provided by the environment at time $t$. Fig.\ref{fig:ch2_rl_diagram} [\cite{SpinningUp2018}] shows the agent-environment interaction loop, where an agent performs an action, receives a reward, and observes the next state. For continuous control policies, actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is is a continuous control signal supplied to the robot, for example, the torque applied to each joint.

\begin{figure*}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.8\columnwidth]{images/ch2/rl_diagram_transparent_bg.png}
\caption{Agent-environment interaction loop.}
\label{fig:ch2_rl_diagram}
\vspace{-3mm}
\end{figure*}

\noindent\textbf{Proximal Policy Optimsation (PPO):}
\\
PPO is a widely used DRL algorithm for continuous control tasks. It was first introduced by \cite{schulman_proximal_2017}, with notable uses for legged robot control in both simulation [\cite{heess_emergence_2017, peng_deepmimic_2018, xie_feedback_2018, yu_learning_2018, lee_composing_2019, xie_allsteps_2020}], and on real legged platforms [\cite{tan_sim--real_2018, xie_learning_2020, rudin_learning_2021}]. PPO is an on-policy algorithm, meaning it trains using the experience collected by running the policy being optimised. On-policy algorithms are particularly suited for evolving training regimes, for example, using curriculum learning (discussed in the following section).

PPO belongs to a family of DRL algorithms known as actor-critic methods [\cite{sutton_reinforcement_1998}] where a neural network policy (the actor) determines the actions an agent should take in the environment, and a second neural network (the critic) evaluates the performance of the policy through a value function. The value function $V^\pi(s_t)$, predicts the discounted sum of future reward given the current state, and running policy $\pi$:

\begin{equation}
    V^\pi(s_t) = \mathbb{E}_{\tau \sim \pi}[R(\tau) | s_0 = s_t]
\end{equation}

The advantage is a zero centered indication of how much better or worse the current state is given the observed reward and the value estimate of the next state. The bootstrapped estimate of the advantage is given by:

\begin{equation}
    \hat{A}(s_t) = r_t + \gamma V^\pi(s_{t+1}) - V^\pi(s_t) 
\end{equation}

In practice, PPO uses general advantage estimation (GAE) [\cite{schulman_gae_2016}], a low variance estimate of the advantage.
% using Monte-Carlo return (non-truncated episode reward). 

PPO is also known as trust region method. PPO works by ensuring that policy updates do not cause the updated policy to perform very different actions to the policy that was used to collect the data. The parameters of the policy $\pi(\theta)$ are updated based on the following clipped loss function:

\begin{equation}
    L^{CLIP}(\theta) = \hat{\mathbb{E}}_t[\text{min}(\hat{r}_t(\theta)\hat{A}_t, \text{clip}(\hat{r}_t(\theta), 1 - \epsilon, 1 + \epsilon)\hat{A}_t)]
\end{equation}

where $\epsilon$ is a tuned clipping parameter, and $\hat{r}_t(\theta)$ is a ratio of the probability of action $a_t$ with the current policy $\pi_\theta(s_t)$, and the policy from the previous update $\pi_{\theta_{old}}(s_t)$:
\begin{equation}
    \hat{r}_t(\theta) = \frac{\pi_\theta(a_t | s_t)}{\pi_{\theta_{old}}(a_t | s_t)} 
\end{equation}

\begin{figure*}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.8\columnwidth]{images/ch2/ppo.png}
\caption{Plots showing the behaviour of the $L^{CLIP}$ loss function of PPO, when the policy performed better than expected $A>0$, and worse than expected $A<0$.}
\label{fig:ch2_ppo}
\vspace{-3mm}
\end{figure*}

The \textit{min} in the loss function ensures that the clipping is one sided depending on if the advantage is positive or negative (shown in Fig. \ref{fig:ch2_ppo}). Intuitively, if we did better than expected, we want to prevent too large of a step in the positive direction, but if we did worse than expected, and the action is now more probable with the new policy, we are allowed to reverse the update that lead to the bad behaviour. Therefore policy updates remain close to the policy that generated the data.

% the gradient of the loss becomes zero for values that result from large changes to the policy prediction (i.e. if the actions of the current policy are very different from the old policy we do not want to update too much), the gradient becomes zero (as shown in Fig. \ref{fig:ch2_ppo}).  In the special case where the advantage is negative, and the action from the new policy is more likely than the with the old policy, we are allowed to reverse the update that lead to the bad behaviour. This is shown in the right diagram of \ref{fig:ch2_ppo}. Therefore policy updates remain close to the policy that generated the data.


% There must be many more examples!



\begin{figure*}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.8\columnwidth]{images/ch2/deep_mimic1.png}
\caption{Characters traversing randomly generated terrains.}
\label{fig:ch2_deep_mimic1}
\vspace{-3mm}
\end{figure*}

Using PPO, \cite{peng_deepmimic_2018} learn complex maneuvers for high degree of freedom characters by following motion capture data. Example behaviours are shown in Fig. \ref{fig:ch2_deep_mimic1}. The reward function encourages matching the expert trajectory:

\begin{equation}
    r_t^I = w^pr^p_t + w^vr^v_t + w^er^e_t + w^cr^c_t
\end{equation}

where $w$ is a tuned weighting for each element, and each element $r_t^{**}$ is defined by:

\begin{equation}
    r_t^{**} = \text{exp}[-w^{**}(\sum_{j}||\hat{q}^{**}_t - q^{**}_t||^2)]
\end{equation}

where $**$ is one of ${p,v,e,c}$ corresponding to joint position, velocity, end effector position, and CoM position, $j$ refers to each element of $**$ (for example each joint or end effector), $w$ is a tuned weighting and $\hat{q}$ refers to the reference motion collected using motion capture. In their work, \cite{peng_deepmimic_2018}  first train the agent on flat terrain, then the policy is augmented to include a heightmap to allow the agent to walk up stairs. While learning from motion capture allows for complex behaviours, it requires having demonstrations of the desired behaviour. 

\cite{peng_deepmimic_2018} further explore the possibilities of having multiple complex behaviours by also learning which behaviour to select using a one-hot selector policy that determines which skill to use. They also construct composite behaviours that combine learned skills. Skills are combined by normalising the value function of each policy, and a new composite policy is trained that is able to perform a set of goal conditioned behaviours. While this work is impressive, it requires all behaviours be available during training, which may not be possible as the number of skills are increased and expensive retraining is required as new skills are included. Furthermore, this method relies on a phase variable supplied as additional information to the policy, meaning skills must complete their full action before transitioning to the next skill.

% \cite{merel_hierarchical_2019} train a humanoid to navigate and walk over gaps using an RGB camera. Policies are trained from snippets of motion capture trajectories, and are then stitched together with a high level selection policy. 

While there have been improvements in the sample efficiency and overall return from continuous DRL algorithms in recent years [\cite{haarnoja_soft_2018, fujimoto_td3_2018, Song2020V-MPO}], PPO is still commonly used for its simplicity, ease of distributed training, and the benefits of on-policy learning. For example, \cite{rudin_learning_2021} recently used PPO to train a walking policy for a quadruped in just 20 minutes using parallel workers on a desktop GPU. The training process included a game-inspired curriculum of increasing terrain complexity. The resulting policy was able to walk up and down stairs with an ANYmal-C quadruped in the real world. \cite{xie_feedback_2018} used PPO to learn a policy that takes as input the robot state and a reference motion and outputs a delta that is then added to the reference motion. This policy is able to control a simulated version of the biped Cassie over undulating terrain. In a followup work this method was applied to the real biped, displaying reduced recovery time after stepping on an unexpected obstacle [\cite{xie_iterative_2019}]. \cite{siekmann_sim--real_2021} use a periodic reward to train an adjustable walking policy also for the Cassie robot in the real world, that allowed the robot to perform complex behaviours such as jumping, skipping, and stepping over difficult obstacles such as stairs.

Usually DRL methods are limited to solving a single task end-to-end, characterised by a scalar reward function. End-to-end methods require costly retraining if new terrains are introduced, and in a real setting it may be intractable to train on the complete set of expected conditions. Furthermore, developing a single policy to perform multiple behaviours can degrade the performance of each behaviour [\cite{lee_robust_2019}].

% On-policy learning benefits from curriculum learning [\cite{yu_learning_2018, rudin_learning_2021}]


% Other algoritms:  
% Reinforce / DDPG? Anything more recent?
% TRPO: [\cite{hwangbo_learning_2019, lee_robust_2019, lee_learning_quad_2020}]
% On-line is preferable to offline learning when.. 
% Is more simple that soft actor-critic (SAC) [\cite{haarnoja_soft_2018}], twin delayed DDPG (TD3) [\cite{fujimoto_td3_2018}], and value maximum posteriori optimisation (V-MPO) [\cite{Song2020V-MPO}]. 


\subsection{Curriculum Learning}

Many examples of curriculum learning (CL) are present throughout
our lives, from progressing through school, playing sport,
or learning a musical instrument [\cite{narvekar_curriculum_2020}]. CL has been applied to a wide range of machine learning domains. The idea of CL is to provide training data to the learning algorithm in order of increasing difficulty [\cite{yu_learning_2018}]. \cite{elman_learning_1993} stated the importance of starting small: learn simpler aspects of a task, then slowly increase the complexity. These ideas were applied to learning grammatical structure, by starting with a simple subset of data and gradually introducing more difficult samples [\cite{elman_learning_1993}]. \cite{bengio_curriculum_2009} highlight that for complex loss functions, CL can guide training towards better regions, helping find more suitable local minima. This results in a faster training time and better generalisation, demonstrated on a shape recognition task, and a natural language task. A summary of curriculum learning methods for deep reinforcement learning (DRL) can be found in \cite{narvekar_curriculum_2020}, and the blog post by \cite{weng_curriculum_2020}.

CL has been applied in continuous control domains such as robotics. \cite{sanger_neural_1994} applied Trajectory Extension Learning, where the desired trajectory for a two joint robot arm slowly moves the robot from a region of solved dynamics to a region where the dynamics are unsolved. The work by \cite{mendoza_curriculum_2017} shows that progressively increasing the number of controllable joints, incrementally moving robot further from the target, and reducing joint velocities improves learning on a Jaco robot arm. 

\cite{karpathy_curriculum_2012} train a dynamic articulated figure called an ``Acrobot" with a curriculum of increasingly difficult maneuvers. In their work, a low level curriculum learns a specific skill, and a high level curriculum specifies which combination of skills are required for a given task. For agents that have an unconstrained base, such as bipeds, several methods employ base stabilisation forces [\cite{van_de_panne_controller_1992, wu_terrain-adaptive_2010, yu_learning_2018}]. 

\cite{yu_learning_2018} demonstrate that employing a virtual assistant that applies external forces to stablise the robot base, as well as encouraging forward motion, can reduce the training time and increase the asymptotic return. The force applied by the virtual assistant is reduced as a success criteria is reached (i.e. if the robot has not fallen after a nominal number of seconds), resulting in walking and running gaits for several simulated bipedal actors (Fig. \ref{fig:ch2_yu_learning1}). In their work, \cite{yu_learning_2018} discuss the different options for curriculum design, including a learner centered curriculum, and an environment-centered curriculum (\ref{fig:ch2_yu_learning2}). This work also demonstrates that with CL, a higher energy penalty can be applied to the magnitude of joint torques, without a detriment to learning [\cite{yu_learning_2018}]. These examples are limited to simple terrains.

\begin{figure*}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.8\columnwidth]{images/ch2/yu_learning1.png}
\caption{Simplified biped walking (top) and running (bottom). 
% Results are trained using environment-centered curriculum learning and mirror symmetry loss.
}
\label{fig:ch2_yu_learning1}
\vspace{-3mm}
\end{figure*}

\begin{figure}[h!tb]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=0.35\columnwidth]{images/ch2/yu_learning_a.png}}
\hspace{0.5cm}
% \subfloat[]{\includegraphics[width=0.3\columnwidth]{images/ch2/yu_learning_b.png}}
\subfloat[]{\includegraphics[width=0.35\columnwidth]{images/ch2/yu_learning_c.png}}
% \hfill
\caption{(a) The learner-centered curriculum determines the lessons adaptively based on the current skill level of the agent. (b) Environment-centered curriculum follows a series of predefined lessons [\cite{yu_learning_2018}].}
\label{fig:ch2_yu_learning2}
% \vspace{-3mm}
\end{figure}

Recent works have seen the adoption of curriculum learning for increasing terrain difficulty [\cite{xie_allsteps_2020, lee_learning_quad_2020, rudin_learning_2021}], as well as a curriculum on reward parameters. \cite{hwangbo_learning_2019} first allow a quadrupedal robot to learn any movements that result in forward motion. During training the reward evolves to encourage actions that produce a desirable walking gait.

% quadruped robot is free to learn an initial walking behaviour, then reward evolution guides the robot towards a more desirable gait throughout training [\cite{hwangbo_learning_2019}]. 



% This work also includes a penalty that encourages symmetrical motions. 

% \begin{equation}
%     \pi_\theta(s) = \Psi_a(\pi_\theta(\Psi_o(s)))
% \end{equation}

% \begin{equation}
%     L_{sym}(\theta) = \sum^B_{i=0}||\pi_\theta(\mathbf{s_i}) - \Psi(\pi_\theta(\Psi_o(\mathbf{s_i})))||^2
% \end{equation}

% \begin{equation}
%     % \pi_\theta* = \underset{\theta}{\text{argmin}} L_{\text{PPO}(\theta) + w L_{sym}(\theta)}
%     \pi_\theta* = \underset{\theta}{\text{argmin}} L_{\text{PPO}}(\theta) + wL_{sym}(\theta)
% \end{equation}




% Our method combines ideas from \cite{yu_learning_2018}, and \cite{rana_multiplicative_2020}, where we stabilise the robot CoM by applying external forces, and also guide exploration using a simple prior controller applying forces to each joint. We apply these ideas, and increase the difficulty of the terrain, resulting in the traversal of complex terrain artifacts.

\section{Behaviour Switching}

Progressive nets and distillation, need to mention these

Behaviour selection is in important property of behaviour based robotics [\cite{arkin_behavior-based_1998}]. For dynamic controllers, it is not only important to know what behaviour to activate, it is vital that behaviours are selected in such a way that the robot always remains in a stable. We are interested in the latter problem, where sequential behaviours that have little or no overlapping states can be safely integrated to allow the robot to perform tasks that are more complex than any single behaviour. 
% Designing a single policy that can display multiple behaviours is challenging, and often results in the degraded performance of individual behaviours [\cite{lee_robust_2019}]

\subsection{Classical Methods for Behaviour Selection}

Need to look at these and slot them in:
\cite{manchester_2011_regions, matallana_2010_estimation}

Classical methods for behaviour selection rely on understanding the model of the system, and knowing the set of states for which a given controller will operate and safely converge to a target set of states. A key component is determining the region of attraction (RoA, also called domain of attraction (DoA)) for each controller, which is defined as the set of states that if a specified controller is activated, the robot will converge to a target set of states defined for that controller. Formally, if each controller $\Phi_i$ has a goal set (or invariant set) $\mathcal{G}(\Phi_i) = \{s_i^*\}$ that defines all of the states the controller operates nominally, then the region of attraction (RoA) for $\Phi_i$ is given by:

\begin{equation}
    \mathcal{R}(\Phi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\Phi_i)\}
\label{eq:roa}
\end{equation}

Controllers can be composed in such a way that the goal set for one controller exists in the RoA of another, thus activating controllers in the correct sequence will drive the robot toward a desired goal state. This sequencing of controllers is known as sequential composition, and the linking of a sequence of controllers together by understanding the RoA and goal set of each has been demonstrated on a juggling robot [\cite{burridge_sequential_1999}]. The sequential composition framework is illustrated in Fig. \ref{fig:cha2_sequential}. 


% where $s=[rs, I]$, and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is the set of states policy $\pi_i$ was designed to operate within (Goal Set or Invariant Set), and $\mathcal{R}(\pi_i)$ is the set of states that will converge to a state in $\mathcal{G}(\pi_i)$. 

\begin{figure*}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.5\columnwidth]{images/ch2/sequential.png}
\caption{The sequential composition of controllers. Each
controller is only active in the part of its domain that is not
already covered by those nearer the goal. Here, $\Phi_3 \succeq \Phi_2 \succeq \Phi_1$ , and $\Phi_1$ is the goal controller.
.}
\label{fig:cha2_sequential}
\vspace{-3mm}
\end{figure*}

Estimating the RoA overlap between controllers can be difficult for robots with high state spaces, however it can be simplified by defining a set of pre and post conditions for each controller [\cite{faloutsos_composable_2001}], defining fixed length control sequences [\cite{peng_deepmimic_2018}], or by providing a rule-based bound on parameters like heading angle and switching frequency [\cite{gregg_control_2012}]. \cite{motahar_composing_2016} switch between straight, left turn, and right turn controllers operating a 3D simulated biped using
a reduced dimension hybrid zero dynamics control law. These methods result in combinations of complex primitives, though they require a mathematically defined RoA, or a hand designed switching criteria for each primitive. RoA expansion can provide a greater overlap between controllers [\cite{borno_domain_2017}]. \cite{borno_domain_2017} estimate the RoA for a simulated humanoid using multiple forward passes of a dynamics model simulation. Using rapidly exploring random trees (RRTs), the closest state within the RoA of a given controller is found, and the new trajectory included in the RoA of the controller (Fig. \ref{fig:ch2_borno}).

% Using pre-trained policies requires a suitable handling of transitions between behaviours. \cite{faloutsos_composable_2001} learns pre and post-conditions for each controller, such that switching only occurs when these conditions have been satisfied.  


\begin{figure*}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.6\columnwidth]{images/ch2/borno1.png}
\caption{RoA expansion by sampling with a RRT [\cite{borno_domain_2017}].
}
\label{fig:ch2_borno}
\vspace{-3mm}
\end{figure*}

% Pics of borno or faloutsos?
% , a similar approach to ours.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Learning Methods for Behaviour Selection}


Combining DRL primitives usually involves training a deep Q network (or a similar discrete switching network) that selects which primitive to use [\cite{liu_learning_2017,merel_hierarchical_2019,lee_robust_2019}], or learning a complex combination of primitives [\cite{peng_mcp_2019}]. \cite{liu_learning_2017} combine control fragments with a Q-learning scheduler that allows highly complex simulated characters perform balancing tasks. \cite{merel_hierarchical_2019} use motion capture to train primitives for a simulated humanoid. Each primitive is spliced into small fragments of known length, and a control fragment selector utilises perception to determine which controller to use at each interval. \cite{lee_robust_2019} learn a switching policy for several complex behaviours that allow a quadruped to recover from a fall, stand, and continue walking. \cite{peng_mcp_2019} learn how to combine pre-trained motion primitives for a simulated humanoid using multiplicative compositional policies (MCP). Using a complex combination of actions results in the smooth transition between behaviours and the emergence of new behaviours created by combining several pre-trained policies [\cite{peng_mcp_2019}]. Other hierarchical approaches learn the primitives and selection network together [\cite{bacon_option-critic_2018}], or with several task-dependent selection networks [\cite{frans_meta_2017}]. Training in each of these examples needs access to all expected environment conditions during training, and adding new primitives requires retraining of the selection policy.

While estimating the complete RoA of a policy is possible for systems with a relatively small state space, such as the single [\cite{berkenkamp_safe_2017, najafi_learning_2016}], or double inverted pendulum [\cite{randlov_combining_2000}], for more complex systems the RoA is difficult to determine. Where it is possible to differentiate between unmodeled regions of the state from those that are well behaved, DRL can guide the agent back to where a classical controller can take over [\cite{najafi_learning_2016}], [\cite{randlov_combining_2000}]. \cite{najafi_learning_2016} train a policy to swing an inverted pendulum to a state where the upright controller can take over. Fig. \ref{fig:cha2_learning_sequential}.a) shows a depiction of the upright, and downward controllers ($\Phi_1$ and $\Phi_2$), without an overlap. In this work, a separate controller was trained with DRL to create an overlap between the existing controllers ($\Phi_3$, shown in green in Fig. \ref{fig:cha2_learning_sequential}.b)). The new behaviour $\Phi_3$ allows the pendulum to move from the downward position ($\Phi_2$), through the goal set of controller $\Phi_3$, to get to the RoA of controller $\Phi_1$, and finally the upward position (i.e. the goal state of controller $\Phi_1$).

\begin{figure}[h!tb]
% \vspace{2mm}
\centering
\subfloat[RoA and goal sets of a sequential
composition controller, where $x_0 \in \mathcal{D}(\Phi_1), x_d \in \mathcal{D}_2(\Phi_2)$, but controller $\Phi_1$ does not prepare controller $\Phi_2$.]{\includegraphics[width=0.5\columnwidth]{images/ch2/learning_sequential_no_overlap.png}}
% \hfill
\hspace{0.5cm}
% \newline
\subfloat[RoA goal sets of the controllers after training (the green ellipse is the trained behaviour).]{\includegraphics[width=0.45\columnwidth]{images/ch2/learning_sequential2.png}}
% \hfill
\caption{Learning sequential composition [\cite{najafi_learning_2016}].}
\label{fig:cha2_learning_sequential}
% \vspace{-3mm}
\end{figure}

% Other work with DRL has shown that expanding the RoA of each primitive with transition policies improves switching [\cite{lee_composing_2019}]. RoA estimation to combine DRL policies is a promising approach to scale the capabilities of legged robots, and is an area of research that requires more investigation.



Hierarchical reinforcement learning (HRL) offers flexibility through architecture, by training all segments of the hierarchy concurrently [\cite{sutton_between_1999, bacon_option-critic_2018, frans_meta_2017,peng_deeploco_2017}], or training parts of the hierarchy separately [\cite{merel_hierarchical_2019}], [\cite{lee_composing_2019}].  When trained together, HRL can improve task level outcomes, such as steering and object tracking [\cite{peng_deeploco_2017}], or improve learning efficiency by reusing low level skills across multiple high level tasks [\cite{frans_meta_2017}]. When trained separately, HRL can break up a large difficult problem into smaller solvable sub-problems [\cite{schaal_dynamic_2006}]. Low level controllers can be refined efficiently using prior knowledge, for example by utilising motion capture data [\cite{peng_deepmimic_2018, merel_hierarchical_2019, peng_mcp_2019}] or behavioural cloning [\cite{strudel_learning_2020}]. For robotics applications it may be difficult to develop controllers for multiple behaviours simultaneously, HRL can break up a large difficult problem into smaller solvable sub-problems [\cite{schaal_dynamic_2006}]. Policy sketches introduce a hierarchical method that uses task specific policies, with each task performed in sequence [\cite{andreas_modular_2017}]. CompILE uses soft boundaries between task segments [\cite{kipf_compile_2019}]. Work by \cite{peng_terrain-adaptive_2016} trains several actor-critic control policies, modulated by the highest critic value in an given state. For these examples there must be a reasonable state overlap between sequential controllers.


% 
% DeepMimic by \cite{peng_deepmimic_2018} combines pre-trained behaviours learned from motion capture, with reliance on a phase variable to determine when one behaviour has been completed.

% In our previous work [\cite{tidd_learning_2021}], we learn when to switch between low level primitives for a simulated biped by randomly sampling from a collection of behaviours.

For dynamic platforms, where separate controllers occupy different subsets of the state, changing behaviours may not result in stable behaviour if there is no overlap between controllers. \cite{lee_composing_2019} learn a proximity predictor to train a transition policy to get an agent to the initial state required by the next controller. Fig. \ref{fig:cha2_lee_composing} outlines this method, where in Fig. \ref{fig:cha2_lee_composing}.a) we see that each policy has a transition policy, Fig. \ref{fig:cha2_lee_composing}.b) shows the training method. Data is collected by recording success and failures. These buffers are used to train a proximity predictor function $P_\omega(s)$, that predicts how close the robot is from a transition state that would result in the successful traversal of the obstacle. Equation \ref{eq:cha2_lee_composing1} shows the loss function for the proximity predictor. Success is a defined parameter relating to the task, for example, if the robot has past the obstacle by 1.5m it was deemed successful. 

\begin{figure}[h!tb]
% \vspace{2mm}
\centering
\subfloat[Our modular network augmented with transition policies. To perform a complex task,
our model repeats the following steps: (1) The meta-policy chooses a primitive policy of index c; (2) The corresponding transition policy helps initiate the chosen primitive policy; (3) The primitive policy executes the skill; and (4) A success or failure signal for the primitive skill is produced.]{\includegraphics[width=0.95\columnwidth]{images/ch2/lee_composing1.png}}
\hfill
\subfloat[Training of transition policies and proximity predictors. After executing a primitive policy, a previously performed transition trajectory is labeled and added to a replay buffer based on the execution success. A proximity predictor is trained on states sampled from the two buffers to output the proximity to the initiation set. The predicted proximity serves as a reward to encourage the transition policy to move toward good initial states for the corresponding primitive policy.]{\includegraphics[width=0.95\columnwidth]{images/ch2/lee_composing2.png}}
% \hfill
\caption{Learning transition policies [\cite{lee_composing_2019}].}
\label{fig:cha2_lee_composing}
% \vspace{-3mm}
\end{figure}
 
\begin{equation}
    L_P(\omega,\mathcal{B}^S, \mathcal{B}^F) = \frac{1}{2}\mathbb{E}_{(s,v) \sim \mathcal{B}^S}[(P_\omega(s) - v)^2] + \frac{1}{2}\mathbb{E}_{(s,v) \sim \mathcal{B}^F}[P_\omega(s)^2] 
\label{eq:cha2_lee_composing1}
\end{equation}

where data is sampled from buffers of success and failures ($\mathcal{B}^S, \mathcal{B}^F$), and $v$ is a linearly discounted function $v = \delta^{step}$. $\delta$ is a decay parameters, and $step$ refers to the number of timesteps required to reach the transition state. Using this prediction as a reward, a transition policy is trained to maximise the reward function ($\gamma$ is a discount factor):

\begin{equation}
    R_{\text{trans}}(\phi) = \mathbb{E}_{(s_0,s_1,...,s_T) \sim \pi_\phi}[\gamma^TP_\omega(s_T) + \sum^{T-1}_{t=0}\gamma^t(P_\omega(s_{t+1}) - P_\omega(s_t))] 
\label{eq:cha2_lee_composing2}
\end{equation}

Other methods that combine pre-trained behaviours learn latent representations of skills [\cite{pertsch_accelerating_2020}] or primitives [\cite{ha_distilling_2020}], enabling interpolation in the latent space. From an offline dataset of experience, \cite{pertsch_accelerating_2020} are able to combine low level controllers in manipulation tasks and locomotion task for a multi-legged agent. \cite{ha_distilling_2020} utilise motion capture to learn latent representations of primitives, then use model predictive control for the high level navigation of a high dimensional humanoid. The FeUdal approach learns a master policy that modulates low-level policies using a learned goal signal [\cite{vezhnevets_feudal_2017}]. Interpolation between behaviours yields natural transitions [\cite{xu_hierarchical_2020}], however in each of these approaches, experience from all behaviours must be available during training. 

% Work by \cite{peng_mcp_2019} combines pre-trained policies using a gating function that learns a multiplicative combination of actsions.
% Our setup policies are also use an intermediate controller, however we show that our method performs more reliably with complex locomotion behaviours.

\section{Navigating Through Narrow Spaces}

Designing an autonomous navigation system to handle difficult terrain scenarios is challenging. Often a set of behaviours is required, where each behaviour has been tuned to handle a unique situation. The recently concluded DARPA Subterranean challenge  [\cite{darpa_darpa_2021}] highlighted the need for agents exploring underground environments to autonomously pass through small gaps like doorways. Costmaps are used by path planners to perform complex maneuvers to traverse difficult terrain [\cite{hudson_heterogeneous_2021}], however the task becomes challenging when gaps that are marginally wider than the robot do not appear as traversable. Common perception modalities, such as occupancy maps, provide a course representation of the world. Distinguishing when a gap is suitable to traverse, and designing a behaviour to get through is an active challenge for mobile platforms.

\subsection{Classical Methods for Robot Navigation}

% Krishan's paper for other methods (Vectore Field Histograms?)
% Vector Field Histograms (VHF) [4] is a real time mo-
% tion planning algorithm that generates a polar histogram to
% represent the polar density of surrounding obstacles. The
% robot’s steering angle is then chosen based on the direction
% exhibiting the least density and cl
% approach, the polar histogram has to be computed at everyoseness to goal. For this
% time step, making it suitable for dynamic obstacle avoidance

Classical methods for autonomous navigation struggle to traverse small gaps. Artificial potential fields (APF) [\cite{khatib_real-time_1986}] is a widely used algorithm for navigation, where the robot is attracted to goal locations, and repelled from obstacles. Vector Field Histograms (VHF) generate the steering angle based on the polar density of surrounding obstacles [\cite{borenstein_vector_1991}]. Bug algorithms have also been used extensively [\cite{mcguire_comparative_2019}], using the idea that the robot moves toward a goal unless an obstacle is encountered, then the robot moves along the obstacle boundary until it can once again move toward the goal. Small gaps are a limitation for each of these methods. Local minima with narrow gaps causes oscillations when the attractive and repelling forces are balanced [\cite{koren_potential_1991}]. 

Many solutions have been proposed for the narrow gaps problem.  \cite{zheng_sun_narrow_2005} introduce a bridge test to detect narrow passages for use with probabilistic roadmap (PRM) planning. Probabilistic planners like PRM and rapidly-exploring random trees (RRTs) rely on verifying path queries with a robot footprint, and therefore also have difficulty with narrow spaces that appear smaller than the robot. \cite{mujahed_admissible_2018} propose an admissibility gap: a virtual gap that satisfies the kinematic constraints of the vehicle to plan through tight spaces. In urban environments, \cite{rusu_laser-based_2009} design a geometric door detection method using 3D point cloud information, provided the door is within a set of specifications. A PR2 robot is able to detect a door and its handles [\cite{meeussen_autonomous_2010}], as well as negotiate the open or closed configuration to get through [\cite{chitta_planning_2010}]. \cite{cosgun_context_2018} detects doors from door signs, and directs a robot through with pointing gestures. \cite{moreno_automatic_2020} generate auxiliary waypoint locations (critical navigation points (CNP)) at problematic narrow regions (Fig. \ref{fig:cha2_moreno}). Sensory errors and coarse perception maps contribute to the failure of these methods where gaps that are less than the robot footprint are not considered for traversal, even though the robot may be able to get through. Classical navigation methods often rely on extensive manual tuning of parameters [\cite{khatib_real-time_1986, hines_virtual_2021, mcguire_comparative_2019}]. Hines et al [\cite{hines_virtual_2021}] design a behaviour stack where each behaviour has a priority, and an admissibility criteria. A behaviour becomes active if it has a higher priority than the current behaviour, and is admissible. Admissibility criteria, and the behaviours themselves, are manually designed. The primary path follow method uses Hybrid A* [\cite{dolgov_path_2010}] to plan a path through a costmap to a goal, considering the vehicle constraints. Manual tuning is a limitation of complex behaviours. Furthermore, in each of these approaches, the robot does not make contact with the environment, limiting its ability to make contact assisted progress through a small gap. Next, we review some of the learning methods for autonomous navigation.

\begin{figure}[h!tb]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=0.3\columnwidth]{images/ch2/moreno1.png}}
% \hfill
\subfloat[]{\includegraphics[width=0.3\columnwidth]{images/ch2/moreno2.png}}
% \hfill
\subfloat[]{\includegraphics[width=0.3\columnwidth]{images/ch2/moreno3.png}}
\hfill
\subfloat[]{\includegraphics[width=0.3\columnwidth]{images/ch2/moreno4.png}}
% \hfill
\subfloat[]{\includegraphics[width=0.3\columnwidth]{images/ch2/moreno5.png}}
% \hfill
\subfloat[]{\includegraphics[width=0.3\columnwidth]{images/ch2/moreno6.png}}
% \hfill
\caption{Detection of a critical navigation point (CNP) in a costmap. All distances between two near edges are computed, and the points yielding the minimum distance are selected. The CNP is finally placed
at the midpoint. [\cite{moreno_automatic_2020}].}
\label{fig:cha2_moreno}
% \vspace{-3mm}
\end{figure}

% \begin{figure*}[htb!]
% % \vspace{2mm}
% \centering
% \includegraphics[width=0.5\columnwidth]{images/ch2/mujahed.png}
% \caption{Extracting gaps. If a ray hits the boundary of the figure, no obstacle point is
% returned (e.g. at I and K). The gaps extracted by the counterclockwise and clockwise
% searches are shown by green and red colors, respectively. In the gap reduction
% process, the gaps indicated by dashed arrows are removed.
% }
% \label{fig:ch2_mujahed}
% \vspace{-3mm}
% \end{figure*}

\subsection{Learning Methods for Robot Navigation}

Learning methods used for navigation have shown promising results for mobile robots in human domains [\cite{rana_multiplicative_2020,bansal_combining_2019,kumar_learning_2019,gupta_cognitive_2019}], and in the field [\cite{kahn_badgr_2020}]. 
Using a prior controller to guide exploration, and decreasing the dependence on the prior as training progresses has improved reliability for robot navigation [\cite{rana_multiplicative_2020}]. This method efficiently learns a navigation policy from an APF prior controller while also learning a confidence for when the learned behaviour should be active, or when the robot should use the prior controller. An ensemble of policies is trained to determine a confidence for running the learned controller. By integrating both methods, the trained policy reduces oscillations caused by the classical controller, and for states not seen in the training data the classical method has priority. With learning methods it is possible to navigate on various surfaces [\cite{kahn_badgr_2020}], and through narrow gaps [\cite{bansal_combining_2019}] using RGB images. BADGR by \cite{kahn_badgr_2020} learn a navigation policy directly from images with a self supervised approach that not only learns to navigate to a waypoint, but also to favour traversing a concrete path over grass. \cite{bansal_combining_2019} learn to navigate through narrow doorways to get to a specified goal location using a monocular camera mounted to a robot. \cite{gupta_cognitive_2019} use end-to-end reinforcement learning to learn an egocentric map and how to plan to a goal. \cite{kumar_learning_2019} learn to plan at a high level of abstraction (turn left, turn right) using video data of expert trajectories. Learning methods reduce some of the hand tuning seen with classical controllers, however with the exception of \cite{rana_multiplicative_2020} they typically do not integrate with pre-existing behaviours. 


% This limits the use of pre-existing behaviour stacks with learned behaviours that can traverse difficult obstacles.

% In our previous work we introduce the idea of developing behaviours separately [\cite{tidd_guided_2020}], then learning when they should be used, either with a supervised approach [\cite{tidd_learning_2021}], or through reinforcement learning [\cite{tidd_learning_2021-1}]. For our problem we require a behaviour that can learn to perform complex maneuvers (such as make contact with a door), and can be integrated into an existing behaviour stack. 



\subsection{Sim-to-real Transfer of Locomotion Policies}

Static mobile robots suffer with less sim-to-real disparity than dynamic platforms. Policies that are trained in simulation have been directly transferred to mobile robots in the real world [\cite{tai_virtual--real_2017, xie_learning_2018, rana_residual_2020}], while behaviours for dynamic legged platforms require system identification [\cite{tan_sim--real_2018}], sim-to-real modelling [\cite{hwangbo_learning_2019, peng_learning_2020, rudin_learning_2021}], and heavy dynamics randomisation [\cite{peng_learning_2020}] during training to allow for policies to jump the reality gap. Furthermore, laser base sensors are less subjected to sim-to-real disparity than cameras and other sensors. \cite{tai_virtual--real_2017} train a policy that learns to avoid obstacles and get to a local target. \cite{xie_learning_2018} learn to switch between a simple controller and a trained policy for reaching a target in the local frame. This work introduced Assisted DPPG (AsDDPG), an extension of deep deterministic policy gradient (DDPG [\cite{Lillicrap2016ContinuousCW}]), where the simple controller provides an exploration policy for efficient learning. \cite{rana_residual_2020} train a navigation policy that sums with an APF prior controller to improve the performance of the prior controller. When the learned behaviour exhibits high uncertainty in a given state, the system switches to rely completely on the prior controller. For each of these examples, policies train in simulation transfer directly to the real robot with no fine tuning. However, each example used a simple differential drive robot (Turtlebot [\cite{tai_virtual--real_2017}], Pioneer [\cite{xie_learning_2018}], PatrolBot mobile \cite{rana_residual_2020}) and operated over a flat consistent surface. For more complex scenarios, (for example a skid steer robot over more challenging terrain), sim-to-real transfer may cause a drop in performance compared with results seen in the simulation. 

In all examples presented, no work considered gaps that are small enough to fall within a margin of error for the perception. The gaps explored are wide enough to be distinguished by the perception system, and no examples describe the requirement of the robot to make contact with a surface in order to get through a small gap. This presents a gap in the literature for small spaces that are marginally wider than the robot, where complex behaviours, such as making contact with the doorway, may be required for traversal. 

% Additionally, with the exception of \cite{xie_learning_2018, rana_residual_2020}, learning methods are not typically integrated with classical methods. 

\section{Summary}

From the reviewed literature, impressive behaviours were shown from both classical and learned methods. As the complexity of the behaviour increases and classical methods become difficult to model, learning approaches become a suitable option. Learning methods are particular suited when perception is linked to action in a complex way, for example for footstep planning. However, the training efficiency of learning models remains low, meaning large numbers of samples are required for training. For complex behaviours it is also challenging to train policies with naive exploration or sparse rewards. Often these policies succumb to local minima or result in overfitting the simulation in unrealistic ways. It remains an underexplored question of how to improve the efficiency of training to allow an agent to traverse complex obstacles. We will investigate this question in chapter \ref{cha:ch3}, and chapter \ref{cha:ch5}.

In many examples seen in the literature there is a form of hierarchical control, where controllers with several levels of abstraction are trained concurrently, and cases where it is beneficial to design separate behaviours and then determine where to activate the appropriate behaviour. For behaviour libraries to scale to more terrains, and for new terrains to be added as the behaviours become available, it is important to understand when it safe to switch between behaviours. For high DoF robots and black box behaviours like neural network policies, it is difficult to know what states are suitable to activate a particular behaviour. While there are examples of learning transition policies when there is little or no overlap between behaviours [\cite{najafi_learning_2016,lee_composing_2019}], for high DoF robots there has not been sufficient research. Chapter \ref{cha:ch4} will investigate learning when to switch between policies, and transitioning between behaviours. Chapter \ref{cha:ch5} will show an example of switching that includes a pre-existing library of manually tuned behaviours.

We have seen examples of navigation algorithms that have been used to pass through small gaps. In classical examples their have been no examples of getting through gaps with path planning methods where the gap is marginally wider than the robot. Learning approaches have shown examples when sensor data can be used directly, for example using a camera or depth sensor. However, for course occupancy maps, where the gap that is larger than the robot may appear smaller in the occupancy map, the robot must make contact with the environment to determine if it can in fact make it through. Chapter \ref{cha:ch5} investigates the challenges of developing a behaviour where the robot is able to make contact with the environment in order to wiggle through. We also consider the challenges that are present in sim-to-real transfer of locomotion policies, and discuss the sources of disparity between the simulation results and those of the robot in the real world.


==> old/Ch3.tex <==
\chapter[Guided Curriculum Learning for Walking Over Complex Terrain]{Guided Curriculum Learning for Walking Over Complex Terrain}
\label{cha:ch3}
% Motivation/contribution/abstract -----------------------


Reliable bipedal walking over complex terrain is a challenging problem, using a curriculum can help learning. Curriculum learning is the idea of starting with an achievable version of a task and increasing the difficulty as a success criteria is met. We propose a 3-stage curriculum to train Deep Reinforcement Learning policies for bipedal walking over various challenging terrains. In the first stage, while applying forces from a target policy to the robot joints and base, the agent starts on an easy terrain and the terrain difficulty is gradually increased. In the second stage, the guiding forces are gradually reduced to zero. Finally, in the third stage, random perturbations with increasing magnitude are applied to the robot base, so the robustness of the policies are improved. In simulation experiments, we show that our approach is effective in learning separate walking policies for five terrain types: flat, hurdles, gaps, stairs, and steps. Moreover, we demonstrate that in the absence of human demonstrations, a simple hand designed walking trajectory is a sufficient prior to learn to traverse complex terrain types. In ablation studies, we show that taking out any one of the three stages of the curriculum degrades the learning performance.

\section{Introduction}
\label{sec:ch3_introduction}


Learning to walk is difficult. Progressing from the stable locomotion of crawling to the more difficult task of walking upright takes on average 4 months for a baby. Once stable walking is achieved, the average infant falls 17 times per hour~\cite{adolph_how_2012}. For a human learning to walk, a curriculum typically occurs from crawling, to standing, to walking, and often with the guidance of an adult or walker. Many examples of curriculum learning are present throughout our lives, from progressing through school, playing sport, or learning a musical instrument~\cite{narvekar_curriculum_2020}. 

\begin{figure*}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=1.2\columnwidth]{images/ch3/fig2.png}
% \includegraphics[width=1.0\columnwidth]{images/ch3/fig2.png}
\caption{We use curriculum learning to train a biped to traverse complex terrain samples. Our learning procedure is divided into three stages. In Stage 1 we use guiding forces that stabilise the robot Centre of Mass and encourage exploration while gradually increasing the difficulty of the terrain. In Stage 2 the guidance forces are slowly reduced. In Stage 3 we increase the magnitude of random perturbations applied to the robot to improve robustness.}
\label{fig:2}
\vspace{-3mm}
\end{figure*}


Controlling a bipedal robot over complex terrain is a challenging task. Classical control methods require meticulous hand design and tuning for each behaviour. Deep Reinforcement Learning (DRL) methods are an alternative where policies are trained through interaction with the environment, and have shown promising results for the task of walking~\cite{peng_deeploco_2017}. However, DRL relies on stochastic exploration with a single scalar reward as a learning signal, which is often difficult to design for a high degree of freedom platform. These restrictions make it difficult for policies to randomly reach the required configuration to traverse particularly challenging terrain types. Curriculum learning offers a way to alleviate these issues for difficult problem domains.

% DRL has been shown to produce policies that closely match motion capture for high degree of freedom humanoid agents, removing much of the complexity of reward design~\cite{peng_deepmimic_2018},~\cite{merel_hierarchical_2019}. These methods require motion capture examples of each behaviour. We show that we do not need perfect demonstrations to train a walking controller, and that a simple walking trajectory is a sufficient prior for a range of complex terrains.

Curriculum learning (CL) applied in machine learning has shown improved learning outcomes in shape recognition and natural language tasks~\cite{elman_learning_1993},~\cite{bengio_curriculum_2009}, with the fundamental idea that easier aspects of a task are learned first, with a gradual increase in difficulty as training progresses. CL has also been used in conjunction with DRL, with similar improvements in robotics manipulation tasks~\cite{sanger_neural_1994},~\cite{mendoza_curriculum_2017}, decision making and navigation~\cite{narvekar_curriculum_2020}, and bipedal walking ~\cite{van_de_panne_guided_1995},~\cite{wu_terrain-adaptive_2010},~\cite{yu_learning_2018}. For bipedal walking, methods that employ curriculum learning show notable reductions in training time and improved final walking performance~\cite{yu_learning_2018}. \cite{yu_learning_2018} employ external guiding forces that stablise the base of the robot, and slowly reduce these forces as a success criteria is reached (if the episode has not terminated after a fixed number of steps). By the end of training the resultant policy can operate on the target domain, free from any external guidance. Our work has similarities to~\cite{yu_learning_2018} where external forces are used to stablise the Centre of Mass (CoM) of the robot. Differently to their work, we apply external forces to each joint, provided by a rudimentary hand crafted walking trajectory, to train policies to traverse complex terrain samples. For each terrain type (flat, gaps, hurdles, stairs, and steps) we train a separate policy following the 3-stage curriculum outlined in Fig~\ref{fig:2}. 
\begin{itemize}
    \item Stage 1: Using guiding forces applied to the CoM and each robot joint, we start from an easy terrain and gradually increment the terrain difficulty
    \item Stage 2: When the terrain is at its most difficult, we slowly decrease the external guiding forces applied to the robot
    \item Stage 3: We increase the magnitude of external perturbations to improve the robustness of the policy
\end{itemize}

Our contributions are as follows:
\begin{itemize}
    \item We propose a 3-stage curriculum learning approach tailored for bipedal walking on complex terrain types
    \item We show that a single rudimentary walking trajectory can be used as a target policy to improve exploration and training outcomes for several difficult terrain types
    \item We perform extensive analysis and ablation studies showing the importance of the design choices for our curriculum approach
    \item We demonstrate the successful traversal of multiple challenging terrain types
\end{itemize}

The organization of this paper is as follows. After reviewing the relevant literature in Sec~\ref{sec:ch3_related_work}, we define the problem of interest in Sec~\ref{sec:ch3_problem} and DRL algorithm used in Sec~\ref{sec:ch3_drl}. Our curriculum learning method is presented in Sec~\ref{sec:ch3_curriculum}, and our experimental results are shown in Sec~\ref{sec:ch3_experiments}. Finally, we conclude with a brief discussion in Sec~\ref{sec:ch3_conclusion}.


\section{Related Work}
\label{sec:ch3_ch3_related_work}


In this section, we review the literature on bipedal walking methods followed by a review of curriculum learning, predominantly in the context of deep reinforcement learning.

\subsection{Bipedal Walking}

Designing controllers for dynamic bipedal walking robots is difficult, particularly when operating over complex terrain~\cite{atkeson_what_2016}. Classical control methods for walking using Zero Moment Point (ZMP)~\cite{kajita_biped_2003} or Capture Point (CP)~\cite{pratt_capture_2006} control, rely on simplified dynamical models such as the spring loaded inverted pendulum (SLIP)~\cite{geyer_compliant_2006}. While classical methods can achieve complex behaviours~\cite{ching-long_shih_ascending_1999},~\cite{gong_feedback_2019},~\cite{xiong_bipedal_2018}, they typically require expert tuning, limiting their extension to more challenging conditions.

Deep reinforcement learning (DRL) has recently demonstrated impressive feats for bipeds in simulation~\cite{heess_emergence_2017},~\cite{peng_deeploco_2017}. Merel et al~\cite{merel_hierarchical_2019} train a humanoid to navigate and walk over gaps using an RGB camera. Policies are trained from snippets of motion capture trajectories, stitched together with a high level selection policy. Peng et al~\cite{peng_deepmimic_2018} learn complex maneuvers for high degree of freedom characters, also following motion capture data. In their work, the agent is first trained on flat terrain, then the policy is augmented to include a heightmap to allow the agent to walk up stairs. While learning from motion capture is promising, it requires having human demonstrations for all terrain conditions. We show it is possible to learn complex behaviours using a simple walking target trajectory. DRL approaches typically require extensive interaction with the target domain, which is a limiting factor for training end-to-end policies that work over a number of different terrains. In our method we train separate policies on small samples of each terrain type, such that we can add to our suite of controllers without retraining any previously trained policies.

\subsection{Curriculum Learning}

Curriculum learning (CL) has been successfully applied to a wide range of machine learning domains. The idea of CL is to provide training data to the learning algorithm in order of increasing difficulty~\cite{yu_learning_2018}. Elman~\cite{elman_learning_1993} stated the importance of starting small: learn simpler aspects of a task, then slowly increase the complexity. These ideas were applied to learning grammatical structure, by starting with a simple subset of data and gradually introducing more difficult samples~\cite{elman_learning_1993}. Bengio et al~\cite{bengio_curriculum_2009} highlight that for complex loss functions, CL can guide training towards better regions, helping find more suitable local minima. This results in a faster training time and better generalisation, demonstrated on a shape recognition task, and a natural language task. A summary of curriculum learning methods for deep reinforcement learning (DRL) can be found in Narvekar et al~\cite{narvekar_curriculum_2020}, and the blog post by Weng~\cite{weng_curriculum_2020}.

CL has been applied in continuous control domains such as robots. Sanger~\cite{sanger_neural_1994} applied Trajectory Extension Learning, where the desired trajectory for a two joint robot arm slowly moves the robot from a region of solved dynamics to a region where the dynamics are unsolved. The work by Mendoza~\cite{mendoza_curriculum_2017} shows that progressively increasing the number of controllable joints, incrementally moving robot further from the target, and reducing joint velocities improves learning on a Jaco robot arm. 

Karpathy and van de Panne~\cite{karpathy_curriculum_2012} train a dynamic articulated figure called an ``Acrobot" with a curriculum of increasingly difficult maneuvers. In their work, a low level curriculum learns a specific skill, and a high level curriculum specifies which combination of skills are required for a given task. For agents that have an unconstrained base, such as bipeds, several methods employ base stabilisation forces~\cite{van_de_panne_controller_1992},~\cite{wu_terrain-adaptive_2010},~\cite{yu_learning_2018}. Yu et al~\cite{yu_learning_2018} shows that employing a virtual assistant that applies external forces to stablise the robot base, as well as encouraging forward motion, can reduce the training time and increase the asymptotic return. The force applied by the virtual assistant is reduced as a success criteria is reached (i.e. if the robot has not fallen after a nominal number of seconds), resulting in walking and running gaits for several simulated bipedal actors~\cite{yu_learning_2018}. This work also demonstrates that with CL, a higher energy penalty can be applied to the magnitude of joint torques, without a detriment to learning. These examples are limited to simple terrain types, whereas our work investigates several complex environments.

Using a prior controller to guide exploration, and decreasing the dependence on the prior as training progresses has shown improved performance for robot navigation~\cite{rana_multiplicative_2020}. Our method combines ideas from Yu et al~\cite{yu_learning_2018}, and Rana et al~\cite{rana_multiplicative_2020}, where we stabilise the robot CoM by applying external forces, and also guide exploration using a simple prior controller applying forces to each joint. We apply these ideas, and increase the difficulty of the terrain, resulting in the traversal of complex terrain artifacts.

\section{Problem Description}
\label{sec:ch3_problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our biped has 12 torque controlled actuators, which we simulate in the 3D Pybullet environment~\cite{coumans_pybullet_2020}. The terrain types we investigate are flat surfaces, gaps, hurdles, stairs, and steps (shown in Fig~\ref{fig:terrains}). The state provided to each policy is $s_t=[rs_t, I_t]$, where $rs_{t}$ is the robot state and $I_t$ is the perception input at time $t$. Fig~\ref{fig:network} shows the robot state and perception input to our policy and the resulting torques that are applied to the agent in Pybullet. 

\noindent\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}, s_{right}, s_{left} ]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot, respectively (four Boolean contact points per foot), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the body Centre of Mass (CoM), $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the CoM and $h_{CoM,t}$ is the height of the robot from the walking surface. $s_{right}$ and $s_{left}$ are Boolean indicators of which foot is in the swing phase, and is updated when the current swing foot makes contact with the ground. All angles except joint angles are represented in the world coordinate frame. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\noindent\textbf{Perception}: Perception is provided from a depth sensor mounted to the robot base, with a resolution of $[48,48,1]$. The depth is a continuous value scaled between $0-1$, equating to a distance of 0.25 and $\SI{2}{\metre}$. The sensor moves with the body in translation and yaw, we assume we are provided with an artificial gimbal that keeps the sensor at a fixed roll and pitch. The sensor is pointed at the robot's feet (the feet are visible) and covers a distance at least two steps in front of the robot as suggested by Zaytsev~\cite{zaytsev_two_2015}. As sampling the sensor is computationally expensive, we reduce the sampling rate to $\SI{20}{\hertz}$, where the rest of the system operates at $\SI{120}{\hertz}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Deep Reinforcement Learning}
\label{sec:ch3_drl}
Curriculum learning in the context of reinforcement learning considers a set of tasks $i\in \mathcal{T}$~\cite{narvekar_curriculum_2020}. For each task $i$ there is a Markov Decision Process $\text{MDP}_i$, defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. We consider a task to be any instance of the curriculum, each policy will experience several tasks. For example, a task may be characterised by a particular gain $K_p$ that determines the magnitude of force applied to the robot, and the response of the environment to a particular torque will depend on the task. The goal of reinforcement learning is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. 

% defined by tuple $\{\mathcal{S}_i,\mathcal{A}_i, R_i, \mathcal{P}_i, \gamma\}$

\subsection{Proximal Policy Optimisation (PPO)}
We choose the on-policy algorithm Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017} to update our policy weights. As we wish to have a single policy (one for each terrain type) that evolves through several MDP's, it is preferred to use an on-policy algorithm. Actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is a torque applied to each joint. We use the implementation of PPO from OpenAI Baselines~\cite{dhariwal_openai_2017}.

\subsection{Simple Target Policy}
\label{sec:ch3_target_policy}
We design a simple target walking trajectory with simulator physics turned off. The target trajectory is a list of joint positions that create a visually accurate walking gait of $\approx\SI{1}{\metre/\second}$. The target trajectory is divided into two segments, one for each foot, with the first set of joint positions corresponding to the impact of the respective foot. Each time the robot foot makes contact with the walking surface, we initialise the target trajectory from the appropriate segment (e.g. if the right foot contacts the ground, we restart the target trajectory with the right segment). We increment the target trajectory with each timestep.


% The target policy in the reward, and in a PD controller in the guidance curriculum (both introduced below). At each timestep we increment the position in the target walking trajectory. To improve the accuracy of our reward predictions and guidance curriculum, we link the target policy to the robot at the point where the swing foot contacts the ground. In other words, our target policy that is an open-loop set of joint positions is now linked to the robot, essentially closing the loop each time the robot swing feet change, i.e. the swing foot for the target trajectory is updated when the swing foot for the robot is updated. We replace the need for a phase variable~\cite{peng_deepmimic_2018},~\cite{merel_hierarchical_2019}, and instead use a Boolean variable that indicates which foot is in swing, and which is in stance. Each terrain type uses the same target trajectory (flat, gaps, hurdles, steps, stairs).

% The target motion could instead be a set of joint positions from motion capture, provided the motion is broken into two segments (for each swing foot), and switching between segments occurs at the same time as the robot. 


\subsection{Reward}
Our reward is inspired by Peng et al in their work mimicking motion capture data~\cite{peng_deepmimic_2018}. Our reward function is the same for each policy, defined as:
\begin{equation}
r_t = goal + pos + vel + base + step + act
\end{equation}
where:
\begin{itemize}[leftmargin=*]
    \item $goal$ is the error between the current heading velocity and goal heading velocity $= w_{goal}\cdot \exp[-c_{goal}\cdot e_{goal}]$.
    \item $pos$ is the error between the joint positions and the target joint positions $= w_{pos}\cdot \exp[-c_{pos}\cdot e_{pos}]$.
    \item $vel$ is the error between the current joint velocities and the target joint velocities (target joint velocities are set to zero) $= w_{vel}\cdot \exp[-c_{vel}\cdot e_{vel}]$.
    \item $base$ is the CoM error from a target height, and zero roll and pitch positions $= w_{base}\cdot \exp[-c_{base}\cdot e_{base}]$. 
    \item $step$ encourages a symmetrical step length ($\text{left}_{step}\approx \text{right}_{step}$ when in contact) $= w_{step}\cdot \exp[-c_{step}\cdot e_{step}]$. 
    \item $act$ is a penalty for excessive torque for each of the $n$ joints $= w_{act}\sum_n(a_t^2)$. 
\end{itemize}

$e$ is the error of each respective element. Parameters $w$ and $c$ are tunable weights, which are fixed for all policies. 

\begin{figure}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=0.95\columnwidth]{images/ch3/network.png}
\includegraphics[width=0.75\columnwidth]{images/ch3/network.png}
\caption{Our policy is a neural network that takes the state (robot state and perception input) $s_t=[rs_t, I_t]$ and returns the torques applied to each joint $a_t$.}
\label{fig:network}
\vspace{-3mm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Curriculum Learning}
\label{sec:ch3_curriculum}
We design our curriculum with the rationale that dynamic platforms are usually supported (e.g. with a crane and harness) while controllers are developed. The learning process is divided into three stages, where $\mathcal{D}$ is the terrain curriculum (Stage 1), $\mathcal{F}$ is the guide curriculum (Stage 2), and $\mathcal{P}$ is the perturbation curriculum (Stage 3), where each stage represents a set of difficulties $\mathcal{D} = \{d_1, d_2, .., d_n\}$, $\mathcal{F} = \{f_1, f_2, .., f_n\}$, and $\mathcal{P} = \{p_1, p_2, .., p_n\}$. To begin learning we select $d_1, f_1$ and $p_1$, i.e all curriculum stages are at the lowest difficulty level. We then proceed to increment the difficulty of Stage 1 to its most difficult setting ($d_1 \rightarrow d_n$), then Stage 2 ($f_1 \rightarrow f_n$), and finally Stage 3 ($p_1 \rightarrow p_n$). During policy training, each increment to the next difficulty level occurs with a \textbf{success criteria}, which we define as the robot successfully reaching the end of the terrain sample three consecutive times. 

\subsection{Stage 1. Terrain Curriculum:}
In the terrain curriculum $\mathcal{D} = \{d_1, d_2, .., d_n\}$, the terrain difficulty is increased by incrementing $d$ up to a final difficulty $n$. In this stage, we apply the guide curriculum and perturbation curriculum at their lowest difficulty. The difficulty range  of each terrain is shown in Fig~\ref{fig:terrains}. Increases to the terrain difficulties are linear, incrementing terrain dimensions by a fixed amount each time the success criteria is achieved. 

% The terrain curriculum allows us to increase the difficulty of the terrain, where for some terrains (like hurdles) the policy fails to traverse the terrain at all, or for others (like gaps) the policy can take much longer to learn the required behaviour.

\subsection{Stage 2. Guide Curriculum:}
\label{sec:ch3_guide_curriculum}
Guide forces are employed from the beginning of training, tracking the target policy explained in Sec.~\ref{sec:ch3_target_policy}. Once the terrain curriculum has completed we begin the guide curriculum $\mathcal{F} = \{f_1, f_2, .., f_n\}$. Guide forces are applied to the CoM of the robot $f_c$ and to each joint $f_j$, where $f_1 = [f_c, f_j]$ is set to the lowest difficulty (highest guide forces).

$f_c$ is a PD controller that is applied to all 6 degrees of freedom of the CoM. 
\begin{equation}
f_c = K_{p_c} (p_{target} - p_{CoM}) + K_{d_c} ( v_{target} - v_{CoM})
\end{equation}
Where $K_{p_c}$ and $K_{d_c}$ are the gains, $p_{target}$ is the target position, $p_{CoM}$ is the observed position, $v_{target}$ is the target velocity, and $v_{CoM}$ is the observed velocity of the robot CoM. The target for the velocity in the forward $x$ direction is $\SI{1}{\meter/\second}$. The height $z$ target position is fixed at a nominal height, the $yaw$ targe follows the yaw of the terrain, and the position targets for the remaining degrees of freedom $y, roll, pitch$, are zero. All velocity targets, except for $x$ velocity, are set to zero. We liken this idea to fixing the robot to a small crane or gantry that supports the body of the robot, and moves forward at the desired velocity.
% This approach has shown reduced training times and increased asymptotic performance for multiple morphologies with a floating base~\cite{yu_learning_2018}.

$f_j$ is a second PD controller that is applied to all 12 actuators tracking our simple target trajectory. Forces applied to each joint are calculated from:
\begin{equation}
f_j = K_{p_j}( J_{t_{target}} - J_t ) + K_{d_j}(Jv_{t_{target}} - Jv_t )
\end{equation}
Where $K_{p_j}$ and $K_{d_j}$ are the gains, $J_{t_{target}}$ is the joint positions of the target trajectory, $J_t$ is the observed joint positions, $Jv_{t_{target}}$ is the target joint velocities, and $Jv_t$ is the observed joint velocities. We found that setting the target velocities to zero was sufficient for training (rather than estimating the target velocities with finite differences).

The guide curriculum involves reducing the guide forces in discrete steps following: $f_2 = 0.65 \cdot f_1$. The external forces are not provided as input to policy, and are considered an artifact of the environment. Once the guide forces decrease below a threshold ($f_n$) Stage 2 is complete.


\subsection{Stage 3. Perturbation Curriculum:}
% \subsection{Stage 3. Adding Perturbations}

Random perturbations applied during training have been shown to improve the robustness of walking policies~\cite{schulman_proximal_2017}. When the other curriculum stages are complete, we increase the magnitude of external perturbations with the perturbation curriculum, $\mathcal{P} = \{p_1, p_2, .., p_n\}$. Perturbations are an impulse force of random magnitude, applied to all 6 degrees of freedom of the CoM. At a random interval of approximately 2.5Hz, and for each DOF, we sample a perturbation force from a uniform distribution $(-p_1,p_1)$, where $p_1$ is increased linearly to the final value $p_n$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:ch3_experiments}


\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[Curved flat terrain initial angle starting at $20\degree$ and width $\SI{1.1}{\meter}$ ]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/flat1.png}}
\hfill
\subfloat[Curved flat terrain final angle
$120\degree$ and width $\SI{0.9}{\meter}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/flat.png}}
\hfill
\subfloat[Hurdles initial height $\SI{13}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/jumps1.png}}
\hfill
\subfloat[Hurdles final height $\SI{38}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/jumps.png}}
\hfill
\subfloat[Gaps initial length $\SI{10}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/gaps1.png}}
\hfill
\subfloat[Gaps final length $\SI{100}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/gaps.png}}
\hfill
\subfloat[Stairs initial height $\SI{1.7}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/stairs1.png}}
\hfill
\subfloat[Stairs final height $\SI{17}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/stairs.png}}
\hfill
\subfloat[Steps initial distance apart $\SI{4}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/steps1.png}}
\hfill
\subfloat[Steps final distance apart $\SI{40}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/steps.png}}
% \hfill
\caption{Our curriculum method traverses complex terrain types. The initial and final terrain sizes used in training are provided.}
\label{fig:terrains}
\vspace{-3mm}
\end{figure}
 
 
In this section we introduce the terrain types used for the test worlds (Sec~\ref{sec:ch3_terrain_types}), and present our simulation results. We evaluate Stage 1 (terrain curriculum), and Stage 2 (guide curriculum) of our method in Sec~\ref{sec:ch3_stage1_stage2}, before analysing Stage 3 (perturbation curriculum) in Sec~\ref{sec:ch3_stage3}. 

\subsection{Terrain Types}
\label{sec:ch3_terrain_types}
For all terrains there is a total of 10 steps of evenly spaced difficulty ($d_1 \rightarrow d_{10}$). The suite of terrains and range of difficulties is shown in Fig~\ref{fig:terrains}. Terrain conditions are selected to test our system with a broad range of scenarios. Examples include the Flat terrain that has curves that require the robot to turn (Fig~\ref{fig:terrains}(a-b)), the Hurdles terrain (Fig~\ref{fig:terrains}(c-d)) that forces the robot to take a high step, and the Steps terrain (Fig~\ref{fig:terrains}(i-j)) where the robot must step with a lateral component.

Each policy is trained on a scenario with two consecutive instances of the same terrain artifact, where an instance refers to a single gap or hurdle, or a random number ($5-8$) of stairs or steps. We found that training on two consecutive artifacts performed better during evaluation than a sample with a single artifact. We evaluate all methods on a sequence of seven consecutive instances of the same terrain artifact at maximum difficulty, making up one trial. We run each policy for 500 trials and record the distance travelled as a percentage of total distance, which we use as our evaluation metric. For all experiments no external disturbance forces are applied when evaluating a policy, except for the perturbation evaluation section of Sec~\ref{sec:ch3_intense}, where perturbations are applied during evaluation. For all experiments, the terrain difficulty at evaluation is set to the highest difficulty (10), except for the domain difficulty section of Sec~\ref{sec:ch3_diff}, where we evaluate our policies on a range of difficulties.


% \subsubsection{Ablation Study}
\subsection{Stage 1 and Stage 2 Analysis}
\label{sec:ch3_stage1_stage2}

\begin{figure*}[ht]
\vspace{-2mm}
\centering
\subfloat[Flat]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_flat.png}}\quad
\subfloat[Gaps]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_gaps.png}}\quad
\subfloat[Hurdles]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_jumps.png}}

\medskip
\vspace{-5mm}
\subfloat[Stairs]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_stairs.png}}\quad
\subfloat[Steps]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_steps.png}}

\caption{Percentage of total distance travelled, evaluated during training showing the comparisons of the Stage 1 and Stage 2 ablation study.}
\label{fig:compare}
\end{figure*}
\begin{table}[h!]
    \vspace{-2mm}
    % \vspace{-45.5mm}https://www.overleaf.com/project/5efc80ce9e222200014e6c84
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         No Stage 1, No Stage 2       & 79.4           & 12.8          & 10.3          & 12.4          & 13.4 \\
         Stage 1, No Stage 2          & 5.5  & 5.3          & 7.1          &  11.5          & 14.2 \\
         No Stage 1, Stage 2          & 88.7           &  1.5          &  1.2          &  43.9          &   1.9 \\
         Stage 1, Stage 2     &  \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}   \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study of Stage 1 and Stage 2 showing percentage of total distance travelled, computed with 500 trials.}
    \label{tab:results_ablation}
    \vspace{-5mm}
\end{table}

This section analyses the effect of Stage 1 and Stage 2 on policy performance in an ablation study. We also investigate three individual aspects of our method: the effect of using success criteria to decay forces for Stage 2, removing the guiding forces applied to the joints, and not linking the target policy to the robot state. For all experiments in this section, the external perturbations are set at the lowest level $p_1$ throughout training, with no external perturbations applied during evaluation.

\subsubsection{Ablation study of Stage 1 and Stage 2}
We investigate the benefit of Stage 1 and Stage 2 of our method by removing one or both stages.

\begin{itemize}[leftmargin=*]

\item\textbf{No Stage 1, No Stage 2:}  The terrain starts at maximum difficulty. Guiding forces are not applied to the robot CoM or joints.

\item\textbf{Stage 1, No Stage 2:} The terrain curriculum is active. Guiding forces are not applied to the robot CoM or joints.

\item\textbf{No Stage 1, Stage 2:} The terrain starts at maximum difficulty. Guide curriculum is active.

\item\textbf{Stage 1, Stage 2:} Both the terrain curriculum and guide curriculum are active. 
\end{itemize}


Fig~\ref{fig:compare} shows the evolution of the percentage of total distance achieved with respect to the number of training steps. We perform this evaluation periodically by pausing training, removing any external forces, setting the terrain difficulty to maximum, and running 500 trials. The final evaluation is provided in Table~\ref{tab:results_ablation}. We can see from Fig~\ref{fig:compare}, and Table~\ref{tab:results_ablation} that both Stage 1 and Stage 2 are important for the development of successful policies for the selected terrain types. Stage 1 is necessary for all terrains except for Flat and Stairs. \textbf{No Stage 1, Stage 2} on the Stairs terrain results in the traversal of a significant portion of the test world (43.9\%). Without Stage 2 the agent learns a one leg hopping gait. For all terrains this gait is unstable (the agent is unable to balance beyond the first hop), except for \textbf{No Stage 1, No Stage 2} on the Flat terrain where the agent successfully traverses 79.4\% of the test world by hopping on one leg. The lowest performance is found with \textbf{No Stage 1, Stage 2} for the Gap, Hurdle, and Steps terrains. For these terrain types, without the terrain curriculum the robot is unable to reach the success criteria required to lower the guidance forces. When evaluated without guide forces, the robot is unable to balance and achieves a much lower result than without any curriculum at all.

\subsubsection{Effect of using success criteria to decay forces}
\begin{table}[h!]
    % \vspace{-45.5mm}
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Force decay with success   &   89.8            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & 58.1  \\  
         Continuous force decay   &  \textbf{97.7}            & 15.2          & 22.8          & 38.7           & \textbf{58.3}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Comparison of force decay used in Stage 2 as percentage of total distance travelled, computed with 500 trials.}
    \label{tab:results_decay}
    \vspace{-2mm}
\end{table}
This section investigates the choice of decay on guidance forces (Stage 2). We compare our method of decay that is dependent on agent success, to decaying the guiding forces at fixed intervals irrespective of the agent success. We found that decaying the guiding forces by $0.995$ each episode was a similar rate to our decay approach (introduced in Sec~\ref{sec:ch3_guide_curriculum}). The results in Table ~\ref{tab:results_decay} show that for the Gaps, Hurdles, and Stairs terrain types, decaying the guide forces continuously performed significantly worse on the test world than our method (Gaps 15.2\% compared to 69.5\%, Hurdles 22.8\% compared to 79.0\%, Stairs 38.7\% compared to 55.8\%). For the Flat and Steps terrain types the continuous decay performed slightly better than decay based on agent success (Flat 89.8\% compared to 97.7\%, Steps 58.1\% compared to 58.3\%). We suspect a decay rate tuned for each terrain type would match or improve the performance of our method for all terrains, though introduces undesirable hand tuning.

\subsubsection{Effect of guide forces on CoM only}
\begin{table}[h!]
    % \vspace{-45.5mm}
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
        Forces on CoM and joints   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
         Forces on CoM only   &  81.6            &  8.6          &  2.7          & 12.2          & 1.0 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Effect of applying guide forces to CoM only, shown as a percentage of total distance travelled, computed with 500 trials.}
    \label{tab:results_guide}
    \vspace{-2mm}
\end{table}
We test the effect of removing the guiding forces on the joints, instead only apply forces to the CoM during Stage 2 Guide Curriculum. We found guiding forces applied only to the base performed worse on all terrains than also applying guiding forces to the joints (Table~\ref{tab:results_guide}). Notably low scores (Gaps 8.6\%, Hurdle 2.7\%, Steps 1.0\%) suggest the agent was unable to decay the guide forces on the CoM, so unable to support itself during evaluation.

\subsubsection{Effect of not linking target policy}
\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}    
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Link to Target Policy   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
         No link to Target Policy          &    54.6           & 38.9          & 40.9          & 28.8          &  15.2 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Effect of linking the target trajectory to the robot, shown as a percentage of total distance travelled, computed with 500 trials.}
    \label{tab:results_no_link}
    \vspace{-2mm}
\end{table}
We investigate the effect of removing the link between the target policy and the robot. Linking is introduced in Sec~\ref{sec:ch3_target_policy}, and refers to resetting the target trajectory with the respective segment (left or right) each time a foot of the robot makes contact with the ground. When the target trajectory is not linked to the robot, the target joint positions are initialised only at the first step. Advancing the target trajectory occurs with each timestep, without any feedback from the robot. We found that not linking the target trajectory with the robot reduced the performance of all terrains in comparison to our method as seen in Table~\ref{tab:results_no_link}. While some policies were able to successfully traverse portions of the test world (Flat 54.6\%, Gaps 38.9\%, Hurdles 40.9\%, Stairs 28.8\%), others such as Steps (15.2\%) performed poorly. We suspect that policies requiring more precise foot placement benefit the most from having the target trajectory linked with the robot steps. This simple method allows us to train policies following a target, without providing the policy with a phase variable (a limitation of related work~\cite{peng_deepmimic_2018},~\cite{merel_hierarchical_2019}). Instead the policy can infer the phase of the walk cycle from joint positions and feet contact information.

\subsection{Stage 3 Analysis}
\label{sec:ch3_stage3}


We now analyse the final stage of our curriculum learning method. In the perturbation curriculum the maximum magnitude of external forces is increased from an initial disturbance of $p_1 = \SI{50}{\newton}$ to a final disturbance of $p_n = \SI{1000}{\newton}$, where perturbations are sampled uniformly for each degree of freedom of the CoM from $\mathcal{U}(-p, p)$. Fig~\ref{fig:stage3} shows the average episode reward for all three stages of training for all terrain types. We can see that Stage 1 completes early in training for all terrain types. Drops in reward are seen early in Stage 2 where the majority of guidance forces are removed, then we see a gradual increase as the agent learns to act without guidance. In Stage 3 we see a large drop in return as the perturbations are increased. At this point in training the agent is operating in the hardest conditions (terrain at highest difficulty, no guiding forces, large perturbations applied to the CoM). We also show the episode reward for policies trained without any part of the curriculum (solid line), and observe the reward for policies trained without a curriculum is much lower than the policies trained with our method.

From Table~\ref{tab:results_stage3} we can see that adding the perturbation curriculum improves performance slightly for all terrain types except the Hurdles terrain (58.5\% compared to 79.0\%). The Hurdles terrain takes the longest for Stage 1 and Stage 2 to complete (as shown in Fig~\ref{fig:stage3}), and therefore has the least time to train with large perturbations. 


\begin{figure}[tb!]
\vspace{-10mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch3/reward.png}
% \includegraphics[width=9 cm, height=7 cm]{images/ch3/reward.png}
\vspace{-10mm}
\caption{Episode rewards for our method (Stage 1, Stage 2, and Stage 3), for each terrain type. The completion of each stage is shown with a circle and change in line colour and type. The first segment (lightest colour, dotted line) is Stage 1, the middle segment shows Stage 2 (dash-dotted line), and the final segment (darkest colour, dashed line) shows the rewards when the perturbation curriculum is applied. The solid coloured lines are the policies trained without a curriculum.}
\label{fig:stage3}
\vspace{-3mm}
\end{figure}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Stage 1 \& 2    &   89.8            & 69.5           &  \textbf{79.0}          & 55.8 & 58.1  \\
         Stage 1, 2 \& 3   &  \textbf{99.9}    & \textbf{72.3}  & 58.5  & \textbf{57.6}  & \textbf{60.5}  \\
        %  Large (1000N)   &  93.0    & 59.5  & 0.0  & 18.9  & 13.2  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Stage 1 \& 2, and Stage 1,2 \& 3 evaluated as percentage of total distance travelled, computed with 500 trials, with no perturbations applied during evaluation.}
    \label{tab:results_stage3}
    \vspace{-2mm}
\end{table}

\subsubsection{Effect of perturbation intensity}
\label{sec:ch3_intense}
In this section we investigate the robustness of our method by applying perturbations during the evaluation. The evaluation perturbation forces are sampled uniformly from $(-\SI{1000}{\newton}, \SI{1000}{\newton})$ and applied to the CoM of the robot. We compare training with small perturbations, training with large perturbations, and our perturbation curriculum.

\begin{itemize}[leftmargin=*]

\item\textbf{Small:} Small perturbations are applied throughout training, sampled uniformly from $(\SI{-50}{\newton}, \SI{50}{\newton})$. This is the same as Stage 1 \& 2.

\item\textbf{Large:} Maximum perturbations are applied throughout training, sampled uniformly from $(\SI{-1000}{\newton}, \SI{1000}{\newton})$.

\item\textbf{Curriculum:} We show the results of the perturbation curriculum (Stage 3), with perturbations applied during evaluation.

\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
         & Flat & Gap & Hurdle & Stairs & Steps \\ 
        %  \multicolumn{6}{l}{\textbf{Curriculum Stage 3 Analysis}}  \\
         \hline
         Small (50N) & 45.9          & 17.8          & 28.5           & 31.6          & 21.7     \\
         Large (1000N) & 81.2          & 18.0          &  21.3           & 22.7          &  9.4   \\
         Curriculum (50N to 1000N)  & \textbf{87.1}          & \textbf{35.7}          & \textbf{28.6}  & \textbf{45.6} & \textbf{24.5}   \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Effect of perturbations during training, shown as a percentage of total distance travelled, computed with 500 trials. Each method is evaluated with maximal perturbations.}
    \label{tab:results_perturbations}
    \vspace{-2mm}
\end{table}

From Table~\ref{tab:results_perturbations}, we can see that our perturbation curriculum (Stage 3) performs best on all terrains compared with applying small (Stage 1 and Stage 2), and large forces throughout training. We notice slight performance gains for Hurdles (28.5\% compared to 28.6\%) and Steps (21.7\% compared to 24.5\%), and larger improvements with Flat (45.9\% compared to 87.1\%), Gaps (17.8\% compared to 35.7\%), and Stairs (31.6\% compared to 45.6\%). For policies trained with large disturbances throughout training we observe reduced performance compared with our method. Our results show that a perturbation curriculum allows for large perturbations during training, with improved outcomes compared to large forces applied for the entirety of training. This methodology can be applied to scenarios where training with perturbations can improve robustness (e.g. simulation to real transfer).

\subsubsection{Effect of test domain difficulty}
\label{sec:ch3_diff}

We test the generalisation of our method (Stages 1, 2 \& 3) in a final evaluation that compares policy performance on terrains that are less difficult, and terrains that are more difficult than the final terrain experienced during training.

\begin{itemize}[leftmargin=*]

\item\textbf{Easy Difficulty:} We evaluate our policies with the easy terrain difficulty $d_1$. 


\item\textbf{Reduced Difficulty:} We evaluate our policies with a terrain difficulty 20\% lower than the final difficulty experienced in training ($d_8$). 

\item\textbf{Normal Difficulty:} We evaluate our policies with the final terrain difficulty experienced in training ($d_{10}$). 

\item\textbf{Increased Difficulty:} We evaluate our policies with a terrain difficulty 20\% higher than the final difficulty experienced in training ($d_{12}$). 
 
\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
         & Flat & Gap & Hurdle & Stairs & Steps \\              
         \hline

        Easy Difficulty           & \textbf{100.0} & 45.3            & 24.5       & \textbf{88.1}          & 12.5   \\
        Reduced Difficulty      & \textbf{100.0} & 15.4            & \textbf{62.3}       & 80.2          & \textbf{87.4}   \\
        Normal Difficulty          & 99.9    & \textbf{72.3}  & 58.5  & 57.6  & 60.5   \\
        Increased Difficulty         & 94.5          & 11.5          & 32.5   & 50.5          &  26.7   \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{The effect of evaluating with terrain difficulty levels that are reduced and increased from the final terrain difficulty reached during training. Shown as a percentage of total distance travelled, computed with 500 trials.}
    \label{tab:results_difficulty}
    \vspace{-2mm}
\end{table}

From Table~\ref{tab:results_difficulty}, we can see how policies adapt to the terrain during training, with some policies (Gaps, Hurdles, Steps) performing poorly when evaluated with an easy terrain difficulty. The Gaps policy has overfit to the final difficulty, performing poorly on reduced (15.4\%) or increased (11.5\%) difficulty. For all other terrain types we can see improved performance on the reduced difficulty terrain, and comparable performance for some terrain types with increased difficulty (Flat 94.5\% compared to 99.9\%, Stairs 50.5\% compared to 57.6\%), suggesting generalisation in these cases. An alternative training strategy that involves training with terrains of multiple difficulties may improve policy performance over a wider range of terrain difficulties.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:ch3_conclusion}
We demonstrate a curriculum learning approach for developing DRL policies for a torque controlled biped traversing complex terrain artifacts. Our agent was successfully able to traverse several difficult terrain types where removal of any component of our multi-stage curriculum resulted in decreased performance or failure to learn. A key idea of our method is that a simple target policy is sufficient to train a policy on various terrains, where much of the behaviour is acquired from the terrain itself.

A limitation of our work is that the curriculum is manually tuned, whereas an adaptive curriculum may be able to learn harder tasks, which is left for future work. We will also investigate methods for switching between these policies such that we can expand the capabilities of our platform.


==> old/Ch3_pdf_old.tex <==




% efficient visuo-motor behaviours. the importance of switching between controllers.  research question 2  RQ1, and RQ2. Statement about efficiency, statement about RQ2 


% Biped, and titan, stairs, steps, hurdles, gaps, and small gaps. Simluation and real world. Dyanmic and static. Learned and traditional controllers.

% Efficiency - using expert trajectories, reward shaping, and reliable switching. 







% This chapter introduces two papers that investigate RQ1, and the first experiments investigating RQ2.  provide solutions to RQ1, , both that investigate the efficiency of learning locomotion behaviours (RQ1), and RQ). Behaviours include biped stuff and titan stuff. Answer to research question 1: \textit{How can complex visuo-motor locomotion behaviours be learned efficiently?}. This chapter also begins the investigation into research question 2: \textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}. Titan switching stuff

% Biped behaviours method

% Summary of Results

% Titan gaps behaviour

% Titan behaviour selection

% Summary of Results

% biped Conclusion wrt research question 1

% titan Conclusion wrt research question 1

% titan Conclusion wrt research question 2

% % \section{Guided Curriculum Learning for Walking Over Complex Terrain}
% % \label{sec:gcl}

% One idea per paragraph. First sentence summarises the whole paragraph, last sentence leads into the next.
% Traditional methods, DRL methods. How do we address the limitations of DRL methods.

% DRL methods have demonstrated the emergence of complex behaviours for locomotion agents [\cite{heess_emergence_2017}], however DRL typically relies on a high number of samples of the agent interacting with the environment. For locomotion over complex obstacles, learning is further complicated by the necessity of perception and the tight coupling to action (visuo-motor policies). Furthermore, naive exploration strategies can result in local minima that may prevent an agent from discovering the necessary behaviour. To reduce these inefficiencies, additional information can be provided to the agent, for example by providing expert demonstrations [\cite{peng_deepmimic_2018}]. While expert knowledge helps to guide the agent out of local minima, expensive skilled demonstrations are required that are close to the desired behaviour for each obstacle. Additionally, instilling expert knowledge by means of reward shaping also requires a large number of samples. This research question investigates how complex behaviours can be achieved without knowing exactly how an expert would perform the behaviour, and by learning with far fewer samples than needed by typical DRL methods.

% Reliable bipedal walking over complex terrain
% is a challenging problem, using a curriculum
% can help learning. Curriculum learning is the
% idea of starting with an achievable version
% of a task and increasing the diculty as a
% success criteria is met. We propose a 3-
% stage curriculum to train Deep Reinforcement
% Learning policies for bipedal walking over
% various challenging terrains. In the rst stage,
% while applying forces from a target policy to
% the robot joints and base, the agent starts
% on an easy terrain and the terrain diculty
% is gradually increased. In the second stage,
% the guiding forces are gradually reduced to
% zero. Finally, in the third stage, random
% perturbations with increasing magnitude are
% applied to the robot base, so the robustness
% of the policies are improved. In simulation
% experiments, we show that our approach is
% eective in learning separate walking policies
% for ve terrain types: 
% at, hurdles, gaps, stairs,
% and steps. Moreover, we demonstrate that in
% the absence of human demonstrations, a simple
% hand designed walking trajectory is a sucient
% prior to learn to traverse complex terrain types.
% In ablation studies, we show that taking out
% any one of the three stages of the curriculum
% degrades the learning performance

% We demonstrate a curriculum learning approach for
% developing DRL policies for a torque controlled biped
% traversing complex terrain artifacts. Our agent was
% successfully able to traverse several dicult terrain types
% where removal of any component of our multi-stage
% curriculum resulted in decreased performance or failure
% to learn. A key idea of our method is that a simple target
% policy is sucient to train a policy on various terrains,
% where much of the behaviour is acquired from the terrain
% itself.

% A limitation of our work is that the curriculum is
% manually tuned, whereas an adaptive curriculum may be
% able to learn harder tasks, which is left for future work.
% We will also investigate methods for switching between
% these policies such that we can expand the capabilities
% of our platform.

% Abstract—The DARPA subterranean challenge requires
% teams of robots to traverse difficult and diverse underground
% environments. Traversing small gaps is one of the challenging
% scenarios that robots encounter. Imperfect sensor information
% makes it difficult for classical navigation methods, where behaviours
% require significant manual fine tuning. In this paper we
% present a deep reinforcement learning method for autonomously
% navigating through small gaps, where contact between the robot
% and the gap may be required. We first learn a gap behaviour
% policy to get through small gaps (only centimeters wider than
% the robot). We then learn a goal-conditioned behaviour selection
% policy that determines when to activate the gap behaviour
% policy. We train our policies in simulation and demonstrate
% their effectiveness with a large tracked robot in simulation and
% on the real platform. In simulation experiments, our approach
% achieves 93% success rate when the gap behaviour is activated
% manually by an operator, and 63% with autonomous activation
% using the behaviour selection policy. In real robot experiments,
% our approach achieves a success rate of 73% with manual
% activation, and 40% with autonomous behaviour selection.
% While we show the feasibility of our approach in simulation,
% the difference in performance between simulated and real world
% scenarios highlight the difficulty of direct sim-to-real transfer
% for deep reinforcement learning policies. In both the simulated
% and real world environments alternative methods were unable
% to traverse the gap.

% We present a reinforcement learning method for developing
% a gap behaviour policy to traverse small gaps. We also
% learn a behaviour selection policy that determines when to
% autonomously activate the gaps behaviour (when a goal is
% through a small gap). We show that our gap behaviour policy
% is more reliable than the current stack of tuned behaviours,
% both in simulation (93% compared to 0%) and on a real
% robot (73% compared to 0%), though we recognise that the
% autonomous behaviour selection needs to be more robust
% before it can be relied upon for fully autonomous integration
% (success rates of 63% in simulation and 40% in real trials).
% We have identified a limitation of transferring from the
% simulation to the real robot by observing the way the robot
% gets stuck on a protruding door frame. Future work will look
% at improving the reliability of the system for a wider range of
% gap scenarios, including updating the simulation to include
% these cases, and adding noise to the occupancy map during
% training to mimic the noisy output of the real perception
% stack.
% A limitation of our method occurs when gaps are smaller
% than the robot. It is likely in these situations the gap
% behaviour policy will still be selected for operation and try
% to traverse the gap. Methods to handle these scenarios will
% be considered in future work.

% Behaviours that allow a dynamic biped to traverse difficult obstacles are challenging to design. Policies that rely on perception, for example to adjust footstep placement and body pose to align a robot with an obstacle, are known as visuo-motor policies. Typically DRL methods require many samples to learn visuo-motor policies. For complex behaviours, policies are subject to local minima where with standard random exploration techniques the agent would never find a way to traverse the obstacle.

% Our approach to efficiently learn these behaviours is to apply curriculum learning (CL). Specifically, we use guided curriculum learning (GCL), a three stage curriculum learning method introduced by this work. We start with a trajectory of joint positions of an expert walking, and apply this expert by means of \textbf{guide forces} using a proportional differential (PD) controller on the robot joints, and external forces on the center of mass (CoM) to move the robot forward. The expert is a rough guide to walking and could be a set of joint positions obtained from motion capture. We train a DRL policy using proximal policy optimisation (PPO) [\cite{schulman_proximal_2017}] using the implementation from \cite{baselines}. Starting with guide forces active, the three stages of GCL, as summarized in Fig.\ref{fig:cha3_fig1}, are:

% \begin{itemize}
%     \item Terrain curriculum: increasing the difficulty of the terrain
%     \item Guide curriculum: reducing the guide forces
%     \item Perturbation curriculum: increasing the external perturbations to improve robustness
% \end{itemize}

% The difficulty of each stage is increased as the robot reaches a milestone. The milestone we use for all difficulty levels in all stages is for the robot to successfully traverse the terrain in the current stage and difficulty three consecutive times. When a stage reaches its most difficult setting, we progress to the next stage.


% Fig.\ref{fig:cha3_fig2} shows the inputs and outputs of our policy. We use the Pybullet environment [\cite{coumans_pybullet_2020}] to showcase our method on a torque controlled biped. A depth image and robot state a provided to a deep neural network policy. The policy output is the joint torques applied to the robot. Fig.\ref{fig:cha3_fig3} shows the initial and final positions of each investigated obstacle (the terrain curriculum of GCL). 

 
 
% We perform a detailed analysis of our curriculum method. We include an ablation of the terrain and guide curriculum (Fig. \ref{fig:ch3_compare}) to show that without either stage, learning is impaired. We investigate several key design decisions, such as continuous vs discrete force decay (Table. \ref{tab:ch3_results_decay}), applying guide forces to the centre of mass (CoM) only (Table. \ref{tab:ch3_results_guide}), and progressing the expert trajectory with swing foot contact (Table. \ref{tab:ch3_results_no_link}).

% The optimal way to decrease guide forces requires further investigation, with the discrete decay with success being the best option for 3 of the 5 terrain times. There are clear benefits to applying forces on the joints as well as the CoM, and for linking the target policy, we can seen an improvement in total distance travelled for all terrain types.  

% Table. \ref{tab:ch3_results_stage3} shows the improvements on robustness of including the perturbation curriculum. Fig. \ref{fig:ch3_stage3} shows the effect of each curriculum stage on training, in comparison to training without a curriculum (solid lines). We also show the effect of having small or large perturbations during training, and show that using a curriculum on disturbances provides a balance between robustness and inability to train (Table \ref{tab:ch3_results_perturbations}). Finally, Table \ref{tab:ch3_results_difficulty} shows the effect of terrain difficulty as a percentage of total distance travelled.



% What does this table add?
% \begin{table}[h!]
%     \vspace{-2mm}
%     % \vspace{-45.5mm}https://www.overleaf.com/project/5efc80ce9e222200014e6c84
%     \centering
%     \begin{adjustbox}{max width=1.0\columnwidth}  
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%          No Stage 1, No Stage 2       & 79.4           & 12.8          & 10.3          & 12.4          & 13.4 \\
%          Stage 1, No Stage 2          & 5.5  & 5.3          & 7.1          &  11.5          & 14.2 \\
%          No Stage 1, Stage 2          & 88.7           &  1.5          &  1.2          &  43.9          &   1.9 \\
%          Stage 1, Stage 2     &  \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}   \\
%     \hline
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Ablation study of Stage 1 and Stage 2 showing percentage of total distance travelled, computed with 500 trials.}
%     \label{tab:results_ablation}
%     \vspace{-5mm}
% \end{table}

% \begin{table}[h!]
%     % \vspace{-45.5mm}
%     \vspace{-2mm}
%     \centering
%     % \begin{adjustbox}{max width=1.0\columnwidth}  
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%          Force decay with success   &   89.8            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & 58.1  \\  
%          Continuous force decay   &  \textbf{97.7}            & 15.2          & 22.8          & 38.7           & \textbf{58.3}  \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{Comparison of force decay used in Stage 2 as percentage of total distance travelled.}
%     \label{tab:ch3_results_decay}
%     \vspace{-2mm}
% \end{table}

% \begin{table}[h!]
%     % \vspace{-45.5mm}
%     \vspace{-2mm}
%     \centering
%     % \begin{adjustbox}{max width=1.0\columnwidth}  
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%         Forces on CoM and joints   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
%          Forces on CoM only   &  81.6            &  8.6          &  2.7          & 12.2          & 1.0 \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{Effect of applying guide forces to CoM only, shown as a percentage of total distance travelled.}
%     \label{tab:ch3_results_guide}
%     \vspace{-2mm}
% \end{table}

% \begin{table}[h!]
%     \vspace{-2mm}
%     \centering
%     % \begin{adjustbox}{max width=1.0\columnwidth}    
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%          Link to Target Policy   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
%          No link to Target Policy          &    54.6           & 38.9          & 40.9          & 28.8          &  15.2 \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{Effect of linking the target trajectory to the robot, shown as a percentage of total distance travelled.}
%     \label{tab:ch3_results_no_link}
%     \vspace{-2mm}
% \end{table}



% \begin{table}[h!]
%     \vspace{-2mm}
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c}
%     % \begin{adjustbox}{max width=1.0\columnwidth}
%     \begin{tabular}{cccccc}
%          & Flat & Gap & Hurdle & Stairs & Steps \\ 
%         %  \multicolumn{6}{l}{\textbf{Curriculum Stage 3 Analysis}}  \\
%          \hline
%          Small (50N) & 45.9          & 17.8          & 28.5           & 31.6          & 21.7     \\
%          Large (1000N) & 81.2          & 18.0          &  21.3           & 22.7          &  9.4   \\
%          Curriculum (50N to 1000N)  & \textbf{87.1}          & \textbf{35.7}          & \textbf{28.6}  & \textbf{45.6} & \textbf{24.5}   \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{Effect of perturbations during training, shown as a percentage of total distance travelled.}
%     \label{tab:ch3_results_perturbations}
%     \vspace{-2mm}
% \end{table}

% \begin{table}[h!]
%     \vspace{-2mm}
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c}
%     % \begin{adjustbox}{max width=1.0\columnwidth}
%     \begin{tabular}{cccccc}
%         % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
%          & Flat & Gap & Hurdle & Stairs & Steps \\              
%          \hline

%         Easy Difficulty           & \textbf{100.0} & 45.3            & 24.5       & \textbf{88.1}          & 12.5   \\
%         Reduced Difficulty      & \textbf{100.0} & 15.4            & \textbf{62.3}       & 80.2          & \textbf{87.4}   \\
%         Normal Difficulty          & 99.9    & \textbf{72.3}  & 58.5  & 57.6  & 60.5   \\
%         Increased Difficulty         & 94.5          & 11.5          & 32.5   & 50.5          &  26.7   \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{The effect of evaluating with terrain difficulty levels that are reduced and increased from the final terrain difficulty reached during training.}
%     \label{tab:ch3_results_difficulty}
%     \vspace{-2mm}
% \end{table}





% \chapter[Passing Through Narrow Gaps with DRL]{Passing Through Narrow Gaps with Deep Reinforcement Learning}
% \label{cha:ch5}
% Motivation/contribution/abstract -----------------------
% \section{Passing Through Narrow Gaps with Deep Reinforcement Learning}
% \label{sec:gaps}


% \chapter[Guided Curriculum Learning for Walking Over Complex Terrain]{Guided Curriculum Learning for Walking Over Complex Terrain}
\chapter[Efficient Learning of Locomotion Behaviours]{Efficient Learning of Behaviours for Robot Locomotion Over Difficult Obstacles}
   
% \item \textbf{Research Question 1: \textit{How can complex visuo-motor locomotion behaviours be learned efficiently, without knowing exactly how an expert would perform the action?}}

\label{cha:ch3}
% Motivation/contribution/abstract -----------------------

% Three paragraphs: Explain motivation, what you did, results

% Final part: What research question you answered, what the contribution was, and what the publication was.

This chapter investigates research question 1: \textit{How can complex visuo-motor locomotion behaviours be learned efficiently?}. The second part of this chapter begins the investigation into research question 2: \textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}. 

% \section{Guided Curriculum Learning for Walking Over Complex Terrain}
% \label{sec:gcl}




Behaviours that allow a dynamic biped to traverse difficult obstacles are challenging to design. Policies that rely on perception, for example to adjust footstep placement and body pose to align a robot with an obstacle, are known as visuo-motor policies. Typically DRL methods require many samples to learn visuo-motor policies. For complex behaviours, policies are subject to local minima where with standard random exploration techniques the agent would never find a way to traverse the obstacle.

Our approach to efficiently learn these behaviours is to apply curriculum learning (CL). Specifically, we use guided curriculum learning (GCL), a three stage curriculum learning method introduced by this work. We start with a trajectory of joint positions of an expert walking, and apply this expert by means of \textbf{guide forces} using a proportional differential (PD) controller on the robot joints, and external forces on the center of mass (CoM) to move the robot forward. The expert is a rough guide to walking and could be a set of joint positions obtained from motion capture. We train a DRL policy using proximal policy optimisation (PPO) [\cite{schulman_proximal_2017}] using the implementation from \cite{baselines}. Starting with guide forces active, the three stages of GCL, as summarized in Fig.\ref{fig:cha3_fig1}, are:

\begin{itemize}
    \item Terrain curriculum: increasing the difficulty of the terrain
    \item Guide curriculum: reducing the guide forces
    \item Perturbation curriculum: increasing the external perturbations to improve robustness
\end{itemize}

The difficulty of each stage is increased as the robot reaches a milestone. The milestone we use for all difficulty levels in all stages is for the robot to successfully traverse the terrain in the current stage and difficulty three consecutive times. When a stage reaches its most difficult setting, we progress to the next stage.

\begin{figure*}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.85\columnwidth]{images/ch3/fig2.png}
\caption{Three stage curriculum learning method to train a biped to traverse complex terrain obstacles.}
\label{fig:cha3_fig1}
\vspace{-3mm}
\end{figure*}

% \begin{figure}[htb!]
\begin{figure}[h!tb]
% \vspace{2mm}
\centering
% \includegraphics[width=0.95\columnwidth]{images/ch3/network.png}
\includegraphics[width=0.8\columnwidth]{images/ch3/network.png}
\caption{Overview of our system.}
\label{fig:cha3_fig2}
\vspace{-3mm}
\end{figure}

% \begin{figure}[htb!]
\begin{figure}[h!tb]
% \vspace{2mm}
\centering
\subfloat[Curved terrain initial angle starting at $20\degree$ and width $\SI{1.1}{\meter}$ ]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/flat1.png}}
% \hfill
\hspace{0.5cm}
\subfloat[Curved terrain final angle
$120\degree$ and width $\SI{0.9}{\meter}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/flat.png}}
\hfill
\subfloat[Hurdles initial height $\SI{13}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/jumps1.png}}
% \hfill
\hspace{0.5cm}
\subfloat[Hurdles final height $\SI{38}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/jumps.png}}
\hfill
\subfloat[Gaps initial length $\SI{10}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/gaps1.png}}
% \hfill
\hspace{0.5cm}
\subfloat[Gaps final length $\SI{100}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/gaps.png}}
\hfill
\subfloat[Stairs initial height $\SI{1.7}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/stairs1.png}}
% \hfill
\hspace{0.5cm}
\subfloat[Stairs final height $\SI{17}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/stairs.png}}
\hfill
\subfloat[Steps initial distance apart $\SI{4}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/steps1.png}}
% \hfill
\hspace{0.5cm}
\subfloat[Steps final distance apart $\SI{40}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/steps.png}}
% \hfill
\caption{The initial and final terrain difficulties used in the first stage of training.}
\label{fig:cha3_fig3}
\vspace{-3mm}
\end{figure}


Fig.\ref{fig:cha3_fig2} shows the inputs and outputs of our policy. We use the Pybullet environment [\cite{coumans_pybullet_2020}] to showcase our method on a torque controlled biped. A depth image and robot state a provided to a deep neural network policy. The policy output is the joint torques applied to the robot. Fig.\ref{fig:cha3_fig3} shows the initial and final positions of each investigated obstacle (the terrain curriculum of GCL). 

 
 
We perform a detailed analysis of our curriculum method. We include an ablation of the terrain and guide curriculum (Fig. \ref{fig:ch3_compare}) to show that without either stage, learning is impaired. We investigate several key design decisions, such as continuous vs discrete force decay (Table. \ref{tab:ch3_results_decay}), applying guide forces to the centre of mass (CoM) only (Table. \ref{tab:ch3_results_guide}), and progressing the expert trajectory with swing foot contact (Table. \ref{tab:ch3_results_no_link}).

% The optimal way to decrease guide forces requires further investigation, with the discrete decay with success being the best option for 3 of the 5 terrain times. There are clear benefits to applying forces on the joints as well as the CoM, and for linking the target policy, we can seen an improvement in total distance travelled for all terrain types.  

Table. \ref{tab:ch3_results_stage3} shows the improvements on robustness of including the perturbation curriculum. Fig. \ref{fig:ch3_stage3} shows the effect of each curriculum stage on training, in comparison to training without a curriculum (solid lines). We also show the effect of having small or large perturbations during training, and show that using a curriculum on disturbances provides a balance between robustness and inability to train (Table \ref{tab:ch3_results_perturbations}). Finally, Table \ref{tab:ch3_results_difficulty} shows the effect of terrain difficulty as a percentage of total distance travelled.

\begin{figure*}[h!]
\vspace{-2mm}
\centering
\subfloat[Flat]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_flat.png}}\quad
\subfloat[Gaps]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_gaps.png}}\quad
\subfloat[Hurdles]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_jumps.png}}
\medskip
\vspace{-5mm}
\subfloat[Stairs]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_stairs.png}}\quad
\subfloat[Steps]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_steps.png}}
\caption{Percentage of total distance travelled, evaluated during training.}
\label{fig:ch3_compare}
\end{figure*}


% What does this table add?
% \begin{table}[h!]
%     \vspace{-2mm}
%     % \vspace{-45.5mm}https://www.overleaf.com/project/5efc80ce9e222200014e6c84
%     \centering
%     \begin{adjustbox}{max width=1.0\columnwidth}  
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%          No Stage 1, No Stage 2       & 79.4           & 12.8          & 10.3          & 12.4          & 13.4 \\
%          Stage 1, No Stage 2          & 5.5  & 5.3          & 7.1          &  11.5          & 14.2 \\
%          No Stage 1, Stage 2          & 88.7           &  1.5          &  1.2          &  43.9          &   1.9 \\
%          Stage 1, Stage 2     &  \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}   \\
%     \hline
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Ablation study of Stage 1 and Stage 2 showing percentage of total distance travelled, computed with 500 trials.}
%     \label{tab:results_ablation}
%     \vspace{-5mm}
% \end{table}

\begin{table}[h!]
    % \vspace{-45.5mm}
    \vspace{-2mm}
    \centering
    % \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Force decay with success   &   89.8            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & 58.1  \\  
         Continuous force decay   &  \textbf{97.7}            & 15.2          & 22.8          & 38.7           & \textbf{58.3}  \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Comparison of force decay used in Stage 2 as percentage of total distance travelled.}
    \label{tab:ch3_results_decay}
    \vspace{-2mm}
\end{table}

\begin{table}[h!]
    % \vspace{-45.5mm}
    \vspace{-2mm}
    \centering
    % \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
        Forces on CoM and joints   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
         Forces on CoM only   &  81.6            &  8.6          &  2.7          & 12.2          & 1.0 \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Effect of applying guide forces to CoM only, shown as a percentage of total distance travelled.}
    \label{tab:ch3_results_guide}
    \vspace{-2mm}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{adjustbox}{max width=1.0\columnwidth}    
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Link to Target Policy   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
         No link to Target Policy          &    54.6           & 38.9          & 40.9          & 28.8          &  15.2 \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Effect of linking the target trajectory to the robot, shown as a percentage of total distance travelled.}
    \label{tab:ch3_results_no_link}
    \vspace{-2mm}
\end{table}

\begin{figure}[tb!]
% \vspace{-10mm}
\vspace{3mm}
\centering
\includegraphics[width=0.75\columnwidth]{images/ch3/reward2.png}
% \includegraphics[width=9 cm, height=7 cm]{images/reward.png}
% \vspace{-10mm}
\caption{Episode rewards for each of the three stages, for each terrain type.}
\label{fig:ch3_stage3}
\vspace{-3mm}
\end{figure}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Stage 1 \& 2    &   89.8            & 69.5           &  \textbf{79.0}          & 55.8 & 58.1  \\
         Stage 1, 2 \& 3   &  \textbf{99.9}    & \textbf{72.3}  & 58.5  & \textbf{57.6}  & \textbf{60.5}  \\
        %  Large (1000N)   &  93.0    & 59.5  & 0.0  & 18.9  & 13.2  \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Stage 1 \& 2, and Stage 1,2 \& 3 evaluated as percentage of total distance travelled.}
    \label{tab:ch3_results_stage3}
    \vspace{-2mm}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
         & Flat & Gap & Hurdle & Stairs & Steps \\ 
        %  \multicolumn{6}{l}{\textbf{Curriculum Stage 3 Analysis}}  \\
         \hline
         Small (50N) & 45.9          & 17.8          & 28.5           & 31.6          & 21.7     \\
         Large (1000N) & 81.2          & 18.0          &  21.3           & 22.7          &  9.4   \\
         Curriculum (50N to 1000N)  & \textbf{87.1}          & \textbf{35.7}          & \textbf{28.6}  & \textbf{45.6} & \textbf{24.5}   \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Effect of perturbations during training, shown as a percentage of total distance travelled.}
    \label{tab:ch3_results_perturbations}
    \vspace{-2mm}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
         & Flat & Gap & Hurdle & Stairs & Steps \\              
         \hline

        Easy Difficulty           & \textbf{100.0} & 45.3            & 24.5       & \textbf{88.1}          & 12.5   \\
        Reduced Difficulty      & \textbf{100.0} & 15.4            & \textbf{62.3}       & 80.2          & \textbf{87.4}   \\
        Normal Difficulty          & 99.9    & \textbf{72.3}  & 58.5  & 57.6  & 60.5   \\
        Increased Difficulty         & 94.5          & 11.5          & 32.5   & 50.5          &  26.7   \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{The effect of evaluating with terrain difficulty levels that are reduced and increased from the final terrain difficulty reached during training.}
    \label{tab:ch3_results_difficulty}
    \vspace{-2mm}
\end{table}





% \chapter[Passing Through Narrow Gaps with DRL]{Passing Through Narrow Gaps with Deep Reinforcement Learning}
% \label{cha:ch5}
% Motivation/contribution/abstract -----------------------
% \section{Passing Through Narrow Gaps with Deep Reinforcement Learning}
% \label{sec:gaps}

Previous chapters have considered traversing obstacles and how to reliably switch between behaviours in the context of simulated biped. This chapter we investigate the research question involving autonomously traversing narrow gaps, and the challenges of deploying behaviours trained in simulation on a real agent. The problem that we are aiming to solve in this chapter is getting a large tracked robot through a doorway (Fig. \ref{fig:cha5_fig1}). 


% Not sure what I'm trying to say here.
% While a tracked robot is statically stable compared with a biped, passing through a tight space and switchinthere are challenges in switching behaviours.

\begin{figure}[htb!]
    % \vspace{2mm}
    \captionsetup[subfigure]{labelformat=empty}
    \centering 
    \subfloat[]{\includegraphics[trim=1cm 1cm 1cm 2cm, clip,width=0.45\columnwidth]{images/ch6/real_door4.png}}
    \hfil
    \subfloat[]{\includegraphics[trim=5.0cm 0.0cm 0.2cm 15.3cm, clip, width=0.5\columnwidth]{images/ch6/real_door2.jpg}}
    \hfil
    \vspace*{-3mm}
    % \hfill
    \caption{We study the problem of traversing narrow gaps with a mobile robot.}
    \label{fig:cha5_fig1}
    %\vspace{-3mm}
\end{figure}


\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[Gap Behaviour]{\includegraphics[trim=1.8cm 3.6cm 1.8cm 3cm, clip, width=0.45\columnwidth]{images/ch6/door1.png}}
\hspace{0.3cm}
\subfloat[Behaviour Selection]{\includegraphics[trim=4.2cm 4.4cm 4cm 3.7cm, clip, width=0.41\columnwidth]{images/ch6/door2.png}}
\caption{The circular markers represent reward targets.}
\label{fig:ch5_doors}
\end{figure}


\begin{figure}[htb!]
    % \vspace{2mm}
    \centering
    \includegraphics[width=\columnwidth]{images/ch6/Fig2.png}
    %\hfill
    \caption{We learn a Gap Behaviour and a Behaviour Selection policy using an occupancy map for perception.}
    \label{fig:cha5_fig2}
    % \vspace{-3mm}
\end{figure}

\begin{figure}[ht!]
    \vspace{-5mm}
    \centering
    % \subfloat[Gap behaviour policy]{\includegraphics[trim=1cm 0.5cm 1cm 2cm, clip, width=0.5\columnwidth]{images/results0.png}}
    \subfloat[Gap Behaviour policy]{\includegraphics[trim=0cm 0.0cm 0cm 0cm, clip, width=0.5\columnwidth]{images/ch6/results0.png}}
    \hfil
    % \subfloat[Behaviour selection policy]{\includegraphics[trim=1cm 1cm 1cm 2cm, clip,width=0.45\columnwidth]{images/results1.png}}
    \subfloat[Behaviour Selection policy]{\includegraphics[trim=0cm 0cm 0cm 0cm, clip,width=0.5\columnwidth]{images/ch6/results1.png}}
    \hfil
    % \hfill
    \caption{Success rates during training for the Gap Behaviour policy and the Behaviour Selection policy.}
    \label{fig:ch5_learning_curves}
    %\vspace{-3mm}
\end{figure}


\begin{figure}[htb!]
    % \vspace{2mm}
    \centering
    \subfloat[Gazebo Simulator]{\includegraphics[trim=3cm 7cm 3cm 6cm, clip, width=0.5\linewidth]{images/ch6/gazebo.png}}
    \hspace{0.3cm}
    \subfloat[Real Robot]{\includegraphics[trim=3cm 4cm 0cm 12.2cm, clip, width=0.4\linewidth]{images/ch6/real_door.jpg}}
    \caption{Experimental setup in simulation and with the real robot.}
    \label{fig:cha5_fig3}
\end{figure}

First we learn a Gap Behaviour policy using ground truth perception with a reward that encourages the robot to line up the gap. Fig.\ref{fig:ch5_doors}.a) shows how we place markers to encourage the robot to first align to the gap before moving through. We then learn a Behaviour Selection policy that learns when to activate the Gap Behaviour, and when to instead default to a pre-existing Behaviour Stack. Fig.\ref{fig:ch5_doors}.b) shows the reward used to train the behaviour selector policy. As the robot moves sequentially between markers 1 to 4, when marker 2 and marker 3 are active, the reward encourages the gaps behaviour to be active. The pipeline once both policies are trained is shown in Fig. \ref{fig:cha5_fig2}. Both the Behaviour Selection policy and the Gap Behaviour use an occupancy map and robot state vector. The Behaviour Selection policy also has a goal waypoint as input and outputs a switch parameter $\tau$ that determines when to use the Gap Behaviour and when to use the pre-existing Behaviour Stack. The Gap Behaviour outputs the forward and heading velocities of the robot. 


Fig. \ref{fig:ch5_learning_curves} shows the progress through training for the Gap Behaviour, and for the Behaviour Selection policy. We also showed the results of training Behaviour Selection as a supervised problem. Using the same amount of data and training updates we saw the reinforcement learning method achieved a faster learning rate and more reliable final policy. We perform an analysis comparing the behaviours in simulation using an occupancy map generated from SLAM data and a simulated Velodyne LiDAR, and also using the same system on a real platform (Fig. \ref{fig:cha5_fig3}). Table \ref{tab:ch5_sim_results} shows the results of experiments in simulation, and Table \ref{tab:ch5_real_results} shows the results for the real experiments. We can see that there is a disparity between the training results, the simulation results, and the real results. 

Here we discuss the sources of the sim-to-real disparity. We observed a difference in training results using ground truth perception and the results from using an occupancy map generated by SLAM. As the simulation dynamics were the same in each case (both in simulation), this difference is likely the effect of a noisy Velodyne model. Adding noise to perception during training may improve these results. We also observed a performance drop when applying these algorithms to the real robot. This disparity was likely the cause of out of distribution examples, and sim-to-real physics differences. In a number of occasions the robot would catch on the door frame, and the wooden surface was much more slippery than the ground surface in the simulation. These issues could be reduced by adding more gap types during training, as well as dynamics randomisation. We leave these investigations for future work.

\begin{table}[h!]
    %\vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    % \begin{adjustbox}{min width=0.75\columnwidth}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Time(s) & Operator Actions \\
       \hline
        Behaviour Stack      & 0.0            &  50.2 &    1  \\
        Manual Gap Behaviour Selection        & 93.3          &  29.7 &    3  \\
        Auto Gap Behaviour Selection  & 63.3          &  45.3 &    1 \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Simulation results for passing through a narrow gap (30 trials)}
    \label{tab:ch5_sim_results}
\end{table}


\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Time(s) & Operator Actions \\
       \hline
        Behaviour Stack              & 0.0           &  44.6 &    1  \\
        Manual Gap Behaviour Selection               & 73.3          &  24.1 &    3  \\
        Auto Gap Behaviour Selection         & 40.0          &  30.9 &    1 \\
    \hline
    \end{tabular}
    % \end{adjustbox}
    \caption{Real robot results for passing through a narrow gap (15 trials).}
    \label{tab:ch5_real_results}
\end{table}





% ``How can we efficiently learn locomotion behaviours for traversing difficult obstacles?"
% ``How can we reliably transition between behaviours?"
% ``What are some of the challenges of training behaviours in simulation for real world applications?"


This chapter presented our first investigation of research question ``How can we efficiently learn locomotion behaviours for traversing difficult obstacles?" The contributions of this paper [\cite{tidd_guided_2020}] are as follows:


This focus of this chapter is the question ``How can we learn to autonomously traverse narrow gaps". We also touch on the first two research questions by first efficiently learning a behaviour for traversing small gaps, then determining when this behaviour should be activated based on the current state and a goal location. Finally, we investigate some of the challenges of training behaviours in simulation for real world applications. The contributions of this chapter (based on the paper [\cite{tidd_passing_2021}]) are as follows:

\begin{itemize}
    \item We proposed a 3-stage curriculum learning approach
    tailored for bipedal walking on complex terrain
    types
    \item  We show that a single rudimentary walking
    trajectory can be used as a target policy to
    improve exploration and training outcomes for
    several difficult terrain types
    \item We perform extensive analysis and ablation studies
    showing the importance of the design choices for our
    curriculum approach, and demonstrate the successful traversal of multiple
    challenging terrain types
    \item We developed a Gap Behaviour policy for controlling a large tracked robot through small gaps
    \item We designed a method to learn when to autonomously activate the Gap Behaviour policy. Our system integrates both learned behaviours and manually designed controllers
    \item We performed proof-of-concept demonstration of the effectiveness of the approach in the real world using a policy trained only in simulation. We identify the some of the sources of disparity, and discuss plans for addressing differences in future work
\end{itemize}

“Guided Curriculum Learning for Walking Over Complex Terrain” was
published at the 2020 Australasian Conference on Robotics and Automation in Brisbane, Australia. 

“Passing Through Narrow Gaps with Deep Reinforcement Learning” was
published at the 2021 IEEE/RSJ International Conference on Intelligent Robots and Systems in Prague, Czech Republic. 
\linebreak
\newpage
\newpage

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/Guided_Curriculum_Learning_for_Walking_Over_Complex_Terrain.pdf}

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/GRC_Statement-of-Contribution_Form_curriculum.pdf}

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/Passing_Through_Narrow_Gaps_with_Deep_Reinforcement_Learning.pdf}

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/GRC_Statement-of-Contribution_Form_passing.pdf}

==> old/Ch3a_mono.tex <==
% \chapter[Guided Curriculum Learning for Walking Over Complex Terrain]{Guided Curriculum Learning for Walking Over Complex Terrain}
\chapter[Guided Curriculum Learning]{Guided Curriculum Learning for Walking Over Complex Terrain}
   
% \item \textbf{Research Question 1: \textit{How can complex visuo-motor locomotion behaviours be learned efficiently, without knowing exactly how an expert would perform the action?}}

\label{cha:ch3a}
% Motivation/contribution/abstract -----------------------



% Three paragraphs: Explain motivation, what you did, results

% Final part: What research question you answered, what the contribution was, and what the publication was.

% \textit{One idea per paragraph. First sentence summarises the whole paragraph, last sentence leads into the next.}

% \textbf{Introduce the work in this chapter: robots, obstacles, DRL with visuo-motor policies}

This chapter presents work on designing behaviours for a simulated bipedal robot walking over difficult obstacles.  The biped uses a depth sensor and negotiates steps, stairs, gaps, and hurdles. The behaviours developed in this section rely on feedback from perception. For example the biped must adjust footstep placement on steps. For these reasons behaviours are difficult to manually design. DRL methods enables the development of visuo-motor policies, however sample efficiency limits their application in complex scenarios. Typically, visuo-motor policies are difficult to train, and requires high levels of interaction between the robot and the environment. Furthermore, for locomotion over difficult obstacles, policies are subject to local minima where commonly used exploration techniques may not be sufficient to direct the robot to the required behaviour. Improving the efficiency of learning behaviours for robot locomotion over difficult obstacles is explored throughout this chapter.

% require many samples. Furthermore, policy training for complex obstacles are subject to local minima where typical exploration techniques may not be sufficient to direct the robot to the required behaviour. The efficiency of learning behaviours for robot locomotion over difficult obstacles is explored throughout this chapter.


% \textbf{Discuss how this chapter answers the research questions: how are behaviours learned efficiently, how is reliable switching achieved.}

The contributions of this chapter are provided by research paper \cite{tidd_guided_2020}, and explores research question 1: the efficient learning of visuo-motor behaviours. Efficient learning is demonstrated by learning behaviours using a simple expert controller with reward shaping. Importantly, the expert is not able to complete the task, it is a rudimentary behaviour that is used to bootstrap learning the complex behaviour. For the complex behaviours required by the biped, a curriculum learning method is introduced to greatly improve training efficiency.  These investigations show the efficient development of difficult behaviours (research questions 1). 

\section{Problem Description}
\label{sec:problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our biped has 12 torque controlled actuators, which we simulate in the 3D Pybullet environment~\cite{coumans_pybullet_2020}. The terrain types we investigate are flat surfaces, gaps, hurdles, stairs, and steps (shown in Fig~\ref{fig:ch3_terrains}). The state provided to each policy is $s_t=[rs_t, I_t]$, where $rs_{t}$ is the robot state and $I_t$ is the perception input at time $t$. Fig~\ref{fig:ch3_network} shows the robot state and perception input to our policy and the resulting torques that are applied to the agent in Pybullet. 

\noindent\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}, s_{right}, s_{left} ]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot, respectively (four Boolean contact points per foot), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the body Centre of Mass (CoM), $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the CoM and $h_{CoM,t}$ is the height of the robot from the walking surface. $s_{right}$ and $s_{left}$ are Boolean indicators of which foot is in the swing phase, and is updated when the current swing foot makes contact with the ground. All angles except joint angles are represented in the world coordinate frame. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\noindent\textbf{Perception}: Perception is provided from a depth sensor mounted to the robot base, with a resolution of $[48,48,1]$. The depth is a continuous value scaled between $0-1$, equating to a distance of 0.25 and $\SI{2}{\metre}$. The sensor moves with the body in translation and yaw, we assume we are provided with an artificial gimbal that keeps the sensor at a fixed roll and pitch. The sensor is pointed at the robot's feet (the feet are visible) and covers a distance at least two steps in front of the robot as suggested by Zaytsev~\cite{zaytsev_two_2015}. As sampling the sensor is computationally expensive, we reduce the sampling rate to $\SI{20}{\hertz}$, where the rest of the system operates at $\SI{120}{\hertz}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Deep Reinforcement Learning}
\label{sec:drl}
Curriculum learning in the context of reinforcement learning considers a set of tasks $i\in \mathcal{T}$~\cite{narvekar_curriculum_2020}. For each task $i$ there is a Markov Decision Process $\text{MDP}_i$, defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. We consider a task to be any instance of the curriculum, each policy will experience several tasks. For example, a task may be characterised by a particular gain $K_p$ that determines the magnitude of force applied to the robot, and the response of the environment to a particular torque will depend on the task. The goal of reinforcement learning is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. 

% defined by tuple $\{\mathcal{S}_i,\mathcal{A}_i, R_i, \mathcal{P}_i, \gamma\}$

\subsection{Proximal Policy Optimisation (PPO)}
We choose the on-policy algorithm Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017} to update our policy weights. As we wish to have a single policy (one for each terrain type) that evolves through several MDP's, it is preferred to use an on-policy algorithm. Actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is a torque applied to each joint. We use the implementation of PPO from OpenAI Baselines~\cite{dhariwal_openai_2017}.

\subsection{Simple Target Policy}
\label{sec:target_policy}
We design a simple target walking trajectory with simulator physics turned off. The target trajectory is a list of joint positions that create a visually accurate walking gait of $\approx\SI{1}{\metre/\second}$. The target trajectory is divided into two segments, one for each foot, with the first set of joint positions corresponding to the impact of the respective foot. Each time the robot foot makes contact with the walking surface, we initialise the target trajectory from the appropriate segment (e.g. if the right foot contacts the ground, we restart the target trajectory with the right segment). We increment the target trajectory with each timestep.


% The target policy in the reward, and in a PD controller in the guidance curriculum (both introduced below). At each timestep we increment the position in the target walking trajectory. To improve the accuracy of our reward predictions and guidance curriculum, we link the target policy to the robot at the point where the swing foot contacts the ground. In other words, our target policy that is an open-loop set of joint positions is now linked to the robot, essentially closing the loop each time the robot swing feet change, i.e. the swing foot for the target trajectory is updated when the swing foot for the robot is updated. We replace the need for a phase variable~\cite{peng_deepmimic_2018},~\cite{merel_hierarchical_2019}, and instead use a Boolean variable that indicates which foot is in swing, and which is in stance. Each terrain type uses the same target trajectory (flat, gaps, hurdles, steps, stairs).

% The target motion could instead be a set of joint positions from motion capture, provided the motion is broken into two segments (for each swing foot), and switching between segments occurs at the same time as the robot. 


\subsection{Reward}
Our reward is inspired by Peng et al in their work mimicking motion capture data~\cite{peng_deepmimic_2018}. Our reward function is the same for each policy, defined as:
\begin{equation}
r_t = goal + pos + vel + base + step + act
\end{equation}
where:
\begin{itemize}[leftmargin=*]
    \item $goal$ is the error between the current heading velocity and goal heading velocity $= w_{goal}\cdot \exp[-c_{goal}\cdot e_{goal}]$.
    \item $pos$ is the error between the joint positions and the target joint positions $= w_{pos}\cdot \exp[-c_{pos}\cdot e_{pos}]$.
    \item $vel$ is the error between the current joint velocities and the target joint velocities (target joint velocities are set to zero) $= w_{vel}\cdot \exp[-c_{vel}\cdot e_{vel}]$.
    \item $base$ is the CoM error from a target height, and zero roll and pitch positions $= w_{base}\cdot \exp[-c_{base}\cdot e_{base}]$. 
    \item $step$ encourages a symmetrical step length ($\text{left}_{step}\approx \text{right}_{step}$ when in contact) $= w_{step}\cdot \exp[-c_{step}\cdot e_{step}]$. 
    \item $act$ is a penalty for excessive torque for each of the $n$ joints $= w_{act}\sum_n(a_t^2)$. 
\end{itemize}

$e$ is the error of each respective element. Parameters $w$ and $c$ are tunable weights, which are fixed for all policies. 

\begin{figure}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=0.95\columnwidth]{images/ch3/network.png}
\includegraphics[width=0.75\columnwidth]{images/ch3/network.png}
\caption{Our policy is a neural network that takes the state (robot state and perception input) $s_t=[rs_t, I_t]$ and returns the torques applied to each joint $a_t$.}
\label{fig:ch3_network}
\vspace{-3mm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Curriculum Learning}
\label{sec:curriculum}
We design our curriculum with the rationale that dynamic platforms are usually supported (e.g. with a crane and harness) while controllers are developed. The learning process is divided into three stages, where $\mathcal{D}$ is the terrain curriculum (Stage 1), $\mathcal{F}$ is the guide curriculum (Stage 2), and $\mathcal{P}$ is the perturbation curriculum (Stage 3), where each stage represents a set of difficulties $\mathcal{D} = \{d_1, d_2, .., d_n\}$, $\mathcal{F} = \{f_1, f_2, .., f_n\}$, and $\mathcal{P} = \{p_1, p_2, .., p_n\}$. To begin learning we select $d_1, f_1$ and $p_1$, i.e all curriculum stages are at the lowest difficulty level. We then proceed to increment the difficulty of Stage 1 to its most difficult setting ($d_1 \rightarrow d_n$), then Stage 2 ($f_1 \rightarrow f_n$), and finally Stage 3 ($p_1 \rightarrow p_n$). During policy training, each increment to the next difficulty level occurs with a \textbf{success criteria}, which we define as the robot successfully reaching the end of the terrain sample three consecutive times. 

\subsection{Stage 1. Terrain Curriculum:}
In the terrain curriculum $\mathcal{D} = \{d_1, d_2, .., d_n\}$, the terrain difficulty is increased by incrementing $d$ up to a final difficulty $n$. In this stage, we apply the guide curriculum and perturbation curriculum at their lowest difficulty. The difficulty range  of each terrain is shown in Fig~\ref{fig:ch3_terrains}. Increases to the terrain difficulties are linear, incrementing terrain dimensions by a fixed amount each time the success criteria is achieved. 

% The terrain curriculum allows us to increase the difficulty of the terrain, where for some terrains (like hurdles) the policy fails to traverse the terrain at all, or for others (like gaps) the policy can take much longer to learn the required behaviour.

\subsection{Stage 2. Guide Curriculum:}
\label{sec:guide_curriculum}
Guide forces are employed from the beginning of training, tracking the target policy explained in Sec.~\ref{sec:target_policy}. Once the terrain curriculum has completed we begin the guide curriculum $\mathcal{F} = \{f_1, f_2, .., f_n\}$. Guide forces are applied to the CoM of the robot $f_c$ and to each joint $f_j$, where $f_1 = [f_c, f_j]$ is set to the lowest difficulty (highest guide forces).

$f_c$ is a PD controller that is applied to all 6 degrees of freedom of the CoM. 
\begin{equation}
f_c = K_{p_c} (p_{target} - p_{CoM}) + K_{d_c} ( v_{target} - v_{CoM})
\end{equation}
Where $K_{p_c}$ and $K_{d_c}$ are the gains, $p_{target}$ is the target position, $p_{CoM}$ is the observed position, $v_{target}$ is the target velocity, and $v_{CoM}$ is the observed velocity of the robot CoM. The target for the velocity in the forward $x$ direction is $\SI{1}{\meter/\second}$. The height $z$ target position is fixed at a nominal height, the $yaw$ targe follows the yaw of the terrain, and the position targets for the remaining degrees of freedom $y, roll, pitch$, are zero. All velocity targets, except for $x$ velocity, are set to zero. We liken this idea to fixing the robot to a small crane or gantry that supports the body of the robot, and moves forward at the desired velocity.
% This approach has shown reduced training times and increased asymptotic performance for multiple morphologies with a floating base~\cite{yu_learning_2018}.

$f_j$ is a second PD controller that is applied to all 12 actuators tracking our simple target trajectory. Forces applied to each joint are calculated from:
\begin{equation}
f_j = K_{p_j}( J_{t_{target}} - J_t ) + K_{d_j}(Jv_{t_{target}} - Jv_t )
\end{equation}
Where $K_{p_j}$ and $K_{d_j}$ are the gains, $J_{t_{target}}$ is the joint positions of the target trajectory, $J_t$ is the observed joint positions, $Jv_{t_{target}}$ is the target joint velocities, and $Jv_t$ is the observed joint velocities. We found that setting the target velocities to zero was sufficient for training (rather than estimating the target velocities with finite differences).

The guide curriculum involves reducing the guide forces in discrete steps following: $f_2 = 0.65 \cdot f_1$. The external forces are not provided as input to policy, and are considered an artifact of the environment. Once the guide forces decrease below a threshold ($f_n$) Stage 2 is complete.


\subsection{Stage 3. Perturbation Curriculum:}
% \subsection{Stage 3. Adding Perturbations}

Random perturbations applied during training have been shown to improve the robustness of walking policies~\cite{schulman_proximal_2017}. When the other curriculum stages are complete, we increase the magnitude of external perturbations with the perturbation curriculum, $\mathcal{P} = \{p_1, p_2, .., p_n\}$. Perturbations are an impulse force of random magnitude, applied to all 6 degrees of freedom of the CoM. At a random interval of approximately 2.5Hz, and for each DOF, we sample a perturbation force from a uniform distribution $(-p_1,p_1)$, where $p_1$ is increased linearly to the final value $p_n$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

 
% \begin{figure*}[tb!]
% % \vspace{2mm}
% \centering
% \subfloat[Curved flat terrain with a bend angle starting at $20\degree$ and increasing to $120\degree$]{\includegraphics[width=\wI cm, height=\hI cm]{images/ch3/flat.png}}
% \hfill
% \subfloat[Hurdles with a height starting at $\SI{6}{\cm}$ and increasing to $\SI{30}{\cm}$]{\includegraphics[width=\wI cm, height=\hI cm]{images/ch3/jumps.png}}
% \hfill
% \subfloat[Gaps with a width starting at $\SI{7}{\cm}$ and increasing to $\SI{70}{\cm}$]{\includegraphics[width=\wI cm, height=\hII cm]{images/ch3/compare_gaps.png}}
% \hfill

% \caption{Using a single walking trajectory as a guide, our curriculum method traverses complex terrain types. The initial and final terrain sizes are provided.}
% \label{fig:ch3_terrains}
% \vspace{-3mm}
% \end{figure*}


\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[Curved flat terrain initial angle starting at $20\degree$ and width $\SI{1.1}{\meter}$ ]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/flat1.png}}
\hfill
\subfloat[Curved flat terrain final angle
$120\degree$ and width $\SI{0.9}{\meter}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/flat.png}}
\hfill
\subfloat[Hurdles initial height $\SI{13}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/jumps1.png}}
\hfill
\subfloat[Hurdles final height $\SI{38}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/jumps.png}}
\hfill
\subfloat[Gaps initial length $\SI{10}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/gaps1.png}}
\hfill
\subfloat[Gaps final length $\SI{100}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/gaps.png}}
\hfill
\subfloat[Stairs initial height $\SI{1.7}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/stairs1.png}}
\hfill
\subfloat[Stairs final height $\SI{17}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/stairs.png}}
\hfill
\subfloat[Steps initial distance apart $\SI{4}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/steps1.png}}
\hfill
\subfloat[Steps final distance apart $\SI{40}{\cm}$]{\includegraphics[width=\w cm, height=\h cm]{images/ch3/steps.png}}
% \hfill
\caption{Our curriculum method traverses complex terrain types. The initial and final terrain sizes used in training are provided.}
\label{fig:ch3_terrains}
\vspace{-3mm}
\end{figure}
 
 
In this section we introduce the terrain types used for the test worlds (Sec~\ref{sec:terrain_types}), and present our simulation results. We evaluate Stage 1 (terrain curriculum), and Stage 2 (guide curriculum) of our method in Sec~\ref{sec:stage1_stage2}, before analysing Stage 3 (perturbation curriculum) in Sec~\ref{sec:stage3}. 

\subsection{Terrain Types}
\label{sec:terrain_types}
For all terrains there is a total of 10 steps of evenly spaced difficulty ($d_1 \rightarrow d_{10}$). The suite of terrains and range of difficulties is shown in Fig~\ref{fig:ch3_terrains}. Terrain conditions are selected to test our system with a broad range of scenarios. Examples include the Flat terrain that has curves that require the robot to turn (Fig~\ref{fig:ch3_terrains}(a-b)), the Hurdles terrain (Fig~\ref{fig:ch3_terrains}(c-d)) that forces the robot to take a high step, and the Steps terrain (Fig~\ref{fig:ch3_terrains}(i-j)) where the robot must step with a lateral component.
% Movements such as turning, high steps, or lateral stepping are not present in the simple target trajectory, yet our policies adapt to the requirements of the terrain. 

% Each terrain example requires the robot to use its perception, this is enforced by randomisation of the starting location of the robot, and randomised aspects of terrain generation (direction of the curve, number of steps or stairs). 

Each policy is trained on a scenario with two consecutive instances of the same terrain artifact, where an instance refers to a single gap or hurdle, or a random number ($5-8$) of stairs or steps. We found that training on two consecutive artifacts performed better during evaluation than a sample with a single artifact. We evaluate all methods on a sequence of seven consecutive instances of the same terrain artifact at maximum difficulty, making up one trial. We run each policy for 500 trials and record the distance travelled as a percentage of total distance, which we use as our evaluation metric. For all experiments no external disturbance forces are applied when evaluating a policy, except for the perturbation evaluation section of Sec~\ref{sec:intense}, where perturbations are applied during evaluation. For all experiments, the terrain difficulty at evaluation is set to the highest difficulty (10), except for the domain difficulty section of Sec~\ref{sec:diff}, where we evaluate our policies on a range of difficulties.

% We train our policies with hyperparameters that are largely unchanged from the OpenAI Baseline defaults~\cite{dhariwal_openai_2017}. 

% We run 16 workers each on a separate thread of a CPU for a maximum of 50 million timesteps (roughly 7 hours), linearly annealing the learning rate to zero throughout training. We observed that Stage 1 usually takes the first 10-20\% of total training time; after that the terrain is at its most difficult for the remainder of training. 


% \subsubsection{Guide Curriculum Evaluation}
% Even for more difficult terrain types we found that with external forces the terrain reaches its maximum difficulty early in training. Reducing the guiding forces however must occur slowly to avoid a local minima where the agent gets stuck in behaviour that fails to complete the task. We investigate several continuous force reduction rates, and compare these to a reduction method based on the environmental curriculum from~\cite{yu_learning_2018}. Plot of decay, yes this is todo.


% \textbf{Decay Types:} We compare several decay types for the second curriculum stage, when the external forces are slowly removed. We look at a linear decay (forces are reduced by a fixed amount), exponential decay (large reductions initially, with tapering reductions as forces get closer to zero), and a sigmoid decay (tapering reductions for large and small gains). The results for these comparisons are found in the first three rows of Table~\ref{tab:ch3_results}. Waiting on results from the HPC.

% We investigate milestone length for decaying the external forces (Stage 2), on the hurdle terrain. Results are shown in plot (TODO - TOTAL REWARD or PERCENTAGE DISTANCE?). We can see that increasing the milestones length..

% \subsubsection{Ablation Study}
\subsection{Stage 1 and Stage 2 Analysis}
\label{sec:stage1_stage2}

\begin{figure*}[ht]
\vspace{-2mm}
\centering
\subfloat[Flat]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_flat.png}}\quad
\subfloat[Gaps]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_gaps.png}}\quad
\subfloat[Hurdles]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_jumps.png}}

\medskip
\vspace{-5mm}
\subfloat[Stairs]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_stairs.png}}\quad
\subfloat[Steps]{\includegraphics[width=.3\textwidth, height=\hIII cm]{images/ch3/compare_steps.png}}

\caption{Percentage of total distance travelled, evaluated during training showing the comparisons of the Stage 1 and Stage 2 ablation study.}
\label{fig:ch3_compare}
\end{figure*}

\begin{table}[h!]
    \vspace{-2mm}
    % \vspace{-45.5mm}https://www.overleaf.com/project/5efc80ce9e222200014e6c84
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         No Stage 1, No Stage 2       & 79.4           & 12.8          & 10.3          & 12.4          & 13.4 \\
         Stage 1, No Stage 2          & 5.5  & 5.3          & 7.1          &  11.5          & 14.2 \\
         No Stage 1, Stage 2          & 88.7           &  1.5          &  1.2          &  43.9          &   1.9 \\
         Stage 1, Stage 2     &  \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}   \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study of Stage 1 and Stage 2 showing percentage of total distance travelled, computed with 500 trials.}
    \label{tab:ch3_results_ablation}
    \vspace{-5mm}
\end{table}
% \begin{table}[h!]
%     % \vspace{-45.5mm}
%     \centering
%     \begin{adjustbox}{max width=1.0\columnwidth}  
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%          No Stage 1, No Stage 2       & 91.1           & 12.7          & 13.9          & 14.9          & 13.5 \\
%          Stage 1, No Stage 2          & \textbf{95.7}  & 14.0          & 14.3          &  3.8          & 15.3 \\
%          No Stage 1, Stage 2          & 89.8           &  1.9          &  2.7          &  1.1          &  1.2 \\
%          Stage 1, Stage 2     &        92.4            & \textbf{78.9} & \textbf{71.6} & \textbf{38.3} & \textbf{60.8}  \\
%     \hline
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Ablation study of Stage 1 and Stage 2 showing percentage of total distance travelled, computed with 500 trials.}
%     \label{tab:ch3_results_ablation}
% \end{table}

% \begin{figure*}[tb!]
% % \vspace{2mm}
% \centering
% \subfloat[Flat]{\includegraphics[width=0.3\textwidth]{images/ch3/compare_flat.png}}
% \hfill
% \subfloat[Hurdles]{\includegraphics[width=0.3\textwidth]{images/ch3/compare_gaps.png}}
% \hfill

% \subfloat[Gaps]{\includegraphics[width=0.3\textwidth]{images/ch3/compare_jumps.png}}
% \hfill
% % \medskip
% \subfloat[Stairs]{\includegraphics[width=0.3\textwidth]{images/ch3/compare_stairs.png}}
% \hfill
% \subfloat[Steps]{\includegraphics[width=0.3\textwidth]{images/ch3/compare_steps.png}}
% \hfill
% \caption{Percentage of total distance travelled, evaluated during training, for the Stage 1 and Stage 2 ablation study.}
% \label{fig:ch3_compare}
% \vspace{-3mm}
% \end{figure*}

% \begin{table*}[]
%     \vspace{3mm}
%     \centering
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%          No Stage 1, No Stage 2       & 37.1          &  8.4          & 14.3         & 13.7          & 18.5 \\https://www.overleaf.com/project/5efc80ce9e222200014e6c84
%          Stage 1, No Stage 2          & 26.0          & 12.9          & 14.6          & 13.1          & 14.3 \\
%          No Stage 1, Stage 2          & 99.6 &          78.7          &  1.9          & 62.7          & 56.9 \\
%          Stage 1, Stage 2     & \textbf{99.8}  & 87.7 & \textbf{78.6} & 58.7 & \textbf{57.2}  \\
%          Continuous Stage 2 decay   & 99.0             & 70.0       & 63.9          & 54.4             & 54.1  \\
%          Guide forces on CoM only   &  83.2          &  \textbf{90.0}  & 42.8          & \textbf{64.2}          & 3.0 \\
%          No link to target          & 53.9          &  66.5         & 34.8          & 49.8          &  4.2 \\
%     \hline
%     \end{tabular}
%     \caption{Analysis of Stage 1 and Stage 2 showing percentage of total distance travelled, computed with 500 trials.}
%     \label{tab:ch3_results1}
% \end{table*}


This section analyses the effect of Stage 1 and Stage 2 on policy performance in an ablation study. We also investigate three individual aspects of our method: the effect of using success criteria to decay forces for Stage 2, removing the guiding forces applied to the joints, and not linking the target policy to the robot state. For all experiments in this section, the external perturbations are set at the lowest level $p_1$ throughout training, with no external perturbations applied during evaluation.

\subsubsection{Ablation study of Stage 1 and Stage 2}
We investigate the benefit of Stage 1 and Stage 2 of our method by removing one or both stages.

\begin{itemize}[leftmargin=*]

\item\textbf{No Stage 1, No Stage 2:}  The terrain starts at maximum difficulty. Guiding forces are not applied to the robot CoM or joints.

\item\textbf{Stage 1, No Stage 2:} The terrain curriculum is active. Guiding forces are not applied to the robot CoM or joints.

\item\textbf{No Stage 1, Stage 2:} The terrain starts at maximum difficulty. Guide curriculum is active.

\item\textbf{Stage 1, Stage 2:} Both the terrain curriculum and guide curriculum are active. 
\end{itemize}


Fig~\ref{fig:ch3_compare} shows the evolution of the percentage of total distance achieved with respect to the number of training steps. We perform this evaluation periodically by pausing training, removing any external forces, setting the terrain difficulty to maximum, and running 500 trials. The final evaluation is provided in Table~\ref{tab:ch3_results_ablation}. We can see from Fig~\ref{fig:ch3_compare}, and Table~\ref{tab:ch3_results_ablation} that both Stage 1 and Stage 2 are important for the development of successful policies for the selected terrain types. Stage 1 is necessary for all terrains except for Flat and Stairs. \textbf{No Stage 1, Stage 2} on the Stairs terrain results in the traversal of a significant portion of the test world (43.9\%). Without Stage 2 the agent learns a one leg hopping gait. For all terrains this gait is unstable (the agent is unable to balance beyond the first hop), except for \textbf{No Stage 1, No Stage 2} on the Flat terrain where the agent successfully traverses 79.4\% of the test world by hopping on one leg. The lowest performance is found with \textbf{No Stage 1, Stage 2} for the Gap, Hurdle, and Steps terrains. For these terrain types, without the terrain curriculum the robot is unable to reach the success criteria required to lower the guidance forces. When evaluated without guide forces, the robot is unable to balance and achieves a much lower result than without any curriculum at all.

% (Flat 89.8\%, Gaps 69.5\%, Hurdles 79.0\%, Stairs 55.8\%, Steps 58.1\%)

% , for each terrain type (evaluated on 7 consecutive instances)

% \begin{table*}[t]
%     % \vspace{-45.5mm}
%     \centering
%     \begin{tabular}{cccccc}
%         %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
%           & Flat & Gap & Hurdle & Stairs & Steps \\
%          \hline
%          No Stage 1, No Stage 2       & 91.1           & 12.7          & 13.9          & 14.9          & 13.5 \\
%          Stage 1, No Stage 2          & \textbf{95.7}  & 14.0          & 14.3          &  3.8          & 15.3 \\
%          No Stage 1, Stage 2          & 89.8           &  1.9          &  2.7          &  1.1          &  1.2 \\
%          Stage 1, Stage 2     &        92.4            & \textbf{78.9} & \textbf{71.6} & \textbf{38.3} & \textbf{60.8}  \\
%          Continuous Stage 2 decay   &  79.1            & 63.9          & 14.2          & 33.5           & 56.7  \\
%          Guide forces on CoM only   &  47.4            &  2.8          &  2.4          & 25.6          &  1.0 \\
%          No link to target          &    7.7           & 54.1          & 53.7          & 17.6          &  14.6 \\
%     \hline
%     \end{tabular}
%     \caption{Analysis of Stage 1 and Stage 2 showing percentage of total distance travelled, computed with 500 trials.}
%     \label{tab:ch3_results1}
% \end{table*}




\subsubsection{Effect of using success criteria to decay forces}
\begin{table}[h!]
    % \vspace{-45.5mm}
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Force decay with success   &   89.8            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & 58.1  \\  
         Continuous force decay   &  \textbf{97.7}            & 15.2          & 22.8          & 38.7           & \textbf{58.3}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Comparison of force decay used in Stage 2 as percentage of total distance travelled, computed with 500 trials.}
    \label{tab:ch3_results_decay}
    \vspace{-2mm}
\end{table}
This section investigates the choice of decay on guidance forces (Stage 2). We compare our method of decay that is dependent on agent success, to decaying the guiding forces at fixed intervals irrespective of the agent success. We found that decaying the guiding forces by $0.995$ each episode was a similar rate to our decay approach (introduced in Sec~\ref{sec:guide_curriculum}). The results in Table ~\ref{tab:ch3_results_decay} show that for the Gaps, Hurdles, and Stairs terrain types, decaying the guide forces continuously performed significantly worse on the test world than our method (Gaps 15.2\% compared to 69.5\%, Hurdles 22.8\% compared to 79.0\%, Stairs 38.7\% compared to 55.8\%). For the Flat and Steps terrain types the continuous decay performed slightly better than decay based on agent success (Flat 89.8\% compared to 97.7\%, Steps 58.1\% compared to 58.3\%). We suspect a decay rate tuned for each terrain type would match or improve the performance of our method for all terrains, though introduces undesirable hand tuning.

\subsubsection{Effect of guide forces on CoM only}
\begin{table}[h!]
    % \vspace{-45.5mm}
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
        Forces on CoM and joints   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
         Forces on CoM only   &  81.6            &  8.6          &  2.7          & 12.2          & 1.0 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Effect of applying guide forces to CoM only, shown as a percentage of total distance travelled, computed with 500 trials.}
    \label{tab:ch3_results_guide}
    \vspace{-2mm}
\end{table}
We test the effect of removing the guiding forces on the joints, instead only apply forces to the CoM during Stage 2 Guide Curriculum. We found guiding forces applied only to the base performed worse on all terrains than also applying guiding forces to the joints (Table~\ref{tab:ch3_results_guide}). Notably low scores (Gaps 8.6\%, Hurdle 2.7\%, Steps 1.0\%) suggest the agent was unable to decay the guide forces on the CoM, so unable to support itself during evaluation.

\subsubsection{Effect of not linking target policy}
\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}    
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Link to Target Policy   &   \textbf{89.8}            & \textbf{69.5}           &  \textbf{79.0}          & \textbf{55.8} & \textbf{58.1}  \\
         No link to Target Policy          &    54.6           & 38.9          & 40.9          & 28.8          &  15.2 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Effect of linking the target trajectory to the robot, shown as a percentage of total distance travelled, computed with 500 trials.}
    \label{tab:ch3_results_no_link}
    \vspace{-2mm}
\end{table}
We investigate the effect of removing the link between the target policy and the robot. Linking is introduced in Sec~\ref{sec:target_policy}, and refers to resetting the target trajectory with the respective segment (left or right) each time a foot of the robot makes contact with the ground. When the target trajectory is not linked to the robot, the target joint positions are initialised only at the first step. Advancing the target trajectory occurs with each timestep, without any feedback from the robot. We found that not linking the target trajectory with the robot reduced the performance of all terrains in comparison to our method as seen in Table~\ref{tab:ch3_results_no_link}. While some policies were able to successfully traverse portions of the test world (Flat 54.6\%, Gaps 38.9\%, Hurdles 40.9\%, Stairs 28.8\%), others such as Steps (15.2\%) performed poorly. We suspect that policies requiring more precise foot placement benefit the most from having the target trajectory linked with the robot steps. This simple method allows us to train policies following a target, without providing the policy with a phase variable (a limitation of related work~\cite{peng_deepmimic_2018},~\cite{merel_hierarchical_2019}). Instead the policy can infer the phase of the walk cycle from joint positions and feet contact information.

\subsection{Stage 3 Analysis}
\label{sec:stage3}

% \begin{table*}[]
%     \vspace{3mm}
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c}
%     \begin{tabular}{cccccc}
%         & Flat & Gap & Hurdle & Stairs & Steps \\ 
%         % \multicolumn{1}{c|}{\textbf{Stage 3 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
%         %  \multicolumn{6}{l}{\textbf{Curriculum Stage 3 Analysis}}  \\
%          \hline
%          Stage 1 and 2    & 99.8                  & \textbf{82.7} & \textbf{78.6} & 80.7                &   77.5  \\
%          Stage 1, 2 and 3 & \textbf{100.0}          & 79.3          & 70.4           & \textbf{80.9}      & \textbf{83.2}     \\

%     \hline
%     \end{tabular}
%     \caption{Stage 1 and 2, and all three stages of the curriculum, as a percentage of total distance travelled, computed with 500 trials. }
%     \label{tab:ch3_results_stage3}
% \end{table*}


We now analyse the final stage of our curriculum learning method. In the perturbation curriculum the maximum magnitude of external forces is increased from an initial disturbance of $p_1 = \SI{50}{\newton}$ to a final disturbance of $p_n = \SI{1000}{\newton}$, where perturbations are sampled uniformly for each degree of freedom of the CoM from $\mathcal{U}(-p, p)$. Fig~\ref{fig:ch3_stage3} shows the average episode reward for all three stages of training for all terrain types. We can see that Stage 1 completes early in training for all terrain types. Drops in reward are seen early in Stage 2 where the majority of guidance forces are removed, then we see a gradual increase as the agent learns to act without guidance. In Stage 3 we see a large drop in return as the perturbations are increased. At this point in training the agent is operating in the hardest conditions (terrain at highest difficulty, no guiding forces, large perturbations applied to the CoM). We also show the episode reward for policies trained without any part of the curriculum (solid line), and observe the reward for policies trained without a curriculum is much lower than the policies trained with our method.

From Table~\ref{tab:ch3_results_stage3} we can see that adding the perturbation curriculum improves performance slightly for all terrain types except the Hurdles terrain (58.5\% compared to 79.0\%). The Hurdles terrain takes the longest for Stage 1 and Stage 2 to complete (as shown in Fig~\ref{fig:ch3_stage3}), and therefore has the least time to train with large perturbations. 

% We note performance could be improved with perturbation tuning for individual terrain types, and that perturbations that are too large can reduce fine grained behaviour improvements.

% did not perform better on the test world than Stage 1 \& 2 (with the exception of the flat terrain: 92.4\% compared to 95.7\%). This can be explained by the Stage 1 \& 2 approach overfitting to the training domain, where increasing perturbations reduces this effect. In the below experiments we test this claim by applying perturbations during evaluation, and assess performance on terrain difficulties that are increased from what are seen during training.
%  We use a single jump from the initial disturbance level to the final disturbance level.
\begin{figure}[tb!]
\vspace{-10mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch3/reward.png}
% \includegraphics[width=9 cm, height=7 cm]{images/ch3/reward.png}
\vspace{-10mm}
\caption{Episode rewards for our method (Stage 1, Stage 2, and Stage 3), for each terrain type. The completion of each stage is shown with a circle and change in line colour and type. The first segment (lightest colour, dotted line) is Stage 1, the middle segment shows Stage 2 (dash-dotted line), and the final segment (darkest colour, dashed line) shows the rewards when the perturbation curriculum is applied. The solid coloured lines are the policies trained without a curriculum.}
\label{fig:ch3_stage3}
\vspace{-3mm}
\end{figure}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{max width=1.0\columnwidth}  
    \begin{tabular}{cccccc}
        %  \multicolumn{1}{c|}{\textbf{Stage 1 and Stage 2 Analysis}} & Flat & Gap & Hurdle & Stairs & Steps \\
          & Flat & Gap & Hurdle & Stairs & Steps \\
         \hline
         Stage 1 \& 2    &   89.8            & 69.5           &  \textbf{79.0}          & 55.8 & 58.1  \\
         Stage 1, 2 \& 3   &  \textbf{99.9}    & \textbf{72.3}  & 58.5  & \textbf{57.6}  & \textbf{60.5}  \\
        %  Large (1000N)   &  93.0    & 59.5  & 0.0  & 18.9  & 13.2  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Stage 1 \& 2, and Stage 1,2 \& 3 evaluated as percentage of total distance travelled, computed with 500 trials, with no perturbations applied during evaluation.}
    \label{tab:ch3_results_stage3}
    \vspace{-2mm}
\end{table}


% Stage 2 completes We observed that Stage 1 usually takes the first 10-20\% of total training time; after that the terrain is at its most difficult for the remainder of training.

% \subsubsection{Effect of Stage 3}
% We compare the results of including Stage 3 in Table~\ref{tab:ch3_results_stage3}, where the first row shows the results for evaluations with Stage 1 and Stage 2, and the second row includes Stage 3. We can see that adding Stage 3 improves the performance of the policies for all terrains.

\subsubsection{Effect of perturbation intensity}
\label{sec:intense}
In this section we investigate the robustness of our method by applying perturbations during the evaluation. The evaluation perturbation forces are sampled uniformly from $(-\SI{1000}{\newton}, \SI{1000}{\newton})$ and applied to the CoM of the robot. We compare training with small perturbations, training with large perturbations, and our perturbation curriculum.

\begin{itemize}[leftmargin=*]

\item\textbf{Small:} Small perturbations are applied throughout training, sampled uniformly from $(\SI{-50}{\newton}, \SI{50}{\newton})$. This is the same as Stage 1 \& 2.

\item\textbf{Large:} Maximum perturbations are applied throughout training, sampled uniformly from $(\SI{-1000}{\newton}, \SI{1000}{\newton})$.

\item\textbf{Curriculum:} We show the results of the perturbation curriculum (Stage 3), with perturbations applied during evaluation.

\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
         & Flat & Gap & Hurdle & Stairs & Steps \\ 
        %  \multicolumn{6}{l}{\textbf{Curriculum Stage 3 Analysis}}  \\
         \hline
         Small (50N) & 45.9          & 17.8          & 28.5           & 31.6          & 21.7     \\
         Large (1000N) & 81.2          & 18.0          &  21.3           & 22.7          &  9.4   \\
         Curriculum (50N to 1000N)  & \textbf{87.1}          & \textbf{35.7}          & \textbf{28.6}  & \textbf{45.6} & \textbf{24.5}   \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Effect of perturbations during training, shown as a percentage of total distance travelled, computed with 500 trials. Each method is evaluated with maximal perturbations.}
    \label{tab:ch3_results_perturbations}
    \vspace{-2mm}
\end{table}

From Table~\ref{tab:ch3_results_perturbations}, we can see that our perturbation curriculum (Stage 3) performs best on all terrains compared with applying small (Stage 1 and Stage 2), and large forces throughout training. We notice slight performance gains for Hurdles (28.5\% compared to 28.6\%) and Steps (21.7\% compared to 24.5\%), and larger improvements with Flat (45.9\% compared to 87.1\%), Gaps (17.8\% compared to 35.7\%), and Stairs (31.6\% compared to 45.6\%). For policies trained with large disturbances throughout training we observe reduced performance compared with our method. Our results show that a perturbation curriculum allows for large perturbations during training, with improved outcomes compared to large forces applied for the entirety of training. This methodology can be applied to scenarios where training with perturbations can improve robustness (e.g. simulation to real transfer).

% and even failure to learni compared with either worse that small perturbations for some terrain types(, Hurdles, Stairs) and detrimental for Steps 9.4\%. 

% We show that using the perturbation curriculum improves robustness (for all terrain types), compared to applying small perturbations throughout training.  

\subsubsection{Effect of test domain difficulty}
\label{sec:diff}

We test the generalisation of our method (Stages 1, 2 \& 3) in a final evaluation that compares policy performance on terrains that are less difficult, and terrains that are more difficult than the final terrain experienced during training.

\begin{itemize}[leftmargin=*]

\item\textbf{Easy Difficulty:} We evaluate our policies with the easy terrain difficulty $d_1$. 


\item\textbf{Reduced Difficulty:} We evaluate our policies with a terrain difficulty 20\% lower than the final difficulty experienced in training ($d_8$). 

\item\textbf{Normal Difficulty:} We evaluate our policies with the final terrain difficulty experienced in training ($d_{10}$). 

\item\textbf{Increased Difficulty:} We evaluate our policies with a terrain difficulty 20\% higher than the final difficulty experienced in training ($d_{12}$). 
 
\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
         & Flat & Gap & Hurdle & Stairs & Steps \\              
         \hline

        Easy Difficulty           & \textbf{100.0} & 45.3            & 24.5       & \textbf{88.1}          & 12.5   \\
        Reduced Difficulty      & \textbf{100.0} & 15.4            & \textbf{62.3}       & 80.2          & \textbf{87.4}   \\
        Normal Difficulty          & 99.9    & \textbf{72.3}  & 58.5  & 57.6  & 60.5   \\
        Increased Difficulty         & 94.5          & 11.5          & 32.5   & 50.5          &  26.7   \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{The effect of evaluating with terrain difficulty levels that are reduced and increased from the final terrain difficulty reached during training. Shown as a percentage of total distance travelled, computed with 500 trials.}
    \label{tab:ch3_results_difficulty}
    \vspace{-2mm}
\end{table}

% From Table~\ref{tab:ch3_results_difficulty}, we can see the Gaps policy has overfit to the final difficulty experienced during training, and has failed to generalise to terrain of reduced (15.4\%) or increased (11.5\%) difficulty. For all other terrain types we observe improved performance on the reduced difficulty terrain, and comparable performance for some terrain types with increased difficulty (Flat 94.5\% compared to 99.9\%, Stairs 50.5\% compared to 57.6\%). Our method requires more investigation to improve the generalisation of our policies to terrain difficulties not seen during training.

From Table~\ref{tab:ch3_results_difficulty}, we can see how policies adapt to the terrain during training, with some policies (Gaps, Hurdles, Steps) performing poorly when evaluated with an easy terrain difficulty. The Gaps policy has overfit to the final difficulty, performing poorly on reduced (15.4\%) or increased (11.5\%) difficulty. For all other terrain types we can see improved performance on the reduced difficulty terrain, and comparable performance for some terrain types with increased difficulty (Flat 94.5\% compared to 99.9\%, Stairs 50.5\% compared to 57.6\%), suggesting generalisation in these cases. An alternative training strategy that involves training with terrains of multiple difficulties may improve policy performance over a wider range of terrain difficulties.


This chapter presented the investigation of research question: \textbf{\textit{How can complex visuo-motor locomotion behaviours be learned efficiently?}} The contributions of this chapter are as follows:

\begin{itemize}
    \item A novel learning approach was demonstrated for training behaviours to traverse complex terrain types with a dynamic biped in simulation. It was shown that a single rudimentary walking trajectory can be used as a target policy to improve exploration and training outcomes for a diverse set of difficult obstacles
    
    % \item We proposed a 3-stage curriculum learning approach
    % tailored for bipedal walking on complex terrain
    % types
    % \item  We show that a single rudimentary walking
    % trajectory can be used as a target policy to
    % improve exploration and training outcomes for
    % several difficult terrain types
    % \item We perform extensive analysis and ablation studies
    % showing the importance of the design choices for our
    % curriculum approach, and demonstrate the successful traversal of multiple
    % challenging terrain types
    % \item We developed a Gap Behaviour policy for controlling a large tracked robot through small gaps
    % \item We designed a method to learn when to autonomously activate the Gap Behaviour policy. Our system integrates both learned behaviours and manually designed controllers
    % \item We performed proof-of-concept demonstration of the effectiveness of the approach in the real world using a policy trained only in simulation. We identify the some of the sources of disparity, and discuss plans for addressing differences in future work
\end{itemize}

“Guided Curriculum Learning for Walking Over Complex Terrain” was
published and presented at the 2020 Australasian Conference on Robotics and Automation held in Brisbane, Australia and virtually. 
\newpage
\newpage

% \includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/Guided_Curriculum_Learning_for_Walking_Over_Complex_Terrain.pdf}

% \includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/GRC_Statement-of-Contribution_Form_curriculum.pdf}

% \includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/Passing_Through_Narrow_Gaps_with_Deep_Reinforcement_Learning.pdf}

% \includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/GRC_Statement-of-Contribution_Form_passing.pdf}


    % \item We proposed a 3-stage curriculum learning approach
    % tailored for bipedal walking on complex terrain
    % types
    % \item  We show that a single rudimentary walking
    % trajectory can be used as a tarfget policy to
    % improve exploration and training outcomes for
    % several difficult terrain types
    % \item We perform extensive analysis and ablation studies
    % showing the importance of the design choices for our
    % curriculum approach, and demonstrate the successful traversal of multiple
    % challenging terrain types
    % \item We developed a Gap Behaviour policy for controlling a large tracked robot through small gaps
    % \item We designed a method to learn when to autonomously activate the Gap Behaviour policy. Our system integrates both learned behaviours and manually designed controllers
    % \item We performed proof-of-concept demonstration of the effectiveness of the approach in the real world using a policy trained only in simulation. We identify the some of the sources of disparity, and discuss plans for addressing differences in future work
    
    
% Three paragraphs: Explain motivation, what you did, results

% Final part: What research question you answered, what the contribution was, and what the publication was.

% \textit{One idea per paragraph. First sentence summarises the whole paragraph, last sentence leads into the next.}

% \textbf{Introduce the work in this chapter: robots, obstacles, DRL with visuo-motor policies}


% policies are subject to local minima where
% Visuo-motor policies can be difficult to train, and require high levels of interaction between the robot and the environment.

% require many samples. Furthermore, policy training for complex obstacles are subject to local minima where typical exploration techniques may not be sufficient to direct the robot to the required behaviour. The efficiency of learning behaviours for robot locomotion over difficult obstacles is explored throughout this chapter.


% \textbf{Discuss how this chapter answers the research questions: how are behaviours learned efficiently, how is reliable switching achieved.}


% The contributions of this chapter are provided by research paper \cite{tidd_guided_2020}, and explores research question 1: the efficient learning of visuo-motor behaviours. Efficient learning is demonstrated by learning behaviours using a simple expert controller with reward shaping. Importantly, the expert is not able to complete the task, it is a rudimentary behaviour that is used to bootstrap learning the complex behaviour. For the complex behaviours required by the biped, a curriculum learning method is introduced to greatly improve training efficiency.  These investigations show the efficient development of difficult behaviours (research questions 1). 

% The behaviours developed in this chapter enable a simulated bipedal robot with a depth sensor to walk over difficult obstacles including steps, stairs, gaps, and hurdles. Curriculum learning is the idea of starting with an achievable version of a task and increasing the difficulty as a success criteria is met. Reliable bipedal walking over complex terrain is a challenging problem, using a curriculum can improve learning outcomes [\cite{yu_learning_2018}].


% . While CL greatly improved the efficiency of learning behaviours, curriculum parameters, for example the decay rate, were determined manually. 
% An adaptive curriculum that alleviated manual tuning could further improve learning efficiency.

% and enable the development of more complex behaviours.

% complex visuo-motor
% following a simple walking trajectory

% Figure \ref{fig:ch3_stage3} shows the effect of each curriculum stage on episode reward during training, where the solid lines show the progress without a curriculum.

% Figure  \label{fig:cha3_fig2} shows the system used for each behaviour. 





% \textbf{Should limitations be discussed here, (currently left for the final discussion}

% \textbf{High level discussion of the methods and results for paper 2}


% \textbf{Conclusions related to the research questions}


% \textbf{Summary of Contributions}




% Previous chapters have considered traversing obstacles and how to reliably switch between behaviours in the context of simulated biped. This chapter we investigate the research question involving autonomously traversing narrow gaps, and the challenges of deploying behaviours trained in simulation on a real agent. The problem that we are aiming to solve in this chapter is getting a large tracked robot through a doorway (Fig. \ref{fig:cha5_fig1}). 


% Not sure what I'm trying to say here.
% While a tracked robot is statically stable compared with a biped, passing through a tight space and switchinthere are challenges in switching behaviours.


% The second scenario explored is a real world application of passing through small gaps with a large tracked platform. The DARPA Subterranean Challenge required teams of robots to traverse difficult and diverse underground environments. Traversing small gaps is one of the challenging scenarios that robots encounter, for example a tunnel entrance, or a doorway (Figure \ref{fig:cha5_fig1}). Path planning methods struggle with imperfect sensor information and low resolution costmaps when gaps marginally wider than the agent are perceived as smaller than the robot footprint. Classical navigation methods require significant manual fine tuning to design behaviours to handle these difficult perception cases. Presented in the second half of this chapter is a DRL method for autonomous navigation through small gaps, where contact between the robot and the gap may be required. A Gap Behaviour policy is trained to get the robot through small gaps (only centimeters wider than the robot) using an occupancy map with a resolution of 10cm. A goal-conditioned Behaviour Selection policy is then trained to determine when to activate the Gap Behaviour policy. The policies trained in simulation are demonstrated on the real platform. Figure \ref{fig:cha5_fig2} shows the pipeline that is applied in the final scenario. The Behaviour Selection policy outputs a switch parameter $\tau$ that determines when to use the Gap Behaviour and when to use the pre-existing Behaviour Stack [\cite{hines_virtual_2021}]. The Gap Behaviour outputs the forward and heading velocities of the robot. 


% \begin{figure}[htb!]
%     % \vspace{2mm}
%     \captionsetup[subfigure]{labelformat=empty}
%     \centering 
%     \subfloat[]{\includegraphics[trim=1cm 1cm 1cm 2cm, clip,width=0.38\columnwidth]{images/ch6/real_door4.png}}
%     \hfil
%     \subfloat[]{\includegraphics[trim=5.0cm 0.0cm 0.2cm 15.3cm, clip, width=0.42\columnwidth]{images/ch6/real_door2.jpg}}
%     \hfil
%     % \vspace*{-3mm}
%     % \hfill
%     \caption{The problem of traversing narrow gaps with a mobile robot was investigated.}
%     \label{fig:cha5_fig1}
%     %\vspace{-3mm}
% \end{figure}





% \begin{figure}[tb!]
% % \vspace{2mm}
% \centering
% \subfloat[Gap Behaviour]{\includegraphics[trim=1.8cm 3.6cm 1.8cm 3cm, clip, width=0.45\columnwidth]{images/ch6/door1.png}}
% \hspace{0.3cm}
% \subfloat[Behaviour Selection]{\includegraphics[trim=4.2cm 4.4cm 4cm 3.7cm, clip, width=0.41\columnwidth]{images/ch6/door2.png}}
% \caption{The circular markers represent reward targets.}
% \label{fig:ch5_doors}
% \end{figure}


% \begin{figure}[htb!]
%     % \vspace{2mm}
%     \centering
%     \includegraphics[width=0.85\columnwidth]{images/ch6/Fig2.png}
%     %\hfill
%     \caption{A Gap Behaviour and a Behaviour Selection policy were trained using an occupancy map and robot state as input. The Behaviour Selection policy determines when  the Gap Behaviour should be active or when the robot should utilise a pre-existing Behaviour Stack.}
%     \label{fig:cha5_fig2}
%     % \vspace{-3mm}
% \end{figure}



% \begin{figure}[ht!]
%     \vspace{-5mm}
%     \centering
%     % \subfloat[Gap behaviour policy]{\includegraphics[trim=1cm 0.5cm 1cm 2cm, clip, width=0.5\columnwidth]{images/results0.png}}
%     \subfloat[Gap Behaviour policy]{\includegraphics[trim=0cm 0.0cm 0cm 0cm, clip, width=0.5\columnwidth]{images/ch6/results0.png}}
%     \hfil
%     % \subfloat[Behaviour selection policy]{\includegraphics[trim=1cm 1cm 1cm 2cm, clip,width=0.45\columnwidth]{images/results1.png}}
%     \subfloat[Behaviour Selection policy]{\includegraphics[trim=0cm 0cm 0cm 0cm, clip,width=0.5\columnwidth]{images/ch6/results1.png}}
%     \hfil
%     % \hfill
%     \caption{Success rates during training for the Gap Behaviour policy and the Behaviour Selection policy.}
%     \label{fig:ch5_learning_curves}
%     %\vspace{-3mm}
% \end{figure}


% \begin{figure}[htb!]
%     % \vspace{2mm}
%     \centering
%     \subfloat[Gazebo Simulator]{\includegraphics[trim=3cm 7cm 3cm 6cm, clip, width=0.5\linewidth]{images/ch6/gazebo.png}}
%     \hspace{0.3cm}
%     \subfloat[Real Robot]{\includegraphics[trim=3cm 4cm 0cm 12.2cm, clip, width=0.4\linewidth]{images/ch6/real_door.jpg}}
%     \caption{Experimental setup in simulation and with the real robot.}
%     \label{fig:cha5_fig3}
% \end{figure}

% In simulation experiments, this approach achieves a success rate of 93\% when the Gap Behaviour is activated manually by an operator, and 63\% with autonomous activation using the Behaviour Selection policy (Table \ref{tab:ch5_sim_results}). In real robot experiments, a drop in performance is observed, with a success rate of 73\% with manual activation, and 40\% with autonomous behaviour selection (Table \ref{tab:ch5_real_results}). While the feasibility of this method is demonstrated in simulation, the difference in performance between simulated and real world scenarios highlights the difficulty of direct sim-to-real transfer for DRL policies. In both the simulated and real world environments alternative methods were unable to traverse the gap. It was demonstrated with these experiments that a behaviour for traversing gap had a good success rate, however the method for switching between sequential behaviours requires further investigation.

% \textbf{Figures and tables}


% The sources of sim-to-real disparity are discussed in this section. A difference in training results was observed when comparing ground truth perception and an occupancy map generated by simultaneous localisation and mapping (SLAM) from a simulated LiDAR. In each case the simulation dynamics were the same, this difference is likely the effect of a noisy Velodyne model. Adding noise to perception during training may improve these results. We also observed a performance drop when applying these algorithms to the real robot. This disparity was likely the cause of out of distribution examples, and sim-to-real physics differences. In a number of occasions the robot would catch on the door frame, and the wooden surface was much more slippery than the ground surface in the simulation. These issues could be reduced by adding more gap types during training, as well as dynamics randomisation. We leave these investigations for future work.

% First we learn a Gap Behaviour policy using ground truth perception with a reward that encourages the robot to line up the gap. Fig.\ref{fig:ch5_doors}.a) shows how we place markers to encourage the robot to first align to the gap before moving through. We then learn a Behaviour Selection policy that learns when to activate the Gap Behaviour, and when to instead default to a pre-existing Behaviour Stack. Fig.\ref{fig:ch5_doors}.b) shows the reward used to train the behaviour selector policy. As the robot moves sequentially between markers 1 to 4, when marker 2 and marker 3 are active, the reward encourages the gaps behaviour to be active. The pipeline once both policies are trained is shown in Fig. \ref{fig:cha5_fig2}. Both the Behaviour Selection policy and the Gap Behaviour use an occupancy map and robot state vector. The Behaviour Selection policy also has a goal waypoint as input and outputs a switch parameter $\tau$ that determines when to use the Gap Behaviour and when to use the pre-existing Behaviour Stack. The Gap Behaviour outputs the forward and heading velocities of the robot. 


% Fig. \ref{fig:ch5_learning_curves} shows the progress through training for the Gap Behaviour, and for the Behaviour Selection policy. We also showed the results of training Behaviour Selection as a supervised problem. Using the same amount of data and training updates we saw the reinforcement learning method achieved a faster learning rate and more reliable final policy. We perform an analysis comparing the behaviours in simulation using an occupancy map generated from SLAM data and a simulated Velodyne LiDAR, and also using the same system on a real platform (Fig. \ref{fig:cha5_fig3}). Table \ref{tab:ch5_sim_results} shows the results of experiments in simulation, and Table \ref{tab:ch5_real_results} shows the results for the real experiments. We can see that there is a disparity between the training results, the simulation results, and the real results. 



% \begin{table}[h!]
%     %\vspace{-2mm}
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c}
%     % \begin{adjustbox}{max width=1.0\columnwidth}
%     % \begin{adjustbox}{min width=0.75\columnwidth}
%     % \begin{adjustbox}{max width=1.0\columnwidth}
%     \begin{tabular}{cccccc}
%         % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
%                                       & Success \% & Time(s) & Operator Actions \\
%       \hline
%         Behaviour Stack      & 0.0            &  50.2 &    1  \\
%         Manual Gap Behaviour Selection        & 93.3          &  29.7 &    3  \\
%         Auto Gap Behaviour Selection  & 63.3          &  45.3 &    1 \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{Simulation results for passing through a narrow gap (30 trials)}
%     \label{tab:ch5_sim_results}
% \end{table}


% \begin{table}[h!]
%     % \vspace{-2mm}
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c}
%     % \begin{adjustbox}{max width=1.0\columnwidth}
%     % \begin{adjustbox}{max width=1.0\columnwidth}
%     \begin{tabular}{cccccc}
%         % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
%                                       & Success \% & Time(s) & Operator Actions \\
%       \hline
%         Behaviour Stack              & 0.0           &  44.6 &    1  \\
%         Manual Gap Behaviour Selection               & 73.3          &  24.1 &    3  \\
%         Auto Gap Behaviour Selection         & 40.0          &  30.9 &    1 \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     % \vspace{-2mm}
%     \caption{Real robot results for passing through a narrow gap (15 trials).}
%     \label{tab:ch5_real_results}
% \end{table}





% ``How can we efficiently learn locomotion behaviours for traversing difficult obstacles?"
% ``How can we reliably transition between behaviours?"
% ``What are some of the challenges of training behaviours in simulation for real world applications?"



==> old/Ch3b_mono.tex <==
% \chapter[Guided Curriculum Learning for Walking Over Complex Terrain]{Guided Curriculum Learning for Walking Over Complex Terrain}
\chapter[Passing Through Narrow Gaps]{Passing Through Narrow Gaps with Deep Reinforcement Learning}
   
% \item \textbf{Research Question 1: \textit{How can complex visuo-motor locomotion behaviours be learned efficiently, without knowing exactly how an expert would perform the action?}}

\label{cha:ch3b}
% Motivation/contribution/abstract -----------------------



% Three paragraphs: Explain motivation, what you did, results

% Final part: What research question you answered, what the contribution was, and what the publication was.

% \textit{One idea per paragraph. First sentence summarises the whole paragraph, last sentence leads into the next.}

% \textbf{Introduce the work in this chapter: robots, obstacles, DRL with visuo-motor policies}

This chapter presents work on designing behaviours for a large tracked robot passing through a narrow gap in a real world application. The tracked platform uses an occupancy map, and must pass through small gaps that are difficult to plan through using traditional methods. The behaviours developed in this section rely on feedback from perception. For example the tracked robot is required to align to the entrance of a narrow doorway. For these reasons behaviours are difficult to manually design. DRL methods enables the development of visuo-motor policies, however sample efficiency limits their application in complex scenarios. Typically, visuo-motor policies are difficult to train, and requires high levels of interaction between the robot and the environment. Furthermore, for locomotion over difficult obstacles, policies are subject to local minima where commonly used exploration techniques may not be sufficient to direct the robot to the required behaviour. Improving the efficiency of learning behaviours for robot locomotion over difficult obstacles is explored throughout this chapter.

% require many samples. Furthermore, policy training for complex obstacles are subject to local minima where typical exploration techniques may not be sufficient to direct the robot to the required behaviour. The efficiency of learning behaviours for robot locomotion over difficult obstacles is explored throughout this chapter.


% \textbf{Discuss how this chapter answers the research questions: how are behaviours learned efficiently, how is reliable switching achieved.}

The contributions of this chapter are provided by research paper \cite{tidd_passing_2021}, exploring research question 1: the efficient learning of visuo-motor behaviours, and introducing the first investigation of reliable switching between behaviours (research question 2). Efficient learning is demonstrated by learning behaviours using a simple expert controller with reward shaping. Importantly, the expert is not able to complete the task, it is a rudimentary behaviour that is used to bootstrap learning the complex behaviour. In addition to the efficient design of behaviours, this chapter also considers the application of controllers to a real world scenario where the learned behaviour for passing through gaps required behaviour switch as it was integrated with a pre-existing behaviour library. These investigations show the efficient development of difficult behaviours, and an approach to switch between sequential behaviours (research questions 1 and 2). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Robotic Platform}
\label{sec:robotic_platform}
The `Titan' all terrain robot (ATR) from BIA5~\cite{bia5_robotic_2021} is a 90Kg tracked vehicle, with a length of 1.4m and a width of 0.78m. It is the primary autonomous platform in a heterogeneous fleet of robots (tracked, legged, aerial) used by team CSIRO Data61's~\cite{hudson_heterogeneous_2021} entry in the SubT Challenge systems track~\cite{darpa_darpa_2021}. The Titan moves with nonholonomic motion following forward and heading velocity commands, and can turn on the spot (skid-steer).

\textbf{Perception Stack:}
Like all robots in team CSIRO Data61, the Titan has a `Catpack' perception system equipped with a tilted spinning Velodyne Lidar, Inertial Measurement Unit (IMU), 4 RGB cameras, and 3 thermal cameras. Each robot performs Simultaneous Localisation and Mapping (SLAM) onboard, providing a height map that is used by local navigation behaviours for fully autonomous navigation. Goals are provided by a higher level planner, encouraging thorough exploration in the search for artifacts (the full specifications of the Catpack and system solution can be found in~\cite{hudson_heterogeneous_2021} and ~\cite{hines_virtual_2021}). 

\textbf{Behaviour Stack:}
Among several manual defined controllers, the primary navigation behaviour is a \textit{path follow} behaviour that takes a goal point and calculates a safe path using hybrid A* search that associates a continuous state with each grid cell (in opposed to discrete cell center in standard A* search), allowing the path to consider vehicle kinematic constraints~\cite{dolgov_path_2010, hines_virtual_2021}. An \textit{orientation correction} behaviour recovers the robot to a level position in the case of extreme roll or pitch, and a \textit{decollide} behaviour will perform a maneuver into a safe location when there is fatal cost within the robot footprint. There is also a teleoperation behaviour (\textit{Joy}) for situations the operator can manually control a robot (when the robot is within communication range with the ground control station). Each behaviour is ranked in order of priority (shown in Fig.~\ref{fig:ch3b_fig2}, behaviour stack), where the admissible behaviour with the highest priority is activated. Each behaviour is responsible for detecting its own admissibility.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\label{sec:method}

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=\columnwidth]{images/ch6/Fig2.png}
%\hfill
\caption{We learn a gap behaviour and a behaviour selection policy using an occupancy map. The behaviour selection policy determines when the gap behaviour should be active based on a goal location, or when we should rely on a manually designed behaviour stack~\cite{hudson_heterogeneous_2021}. The system is trained in simulation, then tested on the real platform.}
\label{fig:ch3b_fig2}
% \vspace{-3mm}
\end{figure}

%Despite a sophisticated perception stack and a well-tuned navigation stack, identifying and traversing narrow gaps remains a challenge. 

Fig.~\ref{fig:ch3b_fig2} outlines our system. The gap behaviour policy receives $s_t = [rs_t, I_t]$ (defined below), and outputs action $a_t$, consisting of forward and angular velocity about the $z$ axis (heading). The behaviour selection policy is also provided with $s_t$, as well as a goal location, and outputs switching parameter $\tau$. The gap behaviour should be activated by the behaviour selection policy when a goal is located behind a small gap, otherwise the behaviour stack should be active.

\subsection{Problem Description}
\label{sec:problem}

Traversing small gaps is important for underground search and rescue scenarios, such as those found in the SubT Challenge~\cite{darpa_darpa_2021}. The SubT Challenge involves detecting and localising artifacts (survivors, backpacks, helmets, etc) in underground environments (mine, urban, cave), where large portions of the course may only be accessible after a narrow constriction. Due to the large scale of the scenarios encountered, teams of robots are required to enter the underground environment, with a limitation that there can only be a single human operator. The human operator can command the robots through any method, though communications to robots are severely limited. Furthermore, coordinating multiple robots while reporting artifact detections in a timed competition (1 hour) presents a significant load on the operator. The robots must be as autonomous as possible. In these search and rescue scenarios the robot is allowed to make contact with the environment, but not intentionally damage it. In this paper we target traversing small doorways.


\subsection{Reinforcement Learning}
\label{sec:rl}

We consider our problem to be a Markov Decision Process $\text{MDP}$, where each state contains all relevant information to make a decision. An MDP is defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. 

With reinforcement learning, the goal is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is the reward at time $t$. Actions are continuous values, sampled from a deep neural network ($a_t\sim\pi_\theta(s_t)$ for the gap behaviour policy, $\tau_t\sim\pi_\phi(s_t, goal)$ for the behaviour selection policy), and $s_t$ includes the robot state $rs_t$ and occupancy map $I_t$ (introduced below). We update each policy with Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}, using the implementation by OpenAI~\cite{dhariwal_openai_2017}.

%  where $a_t = \hat{v}_x, \hat{v}_\omega$ is the linear and angular velocity sent to the robot 
 
\textbf{Robot State $rs_t$:} The robot state is a vector of 7 numbers containing the heading velocity $v_x$, and the angular position and velocities: $roll, pitch, yaw, v_{roll}, v_{pitch}, v_{yaw}$. Velocity terms are calculated with clipped finite differences. These terms are important for determining when the robot has made contact with the wall.

\textbf{Occupancy Map $I_t$:} A binary occupancy map with dimensions $[80,80,1]$ and resolution of 0.1m is provided to the each policy (gap behaviour policy, and behaviour selection policy). A value of 0 indicates a known and unoccupied cell, and a value of 1 indicates an unknown or occupied cell. The occupancy map moves with the $x$, $y$ translation and $yaw$ rotation of the robot, with the center of the robot located at the centre of the occupancy map. During training of both policies, the occupancy map is created using the ground truth position of the door frames and the robot location from the simulation. During testing (both in simulation and on the real robot), the occupancy map is supplied by the perception stack outlined above (Sec.~\ref{sec:robotic_platform}).
%  from the high density point cloud (details are provided in~\cite{hudson_heterogeneous_2021})

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[Gap Behaviour]{\includegraphics[trim=1.8cm 3.6cm 1.8cm 3cm, clip, width=0.45\linewidth]{images/ch6/door1.png}}
\hspace{0.3cm}
\subfloat[Behaviour Selection]{\includegraphics[trim=4.2cm 4.4cm 4cm 3.7cm, clip, width=0.41\linewidth]{images/ch6/door2.png}}

\caption{A simulation of a narrow door. The circular markers represent reward targets. a) The two doorway points are used by the gap behaviour policy. b) Behaviour selection policy uses two pairs of markers.}
\label{fig:ch3b_doors}
\end{figure}

We train a gap behaviour policy to go through small gaps, and a behaviour selection policy that activates the gap behaviour when a goal appears behind a gap. The training setup is show in Fig.~\ref{fig:ch3b_doors}. Fig.~\ref{fig:ch3b_doors}a is used to train the gap behaviour policy, markers depict the entrance and exit to a gap ($m_1,m_2$). Fig.~\ref{fig:ch3b_doors}b shows the setup for training the behaviour selection policy where additional markers show the goal points provided to behaviour selection ($m_1, m_4$).

\subsection{Gap Behaviour Policy}
\label{sec:behaviour}
The gap behaviour receives a stacked robot state message from the previous 5 timesteps: $[rs_t, rs_{t-1}, rs_{t-2}, rs_{t-3}, rs_{t-4}]$. The robot starts from a random initial position in front of a doorway, where the initial position is uniformly selected from a circle 1.5m back from the first marker $m_1$, with a radius of 1.5m. We also randomise the heading of the robot, choosing uniformly between -1.5 and 1.5 radians from the heading perpendicular to the gap. The target marker is set to the initial marker at the entrance to the gap $m_1$. All initial positions and heading ranges are selected based on the field of view of the perception system.

\textbf{Reward:} The reward terms encourage forward progress towards the target marker. Once the robot is within 0.5m of the target marker (initially set to marker $m_1$), the marker through the gap becomes the new target ($m_2$). This encourages the robot to approach the gap with the correct heading to make it through. The reward is defined as:
\[r_t = 1.5 r_{\dot{v}_x} - 0.1r_\theta - 0.05r_a - 0.75r_{\phi} - 0.001r_{s} - 0.25r_{v_{-x}}\]

where $r_{\dot{v}_x}$ is the velocity towards the target marker, $r_\theta$ is the error in heading between the robot and the target marker, $r_a$ is a penalty on angular velocity, $r_{\phi}$ is a penalty on roll and pitch angles, $r_{s}$ is a smoothing cost (previous actions should be close to the current actions), and $r_{v_{-x}}$ is a penalty for going backward. 

We train for 1000 episodes, where episodes are a fixed length of 180 steps (with a timestep of 0.1s), and the policy is updated at the end of an episode. 16 workers (CPU's) run in parallel, performing synchronised policy updates. Each robot is randomly inserted at the beginning of each episode, choosing between 98 different doorways (each with small variations in gap width, and door position). An episode is considered successful if the robot reaches $m_2$ (the marker after the door). All training parameters, including reward coefficients, are tuned empirically using task success.  

% Titan is allowed to make contact with the door

\subsection{Behaviour Selection Policy}
\label{sec:behaviour_selection_method}

% During the SubT challenge there is a single human supervisor for a fleet of 5 or more robots. Autonomy is paramount for success. 
While part of the problem we are considering involves controlling the robot through a narrow gap, to integrate the behaviour into the SubT behaviour stack, we must also know when the gap behaviour should be activated.

We once again use reinforcement learning to train an admissibility prediction that detects when the gap behaviour should be run, and when we should default to the behaviour stack (introduced in Sec:\ref{sec:robotic_platform}). The behaviour selection policy receives the robot state message $rs_t$, occupancy map $I_t$, and a goal location (distance and angle in the robot frame).

As we should only traverse a gap if there is a goal on the other side of the gap, we condition behaviour selection on having a goal. If the goal is on the same side of the gap as the robot, we do not want to activate the gap behaviour, but if is on the the other side we do. We have four markers $[m_1, m_2, m_3, m_4]$, shown in Fig.~\ref{fig:ch3b_doors}b). Markers 1 and 4 are considered goals, and are provided to the behaviour selection policy. These goals would be provided by a higher level exploration planner. Markers 2 and 3 are the same as for the gap behaviour (entrance and exit of the gap) and are used to design the reward.

We start the robot from a random position sampled uniformly from a circle 4.5m before the door marker $m_2$ with a radius of 1.5m. $m_1$ and $m_4$ are also randomly selected from a uniform distribution, $m_1$ is located 1.5m \textit{before} $m_2$, and $m_4$ is located 1.5m \textit{after} $m_3$. The robot heading is randomly sampled from $(-\pi, \pi)$. This heading range is larger than the range used to train the gap behaviour, allowing the behaviour selection policy to be robust to any robot heading, where the gap behaviour is only expected to operate when the gap is in front of the robot.

\textbf{Reward:}
The reward term for behaviour selection is dependent on the current target marker. Once the robot is within 0.5m of a marker, we update the target marker to the next marker in the sequence. The robot should activate the behaviour stack (path follow behaviour) if it has not yet reached $m_1$, or has reached $m_3$. If the robot has reached $m_1$, but has not yet reached $m_3$, it should use the gap behaviour. The reward for behaviour selection is defined as:
\begin{equation}
\label{sup_reward}
    r_t = 
\begin{cases}
    1 - (\tau_t - 0.0)^2,& \text{if the target is } m_1 \text{ or } m_4 \\
    1 - (\tau_t - 1.0)^2,& \text{if the target is } m_2 \text{ or } m_3
\end{cases}
\end{equation}

Where $\tau$, a binary variable, is the output of the behaviour selection policy at time $t$. $\tau$ of 1.0 indicates activating the gap behaviour, and 0.0 the behaviour stack.

% ~\textbf{Path Follow Behaviour} is a proportional controller that minimise the angular position error of the robot and the goal point, and the distance to the goal. Starting the robot from a random position in front of the point, we run the policy determined by the gap detector.  

\textbf{Auxiliary task:} Learning an auxiliary task can help with the learning of visual features~\cite{jaderberg_reinforcement_2016}. We learn an auxiliary task with the behaviour selection policy. As shown in Fig.~\ref{fig:ch3b_fig2}, the auxiliary task shares the convolution layers with behaviour selection, but has two separate fully connected layers. The auxiliary task uses a supervised learning loss to learn the gap width, and location of the gap markers. The auxiliary output is a vector of 5 terms: 
\[aux = [w, m_{2_{dist}}, m_{2_{angle}}, m_{3_{dist}}, m_{3_{angle}}] \]

Where $w$ is gap width, $dist$ and $angle$ are polar coordinates from the respective gap marker ($m_2, m_3$) to the robot ($dist$ is the distance to the robot, $angle$ is the heading error). We train the auxiliary term with mean squared error loss from the ground truth provided by the simulation. Learning the location of the gap has the additional benefit of providing visual information to the operator. If the gap behaviour is activated, the operator can clearly see the gap.

% We train the behaviour selection for 200 updates with 16 workers, randomly choosing between 98 different doorways. Episode lengths are fixed at 300 timesteps.

The gap behaviour policy and the behaviour selection policy are trained in simulation using the Gazebo simulator. We insert walls into the simulator so the robot must drive through gaps (sampled uniformly from $0.8 - 0.85$m). We also add doors in various open configurations. Due to the computational demands of running the full perception stack on a single computer while running multiple agents, the occupancy map is generated from simulation data while training. When the policy is being trained, the occupancy map is generated by inserting blocks into known locations in a global occupancy map, then sampling a robot-centric map using the robot pose ($x,y,yaw$). For testing, we rely on the occupancy map generated by the perception stack, for both simulation and real robot experiments (Sec.~\ref{sec:experiments}.B and Sec.~\ref{sec:experiments}.C).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

\begin{figure}[t!]
    \vspace{-5mm}
    \centering
    % \subfloat[Gap behaviour policy]{\includegraphics[trim=1cm 0.5cm 1cm 2cm, clip, width=0.5\columnwidth]{images/ch6/results0.png}}
    \subfloat[Gap behaviour policy]{\includegraphics[trim=0cm 0.0cm 0cm 0cm, clip, width=0.5\columnwidth]{images/ch6/results0.png}}
    \hfil
    % \subfloat[Behaviour selection policy]{\includegraphics[trim=1cm 1cm 1cm 2cm, clip,width=0.45\columnwidth]{images/ch6/results1.png}}
    \subfloat[Behaviour selection policy]{\includegraphics[trim=0cm 0cm 0cm 0cm, clip,width=0.5\columnwidth]{images/ch6/results1.png}}
    \hfil
    % \hfill
    \caption{Success rates during training for the gap behaviour policy and the behaviour selection policy.}
    \label{fig:ch3b_learning_curves}
    %\vspace{-3mm}
\end{figure}

% \begin{figure}[tb!]
% % \vspace{2mm}
% \centering
% \includegraphics[width=0.65\columnwidth]{images/ch6/selector.png}
% % \includegraphics[width=\columnwidth]{images/ch6/selector.png}
% % \includegraphics[width=\wIII cm, height=\hII cm]{images/ch6/selector.png}
% \hfill
% \caption{We compare training the behaviour selector using a supervised learning approach and a reinforcement learning method, trained with an identical setup for 3 random seeds.}
% \label{fig:ch3b_results_selector}
% % \vspace{-3mm}
% \end{figure}

We first show the results of training our policies (Sec.~\ref{sec:training}). Sec.~\ref{sec:simulation} shows the results in simulation using the perception stack (introduced in ~\ref{sec:problem}), and the real robot results are shown in Sec.~\ref{sec:real}. Fig~\ref{fig:ch3b_modes}.a and b) show the setup for the simulated and real doors.

\subsection{Training Results}
\label{sec:training}

The \textbf{gaps behaviour policy} achieves a success rate of 93.8\% on the simulated environment (98 gaps of random width and door type). The success rate while training is shown in Fig.~\ref{fig:ch3b_learning_curves}.a). The behaviour performs several complex maneuvers that would be difficult to encode manually. These maneuvers include approaching the gap with one corner and making contact with the door, reversing and re-approaching when the robot pitches, and `wiggling' when the robot is part way through but not making progress.

Once the gap behaviour policy is trained, we train the \textbf{behaviour selection policy} with the method from Sec\ref{sec:behaviour_selection_method}. The results shown in Fig~\ref{fig:ch3b_learning_curves}.b), display the success rate for behaviour selection training. We compare using a supervised loss to using our reinforcement learning method for learning behaviour selection:

~\textbf{Supervised Learning:} Behaviour selection could be considered a supervised learning problem where robot state with occupancy map at each timestep are taken as input, and are given a label. We use labels of 0 if the target marker is $m_1$ or $m_4$, and 1 if the target marker is $m_2$ or $m_3$. We update network weights using mean squared error loss.

~\textbf{Reinforcement Learning:}
We train the behaviour selection policy using the reinforcement learning approach introduced in Sec~\ref{sec:behaviour_selection_method}, where we use a reinforcement learning update with the reward from Equation~\ref{sup_reward}.

In both examples we also predict the auxiliary terms, which include door size, and marker locations relative to the robot. Both methods were trained with online data using the same training parameters. As can be seen in Fig.~\ref{fig:ch3b_learning_curves}, the \textbf{reinforcement learning} approach achieves more successful door traversals, with an asymptotic success rate of 88.7\%, compared to 75.8\% with the \textbf{supervised learning} approach. We attribute the difference between the methods on the reinforcement learning approach considering the sum of future behaviour selections, whereas the supervised approach only considers the current timestep. We found that excluding the auxiliary terms from training had very little effect on success rate. We also tested various additional parameters in the reward function but found almost no effect on success rate. We have omitted these results from Fig.~\ref{fig:ch3b_learning_curves}b) for clarity. 

% ~\textbf{Additional Reward Terms:}
% We train with additional reward terms.

% ~\textbf{Supervised Reward with Reinforcement Learning:}
% We use a supervised reward from equation ~\ref{sup_reward}, using reinforcement loss from PPO~\cite{schulman_proximal_2017}.

% ~\textbf{Supervised Reward with Auxiliary Terms:}
% We train a reinforcement learning network to also predict the auxiliary terms, which include door size, and marker locations relative to the robot.


\subsection{Simulation Results}
\label{sec:simulation}

We test our gap behaviour and behaviour selection policies in simulation on an unseen test world, using the ~\textit{perception stack} (Lidar scans are used to produce the occupancy map). The test world has gaps uniformly sampled from $0.8-0.85$m, with random door types. We compare several modes of operation including using the behaviour stack without the gap behaviour, manually activating the gap behaviour, and using the behaviour selection policy to autonomously activate the gap behaviour.

~\textbf{Behaviour Stack:} The current navigation stack used by the Titan platform uses several behaviours described in Sec~\ref{sec:problem}: path follow, orientation correction and decollide. Path follow is the dominant behaviour where hybrid A* search is used to find a path to a local goal. For more details about the behaviour stack see~\cite{hines_virtual_2021} and~\cite{hudson_heterogeneous_2021}. For these experiments the operator inserts a waypoint on the opposite side of a gap.

~\textbf{Manual Gap Behaviour Selection:} The operator can manually call the gap behaviour from a GUI. The operator must first insert a waypoint so the robot approaches the gap (running the behaviour stack), then activate the gap behaviour, and when the robot is through the gap once again activate the behaviour stack to get the robot to the waypoint after the door.

~\textbf{Autonomous Gap Behaviour Selection:} The gap behaviour is autonomously selected when the conditions are met (there is a goal behind a small gap). The operator can place a waypoint on the other side of a door and behaviour selection will activate the behaviour stack or the gap behaviour autonomously. 


\begin{table}[h!]
    %\vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    % \begin{adjustbox}{min width=0.75\columnwidth}
    \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Time(s) & Operator Actions \\
       \hline
        Behaviour Stack      & 0.0            &  50.2 &    1  \\
        Manual Gap Behaviour Selection        & 93.3          &  29.7 &    3  \\
        Auto Gap Behaviour Selection  & 63.3          &  45.3 &    1 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Simulation results for passing through a narrow gap (30 trials)}
    \label{tab:ch3b_sim_results}
\end{table}

% Fig~\ref{fig:ch3b_modes}.c to e) show the three modes of operation. In Fig~\ref{fig:ch3b_modes}.c) the behaviour stack reaches a timeout for all small gaps. Fig~\ref{fig:ch3b_modes}.d) shows the additional operator load for running the gap behaviour manually, and Fig~\ref{fig:ch3b_modes}.e) shows behaviour selection including the auxiliary reward marking the gap position.

We perform 30 trials and present results in Table~\ref{tab:ch3b_sim_results}. We show the average success rate, time until the final waypoint, and the number of operator actions. We can see that the behaviour stack cannot traverse the gap and reaches a timeout (no progress after 30 seconds). Manually activating the gap behaviour has a high success rate (93.3\%), and autonomously selecting behaviours has a reasonable success rate of 63.3\%. Of the failure cases with behaviour selection, the most common cause was the behaviour selector not recognising the gap. We attribute this failure to distribution mismatch between the perception used during training, and the noise introduced by the ~\textit{perception stack}. Other failure cases include the gap behaviour failing, and several cases where oscillation between the gap behaviour and the decollide behaviour caused a timeout on the waypoint. Where decollide did not activate (behaviour selection did not switch back to the behaviour stack midway through the gap), the average time through the gap was 17.3 seconds, suggesting behaviour selection is a viable method, however requires further investigation to ensure robustness.

\begin{figure}[t!]
    % \vspace{2mm}
    \centering
    \subfloat[Gazebo Simulator]{\includegraphics[trim=3cm 7cm 3cm 6cm, clip, width=0.5\linewidth]{images/ch6/gazebo.png}}
    \hspace{0.3cm}
    \subfloat[Real Robot]{\includegraphics[trim=3cm 4cm 0cm 12.2cm, clip, width=0.4\linewidth]{images/ch6/real_door.jpg}}
    \caption{Experimental setup in simulation and with the real robot.}
    \label{fig:ch3b_modes}
\end{figure}

\subsection{Real Robot Results}
\label{sec:real}

% \begin{figure}[tb!]
%     % \vspace{2mm}
%     \centering
%     \subfloat[Real Door]{\includegraphics[width=\w cm, height=\h cm]{images/ch6/real_door.jpg}}
%     \hfil
%     \subfloat[Robot tries to reach goal]{\includegraphics[width=\w cm, height=\h cm]{images/ch6/waypoint1.png}}
%     \hfil
%     \subfloat[Goal timesout]{\includegraphics[width=\w cm, height=\h cm]{images/ch6/Fig5.png}}
%     % \hfill
%     \caption{Real door, waypoint, behaviour, selection.}
%     \label{fig:ch3b_real}
%     \vspace{-3mm}
% \end{figure}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Time(s) & Operator Actions \\
       \hline
        Behaviour Stack              & 0.0           &  44.6 &    1  \\
        Manual Gap Behaviour Selection               & 73.3          &  24.1 &    3  \\
        Auto Gap Behaviour Selection         & 40.0          &  30.9 &    1 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Real robot results for passing through a narrow gap (15 trials).}
    \label{tab:ch3b_real_results}
\end{table}

Table~\ref{tab:ch3b_real_results} show our final experiments applied in a door scenario on a real robot. We use a constructed wooden door rather than a real door as the gap behaviour is allowed to contact the door, which can result in the robot damaging the environment. The constructed door shown in Fig~\ref{fig:ch3b_modes}.b).

We run 15 trials for all experiments, results are shown in Table~\ref{tab:ch3b_real_results}. We confirm our behaviour succeeds in more than 70\% of trials, where the current behaviour stack cannot traverse the gap, timing out after 30 seconds. The behaviour selection method is successful 40\% of the time. Both manually evoking the gap behaviour, and relying on autonomous behaviour selection had the same failure case: the edge of the robot would grab the protrusion of the door and the tracks would spin on the slippery surface. This was not seen in the simulation trials as track slippage is not modeled well in simulation. While this situation may not occur regularly with real doors, future policies will be trained with examples of gaps with small protruding edges. 

Autonomous behaviour selection had a much lower success rate than manually activating the gap behaviour. This is due to the late switching from the behaviour stack to the gap behaviour, and the limitation of our test door (protruding edges). With late switching, the gap behaviour was more likely to get the robot caught on the outer wooden structure of the door. Future behaviour selection models would encourage switching to the gap behaviour earlier, allowing more time to align with the door.

In one case with behaviour selection, the robot was mostly through the gap when the behaviour switched back to the behaviour stack, triggering a decollide behaviour and causing the robot to go in and out of the gap. Training the behaviour selection policy with the marker after the door ($m_3$) further back should result in the gap behaviour being active until after the robot has cleared the door.

While these limitations must be addressed before the behaviour can be properly integrated into the behaviour stack for autonomous operation, the manual activation of the gap behaviour policy has been utilised in a SubT 1 hour test run with 5 different robots (3 Titan's, 1 Ghost Vision60 quadruped, and a drone). A small gap was identified when the behaviour stack timed out at a constriction in the tunnel. The operator manually intervened to execute the gap behaviour policy, resulting in the robot successfully going through the gap.

% shown in Fig~\ref{fig:ch3b_modes}.f),

% \begin{figure}[tb!]
% % \vspace{2mm}
% \centering
% % width=\w cm, height=\h cm
% % \includegraphics[width=\columnwidth]{images/ch6/Fig5.png}
% \includegraphics[width=\w cm, height=\h cm]{images/ch6/Fig5.png}
% \hfill
% \caption{A real use case of the gaps behaviour in a SubT test run. Magenta blocks indicate fatal cost.}
% \label{fig:ch3b_fig5}
% % \vspace{-3mm}
% \end{figure}


This chapter presented the investigation of research question: \textbf{\textit{How can complex visuo-motor locomotion behaviours be learned efficiently?}}, and \textbf{\textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}} The contributions of this chapter are as follows:

\begin{itemize}
    \item A Gap Behaviour, and a Behaviour Selection policy were developed to allow a large mobile robot to autonomously navigate through small gaps. The effectiveness of the these behaviours was demonstrated with behaviours trained in simulation and applied to a real world scenario. Several sources of sim-to-real disparity were identified for improving the system
\end{itemize}


“Passing Through Narrow Gaps with Deep Reinforcement Learning” was published and presented at the 2021 IEEE/RSJ International Conference on Intelligent Robots and Systems held in Prague, Czech Republic and virtually.
\newpage
\newpage

% Motivation/contribution/abstract -----------------------



% Three paragraphs: Explain motivation, what you did, results

% Final part: What research question you answered, what the contribution was, and what the publication was.

% \textit{One idea per paragraph. First sentence summarises the whole paragraph, last sentence leads into the next.}

% \textbf{Introduce the work in this chapter: robots, obstacles, DRL with visuo-motor policies}


% The scenario explored is a real-world application of passing through small gaps with a large tracked platform.
%  Passing through narrow gaps is a challenging problem for mobile robots.
% DRL methods enables the development of visuo-motor policies, however sample efficiency limits their application in complex scenarios. Typically, visuo-motor policies are difficult to train, and requires high levels of interaction between the robot and the environment. Furthermore, for locomotion over difficult obstacles, policies are subject to local minima where commonly used exploration techniques may not be sufficient to direct the robot to the required behaviour. Improving the efficiency of learning behaviours for robot locomotion over difficult obstacles is explored throughout this chapter.

% The behaviours developed in this section rely on feedback from perception to enable the robot to align to the entrance of a narrow doorway.

% The tracked platform uses an occupancy map, and must pass through small gaps that are difficult to plan through using traditional methods. 

% require many samples. Furthermore, policy training for complex obstacles are subject to local minima where typical exploration techniques may not be sufficient to direct the robot to the required behaviour. The efficiency of learning behaviours for robot locomotion over difficult obstacles is explored throughout this chapter.


% \textbf{Discuss how this chapter answers the research questions: how are behaviours learned efficiently, how is reliable switching achieved.}

% The contributions of this chapter are provided by research paper \cite{tidd_passing_2021}, exploring research question 1: the efficient learning of visuo-motor behaviours, and introducing the first investigation of reliable switching between behaviours (research question 2). Efficient learning is demonstrated by learning behaviours using a simple expert controller with reward shaping. Importantly, the expert is not able to complete the task, it is a simple behaviour that is used to bootstrap learning the complex behaviour. In addition to the efficient design of behaviours, this chapter also considers the application of controllers to a real world scenario where the learned behaviour for passing through gaps required behaviour switch as it was integrated with a pre-existing behaviour library. These investigations show the efficient development of difficult behaviours, and an approach to switch between sequential behaviours (research questions 1 and 2). 


%  if the goal location was behind a small door. 
% The output of the Behaviour Selection policy, switch parameter $\tau$, was used to determine when to switch between the Gap Behaviour 

%  Path planning methods struggle with imperfect sensor information and low resolution costmaps when gaps marginally wider than the agent are perceived as smaller than the robot footprint. Classical navigation methods require significant manual fine tuning to design behaviours to handle these difficult perception cases. Presented in this chapter is a DRL method for autonomous navigation through small gaps, where contact between the robot and the gap may be required. 


% The contributions of this chapter are provided by research paper \cite{tidd_passing_2021}, exploring research question 1: the efficient learning of visuo-motor behaviours, and introducing the first investigation of reliable switching between behaviours (research question 2). Efficient learning is demonstrated by learning behaviours using a simple expert controller with reward shaping. Importantly, the expert is not able to complete the task, it is a simple behaviour that is used to bootstrap learning the complex behaviour. In addition to the efficient design of behaviours, this chapter also considers the application of controllers to a real world scenario where the learned behaviour for passing through gaps required behaviour switch as it was integrated with a pre-existing behaviour library. These investigations show the efficient development of difficult behaviours, and an approach to switch between sequential behaviours (research questions 1 and 2). 


% The results from these experiments demonstrate the efficient learning of the Gaps Behaviour, and the reliable switching of behaviours. 

% These experiments showed a 20\% drop in success rate from simulation the real-world. While sim-to-real transfer was demonstrated, factors such as imperfect perception on the real agent, inaccuracies in simulation dynamics, and out of distribution examples seen during deployment create a disparity in performance between the simulation and the real-world scenario. 


% Complex navigation behaviours that require the robot to make contact with the environment are difficult to develop manually, learning methods . Integrating learned behaviours with pre-existing controllers is also challenging. This chapter investigated these challenges, and explored a proof of concept for training policies in simulation and applying them to a real-world scenario. The contributions of this chapter are as follows:

==> old/Ch4.tex <==
\chapter[Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts]{Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts}
\label{cha:ch4}

Legged robots often use separate control policies that are highly engineered for traversing difficult terrain such as stairs, gaps, and steps, where switching between policies is only possible when the robot is in a region that is common to adjacent controllers. Deep Reinforcement Learning (DRL) is a promising alternative to hand-crafted control design, though typically requires the full set of test conditions to be known before training. DRL policies can result in complex (often unrealistic) behaviours that have few or no overlapping regions between adjacent policies, making it difficult to switch behaviours. In this work we develop multiple DRL policies with Curriculum Learning (CL), each that can traverse a single respective terrain condition, while ensuring an overlap between policies. We then train a network for each destination policy that estimates the likelihood of successfully switching from any other policy. We evaluate our switching method on a previously unseen combination of terrain artifacts and show that it performs better than heuristic methods. While our method is trained on individual terrain types, it performs comparably to a Deep Q Network trained on the full set of terrain conditions. This approach allows the development of separate policies in constrained conditions with embedded prior knowledge about each behaviour, that is scalable to any number of behaviours, and prepares DRL methods for applications in the real world.


\section{Introduction}

Legged robots are useful for traversing various terrain conditions where wheeled platforms fail to operate. Terrains that are easily negotiated by humans, however, can present a difficult control problem in robotics \cite{atkeson2016happened}. Consider a delivery driver who jumps down from the delivery vehicle, takes a large step over a break in the sidewalk and walks up the stairs to reach the receiver’s front door. For a last mile delivery robot, it is difficult to design a single locomotion controller that can handle a set of similar tasks. Humanoid robots often use separate control policies that have been meticulously tuned for a specific condition in a constrained setting. 

%Real bipedal robots require harnesses and treadmills to engineer walking policies. Damage to the robot and surroundings is a real risk.

\begin{figure}[tb!]
\centering
\includegraphics[width=1.0\columnwidth]{images/ch4/main_pic.png}
% \caption{We pre-train policies for several artifact types including jumps, gaps and stairs, ensuring an Regions of Attraction (RoA) overlap for each policy. As a new terrain type is detected, we switch policies when the robot is in a state that is in the RoA for the next policy.}
\caption{We design policies for each complex terrain type separately, ensuring common regions of the state between policies. Switching in these common regions results in desirable behaviour from the switched policy. To successfully switch between policies we train a switch estimator for each policy that learns when best to switch. Our method involves training on each artifact type separately, where training on multiple artifact types at once may be unavailable or dangerous.}
\label{fig:main_pic}
\vspace{-3mm}
\end{figure}

For highly dynamic robots such as bipeds, transitioning from one policy to the next may only be possible through a very narrow set of states. Activating a policy when the robot is in an unsuitable configuration for the target policy can result in the robot falling over. We refer to the set of all states from which using a policy will result in a desirable stable behaviour as the Region of Attraction (RoA) of the policy~\cite{burridge_sequential_1999}. A state that is in the RoA for more than one policy presents an opportunity where these policies can be switched such that the agent will eventuate in a stable configuration. A robust policy switching method would reduce robot falls, which is a real problem with humanoid robots \cite{atkeson2016happened,kalyanakrishnan2011learning}.

Deep Reinforcement Learning (DRL) has been shown to be an effective method for developing walking policies~\cite{schulman_proximal_2017,heess_emergence_2017,peng_deeploco_2017}, and eliminates some of the hand engineering that is required by classical controllers. Deep neural networks, however do not provide insight as to where the policies will be stable. Generally, DRL policies train on the domain they are required to operate, either with a single end-to-end policy~\cite{heess_emergence_2017}, or by learning when to switch by interacting with the target environment~\cite{merel_hierarchical_2019}. Developing policies on a real system that requires exposure to a large set of terrain types during training may be difficult. Instead, it is more practical to design separate policies and then determine when to switch. This approach also allows us to embed prior knowledge into controller design (such as a rudimentary walking policy), to improve the learning outcomes of each individual policy~\cite{tidd_guided_2020}.

In this work, we first train individual DRL policies, each capable of traversing a single respective terrain artifact. The RoA of each controller is expanded using curriculum learning, while ensuring there exists a set of states common between policies (RoA overlap). We then train a neural network that estimates the probability of successful switching, given the robot state and target policy. We evaluate our approach on a random sequence of terrain types (an example shown in Fig~\ref{fig:main_pic}). We show that learning to switch is more stable than heuristic methods. We also compare our method to learning approaches trained on the test domain (sequence of terrain artifacts rather than individual artifacts), and show that we have comparable results despite interacting with only one terrain condition at a time.

The contributions of this work are two-fold:
\begin{itemize}
\setlength\itemsep{0pt}
    \item We train DRL policies for each terrain type while expanding the RoA of each policy, and ensuring an overlap between them via Curriculum Learning
    \item We design a policy switching network that estimates when the robot is in the RoA for the next policy by predicting the probability of success switching in the current state
\end{itemize}

The organization of this paper is as follows. After reviewing the relevant literature in Sec~\ref{sec:ch4_related_work}, we describe our method in Sec~\ref{sec:ch4_method}. We define the problem of interest in Sec~\ref{secsec:ch4_problem}, present how we train DRL policies for individual terrain types with curriculum learning in Sec~\ref{secsec:ch4_individual} and describe our switch estimator in Sec~\ref{secsec:ch4_switching}. We present our results in \ref{sec:ch4_experiments}, before concluding with a brief discussion in Sec~\ref{sec:ch4_conclusion}.

%A summary of our contribution is thus presented. First, using DRL we train several policies, each that is capable of traversing a single respective terrain artifact. We increase the RoA of each controller, while ensuring there exists a set of states common between policies (RoA overlap). Secondly, we estimate when the robot is in the RoA of the next policy before switching, thus increasing the stability of the switch. We train a neural network switch estimator for each target policy with data collected from the respective terrain type only. Thirdly, we test our system on a collection of terrain types. %We show that our method for estimating when to switch outperforms several comparative switching methods, and performs comparably with a deep Q learning network that has access to all terrain combinations during training. 
%Fig.~\ref{fig:main_pic} highlights the problem we are addressing and our contributions.


% Deep reinforcement learning (DRL) provides a method to develop visuomotor policies for complex terrain types, though usually does not provide any stability guarantees.

% To develop policies for robots that are equally able as a person and as a human are suitable for tasks such as autonomous last mile delivery, where the robot is required to move  . Complex terrains such as stairs, wide gaps and high ledges, can be easily traversed by a human, though present an extremely challenging task for a robot. A robotic last mile delivery system might be expected to traverse several different types of non-flat surfaces to reach the recipient. 

% It would be difficult to design a single controller for a legged robot to be proficient through a similar range of domains~\cite{?}, instead a suite of controllers is needed. For highly dynamic robots such as bipeds, transitioning from one controller to the next may only be possible in a very narrow set of joint configurations, where switching controllers outside of this configuration would result in instability~\cite{?}. We refer to the set of all states from which using a controller will result in stable behaviour from the robot as the region of attraction (RoA) of the controller~\cite{?}. A state that is in the RoA for more than one controller presents a location where these controllers can be switched such that the agent will eventuate in a stable configuration. 


% A principle benefit to our approach is we do not need access to the combination of all terrain types during training, i.e. once we have trained our set of policies and estimators, we can deploy our system on any combination of terrain artifacts. This is often not the case for other DRL methods where the agent is required to train on the test domain. The idea of training on a single terrain type scales to real systems where it may only be possible to refine a controller in a well constrained setting on a single artifact, and more difficult and unsafe to expose the robot to every terrain condition during training. It is also possible to add controllers for new terrain types without retraining any previous policies, a feature that increases the scope of our control suite to any number of terrain types. 




% Complex terrains such as stairs, wide gaps and high ledges, can be easily traversed by a human, though present an extremely challenging task for a robot. During daily duties, a delivery driver might be expected to walk over several different types of non-flat surfaces to reach their destination. The driver may need to jump down from a step in the delivery vehicle, take a large step over a break in the sidewalk, then walk up several stairs to reach the recipients front door. 

% It would be difficult to design a single controller for a legged robot to be proficient through a similar range of domains, instead a suite of controllers is needed. For highly dynamic robots such as bipeds, transitioning from one controller to the next may only be possible in a very narrow set of joint configurations, where switching controllers outside of this configuration would result in instability.

% Controllers that enable a bipedal robot to work on non-flat surfaces require the controller have information about the walking surface, and can be very challenging to create. Deep reinforcement learning (DRL) methods provide an alternative to hand crafted control designs, and allow the development of complex visuomotor policies. However, DRL methods usually result in a policy trained to work well for a specific task. Furthermore, the policies are highly non linear, often unrealistic, and difficult to analyse with analytical methods. Typical DRL policies have a very narrow set of states for which they are stable, with the possibility of having no states common between controllers. The set of states that are stable for a given controller we refer to as the region of attraction (RoA).

% Our contribution is twofold: we first design controllers that are capable of traversing complex terrain artifacts using DRL, while ensuring the robot motions are not only realistic, they share configuration space with each other controller. Secondly we learn when a robot state is in the region of attraction of a subsequent controller, and by switching controllers in this state we increase the stability of the robot. We show that our method for estimating when to switch outperforms several comparative methods for switching. Fig.~\ref{fig:main_pic} highlights the problem we are addressing and our primary contribution.

% % Our approach looks at designing policies that have overlapping regions of attraction, and learns where these policies overlap such that we can switch between policies at the appropriate time. 


% A principle benefit to our approach is we do not need access to the test domain, i.e. once we have trained our policies and estimators, we can deploy our system on any combination of terrain artifacts. This idea scales to real systems where it may only be possible to refine a controller in a well constrained setting on a single artifact, and more difficult and unsafe to expose the robot to every expected terrain condition during training. It is also possible to add controllers for new terrain types without retraining any previous policies, a feature that scales to any number of terrain types. 


% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% \includegraphics[width=0.75\columnwidth]{images/ch4/legs.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.75\columnwidth]{images/ch4/sim2real_plot.png}}\hfill
% \caption{a) Sim to real test platform, a torque controlled hexapod leg. b) Visualising the reality gap.}
% \label{fig:approach}
% \vspace{-3mm}
% \end{figure}

\section{Related Work}


% \brendan{Classical control and needing primitives}
Controllers developed with bipedal robots with classical methods can perform complex behaviours such as ascending and descending stairs~\cite{ching-long_shih_ascending_1999}, balancing on a Segway~\cite{gong_feedback_2019}, and executing a jump~\cite{xiong_bipedal_2018}. Humanoid robots often employ a set of control primitives, each individually developed and tuned, such as Dynamic Movement Primitives which uses discrete and rhythmic controllers that allow a humanoid robot to play the drums and swing a tennis racket~\cite{schaal_dynamic_2006}. Hauser et al.~\cite{siciliano_using_2008} uses primitives to place and remove a foot from contact, enabling a robot to walk on uneven terrain, up a step, and climb a ladder. Motion capture primitives can be stitched together with Hidden Markov Models to create sequences of motions~\cite{kulic_incremental_2012}. Controllers developed with classical methods usually require extensive human engineering.

% \brendan{Classical Switching}
Linking a sequence of controllers together by understanding where each works has been demonstrated on a juggling robot, the stable switching of behaviours is known as sequential composition~\cite{burridge_sequential_1999}. A key component is determining the region of attraction (RoA) for each policy, which is defined as the set of states that whether engaging a given policy will converge to a target set of states defined for that policy. Estimating the RoA overlap between controllers can be difficult for robots with high state spaces, however it can be simplified by defining a set of pre and post conditions for each controller~\cite{faloutsos_composable_2001}, or by providing a rule-based bound on parameters like heading angle and switching frequency~\cite{gregg_control_2012}. These methods result in combinations of complex primitives, though they require a mathematically defined RoA, or a hand designed switching criteria for each primitive. RoA expansion can also be considered to provide a greater overlap between controllers~\cite{borno_domain_2017}. Borno et al.~\cite{borno_domain_2017} estimates the RoA for a simulated humanoid using multiple forward dynamics model simulations, a similar approach to ours.

% \brendan{DRL}
DRL offers an alternative to classical control methods, policies learn how to act by interacting with the environment. DRL methods have demonstrated bipedal walking over complex terrain~\cite{schulman_proximal_2017,heess_emergence_2017,peng_deeploco_2017}, and performing complex maneuvers replicating motion capture~\cite{peng_deepmimic_2018}. Usually DRL methods are limited to solving a single task end-to-end, characterised by a scalar reward function. End-to-end methods require retraining if new terrains are introduced, and in a real setting it may be intractable to train on the complete set of expected conditions.

% \brendan{DRL with primitives}
Designing a single policy that can display multiple behaviours is challenging, and often results in the degraded performance of individual behaviours~\cite{lee_robust_2019}. Combining DRL primitives usually involves training a deep Q network (or a similar discrete switching network) that selects which primitive to use~\cite{liu_learning_2017,merel_hierarchical_2019,lee_robust_2019}, or learning a complex combination of primitives~\cite{peng_mcp_2019}. Other hierarchical approaches learn the primitives and selection network together~\cite{bacon_option-critic_2018}, or with several task-dependent selection networks~\cite{frans_meta_2017}. Training in each of these examples needs access to all expected environment conditions during training, and adding new primitives requires retraining of the selection policy.

% \brendan{DRL with RoA estimation    }
While estimating the complete RoA of a policy is possible for systems with a relatively small state space, such as the single~\cite{berkenkamp_safe_2017},~\cite{najafi_learning_2016}, or double inverted pendulum~\cite{randlov_combining_2000}, for more complex systems the RoA is difficult to determine. Where it is possible to differentiate between unmodeled regions of the state from those that are well behaved, DRL can guide the agent back to where a classical controller can take over~\cite{najafi_learning_2016},~\cite{randlov_combining_2000}. Other work with DRL has shown that expanding the RoA of each primitive with transition policies improves switching~\cite{lee_composing_2019}. Designing policies with DRL for complex walking robots and  combining these behaviours with RoA estimation is a promising approach to scale the capabilities of legged robots, and is an area of research that requires more investigation. 

% \brendan{Our work}
In our work, we pre-train a set of policies with DRL to traverse complex terrain artifacts. We not only ensure there is a RoA overlap between policies, but also estimate when the overlap occurs such that policies can be switched safely, without the need to train on the complete set of terrain combinations.
% Dynamic humanoid robots have a state space that is very large, with a RoA that is narrow. Expanding the RoA is an approach to ensure sequential policies have a RoA overlap, where switching can safely occur in these states,~\cite{lee_composing_2019}. 
% ~\cite{randla_combining_2000}

% DRL methods that use a switching policy to combine pre-trained policies require activating each policy on all expected terrain conditions during training,, which may be prohibitive in a real setting. Furthermore, any new policy added to the suite requires retraining of the switching mechanism.



% Region of Attraction in RL
% While estimating the complete RoA is possible for systems with a smaller state space~\cite{berkenkamp_safe_2017},~\cite{najafi_learning_2016}, for many systems the RoA is difficult to determine. Dynamic humanoid robots have a state space that is very large, with a RoA that is narrow. Expanding the RoA is an approach to ensure sequential policies have a RoA overlap, where switching can safely occur in these states~\cite{borno_domain_2017},~\cite{lee_composing_2019}. 


% A key advantage of DRL over classical methods is policies that learn to act directly from perception. Perception is advantageous for walking over complex terrain, whether from state information~\cite{lee_composing_2019}, RGB camera~\cite{merel_hierarchical_2019}, or a heightmap~\cite{peng_deeploco_2017}. Resulting policies can walk over narrow paths~\cite{peng_deeploco_2017}, over steps~\cite{heess_emergence_2017}, avoid obstacles, and plan with visual queues~\cite{merel_hierarchical_2019}.


\section{Method}


\begin{figure}[tb!]
\vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch4/fig2.png}
\caption{
We pre-train a suite of deep reinforcement learning (DRL) policies for a set of terrain conditions, and for each policy we train a switch estimator. Using the current policy $\pi_i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $\pi_j$. Each policy $\pi_i$ (where $i \in$ $\{$walk, jump, gaps, stairs$\}$) is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $a_t$ that are the torques applied to each joint. Each switch estimator $\mathcal{E}$ is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $e_j$, where $e_j \in [0,1)$ indicates that the current state is in the region of attraction (RoA) for $\pi_j$: $s_t \in R(\pi_j)$. Switching to $\pi_j$ is safest when $e_j$ is high.
}
\label{fig:method}
\vspace{-3mm}
\end{figure}

A summary of our method is outlined in Fig.~\ref{fig:method}. For each terrain type $i$, where $i \in$ $\{$walk, jump, gaps, stairs$\}$, we train a neural network policy and a switch estimator. We assume access to an oracle terrain detector to determine the upcoming terrain type, and therefore what the next policy will be. The switch estimator $\mathcal{E}_j$ for the next policy $\pi_j$ is activated once the next terrain type is detected, with output $e_j \in [0,1)$ indicating the confidence level that the robot is in the RoA of the next policy.

% : $s_t = \{$ robot state, heightmap $\} \in \mathcal{R}(\pi_j)$.% We evaluate our method on a combination of terrain types and compare our method to several other methods for switching, as well as DRL methods that have been trained on a combination of terrain types. 


\subsection{Problem definition}
\label{secsec:ch4_problem}
The problem we consider is a biped in a 3D environment, with 12 torque controlled actuators using the Pybullet simulator~\cite{coumans_pybullet_2020}. The task of the biped is to navigate obstacles typically navigated by a human delivery driver, as such the robot must traverse stairs, gaps, and a large step. We consider the state $s_t=[rs_t, I_t]$ to be the robot state $rs_{t}$ and heightmap image $I_t$ at time $t$.

\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot, respectively (four Boolean contact points per foot, plus one variable for no points in contact), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the body Centre of Mass (CoM), $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the CoM, and $h_{CoM,t}$ is the height of the CoM above the terrain. All angles except joint angles are represented in the world coordinate frame. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\textbf{Heightmap}: Perception is provided in the form of a heightmap that moves with the x,y,z and yaw positions of the robot body. A heightmap is a common perception method used in robotics, usually extracted from range measuring sensors such as depth cameras, laser scanners or stereo cameras~\cite{fankhauser_universal_2016}. Other work in DRL for walking uses perception from state information~\cite{lee_composing_2019}, RGB cameras~\cite{merel_hierarchical_2019}, or a heightmap~\cite{peng_deeploco_2017}. In early experiments, we found that using a heightmap improved policy performance compared to providing the ground truth terrain pose. The height map is scaled from 0 (the CoM of the robot) to 1 (2m below the CoM), and has a resolution of $[60,40]$, with a grid size of $0.025$m. The robot itself does not appear in the heightmap, and is centred with a larger view in front. The effective field of view is $0.9$m in front, $0.6$m behind, and $0.5$m to each side. A depiction of the heightmap is shown in Fig.~\ref{fig:method}.


\subsection{Training Policies for Individual Terrain Types}
\label{secsec:ch4_individual}
Our switching method requires policies to have a RoA overlap, and provided this condition is met we can employ policies derived from any method. We choose DRL as our method to populate our set of policies. In this section we first introduce the reinforcement learning problem and the algorithm of choice. We then introduce our reward function, and finally our curriculum learning approach that ensures policies have a RoA overlap. 

\textbf{Deep Reinforcement Learning}: We consider our task to be a Markov Decision Process (MDP) defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking $a_t$, and $\gamma$ is a discount factor. The reinforcement learning goal is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. For continuous control, actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is a torque applied to each joint. We update the weights $\theta$ of the policy using Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}.


% We use Proximal Policy Optimisation (PPO) to update a clipped objective function $L(\theta) = \mathbb{E}[\min(\text{ratio}_t\cdot A_t, \text{clip}((\text{ratio}_t, 1 - \epsilon, 1 + \epsilon)A_t)$, where $\text{ratio}_t=\frac{\pi_{\theta}(a_t|s_t)}{\pi_{\theta_{old}(a_t|s_t)}}$ is how far the current policy is from the policy from the previous update, $A_t$ is the advantage calculated with Generalised Advantage Estimation (GAE)~\cite{schulman_high-dimensional_2018}, and $\epsilon$ is a constant clip factor.
% Details can be found in~\cite{schulman_proximal_2017}.

% We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

% We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights~\cite{schulman_proximal_2017}. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse, reduce its probability.

% In practice this loss can result in large updates to the policy that can adversely affect training. Instead we use a loss defined by Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. PPO uses a surrogate loss that is clipped, ensuring policy predictions remain close to the predictions from the previous update. We also apply Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}, leading to a more accurate prediction of $V(s_t)$ and faster convergence.  

% \subsection{Robot Information}

% Remove numbers (put in results).
% \textbf{Reward}: We use the same reward function for each policy. Instead of using motion capture as a reference behaviour~\cite{peng_deepmimic_2018}, we design a simple walking gait target policy, constructed without simulator physics. Every terrain type uses the same target policy, even for the stair, jump, and gap terrains. For our work, a common target policy worked well for all terrain types, however specific target policies might be needed for more complex terrain. Our reward function is defined as:
% \[r_t = goal + pos + vel + base + step + act\]
% where:
% \begin{itemize}[leftmargin=*]
%     \item $goal$ is the error between the current heading velocity and goal heading velocity $= w_{goal}\cdot \exp[-c_{goal}\cdot e_{goal}]$.
%     \item $pos$ is the error between the joint positions and the target joint positions $= w_{pos}\cdot \exp[-c_{pos}\cdot e_{pos}]$.
%     \item $vel$ is the error between the current joint velocities and the target joint velocities (calculated with finite differences as in~\cite{peng_deepmimic_2018}) $= w_{vel}\cdot \exp[-c_{vel}\cdot e_{vel}]$.
%     \item $base$ is the CoM error from a target height, and zero roll and pitch positions $= w_{base}\cdot \exp[-c_{base}\cdot e_{base}]$. 
%     \item $step$ encourages stepping close to the middle of a step when in contact, as well as symmetrical step length ($\text{left}_{step}\approx \text{right}_{step}$ when in contact) $= w_{step}\cdot \exp[-c_{step}\cdot e_{step}]$. 
%     \item $act$ is a penalty for excessive torque for each of the $n$ joints $= w_{act}\sum_n(a_t^2)$. 
% \end{itemize}

% $e$ is the error of each respective element. Parameters $w$ and $c$ are tunable weights, which are fixed for all policies. 

\textbf{Guided Curriculum Learning}: Curriculum learning is a systematic way of increasing the difficulty of a task~\cite{bengio_curriculum_2009}, and results in learning attractive walking gaits quickly~\cite{yu_learning_2018}. In our work, \textbf{Guided Curriculum Learning}~\cite{tidd_guided_2020}, we apply curriculum learning to a sequence of tasks, where each stage is completed before the commencement of the next stage. The difficulty of each curriculum is increased as milestones are reached with average episode reward used as the milestone for all stages: as the robot consistently achieves a threshold reward, the difficulty of the current stage is increased. We employ three stages: increasing terrain difficulty while guided by expert forces, reducing the expert forces, and increasing perturbations. 

The first stage is increasing the terrain difficulty with external guidance from a rudimentary target walking policy. It is in this stage we enforce that all policies start from the same set of initial conditions, thus there exists a set of states that are common between policies (RoA overlap). We apply external forces to stabilise the CoM (similar to~\cite{yu_learning_2018}), and to each joint. Forces applied to each joint are determined from a PD controller tracking the rudimentary target walking policy. Once the respective terrain is at its most difficult setting (maximum stair height, step height, and gap length), all external forces are annealed to zero. The third stage increases the magnitude of perturbations. We found adding strong perturbations early hindered training, while increasing gradually in the last curriculum stage allowed for greater final disturbances and more robust policies. By increasing the perturbations we also increase the RoA of the respective policy, i.e. the set of states the policy can safely operate within is now larger. The full details on our curriculum learning approach, including the reward used for training each policy, can be found in our previous work~\cite{tidd_guided_2020}. 

\begin{figure}[tb!]
\centering
\subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/estimator.png}}
\includegraphics[height=0.3\columnwidth]{images/ch4/estimator.png}}
\hfill
\subfloat[]{%
\includegraphics[height=0.3\columnwidth]{images/ch4/multi_roa.png}}
\hfill
\caption{a) A switch estimator is trained for each policy, with data collected from each terrain type separately. Data points are collected around the switch point and given a label of 1 if the robot reaches the goal state, 0 otherwise. b) Early switching results in successful transitions for some policies (green), whereas switching late is more likely to fail (red).}
\label{fig:estimator}
\vspace{-3mm}
\end{figure}

\subsection{Learning When to Switch}
\label{secsec:ch4_switching}
Switching from one policy to another by estimating when a state is in the RoA for the next policy is an idea that stems from the sequential composition framework~\cite{burridge_sequential_1999}. Each policy $\pi_i$ has a goal set $\mathcal{G}(\pi_i) = \{s_i^*\}$ where $s=[rs, I]$, and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is the set of states policy $\pi_i$ was designed to operate within (Goal Set or Invariant Set), and $\mathcal{R}(\pi_i)$ is the set of states that will converge to a state in $\mathcal{G}(\pi_i)$. 

The complete set of states of the RoA for a complex biped is difficult to determine. Instead, we estimate when the robot is in the RoA of a given policy by training a neural network switch estimator. We train a switch estimator for each policy. In other words, each policy has its own switch estimator that is activated once its respective target terrain type is detected. If we switch policies when the switch estimator for the upcoming policy predicts a high value, then the likelihood of the robot safely traversing the target terrain is increased.

The data collection procedure for switching is as follows. A sample is collected by running $\pi_j$ on terrain condition $i$ and switching to $\pi_i$ a random distance from the terrain artifact (where $j \neq i$). As shown in Fig.~\ref{fig:estimator}a), there are three steps to data collection that occur for each sample: detection, switching, and labelling. Detection occurs when the terrain artifact appears $0.9$m from the robot body. We switch to the target policy at a distance $\sim\mathcal{U}(0,0.9)$m from the artifact. A total of 5 data points (robot state + heightmap) are collected for each sample, including the data point when switching occurred at timestep $t$ and the surrounding data points: $[t-2, t-1, t, t+1, t+2]$. The sample (all 5 data points) is labelled as successful (1) if the robot is able to traverse the terrain artifact and not fall for two complete steps. Otherwise, all data points in the sample are labelled as failed (0).  

% and remain stable for several meters after the terrain artifact

% reaches the goal zone (0.9m after the artifact) while maintaining a nominal $v_{CoM}$ and $h_{CoM}$ as a result of the switch that occur at time $t$. Otherwise, all the data points in the sample are labelled as failed (0). 
% We assume that the states that have close proximity to each other should have a similar success prediction, allowing us to collect five times more data for each sample, while smoothing the switch estimations.


Each switch estimator $\mathcal{E}_i$ is trained to minimise the loss $L(\phi) = (\mathcal{E}_i(s_t) - y_t)^2$, where $\phi$ is the neural network weights, $s_t$ is the state and $y_t$ is the corresponding label for data point $t$. The final layer of the network is a single output with a sigmoid activation. Data is split into 90\% training and 10\% validation, with a 50/50 split of positive and negative labels forced during training and validation. We collected a total of 100000 data points for each terrain type, and trained each switch estimator for 1500 epochs.





% To ensure RoA overlap, each policy must first stand for a random number of timesteps, then walk on a flat surface. We provide as additional input a velocity command input $v_t$. The velocity command parameter $v_t$ is concatenated with the robot state, which is set to 0 for standing, and 1 when the robot should move. 

% \paragraph{First Stage - Learning to Walk}
% The initial curriculum provides external forces to stabilise the centre of mass of the robot similar to~\cite{yu_learning_2018}. In addition, we provide an expert guided force at each actuator. Using our target walking policy introduced in the reward function section, we apply a target torque to each joint, calculated using a PD gain on the error between the robot joint positions and target joint positions. The target torque is added to the torque output from the policy. Importantly, the additional torque from the target PD controller is not considered in the gradient calculations of the policy, and is instead an artifact of the evolving environment. We found that providing this additional torque allows the robot to visit relevant parts of the state early in training, significantly increasing learning. The external forces, including the PD gain used to calculate the target torques, are annealed to zero before the next curriculum stage. Given each policy can walk on a flat surface after the first stage, an alternative approach could use a base walking policy as an initialisation for each policy. However, as the first stage is typically completed within the first 10\% of training, we simply train each policy from a random initialisation.

% \paragraph{Second Stage - Adapting the Terrain}
% After the first stage of training, each policy is capable of walking on a flat surface with no help from external forces. The terrain is slowly changed in the second stage, adding height to stairs and jumps, and length to gaps. Stairs are randomly selected as up or down. Gaps and jumps are added at random distance intervals with flat terrain otherwise. Each policy evolves to traverse its designated terrain condition, while sharing the same initial conditions. The second stage takes about 50\% of the training time (harder terrains take longer).

% \paragraph{Third Stage - Adding External Perturbations}
% In the final stage, and for the remainder of training, we add a curriculum of external perturbations. Adding random external forces is a way to improve the robustness of a policy~\cite{schulman_proximal_2017}, though too much noise early in training is a detrimental to learning. We apply an impulse force of random magnitude to the centre of mass in all 6 degrees of freedom of the torso. The force is sampled from a uniform distribution with a maximum value that is increased with each milestones. The force is applied for a single timestep (impulse), at random intervals of around 2 Hz. Having a dedicated curriculum for external disturbances allows us to use a large force that would otherwise prevent training if employed earlier. Once the third curriculum stage is complete, the maximum linear impulse force is 500N and the maximum torsional impulse force is 250Nm. In depth details and analysis of our sequential curriculum method is left for another work.




% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/ch4/fig2.png}
% \caption{

% We pre-train a suite of policies for a set of terrain conditions, and each policy has a switch estimator. Using the current policy $i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $j$.

% We train a set of RL policies 
% $\pi_i$ on specific terrains where $i \in \{walk, jump, gaps, stairs\}$. 
% Each policy takes the state $s_t = \{robot state, heightmap\}$, and produces the next action, $a_t^i$ specifying the torques for each joint. Each policy also estimates $e_i \in [0,1)$ that the current state is in the region of attraction for this policy $s_t \in R(\pi_j)$. The upcoming policy $j$ is determined by a an assumed classifier of the terrain. The active policy $i$ is switched to $j$ when $e_j$ indicates the state, is in the region of attraction for the next policy .


% We train a set of RL policies $\pi_i$ on specific terrains where $i \in \{walk, jump, gaps, stairs\}$. Each policy takes the state S= {robot state, height map}, and produces the next action, $\a_i$ specifying the torques for each joint. Each policy also estimates $e_i \in [0,1)$ that the current state is in the region of attraction for this policy $S \ in R(\pi_j)$. The upcoming policy $j$ is determined by a an assumed classifier of the terrain. The active policy $i$ is switched to $j$ when $e_j$ indicates the state, is in the region of attraction for the next policy .

% We pre-train a suite of policies for a set of terrain conditions, and each policy has a switch estimator. Using the current policy $i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $j$.

% that determines when the robot is in a safe configuration for switching.

% For each policy $i$ we train a switch estimator with output $e_i$ that indicates when the robot is in a safe configuration to policy $i$.

% \caption{We train a set of policies $\pi$, and a switch estimator for each policy $\mathcal{R}(\pi)$. Each policy and switch estimator is trained on a single terrain artifact, we then evaluate our system in a test world with all artifact types. As the robot detects the next terrain type, the switch estimator indicates when to switch to the next policy.}
% \caption{



% Our system uses a set of pre-trained policies and switch estimators, onefor each terrain condition. We run a single policy at a time, and switch when indicated by the switch estimator for the next policy. A policy is employed The current policy $i$ is employed, passing torques $a_i$ to the robot. When terrain condition $j$ is detected, we evaluate the output of switch estimator $e_j$, and switch the current policy to the next policy $j$ when indicated.

% We then switch to next policy $j$ when the switch estimator output $e_j$ indicates it is safe to switch.

% , and 
% As the next terrain condition $j$ is detected we evaluate the output of the switch estimator, $e_j$. 


% The robot state and heightmap are fed through the current policy
% $e$, $a$

% }

% \label{fig:method}
% \vspace{-3mm}
% \end{figure}


% The perception input is provided by a ground truth of box positions. If the centre of mass is over the current box, then we take current box $ + i$, where $i$ is from $[-1,0,1,2,3]$, i.e. we provide the information of the previous, current, and next 3 boxes relative to the robot centre of mass position. For each box, we provide two corners $x,y$ in robot frame, and $z$ relative to the height of the robot\brendan{should it be robot height? or z offset?}. In total there are $25$ numbers provided to the perception network \brendan{should these be normalised?}. Our perception decision enforces a limit on how close a the robot needs to be to an artifact to detect it.


% \brendan{Network information..
% The heightmap is fed into a convolutional neural network with two layers, and then is concatenated with the robot state, before being fed through two fully connected layers of size 128 before reaching the final layer. All subpolicies and estimators have the same network size.
% }

% We train a set of policies $\pi_i(s_t) \in \Pi$, including a base walking policy, and three terrain artifact policies. The terrain artifacts include stairs, a large gap, and a ledge that requires both feet of the robot to leave the ground.

% Each policy is trained with the same reward, changing the terrain in the second phase of the curriculum makes a policy specialise for a terrain type. Each terrain can walk on flat ground, though through terrain adaption each evolves a slight variant that differs from the original expert policy.


% learn a neural network approximator for $\mathcal{R}(\pi_i)(s_t)$ that predicts 

% by collecting data at transition states, and training an estimator to predict the likelihood of reaching a state in the goal se



% Sequential composition is the idea that moving from one state to another may involve executing several controllers in sequence~\cite{burridge_sequential_1999}. Conceptually, each controller has a set of states that form a funnel, where a robot in any state in the funnel will flow to a convex set of states known as the goal set. Each controller $\pi_i$ has a goal set
% $\mathcal{G}(\pi_i) = \{s_i^*\}$ and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is a set of states controller $\pi_i$ was designed to operate within, and $\mathcal{R}(\pi_i)$ is a set of states that will converge to a state in $\mathcal{G}(\pi_i)$. Thus $\mathcal{R}(\pi_i)$ acts as a funnel, moving any state $s_0$ in its set towards a state in $\mathcal{G}(\pi_i)$. Provided there exists an initial state $s_0\in \mathcal{R}(\pi_i)$, a common state in $\mathcal{G}(\pi_i)$ and $\mathcal{R}(\pi_j)$, and a target state $s_T \in \mathcal{G}(\pi_j)$, then $\pi_i$ can prepare $\pi_j$, shown in notation as $\pi_i \succeq \pi_j$, and therefore controllers can be backchained to move a robot through the state from $s_0$ to $s_T$. We consider switching between policies as a sequential composition problem, where terrain condition $j$ follows terrain condition $i$. \brendan{TODO, reduce this section/make it more relevant}


% how we can estimate when the currently executing policy $\pi_j$ has a RoA overlap between the next required policy $\pi_i$. 



% This switch e sw input 

% We consider the robot state and perception to be the same as for the policies.

% The complete set of states that make up the RoA for a walking controller is difficult to determine. Instead we estimate when the robot is in the RoA of the next policy by collecting data at transition states, and training an estimator to predict the likelihood of reaching a state in the goal set.

% Each policy $\pi_i$ has a goal set $\mathcal{G}(\pi_i)$. For a periodic controller, such as for walking, the goal set is all states visited by the unperturbed policy. For specific terrain artifacts, we define the goal set to be any state a suitable distance after the artifact where the robot maintains a CoM velocity and height typical during walking. 

% A key component to our method is that each element $\{\pi_i, \mathcal{G}(\pi_i),\mathcal{R}(\pi_i)\}$ is only obtained by interaction with terrain condition $i$. To better represent the distribution of transition states each policy may encounter, we first run controller $\pi_j$, where $j \neq i$, before switching to $\pi_i$. 

% Data is collected by running controller $j$ on terrain condition $i$ and switching to controller $i$ at a random distance after the terrain condition has been detected (Fig.~\ref{fig:estimator}a). Terrain detection occurs when the terrain artifact appears $0.9$m from the robot body, a distance consistent with the perception limit. Switching occurs at a distance sampled from $\mathcal{U}(0,0.9)$m from the artifact. We assume we have a method to detect the upcoming terrain type: the agent knows what controller it should use, we tell it when to switch.

% We collect a total of 5 data points when the controller is switched and assign each the same label, including the switch point and the surrounding two data points: $[t-2, t-1, t, t+1, t+2]$. This allows us to collect more data for each trial.

% A neural network is trained to minimise a mean squared error loss to estimate if the current robot state will likely reach the goal set for a given policy. The final layer of the network is a single output with a sigmoid activation. Data is split into 90\% training and 10\% validation, with a 50/50 split of positive and negative labels during training, and for validation. 





% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/plot_alive.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/plot_distance.png}}\hfill
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/plot_success.png}}\hfill
% \caption{a) Sim to real test platform, a torque controlled hexapod leg. b) Visualising the reality gap.}
% \label{fig:approach}
% \vspace{-3mm}
% \end{figure}

% \subsubsection{Success Prediction}

% \subsection{Subpolicies}

% Training curves? Should have some way of testing the claim that policies have overlapping RoA's.

% \subsection{Region of Attraction Estimation}

% \brendan{Should I do the same comparisons on the single environments?}

% We show the baseline results of running each subpolicy on their respective terrain artifacts in Fig.~\ref{tab:roa_results}.
% training on each individual artifact, comparing baselineOur switching method is compared to several other methods, with results displayed in Table.~\ref{tab:roa_results}.


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          & Baseline & Switch Estimate\\   
%          \hline
%          Jumps  & 0.53 &  0.63\\
%          Gaps  & 0.53 &  0.63\\
%          Stairs  & 0.53 &  0.63\\
%          Base  & 0.53 &  0.63\\
%          Zero  & 0.53 &  0.63
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:roa_results}
% \end{table}

% stairs: Thres 0.00 time alive: 0.7091 distance travelled: 0.6733  success: 0.3440
% jumps: Thres 0.00 time alive: 0.9804 distance travelled: 0.9398  success: 0.9120
% gaps: Thres 0.00 time alive: 0.8088 distance travelled: 0.7876  success: 0.6040
% Thres 0.00 time alive: 0.9974 distance travelled: 0.8012  success: 0.8140

% \subsection{Subpolicies}

% \noindent
% \begin{minipage}{0.75\linewidth}

% First version: Many vertical lines, 
% widths of horizontal lines all equal, 
% spacing above\slash below horizontal 
% lines cramped

% \smallskip
% \begin{minipage}{0.9\linewidth}
% \begin{tabularx}{\textwidth}{ |c| *{6}{Y|} }
% % \begin{tabularx}{\textwidth}{ |c| *{6}*{columnwidth/6|} }
% % \begin{tabularx}{\textwidth}{ |c| *{6}*{0.5|} }
% \cline{2-7}
%   \multicolumn{1}{c|}{} 
%  & \multicolumn{3}{c|}{Fantastical aardvarks}  
%  & \multicolumn{3}{c|}{Spelunking elephants}\\
% \hline
%  Foo bar & A & B & C & A & B & C\\
% \hline
%  5  & 87 &  5 &  2 & 82 & 18 & 48\\
%  6  &  5 & 43 &  4 &  7 & 47 &  4\\
%  7  &  7 & 18 & 63 &  2 &  9 & 99\\
% \hline
% \end{tabularx}
% \end{minipage}

% ****** EXAMPLE TABLE ***************
% \begin{minipage}{0.95\linewidth}
% \begin{tabularx}{\textwidth}{c *{6}{Y}}
% \toprule
% Foo bar
%  & \multicolumn{3}{c}{Fantastical aardvarks}  
%  & \multicolumn{3}{c}{Spelunking elephants}\\
% \cmidrule(lr){2-4} \cmidrule(l){5-7}
%   & A & B & C & A & B & C\\
% \midrule
%  5  & 87 &  5 &  2 & 82 & 18 & 48\\
%  6  &  5 & 43 &  4 &  7 & 47 &  4\\
%  7  &  7 & 18 & 63 &  2 &  9 & 99\\
% \bottomrule
% \end{tabularx}
% \captionof{table}{\textbf{How is Regional Accounting Information Processed by Real Estate Forecasters?}}
% \label{tab:1}
% \end{minipage}
% ****** EXAMPLE TABLE ***************

% \begin{minipage}{0.95\linewidth}
% \begin{tabularx}{\textwidth}{c *{7}{Y}}
% \toprule
% %  \multicolumn{7}{c}{Parameter Weights of the Reward Function}\\  
% %  \midrule
% %  & \multicolumn{3}{c}{Spelunking elephants}\\
% % \cmidrule(lr){2-4} \cmidrule(l){5-7}
%   & Goal   & Pos & Vel & CoM & Step & Act \\
% \midrule
%   $w$  & 1.0 & 0.65 & 0.05 & 0.1 & 0.2 & - \\        
%   $c$   & -3.0 & -2.0 & 0.1 & -10.0 & -5.0 & -0.0001 \\
% \bottomrule
% \end{tabularx}
% \captionof{table}{Weights used in the reward function.}
% \label{tab:params}
% \end{minipage}

% Parameters
% \begin{table}[]
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c|c}
%     \begin{tabular}{x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}|x{0.9cm}}
%     % \begin{tabular}{p{2cm}|p{2cm}|p{2cm}}
%          \hline
%   & Goal   & Pos & Vel & CoM & Step & Act \\
%          \hline
%   $w$  & 1.0 & 0.65 & 0.05 & 0.1 & 0.2 & - \\        
%   $c$   & -3.0 & -2.0 & 0.1 & -10.0 & -5.0 & -0.0001 \\
%          \hline
%     \end{tabular}
%     \caption{Parameters used in the reward function.}
%     \label{tab:params}
% \end{table}



% \brendan{I'm not sure where this goes:}

% The parameters used in the reward function are given in Table~\ref{tab:params}. 
In this section, we present the results of our simulation experiments. First, in Sec~\ref{sec:ch4_single} we analyze the performance of each policy on the single artifact type they are trained on. Second, in Sec~\ref{sec:ch4_multi} we present results on terrains that have a sequence of randomly ordered multiple artifact types. In Sec~\ref{sec:ch4_comparison} we discuss how our approach compares with learning methods that are trained directly on the multi-terrains. For performance evaluation, we measure two metrics: 
\begin{itemize}
\setlength\itemsep{0pt}
    \item \textbf{\% Total Distance:} How far the robot has travelled as a percentage of the total terrain length.
    \item \textbf{\% Success:} The percentage of cases where the robot was able to get to the end of the terrain without falling.
\end{itemize}

Each terrain artifact is made up of horizontally stacked boxes, with each trial composed of 7 artifacts. In the single-terrain case all artifacts are of the same type, whereas in the multi-terrain case they are randomly selected among all terrain types. Terrain artifacts consist of Stairs (up and down) with a rise of 0.17m, Gaps that are 0.7m in length, and Steps 0.3m high and 0.16m in length. The terrain width is sampled uniformly from $\mathcal{U}(1.1,1.7)$m and fixed for each trial, flat segments (including the run of stairs) have a length sampled uniformly from $\mathcal{U}(0.36,0.44)$m. 

% Each terrain artifact is made up of horizontally stacked boxes, with each trial composed of exactly 7 artifacts. In the single-terrain case all artifacts are of the same type, whereas in the multi-terrain case they are randomly selected among all terrain types. Each box has a width sampled from $\sim\mathcal{U}(1.1,1.7)$m. Flat segments have a length sampled from $\sim\mathcal{U}(0.36,0.44)$m. Terrain artifacts consist of stairs (up and down) with a rise of 0.17m, gaps of 0.7m in length, and steps that are 0.3m. Gaps and steps have a fixed length of 0.7 and 0.16m respectively. 

%  Each box length (except for the gaps and jumps artifact) are sampled from $\mathcal{U}(0.36,0.44)$, this is different from artifact training where box lengths are fixed for a whole trial.
\subsection{Single Artifact Type Terrains}
\label{sec:ch4_single}

Table~\ref{tab:individual_results} shows the percentage of total track distance covered and the success rate for each terrain type. Each policy is evaluated for 500 trials with 7 artifacts per trial. In these results no switching occurs. The Walk policy had the highest success rate with 99.2\%, which was expected because the robot was on flat surface. Jumps policy on step artifacts performed second best, with 91.2\% success rate. The Gaps and Stairs policies were the least successful, reaching to the final zone only 60.4\% and 34.4\% of the time. Percentage of the total distance metric was consistent with the success rates.

% \brendan{Statement about these results? What do they mean, why is the success rate so low for stairs (and gaps)? Should it correlate/provide an upper bound to switching?}
% Thres 0.00 time alive: 0.9955 distance travelled: 0.9766  success: 0.9920
% \smallskip
% \begin{minipage}{0.7\linewidth}
% \begin{tabularx}{\textwidth}{c| *{3}{Y}}
% \toprule
% \multicolumn{3}{c}{Results of 500 Trials on a Single Terrain World}\\
% \midrule
%  Artifact Type & Percentage of Total Distance & Success Rate \\   
% \midrule
%          Walk   & 0.9766 & 0.9920 \\
%          Jumps  & 0.9398 & 0.9120 \\
%          Gaps   & 0.7876 & 0.6040 \\
%          Stairs & 0.6733 & 0.3440 \\
% \bottomrule
% \end{tabularx}
% \captionof{table}{Weights used in the reward function.}
% \label{tab:individual_results}
% \end{minipage}

% |p{3cm}||p{3cm}|p{3cm}|p{3cm}| 
\begin{table}[]
    \vspace{3mm}
    \centering
    \begin{tabular}{c|c|c}

    % \begin{tabular}{p{2cm}|p{2cm}|p{2cm}}
         %\hline
         %\multicolumn{3}{c}{Results of 500 Trials on a Single Terrain World}\\
         \hline
         Policy & \% Total Dist. & \% Success \\   
         \hline
         Walk   & \textbf{97.6} & \textbf{99.2} \\
         Jumps  & 93.9 & 91.2 \\
         Gaps   & 78.7 & 60.4 \\
         Stairs & 67.3 & 34.4 \\
         \hline
    \end{tabular}
    \caption{Results of each individual policy on its corresponding terrain type (i.e. Walking policy on flat terrain). \% of total track distance covered and \% success is shown.}
    \label{tab:individual_results}
\end{table}

% \subsection{Test World}

\subsection{Multiple Artifact Type Terrains}
\label{sec:ch4_multi}
Our switching method is compared with several other methods, with results displayed in Table~\ref{tab:test_results}. All tests are performed with 2500 trials of a test world consisting of 7 terrain artifacts randomly selected from gaps, jumps and stairs. Each trial begins with a flat segment and the walk policy. Artifacts are restricted so there may not be two sequential artifacts of the same type. For the combination test worlds, only widths are fixed for an episode, each box length is randomly chosen. The number of boxes in each artifact varies from 4 to 9, while ensuring at least 0.9m of flat surface before each artifact to be consistent with how our switch estimator data is collected.

% While training policies, the terrain for an episode has a fixed length and width. 



%\subsubsection{Comparisons}

We compare our policy switching method with several heuristic methods, with the only difference between the methods being the timing of the switching.
\begin{itemize}[leftmargin=*]
    \item \textbf{Random:} Switching occurs a random distance after the artifact is detected.
    \item \textbf{On detection:} Switching occurs as soon as a next artifact is detected.
    \item \textbf{Lookup table:} We evaluate the optimal distance to switch for all switch combinations. On each artifact separately, we record the success rate of switching from any other policy to the target policy from 0 to 0.9m from the artifact (0.01m resolution).  Therefore, each switchable combination (e.g. $\pi_j$ to $\pi_i$) has a table of size $90$. We then take the $\arg\max$ of each permutation to determine the optimal switch distance for each artifact given the current policy and the target policy.
    \item \textbf{Centre of mass over feet:} Having the CoM over the support polygon created by the grounded foot is a well known  criteria for the stability of legged robots~\cite{faloutsos_composable_2001}. We switch when the following two conditions are true: 1) CoM is over the support polygon and 2) Both feet are within a tolerance distance to each other.%, switching when these conditions are met encourages RoA overlap as all policies share this configuration.% If the condition is not met and the robot is within 1cm of the artifact, switching is forced.
    \item \textbf{Our switch estimator:} We predict the probability of success for switching in the current state with our switch estimators. We threshold our predictions at 0.85 which empirically gave the best overall success for transitions. If terrain condition $i$ is detected and $\mathcal{E}_i(s_t) \geqslant 0.85$ we switch to $\pi_i$. 
\end{itemize}

For \textbf{CoM over feet} and our \textbf{Switch Estimator} methods, if there is no state where the condition to switch is met, then we force-switch to next policy when the robot is within 1cm of the corresponding artifact.% e2e
% [0.95834 0.92776 0.902  ]
% [0.00494473 0.00441479 0.01344619]
% 106 46 94 246


% [0.46104 0.7821  0.7946  0.82184 0.83734 0.82776] [0.01048286 0.01384789 0.00930011 0.01266074 0.01296528 0.00892829]

% np.array([0.8544, 0.8284, 0.7160])

% 0.4610  0.4271 & 0.1012\\
%          On detection  & 0.7821 &  0.7560 & 0.6012\\
%          Q table & 0.7946 &  0.76356  & 0.5908 \\
%          CoM over feet  &  0.8218 & 0.7914 & 0.6680\\
%          Our RoA estimator & \textbf{0.8530} & \textbf{0.8247} & \textbf{0.7148} \\   
%          \hline
%          End to end  & - &  - & -\\
%          DQN  & \textbf{0.86428} & \textbf{0.83218} & \textbf{0.7240}\\
%          \hline

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%     % \begin{tabular}{p{3cm}|x{1cm}|x{1cm}|x{1cm}}
%         %\hline
%         %\multicolumn{4}{c}{Artifact Type When Failure Occurs}\\
%         \hline
%          Switch method & Gaps & Jumps & Stairs\\   
%          \hline
%          Random  & 70.6 & 11.6 & 7.6  \\
%          On detection  & 21.4 & 3.3 & 15.2 \\
%          Lookup table  &  21.2 & 4.7 & 14.9 \\
%          CoM over feet  &  17.6 & 2.7 & 12.9 \\
%          Ours & 16.7 & 2.4 & 9.4\\
%          \hline
%          *DQN &  15.1 & 3.7 & 8.8  \\
%          *End to end & 4.2 & 1.8 & 3.7  \\
%         \hline
%     \end{tabular}
%     \caption{The artifact the robot was over when failure occurs, as a total percentage of all failures.\\ *Trained on the test domain (combinations of terrain types).}
%     \label{tab:failures}
% \end{table}

\begin{table}[]
    \vspace{3mm}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
         %\hline
         %\multicolumn{3}{c}{Results of 2500 Trials on a Multi Terrain World}\\
         \hline
         Switch Method & \scriptsize{\% Total Dist.} & \scriptsize{\% Success} & \scriptsize{\% Gap Fail} & \scriptsize{\% Jump Fail} & \scriptsize{\% Stair Fail}\\   
         \hline
         Random  & 42.7 & 10.1 & 70.6 & 11.6 & \textbf{7.6} \\
         On detection  &   75.6 & 60.1 & 21.4 & 3.3 & 15.2 \\
         Lookup table &   76.3  & 59.0  &  21.2 & 4.7 & 14.9\\
         CoM over feet  & 79.1 & 66.8 &  17.6 & 2.7 & 12.9 \\
         Ours & \textbf{82.4} & \textbf{71.4} & \textbf{16.7} & \textbf{2.4} & 9.4\\   
         \hline
         *DQN  &  83.2 & 72.4 &  15.1 & 3.7 & 8.8  \\
         *End-to-end  &  \textbf{92.7} & \textbf{90.2} & \textbf{4.2} & \textbf{1.8} & \textbf{3.7}\\
         \hline
    \end{tabular}
    \caption{Results of each switching method on multi-terrain test worlds (500 trials). The \% of the total distance covered, and the success rate for the robot reaching the end of the trial is shown. The final three columns show the \% of failures for each artifact type.\\ *Trained on the test domain (combinations of terrain types).}
    \label{tab:test_results}
\end{table}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}
%          \hline
%          \multicolumn{3}{c}{Results of 2500 Trials on a Multi Terrain World}\\
%          \hline
%          Switch Method & Percentage of Total Distance & Success Rate\\   
%          \hline
%          Our switch estimator & \textbf{0.8247} & \textbf{0.7148} \\   
%          \hline
%          End to end  &  \textbf{0.92776} & \textbf{0.9020}\\
%          DQN  &  0.8322 & 0.7240\\
%          \hline
%     \end{tabular}
%     \caption{Results from 2500 trials on a random test world for each switching method. We record the percentage of the total distance reached, and the success rate for the robot reaching the end of the trial.}    \label{tab:test_e2e_results}
% \end{table}


Table~\ref{tab:test_results} shows the results for multi-terrain test worlds. For less dynamic platforms it may be possible to switch controllers at any time after obstacle detection, however that was not the case for our scenarios: random switching performed the worst as expected with only 10.1\% success rate. Switching as soon as an artifact is detected does better than randomly switching with 60.1\% success, we suggest this is because switching early might give the policies enough time to align to an artifact. Fig.~\ref{fig:estimator}.b) shows it is preferential to switch early for some policies. \textbf{Lookup table} method performed similarly to the \textbf{On Detection} method. \textbf{CoM over feet} method performed relatively well with 66.8\% success. An advantage of this method is that it does not require further data collection once individual policies are trained, providing insight into where RoA overlap occurs for most policies. Our switching method was the most robust, whilst following our condition that we only have access to each individual terrain artifact at training time, traversing 82.4\% of the terrain and reaching the final zone in 71.4\% of trials.

Fig.~\ref{fig:plot} shows a single trial of the test world using our method. We can see the switch estimator predictions for each policy in the top figure, and the times our predictions prevented early switching (vertical green lines show detection, vertical red lines show when switching occurs). We can also see in the bottom plot the times that the CoM is over the feet, and instances our estimator switched outside of these regions ($\text{timestep}\approx875$).

The final three columns of Table~\ref{tab:test_results} shows the failure distribution of each switch method. We record where the robot was when failure occurs, given as a percentage of all trials. For each method, the most failures happened after switching to the Gaps policy. For instance, it contributed to to 16.7\% of a total (28.6\%) failures for our switching method. For all terrain types, these results show less failures than the single terrain experiments reported in Table~\ref{tab:individual_results}. This suggests we are improving the robustness of each policy using our switch estimator.

% This provides insight into where our system requires more robust policies, and more reliable swic

% This is in contrast to the results reported in Table~\ref{tab:individual_results}, where the Stairs policy was the least reliable. 

% We believe that this is because in the single artifact type case, the Stairs policy does not get a chance to stabilise for the upcoming Stairs artifact, whereas in the multi artifact type case, the flat portion of the following non-Stair artifact allows the robot to stabilise.

%We believe that after a  segment of stairs in the test conditions, the flat portion of the following non-stair artifact allows the robot to stabilise.

% Table.~\ref{tab:individual_results} shows the gaps policy on a single terrain has a failure rate of 39.6\%, indicating that our switch estimator 

% This is in contrast to the results in table.~\ref{tab:individual_results} where the stair controller was the least stable

% Performance improvements for each policy are consistent with the results from Table.~\ref{tab:test_results}, though interestingly do not match the baseline performances from table.~\ref{tab:individual_results}. This information can potentially be used to improve particular policies, and if necessary look at specific regions where new policies are required.

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \hline
%         \multicolumn{5}{c}{Artifact Failure Count}\\
%         \hline
%          Switch method & Gaps & Jumps & Stairs & Total\\   
%          \hline
%          Random switching  & 1759 & 289 & 190 & 2238 \\
%          On detection  & 535 & 82 & 380 & 997\\
%          Look up table  &  529 & 118 & 372 & 1019\\
%          CoM over feet  &  441 & 67 & 323 & 831\\
%          Our switch estimator & 416 & 60 & 235 & 711\\
%          \hline
%          End to end & 106 & 46 & 94 & 246 \\
%          DQN &  377 & 92 & 221 &  690\\
%         \hline
%     \end{tabular}
%     \caption{A record of the artifact the robot was over when failure occurs for each switching method.}
%     \label{tab:failures}
% \end{table}


% 0.706429490616622	0.116064879356568	0.07630563002681
% 0.214	0.0328	0.152
% 0.212430618253189	0.047385279685967	0.149384102060844
% 0.176187725631769	0.026767749699158	0.129044524669073
% 0.166868073136428	0.024067510548523	0.094264416315049
% #DIV/0!	#DIV/0!	#DIV/0!
% 0.042227642276423	0.018325203252033	0.037447154471545
% 0.1508	0.0368	0.0884

%  Switch method & Gaps & Jumps & Stairs\\   
%  \hline
%  Random switching  & 0.7064 & 0.1161 & 0.0763  \\
%  On detection  & 0.2140 & 0.0328 & 0.1520 \\
%  Look up table  &  0.2124 & 0.0474 & 0.1494 \\
%  CoM over feet  &  0.1762 & 0.02677 & 0.1290 \\
%  Our switch estimator & 0.1669 & 0.0241 & 0.0943\\
%  \hline
%  *DQN &  0.1508 & 0.0368 & 0.0884  \\
%  *End to end & 0.0422 & 0.0183 & 0.0374  \\

% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%     % \begin{tabular}{p{3cm}|x{1cm}|x{1cm}|x{1cm}}
%         %\hline
%         %\multicolumn{4}{c}{Artifact Type When Failure Occurs}\\
%         \hline
%          Switch method & Gaps & Jumps & Stairs\\   
%          \hline
%          Random  & 70.6 & 11.6 & 7.6  \\
%          On detection  & 21.4 & 3.3 & 15.2 \\
%          Lookup table  &  21.2 & 4.7 & 14.9 \\
%          CoM over feet  &  17.6 & 2.7 & 12.9 \\
%          Ours & 16.7 & 2.4 & 9.4\\
%          \hline
%          *DQN &  15.1 & 3.7 & 8.8  \\
%          *End to end & 4.2 & 1.8 & 3.7  \\
%         \hline
%     \end{tabular}
%     \caption{The artifact the robot was over when failure occurs, as a total percentage of all failures.\\ *Trained on the test domain (combinations of terrain types).}
%     \label{tab:failures}
% \end{table}

\subsection{Comparison with training on multiple artifact terrains}
\label{sec:ch4_comparison}

For completeness, we also look at other methods that involve training on a full combination of terrain artifacts, including training a Deep Q Network (DQN) using our pre-trained policies, and a single end-to-end policy. Results are displayed in the last two rows of Table.~\ref{tab:test_results}. The DQN was provided with the artifact detection in the form of a one hot encoding appended to the robot state, and received the same reward as each policy, with an additional reward provided by our oracle terrain detector. We note that without the additional reward provided by the oracle the DQN failed to learn. For the end-to-end learning method, we applied the same reward and curriculum learning approach (from~\cite{tidd_guided_2020}) as our policies. Robot state + heightmap is provided as input, and torques are generated at the output. We note that without the curriculum the end-to-end method failed to learn.

Our estimator performs similarly to the DQN despite not seeing more than one terrain artifact type during training (71.4\% success compared to 72.4\%). While learning was substantially longer for the end-to-end policy (approx. 3 times longer than an individual policy), it performed the best with 90.2\% success rate. While these methods trained on the test domain perform well, it may not be possible to train on all expected terrain conditions on a real platform, where training policies separately allows us to refine each policy in a constrained setting.

% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/plot_alive.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/plot_distance.png}}\hfill
% \hfill
% \subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/plot_success.png}}\hfill
% \caption{Graphical representation of Table.~\ref{tab:test_results} including the standard deviation from the 5 random seeds. a) Shows the portion of time alive compared to the total possible time for a given trial, b) is the portion of distance covered, and c) is the success rate for reaching the end of a trial sequence.}
% \label{fig:test_results}
% \vspace{-3mm}
% \end{figure}



\begin{figure}[tb!]
\vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch4/plot.png}
\caption{Our method on a single trial in the test world. The top figure shows the switch estimate from the time the next artifact is detected until the robot has past the artifact. The bottom figure shows the terrain (pink) with foot (blue and green) and CoM height (red) when the CoM is over the stance foot. Green vertical lines indicate when the terrain was detected, red vertical lines show when switching occurred.}
\label{fig:plot}
% \vspace{-3mm}
\end{figure}

% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/ch4/main_pic.png}
% % \caption{We pre-train policies for several artifact types including jumps, gaps and stairs, ensuring an Regions of Attraction (RoA) overlap for each policy. As a new terrain type is detected, we switch policies when the robot is in a state that is in the RoA for the next policy.}
% \caption{We design policies for each complex terrain type separately, ensuring common regions of the state between policies. Switching in these common regions results in desirable behaviour from the switched policy. To successfully switch between policies we train a switch estimator for each policy that learns when best to switch. Our method involves training on each artifact type separately, where training on multiple artifact types at once may be unavailable or dangerous.}
% \label{fig:plot}
% \vspace{-3mm}
% \end{figure}

% \caption{Our method on a single trial in the test world. The top figure shows the switch estimate from the time the next artifact is detected until the robot has past the artifact. The middle plot is the current policy being deployed, and when the switching occurs to the next policy. The bottom figure shows the terrain with foot and CoM height when the CoM is over the stance foot.}


% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c|c}
%         \hline
%          & Time Alive & Distance & Success \\   
%          \hline
%          End to end  & 0.5249 &  0.4933 & 0.24\\
%          DQN  & 0.86428 & 0.83218 & 0.7240\\
         
%          \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:other_results}
% \end{table}

% \begin{figure}[tb!]
% \centering
% \includegraphics[width=1.0\columnwidth]{images/ch4/gaps_q_table.png}
% \caption{}
% \label{fig:q_table}
% \vspace{-3mm}
% \end{figure}



% Results summary:
% \begin{itemize}
%     \item TODO: Way to show that subpolicies have regions of attractions that overlap:
%     \begin{itemize}
%         \item Train subpolicies without controller overlap: no expert in reward, no expert cur?
%         \item Evaluate individual policies
%         \item Run baseline
%     \end{itemize}
%     \item Evaluate individual policies, 
%     \item Evaluate likelihoods for sections: graphics
%     \item Evaluate switching at given step
%     \item Evaluate success criteria
%     \item compare baseline, switching, and ours
% \end{itemize}
% Notes:
% \begin{itemize}
%     \item Compare the amount of information needed to switch: 
%     \begin{itemize}
%         \item none (switch as soon as artifact detected)
%         \item Randomly switch after an artifact detected
%         \item Switch based on distance since artifact detected
%         \item Mine: switch when configuration good: i.e. roa estimate
        
%     \end{itemize}
%     \item Histogram for each
%     \item Look at simple things like when is switching good between the methods: when foot is down (left foot over right?), where is the com. Any patterns. feature engineering: wider vs deeper. 
%     \item Other things to consider: training time (samples). Compare how good each method is on the training domain compared to the test..
%     \item success criteria may effect all results, evaluate some of these.
% \end{itemize}


% What plots should I have?

% Subpolicy results

% Results of individual experiments. Pics of 


% We evaluate our switching method on a test world. The test world is a random sequence of 7 terrain artifacts, with a distance of around 19m and dimensions drawn from the same uniform distributions as the training examples. Each test is performed 100 times, equating to 700 interactions with artifacts. The results are shown in table~\ref{tab:results}. 

% We compare our switching method to several benchmarks, with a baseline of switching controllers as soon as the robot's perception detects the next artifact. We try switching when the feet are close together and the centre of mass is over the feet. 

% After each run we record how long the robot has been alive out of a possible 3000 timesteps, how far the robot has walked out of the total terrain distance, and if the robot has successfully made it to the final flat area at the end of the terrain sequence.

% We evaluate several thresholds for success criteria.



\section{Results}
\section{Discussion}
% Where it is challenging to access to the full set of conditions during development, walking over complex terrain requires specialist policies to navigate difficult terrain types. In order to successfully transition between policies, we show that learning when to switch can occur in single terrain conditions, leading to a scalable method where any number of policies can be added to the control suite as required. 
We introduce a novel method for estimating when to switch between a set a of pre-trained policies. We show that our method improves the stability of switching compared to heuristic methods, where policies and switch estimators only have access to a single terrain during training. Our method also performs comparable to a DQN trained on test conditions (all terrain types), which may not be possible for real systems. By designing policies separately we are able to refine controllers in a constrained setting, and embed prior knowledge about the the required behaviour. Similar to the human delivery driver, our bipedal agent can traverse several difficult terrain types, and by understanding when to switch between behaviours our method can scale to any number of terrain conditions.

We design our policies with an overlapping Region of Attraction (RoA). However, this may not always be the possible, particularly for specialist policies where the RoA represents a very narrow set of states that do not overlap with a simple walking policy. Future work will look at evoking a setup policy that expands the RoA of a given policy to ensure this overlap exists. A limitation of our method is the assumption that we have a terrain oracle, learning to identify the upcoming terrain type is left for future work. We believe that harnessing the capabilities of DRL and combining controllers in a modular way will allow us to expand the locomotion capabilities of legged robots. 

% \brendan{TODO:}
% \brendan{
% \begin{itemize}
%     \item switch plots
%     \item end to end
%     \item DQN
%     \item q table plot
%     \item results
%     \item subpolicies results
%     \item baseline table
% \end{itemize}
% }




==> old/Ch4_mono.tex <==
% \chapter[Learning to Transition Between Dynamic Behaviours]{Learning to Transition Between Complex Behaviours}

% \chapter[Learning to Switch Between Behaviours]{Learning When to Switch Between Sequential Behaviours}
\chapter[Learning When to Switch]{Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts}

% \item \textbf{Research Question 2: \textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}}

\label{cha:ch4}
% Motivation/contribution/abstract -----------------------

% \section{Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts}
% \label{sec:sec_switch}

This chapter investigates research question 2, exploring the safe switch location for sequential behaviours. The work presented in this chapter has been published at IROS 2021 [\cite{tidd_learning_2021}]. Chapters \ref{cha:ch3a} and \ref{cha:ch3b} discussed methods for efficiently learning separate locomotion behaviours, this chapter considers combining behaviours to traverse a sequence of obstacles. Dynamic platforms such as bipeds rely on controllers that consider the stability of the robot during operation. Switching from one behaviour to the next must occur when stability is ensured by the receiving controller. In Chapter \ref{cha:Introduction} the concepts region of attraction (RoA), and RoA overlap were introduced. To safely switch, sequential behaviours must have a RoA overlap. This chapter considers the effect of overlapping regions on safe switching, and explores when a reliable switch state occurs for specific behaviours.

\begin{figure}[htb!]
\centering
\includegraphics[width=1.0\columnwidth]{images/ch4/main_pic.png}
\caption{Switching between behaviours is necessary to traverse a sequence of obstacles.}
\label{fig:ch4_cha4_fig1}
% \vspace{-3mm}
\end{figure}

The goal of this chapter is to use behaviours developed with the methods outlined in Chapter \ref{cha:ch3a} to reliably traverse a sequence of obstacles containing stairs, gaps, and hurdles (as depicted in Figure \ref{fig:ch4_cha4_fig1}). 
Bipedal robots often use separate control policies that are specifically designed for traversing difficult obstacles where switching between policies must occur while in the RoA of the next policy. To achieve this, a novel Switch Estimator policy learned to predict when the robot was in a suitable state to switch to an upcoming target policy. The Switch Estimator was trained with supervised learning using data collected by recording the state the switch occurred, and the label corresponding to if the robot was able to successfully traverse the obstacle (Figure \ref{fig:ch4_cha4_fig3}). Additionally, the criticality of overlapping states was investigated by comparing the effect of initial conditions on the reliability of switching. To ensure an overlap, each behaviour was first required to stand the robot in place for a short duration before commencing the behaviour. 


\section{Method}
\label{sec:method}


\begin{figure}[tb!]
\vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch4/fig2.png}
\caption{
We pre-train a suite of deep reinforcement learning (DRL) policies for a set of terrain conditions, and for each policy we train a switch estimator. Using the current policy $\pi_i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $\pi_j$. Each policy $\pi_i$ (where $i \in$ $\{$walk, jump, gaps, stairs$\}$) is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $a_t$ that are the torques applied to each joint. Each switch estimator $\mathcal{E}$ is a neural network with inputs $s_t=\{$robot state, heightmap$\}$ and outputs $e_j$, where $e_j \in [0,1)$ indicates that the current state is in the region of attraction (RoA) for $\pi_j$: $s_t \in R(\pi_j)$. Switching to $\pi_j$ is safest when $e_j$ is high.
}
\label{fig:ch4_method}
\vspace{-3mm}
\end{figure}

A summary of our method is outlined in Fig.~\ref{fig:ch4_method}. For each terrain type $i$, where $i \in$ $\{$walk, jump, gaps, stairs$\}$, we train a neural network policy and a switch estimator. We assume access to an oracle terrain detector to determine the upcoming terrain type, and therefore what the next policy will be. The switch estimator $\mathcal{E}_j$ for the next policy $\pi_j$ is activated once the next terrain type is detected, with output $e_j \in [0,1)$ indicating the confidence level that the robot is in the RoA of the next policy.

% : $s_t = \{$ robot state, heightmap $\} \in \mathcal{R}(\pi_j)$.% We evaluate our method on a combination of terrain types and compare our method to several other methods for switching, as well as DRL methods that have been trained on a combination of terrain types. 


\subsection{Problem definition}
\label{secsec:problem}
The problem we consider is a biped in a 3D environment, with 12 torque controlled actuators using the Pybullet simulator~\cite{coumans_pybullet_2020}. The task of the biped is to navigate obstacles typically navigated by a human delivery driver, as such the robot must traverse stairs, gaps, and a large step. We consider the state $s_t=[rs_t, I_t]$ to be the robot state $rs_{t}$ and heightmap image $I_t$ at time $t$.

% The biped model has a mass of 54kg, and uses an average torque of TODOwhen walking on a flat surface with torque limits of TODO.

\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot, respectively (four Boolean contact points per foot, plus one variable for no points in contact), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the body Centre of Mass (CoM), $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the CoM, and $h_{CoM,t}$ is the height of the CoM above the terrain. All angles except joint angles are represented in the world coordinate frame. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\textbf{Heightmap}: Perception is provided in the form of a heightmap that moves with the x,y,z and yaw positions of the robot body. A heightmap is a common perception method used in robotics, usually extracted from range measuring sensors such as depth cameras, laser scanners or stereo cameras~\cite{fankhauser_universal_2016}. Other work in DRL for walking uses perception from state information~\cite{lee_composing_2019}, RGB cameras~\cite{merel_hierarchical_2019}, or a heightmap~\cite{peng_deeploco_2017}. In early experiments, we found that using a heightmap improved policy performance compared to providing the ground truth terrain pose. The height map is scaled from 0 (the CoM of the robot) to 1 (2m below the CoM), and has a resolution of $[60,40]$, with a grid size of $0.025$m. The robot itself does not appear in the heightmap, and is centred with a larger view in front. The effective field of view is $0.9$m in front, $0.6$m behind, and $0.5$m to each side. A depiction of the heightmap is shown in Fig.~\ref{fig:ch4_method}.


\subsection{Training Policies for Individual Terrain Types}
\label{secsec:individual}
Our switching method requires policies to have a RoA overlap, and provided this condition is met we can employ policies derived from any method. We choose DRL as our method to populate our set of policies. In this section we first introduce the reinforcement learning problem and the algorithm of choice. We then introduce our reward function, and finally our curriculum learning approach that ensures policies have a RoA overlap. 

\textbf{Deep Reinforcement Learning}: We consider our task to be a Markov Decision Process (MDP) defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking $a_t$, and $\gamma$ is a discount factor. The reinforcement learning goal is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. For continuous control, actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is a torque applied to each joint. We update the weights $\theta$ of the policy using Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}.


\textbf{Guided Curriculum Learning}: Curriculum learning is a systematic way of increasing the difficulty of a task~\cite{bengio_curriculum_2009}, and results in learning attractive walking gaits quickly~\cite{yu_learning_2018}. In our work, \textbf{Guided Curriculum Learning}~\cite{tidd_guided_2020}, we apply curriculum learning to a sequence of tasks, where each stage is completed before the commencement of the next stage. The difficulty of each curriculum is increased as milestones are reached with average episode reward used as the milestone for all stages: as the robot consistently achieves a threshold reward, the difficulty of the current stage is increased. We employ three stages: increasing terrain difficulty while guided by expert forces, reducing the expert forces, and increasing perturbations. 

The first stage is increasing the terrain difficulty with external guidance from a rudimentary target walking policy. We apply external forces to stabilise the CoM (similar to~\cite{yu_learning_2018}), and to each joint. Forces applied to each joint are determined from a PD controller tracking the rudimentary target walking policy. Once the respective terrain is at its most difficult setting (maximum stair height, step height, and gap length), all external forces are annealed to zero. The third stage increases the magnitude of perturbations. We found adding strong perturbations early hindered training, while increasing gradually in the last curriculum stage allowed for greater final disturbances and more robust policies. By increasing the perturbations we also increase the RoA of the respective policy, i.e. the set of states the policy can safely operate within is now larger. The full details on our curriculum learning approach, including the reward used for training each policy, can be found in our previous work~\cite{tidd_guided_2020}. We extend this work by comparing the effect of starting all policies from the same set of initial conditions (a standing pose), compared to starting from a random joint configuration, and thus enforce there to be a set of states that are common between policies (RoA overlap). The policies must pause for a short duration (0.5 seconds) before commencing the location behaviour. 

\begin{figure}[tb!]
\centering
\subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/estimator.png}}
\includegraphics[height=0.3\columnwidth]{images/ch4/estimator.png}}
\hfill
\subfloat[]{%
\includegraphics[height=0.3\columnwidth]{images/ch4/multi_roa.png}}
\hfill
\caption{a) A switch estimator is trained for each policy, with data collected from each terrain type separately. Data points are collected around the switch point and given a label of 1 if the robot reaches the goal state, 0 otherwise. b) Early switching results in successful transitions for some policies (green), whereas switching late is more likely to fail (red).}
\label{fig:ch4_estimator}
\vspace{-3mm}
\end{figure}

\subsection{Learning When to Switch}
\label{secsec:switching}
Switching from one policy to another by estimating when a state is in the RoA for the next policy is an idea that stems from the sequential composition framework~\cite{burridge_sequential_1999}. Each policy $\pi_i$ has a goal set $\mathcal{G}(\pi_i) = \{s_i^*\}$ where $s=[rs, I]$, and a Region of Attraction (RoA) $\mathcal{R}(\pi_i) = \{s_0 \in \mathcal{S} : \lim_{t\to\infty} s(t,s_0) = \mathcal{G}(\pi_i)\}$. $\mathcal{G}(\pi_i)$ is the set of states policy $\pi_i$ was designed to operate within (Goal or Invariant Set), and $\mathcal{R}(\pi_i)$ is the set of states that will converge to a state in $\mathcal{G}(\pi_i)$. 

The complete set of states of the RoA for a complex biped is difficult to determine. Instead, we estimate when the robot is in the RoA of a given policy by training a neural network switch estimator. We train a switch estimator for each policy. In other words, each policy has its own switch estimator that is activated once its respective target terrain type is detected. If we switch policies when the switch estimator for the upcoming policy predicts a high value, then the likelihood of the robot safely traversing the target terrain is increased.

The data collection procedure for switching is as follows. A sample is collected by running $\pi_j$ on terrain condition $i$ and switching to $\pi_i$ a random distance from the terrain artifact (where $j \neq i$). As shown in Fig.~\ref{fig:ch4_estimator}a), there are three steps to data collection that occur for each sample: detection, switching, and labelling. Detection occurs when the terrain artifact appears $0.9$m from the robot body. We switch to the target policy at a distance $\sim\mathcal{U}(0,0.9)$m from the artifact. A total of 5 data points (robot state + heightmap) are collected for each sample, including the data point when switching occurred at timestep $t$ and the surrounding data points: $[t-2, t-1, t, t+1, t+2]$. The sample (all 5 data points) is labelled as successful (1) if the robot is able to traverse the terrain artifact and remain stable for two complete steps past the terrain. Otherwise, all data points in the sample are labelled as failed (0).  

% and remain stable for several meters after the terrain artifact

% reaches the goal zone (0.9m after the artifact) while maintaining a nominal $v_{CoM}$ and $h_{CoM}$ as a result of the switch that occur at time $t$. Otherwise, all the data points in the sample are labelled as failed (0). 
% We assume that the states that have close proximity to each other should have a similar success prediction, allowing us to collect five times more data for each sample, while smoothing the switch estimations.


Each switch estimator $\mathcal{E}_i$ is trained to minimise the loss $L(\phi) = (\mathcal{E}_i(s_t) - y_t)^2$, where $\phi$ is the neural network weights, $s_t$ is the state and $y_t$ is the corresponding label for data point $t$. The final layer of the network is a single output with a sigmoid activation. Data is split into 90\% training and 10\% validation, with a 50/50 split of positive and negative labels forced during training and validation. We collected a total of 100000 data points for each terrain type, and trained each switch estimator for 1500 epochs.


\section{Experiments}
\label{sec:experiments}

% The parameters used in the reward function are given in Table~\ref{tab:ch4_params}. 
In this section, we present the results of our simulation experiments. First, in Sec~\ref{sec:single} we analyze the performance of each policy on the single artifact type they are trained on. Second, in Sec~\ref{sec:multi} we present results on terrains that have a sequence of randomly ordered multiple artifact types. In Sec~\ref{sec:comparison} we discuss how our approach compares with learning methods that are trained directly on the multi-terrains. For performance evaluation, we measure two metrics: 
\begin{itemize}
\setlength\itemsep{0pt}
    \item \textbf{\% Total Distance:} How far the robot has travelled as a percentage of the total terrain length.
    \item \textbf{\% Success:} The percentage of cases where the robot was able to get to the end of the terrain without falling.
\end{itemize}

Each terrain artifact is made up of horizontally stacked boxes, with each trial composed of 7 artifacts. In the single-terrain case all artifacts are of the same type, whereas in the multi-terrain case they are randomly selected among all terrain types. Terrain artifacts consist of Stairs (up and down) with a rise of 0.17m, Gaps that are 0.7m in length, and Steps 0.3m high and 0.16m in length (the size of each obstacle is kept fixed). The terrain width is sampled uniformly from $\mathcal{U}(1.1,1.7)$m and fixed for each trial, flat segments (including the run of stairs) have a length sampled uniformly from $\mathcal{U}(0.36,0.44)$m. We do not consider the efficacy of policies on terrains outside of these ranges, some discussion on out of distribution operation is presented in~\cite{tidd_guided_2020}. 

%  Each box length (except for the gaps and jumps artifact) are sampled from $\mathcal{U}(0.36,0.44)$, this is different from artifact training where box lengths are fixed for a whole trial.
\subsection{Single Artifact Type Terrains}
\label{sec:single}

Table~\ref{tab:ch4_individual_results} shows the percentage of total track distance covered and the success rate for each terrain type. Each policy is evaluated for 500 trials with 7 artifacts per trial. In these results no switching occurs. We evaluate two sets of policies according to the initial conditions: if the robot started with a standing joint configuration and was required to pause for a short duration before walking, or if the robot started with a random joint configuration with no pause. Of the policies starting from a standing joint configuration, the Jumps policy performed best, with a success rate of 87.8\%. Both conditions for starting state were effective at learning policies, though we observed that random initial joint positions resulted in more successful policies for the Gaps and Stair artifacts (75.5\% and 59.0\%). We suggest this improvement may be the result of imposing fewer state limitations on the emergent behaviours. The percentage of the total distance metric was consistent with the success rates.

%  The Gaps and Stairs policies were the least successful, reaching to the final zone only 56.3\% and 52.1\% of the time.

% The Walk policy had the highest success rate with 99.2\%, which was expected because the robot was on flat surface.

% |p{3cm}||p{3cm}|p{3cm}|p{3cm}| 
\begin{table}[]
    \vspace{3mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c|c|c}
    % \begin{tabular}{c|c|c}
    % \begin{tabular}{|c|cc|cc|}

    % \begin{tabular}{p{1.cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
    \begin{tabular}{M{0.9cm}|M{1.65cm}|M{1.5cm}|M{1.65cm}|M{1.5cm}}
    % \begin{tabular}{p{2cm}|p{2cm}|p{2cm}}
         %\hline
         %\multicolumn{3}{c}{Results of 500 Trials on a Single Terrain World}\\
        %  \hline
        % %  Policy & \% Total Dist. & \% Success \\   
        %  Policy & \multicolumn{2}{c|}{\% Total Dist.} & \multicolumn{2}{c|}{\% Success}\\
        %  \hline
        % %  Walk   & \textbf{97.6} & \textbf{99.2} \\
        %  Walk   & \multicolumn{2}{c|}{\textbf{97.6}} & \multicolumn{2}{c|}{\textbf{99.2}} \\
        %  Jumps  & 93.9 & 86.2 & 91.2 & 77.5\\
        %  Gaps   & 78.7 & 87.4 & 60.4 & 75.5 \\
        %  Stairs & 67.3 & 78.7 & 34.4 & 59 \\
         
         Policy & \% Total Dist. &\% Success & \% Total Dist. rand & \% Success rand\\
         \hline
        %  Walk   & \textbf{97.6} & \textbf{99.2} \\
        %  Walk   & \textbf{97.6} & \textbf{99.2} & \textbf{97.6} & \textbf{99.2}\\
         Jumps  & 93.1 & 87.8 & 86.2 & 77.5\\
         Gaps   & 76.0 & 56.3  & 87.4 & 75.5 \\
         Stairs & 71.4 & 52.1  & 78.7 & 59.0 \\
         
        
        % Original format and results:
        % \hline
        % Policy & \% Total Dist. & \% Success \\ 
        % \hline
        %  Walk   & \textbf{97.6} & \textbf{99.2} \\
        %  Jumps  & 93.9 & 91.2 \\
        %  Gaps   & 78.7 & 60.4 \\
        %  Stairs & 67.3 & 34.4 \\
         
         \hline
    \end{tabular}
    \caption{Results of each individual policy on its corresponding terrain type. \% of total track distance covered and \% success is shown. We also report the success of policies that are trained with random initial joint positions.}
    \label{tab:ch4_individual_results}
\end{table}

% \subsection{Test World}

\subsection{Multiple Artifact Type Terrains}
\label{sec:multi}
Our switching method is compared with several other methods, with results displayed in Table~\ref{tab:ch4_test_results}. All tests are performed with 2500 trials of a test world consisting of 7 terrain artifacts randomly selected from gaps, jumps and stairs. Each trial begins with a flat segment and the walk policy. Artifacts are restricted so there may not be two sequential artifacts of the same type. For the combination test worlds, only widths are fixed for an episode, each box length is randomly chosen. The number of boxes in each artifact varies from 4 to 9, while ensuring at least 0.9m of flat surface before each artifact to be consistent with how our switch estimator data is collected.


%\subsubsection{Comparisons}

We compare our policy switching method with several heuristic methods, with the only difference between the methods being the timing of the switching.
\begin{itemize}[leftmargin=*]
    \item \textbf{Random:} Switching occurs a random distance after the artifact is detected.
    \item \textbf{On detection:} Switching occurs as soon as a next artifact is detected.
    \item \textbf{Lookup table:} We evaluate the optimal distance to switch for all switch combinations. On each artifact separately, we record the success rate of switching from any other policy to the target policy from 0 to 0.9m from the artifact (0.01m resolution).  Therefore, each switchable combination (e.g. $\pi_j$ to $\pi_i$) has a table of size $90$. We then take the $\arg\max$ of each permutation to determine the optimal switch distance for each artifact given the current policy and the target policy.
    \item \textbf{Centre of mass over feet:} Having the CoM over the support polygon created by the grounded foot is a well known  criteria for the stability of legged robots~\cite{faloutsos_composable_2001}. We switch when the following two conditions are true: 1) CoM is over the support polygon and 2) Both feet are within a tolerance distance to each other.%, switching when these conditions are met encourages RoA overlap as all policies share this configuration.% If the condition is not met and the robot is within 1cm of the artifact, switching is forced.
    \item \textbf{Our switch estimator:} We predict the probability of success for switching in the current state with our switch estimators. We threshold our predictions at 0.85 which empirically gave the best overall success for transitions. If terrain condition $i$ is detected and $\mathcal{E}_i(s_t) \geqslant 0.85$ we switch to $\pi_i$. All policies are trained by starting with the same initial state (a standing configuration), followed by a small pause before the robot attempts the respective terrain.
    \item \textbf{Our switch estimator without region of attraction overlap:} We test our method using policies trained without considering a region of attraction overlap. The robot is initialised from a random set of joint positions, and is not required to pause before commencing locomotion. All other training and terrain properties are consistent with our switch estimator method, and all policies achieve comparable, or better success rates than policies forced to start from a standing initial state (Table.~\ref{tab:ch4_individual_results}).
\end{itemize}

For \textbf{CoM over feet} and our \textbf{Switch Estimator} methods, if there is no state where the condition to switch is met, then we force-switch to next policy when the robot is within 1cm of the corresponding artifact (other methods switch at a specified distance to the artifact).% e2e
% [0.95834 0.92776 0.902  ]
% [0.00494473 0.00441479 0.01344619]
% 106 46 94 246

\begin{table}[]
    \vspace{3mm}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
         %\hline
         %\multicolumn{3}{c}{Results of 2500 Trials on a Multi Terrain World}\\
         \hline
         Switch Method & \scriptsize{\% Total Dist.} & \scriptsize{\% Success} & \scriptsize{\% Gap Fail} & \scriptsize{\% Jump Fail} & \scriptsize{\% Stair Fail}\\   
         \hline
         Random  & 42.7 & 10.1 & 70.6 & 11.6 & \textbf{7.6} \\
         On detection  &   75.6 & 60.1 & 21.4 & 3.3 & 15.2 \\
         Lookup table &   76.3  & 59.0  &  21.2 & 4.7 & 14.9\\
         CoM over feet  & 79.1 & 66.8 &  17.6 & 2.7 & 12.9 \\
         Ours & \textbf{82.4} & \textbf{71.4} & \textbf{16.7} & \textbf{2.4} & 9.4\\   
         Ours no overlap& 17.5 & 0.7 &  58.6 & 12.9 & 27.7 \\   
         \hline
         *DQN  &  83.2 & 72.4 &  15.1 & 3.7 & 8.8  \\
         *End-to-end  &  \textbf{92.7} & \textbf{90.2} & \textbf{4.2} & \textbf{1.8} & \textbf{3.7}\\
         \hline
    \end{tabular}
    \caption{Results of each switching method on multi-terrain test worlds (2500 trials). The \% of the total distance covered, and the success rate for the robot reaching the end of the trial is shown. The final three columns show the \% of failures for each artifact type.\\ *Trained on the test domain (combinations of terrain types).}
    \label{tab:ch4_test_results}
\end{table}


Table~\ref{tab:ch4_test_results} shows the results for multi-terrain test worlds. For less dynamic platforms it may be possible to switch controllers at any time after obstacle detection, however that was not the case for our scenarios: \textbf{Random} switching performed the worst as expected with only 10.1\% success rate. Switching as soon as an artifact is detected does better than randomly switching with 60.1\% success, we suggest this is because switching early might give the policies enough time to align to an artifact. Fig.~\ref{fig:ch4_estimator}.b) shows it is preferential to switch early for some policies. \textbf{Lookup table} method performed similarly to the \textbf{On Detection} method. \textbf{CoM over feet} method performed relatively well with 66.8\% success. An advantage of this method is that it does not require further data collection once individual policies are trained, providing insight into where RoA overlap occurs for most policies.  \textbf{Our} switching method was the most robust, whilst following our condition that we only have access to individual terrain artifact at training time, traversing 82.4\% of the terrain and reaching the final zone in 71.4\% of trials. Finally, we show the effect of training policies without considering RoA overlap. \textbf{Ours no overlap} performed poorly. Despite the capabilities of the individual behaviours reported in Table.~\ref{tab:ch4_individual_results}, policies trained without explicit state overlap are unable to successfully complete the multi terrain test environment. This result highlights the importance of RoA consideration when training dynamic policies where switching between controllers may be required. 

Fig.~\ref{fig:ch4_plot} shows a single trial of the test world using our method. We can see the switch estimator predictions for each policy in the top figure, and the times our predictions prevented early switching (vertical green lines show detection, vertical red lines show when switching occurs). We can also see in the bottom plot the times that the CoM is over the feet, and instances our estimator switched outside of these regions ($\text{timestep}\approx875$).

The final three columns of Table~\ref{tab:ch4_test_results} shows the failure distribution of each switch method. We record where the robot was when failure occurs, given as a percentage of all trials. For each method, the most failures happened after switching to the Gaps policy. For instance, it contributed to to 16.7\% of a total (28.6\%) failures for our switching method. For all terrain types, these results show less failures than the single terrain experiments reported in Table~\ref{tab:ch4_individual_results}. This suggests we are improving the overall robustness of our behaviour suite using our switch estimator.


\subsection{Comparison with training on multiple artifact terrains}
\label{sec:comparison}

For completeness, we also look at other methods that involve training on a full combination of terrain artifacts, including training a \textbf{Deep Q Network (DQN)} using our pre-trained policies, and a single \textbf{end-to-end policy}. Results are displayed in the last two rows of Table.~\ref{tab:ch4_test_results}. The \textbf{DQN} was provided with the artifact detection in the form of a one hot encoding appended to the robot state, and received the same reward as each policy, with an additional reward provided by our oracle terrain detector encouraging the activation of the correct policy. We note that without the additional reward provided by the oracle the \textbf{DQN} failed to learn. For the \textbf{end-to-end} learning method, we applied the same reward and curriculum learning approach (from~\cite{tidd_guided_2020}) as our policies. Robot state + heightmap is provided as input, and torques are generated at the output. We note that without the curriculum the \textbf{end-to-end} method failed to learn.

Our estimator performs similarly to the \textbf{DQN} despite not seeing more than one terrain artifact type during training (71.4\% success compared to 72.4\%). While learning was substantially longer for the \textbf{end-to-end} policy (approx. two times longer than an individual policy), it performed the best with 90.2\% success rate. While these methods trained on the test domain perform well, it may not be possible to train on all expected terrain conditions on a real platform, where training policies separately allows us to refine each policy in a constrained setting. 

% Furthermore, our method can include new behaviours as they become available, where the \textbf{DQN} and \textbf{end-to-end} methods fail when a new terrain is introduced.

We consider the case where a new terrain is introduced to an existing behaviour suite with two behaviours. With our method, we train a policy for the new terrain obstacle, and retrain the switch estimator for each policy (three in total) to include the new behaviour. We record the wall clock time for training a single policy and the respective switch estimators, and compare to the time to retrain the \textbf{DQN} and \textbf{end-to-end} methods. It takes approximately 17 hours to train a single policy, and an hour to collect data and train a single switch estimator. The \textbf{DQN} method takes about 8 hours to train (after the new policy is available), and the \textbf{end-to-end} method takes roughly 34 hours to train. Table.\ref{tab:ch4_re_training} shows an estimate of wall clock time for each method when a new obstacle is introduced. It can be seen that our method is the most efficient to incorporate new behaviours. Furthermore, our method has the same training complexity as new behaviours become available, where the training becomes more difficult for the \textbf{DQN} and \textbf{end-to-end} methods as more diverse obstacles are introduced. A current limitation of our method is that we collect switching data from all available behaviours, requiring retraining of all switch estimators with each new behaviour. This could be improved by collecting data from a common walking policy, where only a single switch estimator would be trained with a new behaviour. We leave this improvement for future work.


% Table~\ref{tab:ch4_re_training} shows the wall clock training time for all 3 methods when a new terrain is introduced. \textbf{TODO:} make sure $\pi_i$ is the default flat policy only

\begin{table}[]
    \vspace{3mm}
    \centering
    \begin{tabular}{c|c|c}
         \hline
         \scriptsize{\textbf{DQN (hrs)}} & \scriptsize{\textbf{end-to-end (hrs)}} & \scriptsize{\textbf{Ours (hrs)}}\\   
         \hline
         25 & 34 & \textbf{20} \\
         \hline
    \end{tabular}
    \caption{Wall clock time for retraining when a new terrain is introduced. Each method is trained with the same number of CPU cores of the same architecture.}
    \label{tab:ch4_re_training}
\end{table}




\begin{figure}[tb!]
\vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch4/plot.png}
\caption{Our method on a single trial in the test world. The top figure shows the switch estimate from the time the next artifact is detected until the robot has past the artifact. The bottom figure shows the terrain (pink) with foot (blue and green) and CoM height (red) when the CoM is over the stance foot. Green vertical lines indicate when the terrain was detected, red vertical lines show when switching occurred.}
\label{fig:ch4_plot}
% \vspace{-3mm}
\end{figure}


This chapter investigated research question: \textbf{\textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}} Behaviour switching was demonstrated with a biped learning switch states between discrete behaviours. The contributions of this chapter, from \cite{tidd_learning_2021} are as follows:

\begin{itemize}
    % \item Using policies developed in the previous chapter, we investigate  the effect of state overlap on safe policy switching
    % \item We design a policy switching network that estimates when the  robot is in the RoA for the next policy by predicting the probability  of success by switching in the current state
    \item The effect of state overlap on safe policy switching was investigated by training diverse policies with common initial conditions. The results showed that initiating each policy with the same configuration provided sufficient RoA overlap for reliable behaviour switching
    \item A policy switching network was designed to estimate the likelihood of success for switching policies in a given state, improving the reliability of traversing a sequence of obstacles
\end{itemize}

“Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts” was
published and presented at the 2021 IEEE/RSJ International Conference on Intelligent Robots and Systems held in Prague, Czech Republic and virtually. 
\newpage
\newpage



==> old/Ch4_pdf_old.tex <==
% \chapter[Learning to Transition Between Dynamic Behaviours]{Learning to Transition Between Complex Behaviours}

% \chapter[Learning to Switch Between Behaviours]{Learning When to Switch Between Sequential Behaviours}
\chapter[Learning When to Switch]{Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts}

% \item \textbf{Research Question 2: \textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}}

\label{cha:ch4}
% Motivation/contribution/abstract -----------------------

% \section{Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts}
% \label{sec:sec_switch}

Chapter \ref{cha:ch3} discussed methods for efficiently learning locomotion behaviours, investigating how  for a dynamic biped traversing complex obstacles. These behaviours were created on separate terrain examples. 

apply these behaviours as a set to traverse a sequence of obstacles (as shown in Fig.~\ref{fig:cha4_fig1}) we must be able to switch between controllers. In this chapter we investigate research question 2: \textit{``How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?"}

\begin{figure}[htb!]
\centering
\includegraphics[width=1.0\columnwidth]{images/ch4/main_pic.png}
\caption{Switching between policies to traverse a sequence of obstacles.}
\label{fig:cha4_fig1}
% \vspace{-3mm}
\end{figure}

This chapter is constructed from two papers: the first paper ``Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts" [\cite{tidd_learning_2021}] , discusses the effect of RoA overlap when training policies, and learns a Switch Estimator policy to determine when the robot is in a suitable state to switch to a particular policy. The second paper, ``Learning Setup Policies: Reliable Transition Between Locomotion Behaviours" [\cite{tidd_learning_2021-1}], looks at how we can bridge the gap when there is no overlap between adjacent policies.



% Dynamic walking requires the robot to undergo a periods of controlled falling throughout its step cycle. Through this falling period, the robot does not have control authority over the contact with the ground. 

% Using these behaviours, we now investigate research question 2: ``How can we reliably transition between behaviours?" Switching between dynamic behaviours requires the robot be in a suitable state for the next behaviour. 

% Behaviour based locomotion requires that controllers can be switched to the most appropriate behaviour for the terrain conditions. Switching to a behaviour while the robot is not in an compatible state for the new controller can result in undesired behaviour or instability (particularly if the robot is highly dynamic). While classical methods rely on explicitly knowing the set of states that a controller will converge to a stable behaviour, (known as the region of attraction (RoA) for the controller), it may be difficult to know this complete set. Agents with a high degree of freedom (DoF), black box controllers, and pose relative to terrain obstacles make it difficult to formulate the complete set of states within a controllers RoA. Furthermore, for complex behaviours, there may be little or no overlap between the RoA's of two sequential controllers, meaning that a stable switch point may not exist. We aim to investigate how we can determine when a good switch location occurs, and how we can prepare the robot for an upcoming behaviour if there is no suitable overlap. 

% Learning when to switch is important. Fig.~\ref{fig:cha4_fig1}. Fig.~\ref{fig:cha4_fig2}. Fig.~\ref{fig:cha4_fig3}.

% Methohds

\begin{figure}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch4/fig2.png}
\caption{Using a Switch Estimator for improving the reliability of changing behaviours after a new terrain is detected.}
\label{fig:cha4_fig2}
% \vspace{-3mm}
\end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=0.9\columnwidth]{images/ch4/estimator.png}
\hfill
\caption{The Switch Estimator is trained with data collected from each policy on its respective terrain.}
\label{fig:cha4_fig3}
% \vspace{-3mm}
\end{figure}

\begin{table}[htb!]
    % \vspace{3mm}
    \centering
    % \begin{tabular}{p{1.5cm}|M{2.5cm}|M{2.5cm}|M{2.5cm}|M{2.5cm}}
    \begin{tabular}{p{1.5cm}M{2.5cm}M{2.5cm}M{2.5cm}M{2.5cm}}
    % \begin{tabular}{c|c|c|c|c}
         Policy & \% Total Dist. &\% Success & \% Total Dist. no Overlap & \% Success  no Overlap\\
         \hline
         Jumps  & \textbf{93.9} & \textbf{91.2} & 86.2 & 77.5\\
         Gaps   & 78.7 & 60.4  & \textbf{87.4} & \textbf{75.5} \\
         Stairs & 67.3 & 34.4  & \textbf{78.7} & \textbf{59} \\
         \hline
    \end{tabular}
    \caption{Results of each individual policy on its corresponding terrain type, starting from a standing initial joint positions, and from random initial joint positions (no Overlap).}
    \label{tab:ch4a_individual_results}
\end{table}



\begin{table}[htb!]
    % \vspace{3mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    \begin{tabular}{cccccc}
         %\hline
         %\multicolumn{3}{c}{Results of 2500 Trials on a Multi Terrain World}\\
        %  \hline
        %  Switch Method & \scriptsize{\% Total Dist.} & \scriptsize{\% Success} & \scriptsize{\% Gap Fail} & \scriptsize{\% Jump Fail} & \scriptsize{\% Stair Fail}\\   
          Switch Method & \% Total Dist. & \% Success & \% Gap Fail & \% Jump Fail & \% Stair Fail\\   
         \hline
         Random  & 42.7 & 10.1 & 70.6 & 11.6 & \textbf{7.6} \\
         On detection  &   75.6 & 60.1 & 21.4 & 3.3 & 15.2 \\
         Lookup table &   76.3  & 59.0  &  21.2 & 4.7 & 14.9\\
         CoM over feet  & 79.1 & 66.8 &  17.6 & 2.7 & 12.9 \\
         Ours & \textbf{82.4} & \textbf{71.4} & \textbf{16.7} & \textbf{2.4} & 9.4\\   
         Ours no overlap& 17.5 & 0.7 &  58.6 & 12.9 & 27.7 \\   
         \hline
         *DQN  &  83.2 & 72.4 &  15.1 & 3.7 & 8.8  \\
         *End-to-end  &  \textbf{92.7} & \textbf{90.2} & \textbf{4.2} & \textbf{1.8} & \textbf{3.7}\\
         \hline
    \end{tabular}
    \caption{Results of each switching method on multi-terrain test worlds (2500 trials).}
    \label{tab:ch4a_test_results}
\end{table}

\begin{table}[htb!]
    % \vspace{3mm}
    \centering
    \begin{tabular}{ccc}
        %  \hline
         \textbf{DQN (hrs)} & \textbf{end-to-end (hrs)} & \textbf{Ours (hrs)}\\  
        %   \scriptsize{\textbf{DQN (hrs)}} & \scriptsize{\textbf{end-to-end (hrs)}} & \scriptsize{\textbf{Ours (hrs)}}\\  
         \hline
        %  70.6 & 11.6 & \textbf{7.6} \\WTF? where did these numbers come frome?
           25 & 34 & \textbf{20} \\
         \hline
    \end{tabular}
    \caption{Wall clock time for retraining when a new terrain is introduced.}
    \label{tab:ch4a_re_training}
\end{table}

\begin{figure}[htb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch4/plot.png}
\caption{Our method on a single trial in the test world.}
\label{fig:ch4a_plot}
% \vspace{-3mm}
\end{figure}


% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% % \includegraphics[width=0.5\columnwidth]{images/ch4/estimator.png}}
% \includegraphics[height=0.3\columnwidth]{images/ch4/estimator.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[height=0.3\columnwidth]{images/ch4/multi_roa.png}}
% \hfill
% \caption{a) The Switch Estimator is trained with data collected from each policy. b) Switching locations and resulting success.}
% \label{fig:cha4_fig3}
% % \vspace{-3mm}
% \end{figure}


Fig.~\ref{fig:cha4_fig2} shows the pipeline for running multiple behaviours and their respective Switch Estimator policy. Once a new terrain is detected, the Switch Estimator for the next policy determines when the robot is in a safe state for switching. Switch Estimators are trained by collecting data by randomly switching between behaviours and assigning labels to states based on the successful traversal of the terrain (Fig.~\ref{fig:cha4_fig3}).


Table \ref{tab:ch4a_individual_results} shows the success rates for each terrain type if the robot started each episode from a standing pose, or from random initial joint positions (no overlap). Table \ref{tab:ch4a_test_results} compares several switching methods, and shows that not only is learning when to switch the most successful method for reliable switching, it is also vital there is an overlap between behaviours. Methods with access to the full terrain during training (DQN and end-to-end) perform better overall, however our method can be retrained more efficiently when a new terrain is introduced (Table \ref{tab:ch4a_re_training}). We can see the Switch Estimator predictions for a single episode over a sequence of terrain types terrain types (Fig.\ref{fig:ch4a_plot}).

% In order to ensure policies trained on separate terrains have a set of common states, we started the robot from the same initial standing pose. 

% \section{Learning Setup Policies: Reliable Transition Between Locomotion Behaviours}
% \label{sec:sec_setup}
% Motivation/contribution/abstract -----------------------


%     \item How can we reliably transition between behaviours? \\
    
%         Behaviour based locomotion requires that controllers can be switched to the most appropriate behaviour for the terrain conditions. Switching to a behaviour while the robot is not in an compatible state for the new controller can result in undesired behaviour or instability (particularly if the robot is highly dynamic). While classical methods rely on explicitly knowing the set of states that a controller will converge to a stable behaviour, (known as the region of attraction (RoA) for the controller), it may be difficult to know this complete set. Agents with a high degree of freedom (DoF), black box controllers, and pose relative to terrain obstacles make it difficult to formulate the complete set of states within a controllers RoA. Furthermore, for complex behaviours, there may be little or no overlap between the RoA's of two sequential controllers, meaning that a stable switch point may not exist. We aim to investigate how we can determine when a good switch location occurs, and how we can prepare the robot for an upcoming behaviour if is no suitable overlap. 

In this chapter we investigate the research question ``How can we reliably transition between behaviours?" The contributions of this chapter, from the two included papers [\cite{tidd_learning_2021}, \cite{tidd_learning_2021-1}] are as follows:

\begin{itemize}
    \item Using policies developed in the previous chapter, we investigate  the effect of state overlap on safe policy switching
    \item We design a policy switching network that estimates when the  robot is in the RoA for the next policy by predicting the probability  of success by switching in the current state
\end{itemize}

“Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts” was
published at the 2021 IEEE/RSJ International Conference on Intelligent Robots and Systems in Prague, Czech Republic. 
\linebreak
\newpage
\newpage

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/Learning_When_to_Switch__Composing_Controllers_to_Traverse_a_Sequence_of_Terrain_Artifacts.pdf}

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/GRC_Statement-of-Contribution_Form_switching.pdf}

    % \item Using policies developed in the previous chapter, we investigate  the effect of state overlap on safe policy switching
    % \item We design a policy switching network that estimates when the  robot is in the RoA for the next policy by predicting the probability  of success by switching in the current state

%  Bipedal robots often use separate control policies that are specifically designed for a given condition, where reliable behaviour switching occurs when the robot is in the RoA of the next behaviour.

% Methods with access to the full terrain during training (DQN and end-to-end) perform better overall, however our method can be retrained more efficiently when a new terrain is introduced (Table \ref{tab:ch4a_re_training}).


% \begin{table}[htb!]
%     % \vspace{3mm}
%     \centering
%     \begin{tabular}{ccc}
%         %  \hline
%          \textbf{DQN (hrs)} & \textbf{end-to-end (hrs)} & \textbf{Ours (hrs)}\\  
%         %   \scriptsize{\textbf{DQN (hrs)}} & \scriptsize{\textbf{end-to-end (hrs)}} & \scriptsize{\textbf{Ours (hrs)}}\\  
%          \hline
%         %  70.6 & 11.6 & \textbf{7.6} \\WTF? where did these numbers come frome?
%           25 & 34 & \textbf{20} \\
%          \hline
%     \end{tabular}
%     \caption{Wall clock time for retraining when a new terrain is introduced.}
%     \label{tab:ch4a_re_training}
% \end{table}


% Table



%  This objective requires the reliable Using these behaviours, the object of .A Switch Estimator policy was trained to determine when the robot is in a suitable state for switching to the behaviour most suited for the upcoming obstacle. Additionally, 

% To understand the effect of state overlap for controller switching, the initial conditions

% where switching between policies is only possible when the robot is in a region that is common to adjacent controllers. Deep Reinforcement Learning (DRL) is a promising alternative to hand-crafted control design, though typically requires the full set of test conditions to be known before training. DRL policies can result in complex (often unrealistic) behaviours that have few or no overlapping regions between adjacent policies, making it difficult to switch behaviours. In this work we develop multiple DRL policies with Curriculum Learning (CL), each that can traverse a single respective terrain condition, while ensuring an overlap between policies. We then train a network for each destination policy that estimates the likelihood of successfully switching from any other policy. We evaluate our switching method on a previously unseen combination of terrain artifacts and show that it performs better than heuristic methods. While our method is trained on individual terrain types, it performs comparably to a Deep Q Network trained on the full set of terrain conditions. This approach allows the development of separate policies in constrained conditions with embedded prior knowledge about each behaviour, that is scalable to any number of behaviours, and prepares DRL methods for applications in the real world.

% Results

% Contributions


% Chapter \ref{cha:ch3} discussed methods for efficiently learning locomotion behaviours, investigating how  for a dynamic biped traversing complex obstacles. These behaviours were created on separate terrain examples. 

% apply these behaviours as a set to traverse a sequence of obstacles (as shown in Fig.~\ref{fig:cha4_fig1}) we must be able to switch between controllers. In this chapter we investigate research question 2: \textit{``How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?"}


% This chapter is constructed from two papers: the first paper ``Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts" [\cite{tidd_learning_2021}] , discusses the effect of RoA overlap when training policies, and learns a Switch Estimator policy to determine when the robot is in a suitable state to switch to a particular policy. The second paper, ``Learning Setup Policies: Reliable Transition Between Locomotion Behaviours" [\cite{tidd_learning_2021-1}], looks at how we can bridge the gap when there is no overlap between adjacent policies.



% Dynamic walking requires the robot to undergo a periods of controlled falling throughout its step cycle. Through this falling period, the robot does not have control authority over the contact with the ground. 

% Using these behaviours, we now investigate research question 2: ``How can we reliably transition between behaviours?" Switching between dynamic behaviours requires the robot be in a suitable state for the next behaviour. 

% Behaviour based locomotion requires that controllers can be switched to the most appropriate behaviour for the terrain conditions. Switching to a behaviour while the robot is not in an compatible state for the new controller can result in undesired behaviour or instability (particularly if the robot is highly dynamic). While classical methods rely on explicitly knowing the set of states that a controller will converge to a stable behaviour, (known as the region of attraction (RoA) for the controller), it may be difficult to know this complete set. Agents with a high degree of freedom (DoF), black box controllers, and pose relative to terrain obstacles make it difficult to formulate the complete set of states within a controllers RoA. Furthermore, for complex behaviours, there may be little or no overlap between the RoA's of two sequential controllers, meaning that a stable switch point may not exist. We aim to investigate how we can determine when a good switch location occurs, and how we can prepare the robot for an upcoming behaviour if there is no suitable overlap. 

% Learning when to switch is important. Fig.~\ref{fig:cha4_fig1}. Fig.~\ref{fig:cha4_fig2}. Fig.~\ref{fig:cha4_fig3}.

% Methohds



% \begin{table}[htb!]
%     % \vspace{3mm}
%     \centering
%     % \begin{tabular}{p{1.5cm}|M{2.5cm}|M{2.5cm}|M{2.5cm}|M{2.5cm}}
%     \begin{tabular}{p{1.5cm}M{2.5cm}M{2.5cm}M{2.5cm}M{2.5cm}}
%     % \begin{tabular}{c|c|c|c|c}
%          Policy & \% Total Dist. &\% Success & \% Total Dist. no Overlap & \% Success  no Overlap\\
%          \hline
%          Jumps  & \textbf{93.9} & \textbf{91.2} & 86.2 & 77.5\\
%          Gaps   & 78.7 & 60.4  & \textbf{87.4} & \textbf{75.5} \\
%          Stairs & 67.3 & 34.4  & \textbf{78.7} & \textbf{59} \\
%          \hline
%     \end{tabular}
%     \caption{Results of each individual policy on its corresponding terrain type, starting from a standing initial joint positions, and from random initial joint positions (no Overlap).}
%     \label{tab:ch4a_individual_results}
% \end{table}




% \begin{figure}[htb!]
% % \vspace{2mm}
% \centering
% \includegraphics[width=0.95\columnwidth]{images/ch4/plot.png}
% \caption{Our method on a single trial in the test world.}
% \label{fig:ch4a_plot}
% % \vspace{-3mm}
% \end{figure}


% \begin{figure}[tb!]
% \centering
% \subfloat[]{%
% % \includegraphics[width=0.5\columnwidth]{images/ch4/estimator.png}}
% \includegraphics[height=0.3\columnwidth]{images/ch4/estimator.png}}
% \hfill
% \subfloat[]{%
% \includegraphics[height=0.3\columnwidth]{images/ch4/multi_roa.png}}
% \hfill
% \caption{a) The Switch Estimator is trained with data collected from each policy. b) Switching locations and resulting success.}
% \label{fig:cha4_fig3}
% % \vspace{-3mm}
% \end{figure}


% Fig.~\ref{fig:cha4_fig2} shows the pipeline for running multiple behaviours and their respective Switch Estimator policy. Once a new terrain is detected, the Switch Estimator for the next policy determines when the robot is in a safe state for switching. Switch Estimators are trained by collecting data by randomly switching between behaviours and assigning labels to states based on the successful traversal of the terrain (Fig.~\ref{fig:cha4_fig3}).


% Table \ref{tab:ch4a_individual_results} shows the success rates for each terrain type if the robot started each episode from a standing pose, or from random initial joint positions (no overlap). Table \ref{tab:ch4a_test_results} compares several switching methods, and shows that not only is learning when to switch the most successful method for reliable switching, it is also vital there is an overlap between behaviours. Methods with access to the full terrain during training (DQN and end-to-end) perform better overall, however our method can be retrained more efficiently when a new terrain is introduced (Table \ref{tab:ch4a_re_training}). We can see the Switch Estimator predictions for a single episode over a sequence of terrain types terrain types (Fig.\ref{fig:ch4a_plot}).

% In order to ensure policies trained on separate terrains have a set of common states, we started the robot from the same initial standing pose. 

% \section{Learning Setup Policies: Reliable Transition Between Locomotion Behaviours}
% \label{sec:sec_setup}
% Motivation/contribution/abstract -----------------------


%     \item How can we reliably transition between behaviours? \\
    
%         Behaviour based locomotion requires that controllers can be switched to the most appropriate behaviour for the terrain conditions. Switching to a behaviour while the robot is not in an compatible state for the new controller can result in undesired behaviour or instability (particularly if the robot is highly dynamic). While classical methods rely on explicitly knowing the set of states that a controller will converge to a stable behaviour, (known as the region of attraction (RoA) for the controller), it may be difficult to know this complete set. Agents with a high degree of freedom (DoF), black box controllers, and pose relative to terrain obstacles make it difficult to formulate the complete set of states within a controllers RoA. Furthermore, for complex behaviours, there may be little or no overlap between the RoA's of two sequential controllers, meaning that a stable switch point may not exist. We aim to investigate how we can determine when a good switch location occurs, and how we can prepare the robot for an upcoming behaviour if is no suitable overlap. 


==> old/Ch4_pdf_separate.tex <==
\chapter[Learning to Transition Between Dynamic Behaviours]{Learning to Transition Between Dynamic Behaviours}
\label{cha:ch4}
% Motivation/contribution/abstract -----------------------

\section{Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts}
\label{sec:sec_switch}


Learning when to switch is important. Fig.~\ref{fig:cha4_fig1}. Fig.~\ref{fig:cha4_fig2}. Fig.~\ref{fig:cha4_fig3}.

\begin{figure}[htb!]
\centering
\includegraphics[width=1.0\columnwidth]{images/ch4/main_pic.png}
\caption{To successfully switch between policies we train a switch estimator for each policy that learns when best to switch.}
\label{fig:cha4_fig1}
\vspace{-3mm}
\end{figure}

\begin{figure}[htb!]
\vspace{2mm}
\centering
\includegraphics[width=0.95\columnwidth]{images/ch4/fig2.png}
\caption{Using the current policy $\pi_i$, and detecting upcoming terrain type $j$, we use the switch estimator output $e_j$ to determine when the robot is in a suitable configuration to safely switch to the next policy $\pi_j$.}
\label{fig:cha4_fig2}
\vspace{-3mm}
\end{figure}

\begin{figure}[tb!]
\centering
\subfloat[]{%
% \includegraphics[width=0.5\columnwidth]{images/ch4/estimator.png}}
\includegraphics[height=0.3\columnwidth]{images/ch4/estimator.png}}
\hfill
\subfloat[]{%
\includegraphics[height=0.3\columnwidth]{images/ch4/multi_roa.png}}
\hfill
\caption{a) A switch estimator is trained with data collected from each policy. b) Early switching results in successful transitions for some policies (green), whereas switching late is more likely to fail (red).}
\label{fig:cha4_fig3}
\vspace{-3mm}
\end{figure}


The research question answering:

The contributions of this paper.

“Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts” was
published at the 2021 IEEE/RSJ International Conference on Intelligent Robots and Systems in Prague, Czech Republic. 
\linebreak
\newpage

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/Learning_When_to_Switch__Composing_Controllers_to_Traverse_a_Sequence_of_Terrain_Artifacts.pdf}

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/GRC_Statement-of-Contribution_Form_switching.pdf}

% =======================================================================
% -----------------------------------------------------------------------
% =======================================================================

\section{Learning Setup Policies: Reliable Transition Between Locomotion Behaviours}
\label{sec:sec_setup}
% Motivation/contribution/abstract -----------------------

\begin{figure}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth,natwidth=610,natheight=642]{images/ch5/Fig1.png}
\includegraphics[width=\columnwidth]{images/ch5/Fig1.png}
% \includegraphics[width=\columnwidth]{images/ch5/Fig1_err.png}
\hfill
\caption{The trajectory of the walking policy $i$ (shown with a blue line), does not intersect with the trajectory of the target policy $j$ (green line). Our setup policy provides a trajectory that prepares the robot for the upcoming target policy (orange line).}
\label{fig:cha4_setup_fig1}
% \vspace{-3mm}
\end{figure}
% How can we leverage subpolicy learning to improve learning outcomes?
Our contributions are as follows:
\begin{itemize}
    \item Using pre-trained policies, we develop a \textbf{Setup Policy} that significantly improves the success rate from transitioning from a default walking policy to a target policy (from 1.5$\%$ success rate without Setup Policies to 82$\%$). The setup policy also learns when to switch to the target policy. 
    \item We introduce a novel reward, called \textbf{Advantage Weighted Target Value}, based on the performance of the subsequent policy.
    \item We show that we can use our setup policies with several difficult terrain types, allowing for a modular control suite, combining policies that have been trained separately.
\end{itemize}


\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=\columnwidth]{images/ch5/Fig2.png}}
\hfill
\subfloat[]{\includegraphics[width=\columnwidth]{images/ch5/Fig3.png}}
% \hfill
\caption{a) A terrain classifier selects which module should be utilised. b) Each module (Target Policy and Setup Policy) is trained on a single terrain type.}
\label{fig:cha4_setup_fig2}
% \vspace{-3mm}
\end{figure}

\begin{figure*}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth]{images/ch5/Fig1_2.png}
\includegraphics[width=\textwidth]{images/ch5/all.png}
\hfill
\caption{Setup policies allow us to transition between behaviours to traverse several complex terrains.}
\label{fig:cha4_setup_fig3}
% \vspace{-3mm}
\end{figure*}


The research question answering:

The contributions of this paper.

“Learning Setup Policies: Reliable Transition Between Locomotion Behaviours” was
in submission for the IEEE Robotics and Automation Letters (RA-L). 
\linebreak
\newpage

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/Learning_Setup_Policies__Reliable_Transition_Between_Locomotion_Behaviours.pdf}

\includepdf[pages=-,pagecommand={},width=\textwidth]{pdfs/GRC_Statement-of-Contribution_Form_setup.pdf}

==> old/Ch5.tex <==
% Ch5.tex
\chapter[Learning Setup Policies: Reliable Transition Between Locomotion Behaviours]{Learning Setup Policies: Reliable Transition Between Locomotion Behaviours}
\label{cha:ch5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Dynamic platforms that operate over many unique terrain conditions typically require multiple controllers. To transition safely between controllers, there must be an overlap of states between adjacent controllers. We develop a novel method for training Setup Policies that bridge the trajectories between pre-trained Deep Reinforcement Learning (DRL) policies. We demonstrate our method with a simulated biped traversing a difficult jump terrain, where a single policy fails to learn the task, and switching between pre-trained policies without Setup Policies also fails. We perform an ablation of key components of our system, and show that our method outperforms others that learn transition policies. We demonstrate our method with several difficult and diverse terrain types, and show that we can use Setup Policies as part of a modular control suite to successfully traverse a sequence of complex terrains. We show that using Setup Policies improves the success rate for traversing a single difficult jump terrain (from 1.5$\%$ success rate without Setup Policies to 82$\%$), and a sequence of various terrains (from 6.5$\%$ without Setup Policies to 29.1$\%$).


% \textbf{why do I care?}
% , as it may not be possible to safely switch between controllers outside of the overlapping states.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:introduction}

Bipedal robots have the capability to cover a span of terrains that humans can traverse. This makes bipeds an appealing locomotion option for robots in human environments. It is impractical, however, to design a single controller that works over all required environments, particularly if all conditions are not known a priori. For robots to be able to perform a number of diverse behaviours, it is desirable for a control suite to be modular, where any number of behaviours can be added with minimal retraining.

% included in the control repertoire. 
% Ideally, as new conditions are identified and new controllers become available, the new behaviours can be added to the control suite with minimal retraining.
 
Deep Reinforcement Learning (DRL) is an appealing method for developing behaviours for legged platforms. However, such DRL policies are usually trained in the same terrain they are expected to operate, though it is unlikely that the agent would have access to a complete set of terrain conditions during policy training before deployment. Controllers for dynamic platforms are typically developed and tuned with harnesses and treadmills in order to minimise potential damage to the robot and the environment. These restrictions limit the development of controllers over an exhaustive collection of terrain conditions. Furthermore, it is preferable to not re-design controllers that have already been tuned, whereas DRL methods typically require retraining if the target conditions are evolved to included new terrains. We propose training a \textit{Setup Policy} to transition between two pre-trained policies targeting different terrains.

A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over if controllers are switched when the robot is not in a safe region for the subsequent controller. Figure~\ref{fig:fig1} shows our primary contribution: a Setup Policy that prepares the robot for the necessary controller to traverse the upcoming terrain artifact. With our method, we can transition between existing behaviours, allowing pre-trained DRL policies to be combined. 

% We propose a modular approach to developing a control suite for a biped expected to traverse a number of difficult terrain artifacts, where all terrain conditions are not known when training each module. A modular control suite for a dynamic platform requires careful design. Simply switching between controllers may result in the robot falling over. Figure~\ref{fig:fig1} shows our primary contribution: a setup policy that prepares the robot for the upcoming terrain artifact. With our method, we can safely transition between behaviours that are developed separately, such that any number of pre-trained DRL policies can be combined, without any re-training of low level policies.  

\begin{figure}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth,natwidth=610,natheight=642]{images/ch5/Fig1.png}
\includegraphics[width=\columnwidth]{images/ch5/Fig1.png}
% \includegraphics[width=\columnwidth]{images/ch5/Fig1_err.png}
\hfill
\caption{As the robot approaches a difficult terrain artifact, it must move into position for target policy $j$. The trajectory of the walking policy $i$ (shown with a blue line), does not intersect with the trajectory of the target policy $j$ (green line). Our setup policy provides a trajectory that prepares the robot for the upcoming target policy (orange line).}
\label{fig:fig1}
% \vspace{-3mm}
\end{figure}
% How can we leverage subpolicy learning to improve learning outcomes?
Our contributions are as follows:
\begin{itemize}
    \item Using pre-trained policies, we develop a \textbf{Setup Policy} that significantly improves the success rate from transitioning from a default walking policy to a target policy (from 1.5$\%$ success rate without Setup Policies to 82$\%$). The setup policy also learns when to switch to the target policy. 
    \item We introduce a novel reward, called \textbf{Advantage Weighted Target Value}, based on the performance of the subsequent policy.
    \item We show that we can use our setup policies with several difficult terrain types, allowing for a modular control suite, combining policies that have been trained separately.
\end{itemize}

% The organization of this paper is as follows. After reviewing the relevant literature in Sec~\ref{sec:related_work}, we define the problem in Sec~\ref{sec:problem}, the learning algorithm in Sec~\ref{sec:ppo}, and our method for developing setup policies in Sec~\ref{sec:setup}. Our experimental results and comparisons are shown in Sec~\ref{sec:experiments}. Finally, we conclude with a brief discussion in Sec~\ref{sec:conclusion}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:related_work}
% Related work should also be story, starting from the start of the problem, highlighting what is missing, and refining to the specific paper that is closest to ours. Goal is to find gaps, start broad, and funnel into specifics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Deep reinforcement learning (DRL) has demonstrated impressive results for locomotion tasks in recent works~\cite{schulman_proximal_2017, heess_emergence_2017, peng_deeploco_2017, peng_deepmimic_2018, xie_allsteps_2020}. Typically DRL policies optimise a single reward function, as new environments and behaviours are introduced costly retraining is required. Furthermore, developing a single policy to perform multiple behaviours can degrade the performance of each behaviour~\cite{lee_robust_2019}.

Hierarchical reinforcement learning (HRL) offers flexibility through architecture, involving training all segments of the hierarchy concurrently~\cite{sutton_between_1999, bacon_option-critic_2018, frans_meta_2018,peng_deeploco_2017}, or training parts of the hierarchy separately~\cite{merel_hierarchical_2019},~\cite{lee_composing_2019}.  When trained together, HRL can improve task level outcomes, such as steering and object tracking~\cite{peng_deeploco_2017}, or improve learning efficiency by reusing low level skills across multiple high level tasks~\cite{frans_meta_2018}. When trained separately, low level controllers can be refined efficiently using prior knowledge, such as by utilising motion capture data~\cite{peng_deepmimic_2018, merel_hierarchical_2019, peng_mcp_2019} or inverse reinforcement learning~\cite{strudel_learning_2020}. For robotics applications it may be difficult to develop controllers for multiple behaviours simultaneously. Using pre-trained primitives can break up a large difficult problem into smaller solvable sub-problems~\cite{schaal_dynamic_2006}.

Using pre-trained policies requires a suitable handling of transitions between behaviours. Faloutsos et al~\cite{faloutsos_composable_2001} learns pre and post-conditions for each controller, such that switching only occurs when these conditions have been satisfied. DeepMimic by Peng et al~\cite{peng_deepmimic_2018} combines pre-trained behaviours learned from motion capture, with reliance on a phase variable to determine when one behaviour has been completed. Policy sketches introduce a hierarchical method that uses task specific policies, with each task performed in sequence~\cite{andreas_modular_2017}. CompILE uses soft boundaries between task segments~\cite{kipf_compile_2019}. Work by Peng et al~\cite{peng_terrain-adaptive_2016} trains several actor-critic control policies, modulated by the highest critic value in an given state. For these examples there must be a reasonable state overlap between sequential controllers.

Other methods that combine pre-trained behaviours learn latent representations of skills~\cite{pertsch_accelerating_2020} or primitives~\cite{ha_distilling_2020}, enabling interpolation in the latent space. From an offline dataset of experience, Pertsch et al~\cite{pertsch_accelerating_2020} are able to combine low level controllers in manipulation tasks and locomotion task for a multi-legged agent. Ha et al~\cite{ha_distilling_2020} utilise motion capture to learn latent representations of primitives, then use model predictive control for the high level navigation of a high dimensional humanoid. The FeUdal approach learns a master policy that modulates
low-level policies using a learned goal signal~\cite{vezhnevets_feudal_2017}. Work by Peng et al~\cite{peng_mcp_2019} combines pre-trained policies using a gating function that learns a multiplicative combination of actions. In our previous work~\cite{tidd_learning_2020}, we learn when to switch between low level primitives for a simulated biped by randomly sampling from a collection of behaviours. Interpolation between behaviours yields natural transitions~\cite{xu_hierarchical_2020}, however in each of these approaches, experience from all behaviours must be available during training. 

For dynamic platforms, where separate controllers occupy different subsets of the state, changing behaviours may not result in stable behaviour if there is no overlap between controllers. Lee et al~\cite{lee_composing_2019} learn a proximity predictor to train a transition policy to get an agent to the initial state required by the next controller. Our setup policies are also use an intermediate controller, however we show that our method performs more reliably with complex locomotion behaviours.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Berkencamp, and mace use values to estimate when to use controllers.
% Composing paper. Something more specific about our method: advantage weighted value, this is a primary contribution. Training on sample only. Scaling to any number of policies, only needing data to train classifier, (no training of policies on anything but samples).


% sequential decision making tasks
% with greater sample efficiency than their non-hierarchical counterparts because hierarchical agents can break down tasks into sets of subtasks that only require short
% sequences of decisions.LEARNING MULTI-LEVEL HIERARCHIES WITH
% HINDSIGHT Andrew Levy , Hierarchical Actor-Critic (HAC), . Yet, learning multiple
% levels of policies in parallel is hard because it is inherently unstable: changes in
% a policy at one level of the hierarchy may cause changes in the transition and reward functions at higher levels in the hierarchy, making it difficult to jointly learn
% multiple levels of policies.  The main idea behind HAC is to train each level of the
% hierarchy independently of the lower levels by training each level as if the lower
% level policies are already optimal.

% HIRO Data-Efficient Hierarchical Reinforcement Learning Ofir Nachum - Use reward relabeling - High level give goals to low level. rewards from the environment are reused, temporal abstraction, off-policy.


% The first category lets a high-level policy select a low-level skill to execute [13, 14, 15, 28],
% which we refer to as the selector methods. In the second category, a subgoal is set for the low level by
% high-level policies [8, 9, 11, 10, 25], which we refer to as subgoal-based methods.

% % \subsection{Hierarchical RL}

% % \subsection{Transition Policies and Modular RL}
% % \textbf{ TODO Transition papers
% \begin{itemize}
%     \item sutton \cite{Sutton2017ReinforcementA.G.}
%     \item HRL \cite{sutton_between_1999} - introduces options, a framework for splitting mdp into temporally abstracted options.
%     \item m, HRL with Advantage function-based Auxiliary Rewards \cite{li et al} - Use the advantage of the high level policy as dense reward signal for an otherwise sparse reward problem,  improving pre-trained low level policies for navigation with legged locomotion.
%     \item 
%     \item COMPOSING COMPLEX SKILLS BY LEARNING TRANSITION POLICIES~\cite{lee_composing_2019}
%     \item MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies~\cite{peng_mcp_2019}
%     \item  MCP: Learning Composable Hierarchical Control with Multiplicative Compositional Policies

%     \item Robust Recovery Controller for a Quadrupedal Robot using Deep Reinforcement Learning\cite{lee_robust_2019}
%     \item Modular multitask reinforcement learning with
% policy sketches \cite{andreas_modular_2017}
%     \item The option-critic architecture \cite{bacon_option-critic_2018}
%     \item DIVIDE-AND-CONQUER REINFORCEMENT LEARNING \cite{ghosh_divide-and-conquer_2018}
%     \item distillation - PLAID
%     \item progressive learning? progressive nets?
%     \item FeUdal Networks for Hierarchical Reinforcement Learning Alexander Sasha Vezhnevets \cite{vezhnevets_feudal_2017}
%     \item Terrain-Adaptive Locomotion Skills Using Deep Reinforcement Learning peng: relies on taking an action based on its value, (overestimated)
%     \item bekencamp - value to predict roa of pendulum (overestimated)
% \end{itemize}


% \begin{itemize}
%     \item Composable Controllers for Physics-Based Character Animation~\cite{faloutsos_composable_2001}
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Method}
\label{sec:method}

In this section we describe the problem we are solving and our method for training setup policies. 

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=\columnwidth]{images/ch5/Fig2.png}}
\hfill
\subfloat[]{\includegraphics[width=\columnwidth]{images/ch5/Fig3.png}}
% \hfill
\caption{a) shows the modular pipeline. A terrain classifier selects which module should be utilised, and the torque from the output of the selected module is applied to the robot, returning robot state and depth image. b) Each module is pre-trained on a single terrain type. The Target Policy has been designed to traverse a specific terrain condition. The Setup Policy guides the trajectory of the robot from a default walking controller to the Target Policy, also learning when to switch to the Target Policy.}
\label{fig:fig2}
% \vspace{-3mm}
\end{figure}

\subsection{Problem Description}
\label{sec:problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We investigate composing controllers for a dynamic platform with little or no state overlap between adjacent behaviours. An example of where this occurs when a bipedal robot performs a jump over a large block. In this scenario, the robot walks up to the block using a walking policy and then performs a jump with a terrain-specific target policy, where the behaviour involves jumping with both feet. Fig~\ref{fig:fig1} shows that the trajectory of the walk policy does not intersect with the trajectory of the target policy, therefore we require an intermediate policy. Our agent has 12 torque controlled actuators, simulated in Pybullet~\cite{coumans_pybullet_2020}. 

We select which terrain module to employ using an oracle terrain classifier (Fig~\ref{fig:fig2}a). From a default walking policy, we utilise a Setup Policy that prepares the robot for the Target Policy (Fig~\ref{fig:fig2}b)). When to switch from the Setup Policy to the Target Policy is also a learned output of the Setup Policy. We first study the traversal of a single difficult terrain artifact that requires walking on a flat surface and performing a jump. We then consider several diverse terrain types (gaps, hurdles, stairs, and steps). The state provided to each policy is $s_t=[rs_t, I_t]$, where $rs_{t}$ is the robot state and $I_t$ is the perception input at time $t$. 

\noindent\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}, s_{right}, s_{left} ]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot, respectively (four Boolean contact points per foot), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the body Centre of Mass (CoM), $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the CoM and $h_{CoM,t}$ is the height of the robot from the walking surface. $s_{right}$ and $s_{left}$ are Boolean indicators of which foot is in the swing phase, and is updated when the current swing foot makes contact with the ground. All angles except joint angles are represented in the world coordinate frame. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\noindent\textbf{Perception}: Perception is a depth sensor mounted to the robot base, with a resolution of $[48,48,1]$. Each pixel is a continuous value scaled between $0-1$, measuring a distance between 0.25 and $\SI{2}{\metre}$ from the robot base. The sensor moves with the body in translation and yaw, we provide an artificial gimbal to keep the sensor fixed in roll and pitch. The sensor is pointed at the robot's feet (the feet are visible) and covers at least two steps in front of the robot~\cite{zaytsev_two_2015}. We reduce the sampling rate of the perception to $\SI{20}{\hertz}$ (reducing computational complexity), where the simulator operates at $\SI{120}{\hertz}$.

\subsection{Deep Reinforcement Learning for Continuous Control}
\label{sec:ppo}
 
We consider our task to be a Markov Decision Process $\text{MDP}$, defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. 

The goal of reinforcement learning is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. Actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is a torque applied to each joint. Each policy is trained with Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. We use the implementation of PPO from OpenAI Baselines~\cite{dhariwal_openai_2017}.

% We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

% We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[-\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse reduce its probability.

% In practice this loss can be noisy, and result in large updates to the policy. Insteasd we use Proximal Policy Optimisation~\cite{schulman_proximal_2017}, which uses a surrogate loss that is clipped, preventing policy updates that are too large. We also use Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}. 


\subsection{Training Setup Policies}
\label{sec:setup}

For each target terrain type we train a Setup Policy with the purpose of bridging the trajectories of a default walking policy and the policy for the upcoming terrain condition. The algorithm for training each Setup Policy is shown in Algorithm~\ref{alg:setup}. 

\textbf{Default Policy}: 
The Default Policy is a pre-trained policy designed to walk on a flat surface. When training a Setup Policy we always begin with the Default Policy until the terrain artifact is detected by an oracle. Once the terrain has been traversed, we switch back to the Default Policy when a termination criteria is reached ($\tau_\theta$, defined below). We initialise the Setup Policy from the default walking policy such that the robot continues to walk towards the terrain artifact while learning how to setup the target policy.

\textbf{Setup Policy}: 
When terrain type $i$ is detected, we switch immediately from the Default Policy to the Setup Policy for terrain type $i$, denoted as $\pi_\phi^i$. While training we are given access to an oracle terrain detector that indicates when the robot is a fixed distance from the terrain artifact. The Setup Policy outputs joint torques $a_i$, and switch condition $\tau_\phi$. If the switch condition is met, we immediately switch to the Target Policy.

\textbf{Target Policy}: 
The Target Policy for terrain type $i$, denoted as $\pi_\theta^i$, is trained with curriculum learning following the method outlined in our previous work~\cite{tidd_guided_2020}. We also define a termination condition $\tau_\theta$ that denotes switching from the Target Policy back to the Default Policy. For the the termination condition to be reached the robot must be have successfully traversed the terrain artifact, have both feet in contact with the ground plane, and a positive forward velocity $vx$. This condition is the same for all artifact types.

\textbf{Setup Policy Reward}: 
We design a reward function to motivate the Setup Policy to transition the robot from states visited by the Default Policy to states required by the Target Policy. We note the value function of the Target Policy, $\hat{V}(s_t) = \sum_{t=0}^{T}\gamma^tr_t$, (where $r_t$ is the original reward afforded by the environment for the Target Policy), provides an estimate of what return we can expect if we run the Target Policy from $s_t$. However, value functions are notoriously over optimistic for states that have not been visited~\cite{haarnoja_soft_2018} (such as those we might experience by running the Default Policy).

We observe the advantage is a zero centered estimate of the effect of running action $a_t\sim\pi_\theta^i (s_t)$, given by the advantage for the Target Policy:

\begin{equation}
    \hat{A}(s_t, a_t) = r_t + \gamma\hat{V}(s_{t+1)} - \hat{V}(s_t)
\end{equation}

where $r_t$ is the Target Policy reward. (details can be found in our previous work~\cite{tidd_guided_2020}).

Using advantage $\hat{A}(s_t, a_t)$ as a confidence for the accuracy of $\hat{V}(s_t)$, we define the reward from the \textbf{Advantage Weighted Target Value}:
\begin{equation}
    \hat{r}_t = ( 1 - \text{min}(\alpha\hat{A}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}(s_t)
\end{equation}

Where $\alpha$ and $\beta$ are scaling factors we set to 0.15 and 0.01 respectively. Intuitively, for states where the Target Policy value function $\hat{V}(s_t)$ is accurate, the Target Policy advantage $\hat{A}$ will be close to zero, thus the Setup Policy will learn to maximise $\hat{V}$. States where $\hat{A}$ is far from zero will reduce the effect of an overconfident $\hat{V}$.

\textbf{Extended Reward}: 
One issue with training Setup Policies is the delayed effect of actions, where once switched to the Target policy, the Setup Policy is no longer acting on the environment or receiving a reward. Once the Setup Policy has transitioned to the Target Policy, we must provide the Setup Policy with information regarding the performance of the robot since switching. Our method for solving this problem is to provide the additional reward obtained \textit{after} switching, by including an extended reward in the rollout buffer of the Setup Policy. We add this extended reward to the last element of the Setup Policy buffer: 
\begin{equation}
    % \text{Buffer}[\hat{r}][-1] \mathrel{+}= \hat{r}_t    
    \hat{r}_{final} = \hat{r}_{final} + \hat{r}_t 
\end{equation}
where $\hat{r}_{final}$ is the final reward entry received by the Setup Policy, and $\hat{r}$ is the reward received at time $t$, after the Setup Policy has transitioned to the Target Policy. For algorithmic stability, we clear all but the last entry of the buffer after each training update. The procedure for training Setup Policies is provided in Algorithm~\ref{alg:setup}. Note that the termination variable $\tau_t$ (line 7) is either $\tau_\phi$ if the Current Policy is the Setup Policy, or $\tau_\theta$ if the Current Policy is the Target Policy.

\begin{algorithm}
	\caption{Setup Before Switching} 
	\begin{algorithmic}[1]
      \State Load Target Policy. Load Default Policy
      \State Initialise Setup Policy from Default Policy
      \State Initialise Buffer
        \State Current Policy $\gets$ Default Policy
		\For {$iteration=1,2,\ldots$}
		    \While {not $done$}
    		    \State $a_t, \tau_t \sim $ Current Policy$(s_t)$ 
    		  %  \State ($\tau_t = \tau_\theta || \tau_\phi$)
    		    %\Comment{$\tau_\theta$ if Current Policy == }
    		    \State $s_{t+1}, r_t, done = env.step(a_t)$
    		    \If{Terrain detected}
    	            \State $\hat{A}(s_t, a_t) = r_t + \gamma\hat{V}(s_{t+1}) - \hat{V}(s_t)$
        		    \State $\hat{r}_t = (1 - \alpha\hat{A}(s_t, a_t)^2)\cdot \beta\hat{V}(s_t)$
        		    \If{Current Policy == Default Policy}
        		        \State Current Policy $\gets$ Setup Policy 
            		\ElsIf{Current Policy == Setup Policy}
        		        \State Store $s_t$, $a_t$, $\hat{r}_t$, $\tau_\phi$ into Buffer
                        \If{Buffer Full}
                            \State PPO Training Update
                            \State Clear buffer (except last entry)
                        \EndIf
            		    \If {$\tau_\phi$}
            		        \State Current Policy $\gets$ Target Policy 
            		    \EndIf
        			\ElsIf{$\tau_\theta$}
        			    \State Current Policy $\gets$ Default Policy
        		    \EndIf
        		    \If{Current Policy != Setup Policy}
        			 %   \State Buffer$[\hat{r}][-1] \mathrel{+}= \hat{r}_t$
        			    \State $\hat{r}_{final} = \hat{r}_{final} + \hat{r}_t$ 
        			\EndIf
        		\EndIf
        		\State $s_t = s_{t+1}$
        	\EndWhile
		\EndFor
	\end{algorithmic} 
\label{alg:setup}
\end{algorithm}

% \subsection{Terrain Classification}
% \label{sec:classifier}

% Classifier Network \textbf{TBD}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

We evaluate our method with a biped in simulation. Initial evaluations are performed with a single difficult terrain (Sec~\ref{sec:ablation}, Sec~\ref{sec:reward_choice}, Sec~\ref{sec:comparisons}), before adding more behaviours in Sec~\ref{sec:multi_terrain}. The difficult terrain is a sample of flat terrain with a single block 70cm high, and 30cm in length (in the forward direction of the robot), an example is shown in Fig.~\ref{fig:fig1}. We perform training and evaluation on a single terrain sample, starting the robot from a random $x$ (forward direction) uniformly sampled from $(0.0, 2.2)\si{\meter}$ before the terrain artifact, $y$ (strafe) uniformly sampled from $(-0.6, 0.6)\si{\meter}$, and heading (yaw) uniformly sampled from $(-0.3, 0.3)\si{\radian}$. All experiments are evaluated by pausing training and performing 100 evaluation runs, and recording both the Success percentage and Distance percentage. Success \% is defined as the average success rate to reach a goal location several meters past the terrain artifact. Distance \% is the percentage of total distance the agent successfully traversed of the terrain.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effect of Using Initialisation and Extended Reward}
\label{sec:ablation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We perform an ablation to study the effect of initialising the Setup Policy from the walking policy, and the effect of extending the reward after the Setup Policy has transitioned to the Target Policy. In all experiments the Default Policy is used until the terrain is detected, then the Setup Policy is activated until the termination signal $\tau_\phi$ indicates switching to the Target Policy, and $\tau_\theta$ then results in switching back to the Default Policy.

\begin{itemize}[leftmargin=*]

\item\textbf{Without Initialisation:} We evaluate our method without initialising the Setup Policy from the Default Walk Policy, i.e. the Setup Policy is randomly initialised.

\item\textbf{Without Extended Reward:} We evaluate our method without including reward after the Setup Policy has switched to the Target Policy. 

\item\textbf{Full Method:} Our method uses a Setup Policy initialised from the Default Walk Policy, and receives reward signal after the Setup Policy has transitioned to the Target Policy. 

\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Initialisation        & 38.8      & 73.2  \\
        Without Extended Reward       & 12.3      & 58.3  \\
        Full Method                          & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study for Initialising from Walk Policy and Extended Rewards, on a single jump terrain sample.}
    \label{tab:results}
\end{table}

We can see that initialising the Setup Policy with the default walking policy and extending the reward improves learning outcomes as shown in Table~\ref{tab:results}, where our method achieves 82.2\% success compared to 38.8\% (without initialisation from the default walking policy) and 12.3\% (without extended reward). It is worth noting that training without initialisation from the walking policy required many more training steps to reach an asymptotic result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setup Policy Reward Choice}
\label{sec:reward_choice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For training the setup policy, we investigate several options for the reward provided at each timestep. For each reward type we evaluate with three different random seeds, results are shown in Fig~\ref{fig:results}.

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=\columnwidth]{images/ch5/results.png}
\hfill
\caption{We investigate several options for the reward function used by the Setup Policy on the difficult jump terrain. We show the percentage of successful runs (robot reaches several meters after the jump) from three different random seeds.}
\label{fig:results}
% \vspace{-3mm}
\end{figure}

\begin{itemize}[leftmargin=*]
\item\textbf{Original:} The reward the same that is used to train the Target Policy (See~\cite{tidd_guided_2020} for details of the reward function). 

\item\textbf{Constant:} At each timestep a constant reward of 1.5 is given.

\item\textbf{Target Torque:} We match the output of the Target Policy torque by minimising the error between the Setup Policy and the Target Policy: $\exp[-2.0\cdot (\pi_\phi(s_t) - \pi_\theta(s_t))^2]$.

\item\textbf{Target Value:} We evaluate the effect of maximising the Target Policy value function $\beta\hat{V}(s_t)$, where $\beta$ is scaling factor 0.01.

\item\textbf{Advantage Weighted Target Value:} We evaluate the reward based on the Target Policy advantage $\hat{A}$ and value function $\hat{V}$: $( 1 - \text{min}(\alpha\hat{A}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}(s_t)$, where $\alpha$ and $\beta$ are scaling factors 0.15 and 0.01 respectively.

\end{itemize}

It can be seen from Fig~\ref{fig:results} that a reward using \textbf{Advantage Weighted Target Value} performs better than other reward choices, achieving the highest average success rate (78.7\%). Using the Target Value reaches a success rate of 63.9\%. This disparity, and the large variation in the Target Value (green line), shows the effect of over estimation bias often seen with value functions, validating our idea that weighting the value by the advantage reduces the affect of this bias when training Setup Policies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparisons}
\label{sec:comparisons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We compare our method for training Setup Policies with several other methods, including end to end methods, without using Setup Policies, and a method that learns a proximity prediction~\cite{lee_composing_2019}.

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success\% & Distance\% \\
       \hline
        Single Policy                 & 0.0           & 11.3  \\
        Single Policy With Curriculum & 0.0           &  3.8 \\
        No Setup Policy               & 1.5           & 51.3 \\
        Learn When to Switch          & 0.0           & 44.2  \\
        Proximity Prediction         & 51.3           & 82.4 \\
        Setup Policy (Ours)                         & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{}
    \label{tab:results_compare}
\end{table}

\begin{itemize}[leftmargin=*]

\begin{figure*}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth]{images/ch5/Fig1_2.png}
\includegraphics[width=\textwidth]{images/ch5/all.png}
\hfill
\caption{Setup policies allow us to transition between behaviours to traverse several complex terrains.}
\label{fig:multi}
% \vspace{-3mm}
\end{figure*}

\item\textbf{Single Policy:} We train a single end to end policy on the terrain sample.

\item\textbf{Single Policy With Curriculum:} We utilise curriculum learning to train a single end to end policy on the terrain sample (using the method defined in~\cite{tidd_guided_2020}).

\item\textbf{No Setup Policy:} We switch to the Target Policy from the Default Policy as soon as the terrain oracle detects the next terrain.

\item\textbf{Learn When to Switch:} We collect data by switching from the Default Policy to the Target Policy at random distances from the Jump. We use supervised learning to learn when the robot is in an suitable state to switch. Details of this method is found in our previous work~\cite{tidd_learning_2020}.

\item\textbf{Proximity Prediction:} We follow the method defined by Lee et al~\cite{lee_composing_2019} to train Setup Policies using a proximity predictor function $P(s_t)$. $P(s_t)$ outputs a continuous value that indicates how close the agent is to a configuration that resulted in successful traversal. $P_(s_t)$ is trained using supervised learning from success and failure buffers. The reward used to train the Setup Policy is the dense reward created by  $P(s_{t+1}) - P(s_{t})$, encouraging the agent to move closer to a successful switching configuration. For accurate comparison we initialise the transition policy with weights from the walk policy.

\item\textbf{Setup Policy (Ours):} We follow Algorithm~\ref{alg:setup} to train Setup Policies. 

\end{itemize}

We can see from Table~\ref{tab:results_compare} that our method for developing Setup Policies performs the best (82.2\% success rate), compared to other methods. A single policy was unable to traverse the difficult jump terrain, even after an extended learning time and with curriculum learning. We show that Setup Policies are necessary for this problem, with \textbf{No Setup Policy} unable to successfully traverse the terrain (1.5\% success). \textbf{Learning When to Switch} also performed poorly as there are very few states that overlap between the Default Policy and the Target Policy for the switch estimator to learn. The \textbf{Proximity Prediction} method was able to successfully traverse the jump 51.3\% of the time. It is worth noting that this method required approximately three times more training episodes than our method to reach the provided results, despite also being initialised from the Default Policy.

These experiments show that for the difficult jump terrain, we require a specialised Target Policy dedicated to learning the complex jumping behaviour. We show that this specialised policy has a trajectory that does not overlap with the Default Policy, and thus Setup Policies are required. Our method for learning a Setup Policy method achieves the highest performance on this difficult task.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Multiple Terrain Types}
\label{sec:multi_terrain}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


For our final experiment we train Setup Policies for several additional terrain types. In total we now have modules for Jumps, Gaps, Hurdles, Stairs, and Steps. Fig~\ref{fig:multi} shows a sequence with each terrain type. We follow the pipeline shown in Fig~\ref{fig:fig2}a), where a terrain oracle determines which module should be selected. On selection, the Setup Policy is employed until it determines when to switch to the Target Policy.
Termination criteria $\tau_\theta$ (introduced in Sec~\ref{sec:method}) determines when to switch back to the Default Policy for the Jump Policy only. All other policies resemble the behaviour of the Default Policy on flat terrain, i.e. we continue using the Target Policy after the terrain has been traversed for Gaps, Hurdles, Stairs, and Steps, until the oracle determines the terrain has changed.

We evaluate with 7 randomly selected terrains types in sequence. We perform 500 runs, with a total of 3500 various terrain types to be traversed. In Table~\ref{tab:multi_results} we show the percentage of total distance travelled and success rate with and without using Setup Policies. A successful run in this scenario is defined as reaching the last terrain in the sequence. Table~\ref{tab:multi_breakdown} shows the individual performance of the agent for each terrain type (number of successful traversals / total traversals).

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.71\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Setup Policies        & 6.5      & 32.9  \\
        With Setup Policies       & \textbf{29.1}      & \textbf{62.8}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success rate and percent total distance travelled for 500 episodes of 7 randomly selected terrain types.}
    \label{tab:multi_results}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{min width=0.95\columnwidth}
    \begin{tabular}{cccccc}
                                      & Jump & Gap & Hurdle & Stairs & Steps \\
      \hline
        Without Setup Policies       & 5.8\%      & 88.8\%  & 89.3\% &  96.3\% & 83.9\%  \\
        With Setup Policies        & \textbf{67.7\%}      & \textbf{93.0\%}  & \textbf{91.3\%} &  \textbf{97.1\%} & \textbf{88.8\%}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Percent of successful traversals for each terrain type from 500 episodes of 7 randomly selected terrain types.}
    \label{tab:multi_breakdown}
\end{table}

We can see from these results that Setup Policies improve the success rate compared to switching policies without this intermediate policy (29.1\% success compared to 6.5\%). From Table~\ref{tab:multi_results} we can see that Setup Policies are most critical for traversing the difficult Jump terrain (67.7\% compared with 5.8\%), though show improvements for all terrain types. There is a clear room for improvement for the Jump terrain. We attribute this low success rate (67.6\% compared to the single Jump terrain success rate of 82.2\%) to out of distribution states, i.e. the robot visits states in the terrain sequence that it does not experience when training the Setup Policy. Training Setup Policies for wider range of states will be investigated in future work. 

% It is worth mentioning that while we evaluate the success rate of individual terrains in Table~\ref{tab:multi_breakdown}, we show the success rate of traversing all 7 terrains in sequence in Table~\ref{tab:multi_results}, which should explain the lower success rate figure. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

It is common practice for legged robots to have separate locomotion policies to traverse different terrain conditions. We propose Setup Policies that allows smooth transition from one locomotion policy to a target policy for a dynamic biped. We use deep reinforcement learning to learn the Setup Policies for which we introduce a novel reward based on the Advantage Weighted Target Value, utilising the value prediction of the Target Policy in the reward for the Setup Policy. 

In simulation experiments for transitioning from a Walking policy to a Jumping policy, we show using an in-between Setup Policy yields a higher success rate compared to using a single policy (0$\%$ success rate), or the two policies without the Setup Policy (from 1.5$\%$ success rate without Setup Policies to 82$\%$). We further show that our method is scalable to other terrain types, and demonstrate the effectiveness of the approach on a sequence of difficult terrain conditions, improving the success rate from 6.5$\%$ without Setup Policies to 29.1$\%$.

A limitation of our method is that the Setup Policies are trained from a default walking policy. We would like to improve the scope of the Setup Policies such that a wider range of states are funnelled toward the Target Policy. A significant assumption in this work is that we have access to a terrain oracle; removing this dependency will also be investigated in future work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%  However, for complex behaviours, there may not be a RoA overlap.

% For classical methods that rely on the RoA set to be explicitly known, controllers can be composed by funneling one behaviour into the next. This is only possible when the set of states visited by an agent when a controller is running nominally (the goal set) of one behaviour exists in the RoA of the next [\cite{burridge_sequential_1999}].

% if an active controller cannot behave nominally from the current state. 
% preparing an agent for an upcoming behaviour such that safe switching can occur. 

% These scenarios can prevent the robot from reliably reaching a safe switch state, t
% Not only is there a risk of instability when switching without RoA overlap, it is also possible that only part of a behaviours goal set exists in the RoA of the next behaviour. This situation creates a partial, or incomplete RoA overlap, and can occur with periodic behaviours such as walking, or factors external to the robot such as obstacle proximity and can prevent the robot from reaching an overlapping state.


% This leaves a partial, or incomplete RoA overlap, where reliable switching is difficult. 

% This chapter is motivated by situations when such a state cannot be reached reliably.

% means there are states from one behaviour that will take the robot out of the RoA for the next. This is defined here as a partial, or incomplete 

% Previous definitions of RoA 


% Region of attraction (RoA) refers to the set of states, from any of which a controller will converge to its nominal behaviour given time. For a switch location to exist between two controllers, there must be common states in the RoA set of each controller. If a common state does not exist, or a controller does not have enough time. This chapter considers these issues.

% This could go somewhere 
% Behaviours may also have partial, or incomplete overlap, where some of the states in the goal set exist in the RoA of the next controller, but not all. This can be predicated on terrain, or periodic behaviours. 



% This is how we answer RQ2 and 3. 



% The method uses policies initialised from a default policy (a walking controller), a novel reward that guides the robot toward the target behaviour, and an extended reward that provides training signal after switching occurs.

% that estimates how well the robot will perform compared to the target behaviour. The  uses  Figure  shows the performance of several alternative reward functions. From the low variance performance of this and to minimise over estimation bias from the target value function. 




% \textbf{\textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}}

% \textbf{\textit{How can the reliability of switching between complex behaviours be improved?}}


% For behaviours that are have few or no overlapping states, we train Setup Policies enable to the robot to transition between the trajectory of the current policy, and the trajectory of the Target Policy (Fig.~\ref{fig:cha4_setup_fig1}). Instead of a Switch Estimator, the Setup Policy also determines when we should switch to the Target Policy. Fig.~\ref{fig:cha4_setup_fig2}.a) shows the pipeline where a module is selected based on the current terrain. The selected module, (Fig.~\ref{fig:cha4_setup_fig2}.b), will first use the Setup Policy, then switch to the Target Policy when the robot is in a suitable state determined by the Setup Policy. We test our approach on a difficult jump behaviour, as shown in Fig.~\ref{fig:cha4_setup_fig1}, that requires the robot to jump with both feet to land on top of the 70cm obstacle.

% Setup Policies are initialised from a walking policy. We use an extended reward that considers the reward obtained from the moment a Setup Policy is activated, and the reward obtained after switching to the Target Policy.  Table. \ref{tab:ch4b_results} shows that Setup Policies require both of these features. 


% \begin{table}[h!]
%     % \vspace{-2mm}
%     \centering
%     % \begin{tabular}{c|c|c|c|c|c}
%     % \begin{adjustbox}{max width=1.0\columnwidth}
%     % \begin{adjustbox}{min width=0.8\columnwidth}
%     \begin{tabular}{cccccc}
%         % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
%                                       & Success \% & Distance \% \\
%       \hline
%         Without Initialisation        & 38.8      & 73.2  \\
%         Without Extended Reward       & 12.3      & 58.3  \\
%         Full Method                          & \textbf{82.2} & \textbf{96.1}\\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{The effect of initialising from walking policy, and considering the reward after switching to the Target Policy.}
%     \label{tab:ch4b_results}
% \end{table}




% Fig. \ref{fig:ch4b_results} shows the effect of various reward functions on Setup Policy learning. The best reward was constructed by scaling the value estimate of the Target Policy by the advantage in the current state. The value function of the Target Policy is an estimate of the sum of future rewards for running policy $\pi_j$: $\hat{V}^{\pi_j}(s_t) = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is the reward afforded by the environment at time $t$. Remembering that the advantage is a zero centered estimate of the effect of running action $a_t\sim\pi_\theta (s_t)$:

% \begin{equation}
%     \hat{A}^{\pi_j}(s_t, a_t) = r_t + \gamma\hat{V}^{\pi_j}(s_{t+1)} - \hat{V}^{\pi_j}(s_t)
% \end{equation}

% We note the value function of the Target Policy, $\hat{V}(s_t) = \sum_{t=0}^{T}\gamma^tr_t$, (where $r_t$ is the original reward afforded by the environment for the Target Policy), provides an estimate of what return we can expect if we run the Target Policy from $s_t$. However, value functions are notoriously over optimistic for states that have not been visited~\cite{haarnoja_soft_2018} (such as those we might experience by running the Default Policy).

% Using advantage $\hat{A}^{\pi_j}(s_t, a_t)$ as a confidence for the accuracy of $\hat{V}^{\pi_j}(s_t)$, we define the reward \textbf{Advantage Weighted Target Value} used for training the Setup Policy for Target Policy $\pi_j$:

% \begin{equation}
%     \hat{r}_t = ( 1 - \text{min}(\alpha\hat{A}^{\pi_j}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}^{\pi_j}(s_t)
% \label{eq:ch4_setup}
% \end{equation}

% where $\alpha$ and $\beta$ are scaling factors are tuned empirically (set to 0.15 and 0.01 respectively). 

% Table \ref{tab:ch4b_results_compare} shows the comparison of our Setup Policy method with several other methods for switching or learning transition policies. Importantly, for the complex jump behaviour, learning when to switch is not enough to successfully transition between walking and jumping. Finally, Table \ref{tab:ch4b_multi_results} shows that Setup Policies are required for traversing a sequence of complex obstacles, and Table \ref{tab:ch4b_multi_breakdown} shows which terrain types contributed most to failure.

% Using Setup Policies, we are able to traverse a complex sequence of terrain obstacles (Fig.~\ref{fig:cha4_setup_fig3}), where sequential behaviours do not necessarily have an overlapping RoA.



% \begin{table}[h!]
%     % \vspace{-2mm}
%     \centering
%     % \begin{adjustbox}{min width=0.95\columnwidth}
%     \begin{tabular}{cccccc}
%                                       & Jump & Gap & Hurdle & Stairs & Steps \\
%       \hline
%         Without Setup Policies       & 710      & 90  & \textbf{43} &  \textbf{20} & \textbf{90}  \\
%         With Setup Policies        & \textbf{420}      & \textbf{70}  & 73 & 36 & 144 \\
%     \hline
%     \end{tabular}
%     % \end{adjustbox}
%     \caption{Number of failures by terrain type from 1000 episodes of 7 randomly selected terrain types.}
%     \label{tab:ch4b_multi_breakdown}
% \end{table}


% =======================================================================
% -----------------------------------------------------------------------
% =======================================================================

% \item We develop a Setup Policy that significantly improves the success rate from transitioning from a default walking policy to a Target Policy (from 1.5\% success rate without Setup Policies to 82\% for a difficult 70cm jump). The setup policy also learns when to switch to the target policy
    % \item We introduce a novel reward, called Advantage Weighted Target Value, based on the performance of the Target Policy
    % \item We show that we can use our Setup Policies with several difficult  terrain types, allowing for a modular control suite by combining policies that have been trained separately
    
% The behaviour switch methods discussed in Chapter \ref{cha:ch3b} and \ref{cha:ch4} required access to all behaviours during training or data collection. 


==> old/Ch5_mono.tex <==
\chapter[Learning Setup Policies]{Learning Setup Policies: Reliable Transition Between Locomotion Behaviours}

% \item \textbf{Research Question 3: \textit{How can an agent prepare to activate a desired behaviour when there is no suitable switch location?}}

% Extended abstract

\label{cha:ch5}
% =======================================================
% -------------------------------------------------------
% =======================================================
% {How can an agent prepare for an upcoming behaviour such that safe switching can occur?}}
Chapter \ref{cha:ch4} investigated a method for determining a switch location for sequential behaviours, this chapter considers preparing an agent for an upcoming behaviour such that safe switching can occur. Dynamic behaviours are particularly sensitive to instability if an active controller cannot behave nominally from the current state. For classical methods that rely on the RoA set to be explicitly understood, controllers can be composed by funneling one behaviour into the next. This is possible when the set of states visited by an agent when a controller is running nominally (the goal set) of one behaviour exists in the RoA of the next [\cite{burridge_sequential_1999}]. However, for complex behaviours, there may not be a RoA overlap. Furthermore, periodic behaviours such as walking, or the proximity of the robot to an obstacle may result in a partial, or incomplete overlap, preventing the timely activation of the target behaviour. Transitioning between behaviours despite these limitations is investigated in this chapter.

% These scenarios can prevent the robot from reliably reaching a safe switch state, t
% Not only is there a risk of instability when switching without RoA overlap, it is also possible that only part of a behaviours goal set exists in the RoA of the next behaviour. This situation creates a partial, or incomplete RoA overlap, and can occur with periodic behaviours such as walking, or factors external to the robot such as obstacle proximity and can prevent the robot from reaching an overlapping state.


% This leaves a partial, or incomplete RoA overlap, where reliable switching is difficult. 

% This chapter is motivated by situations when such a state cannot be reached reliably.

% means there are states from one behaviour that will take the robot out of the RoA for the next. This is defined here as a partial, or incomplete 

% Previous definitions of RoA 


% Region of attraction (RoA) refers to the set of states, from any of which a controller will converge to its nominal behaviour given time. For a switch location to exist between two controllers, there must be common states in the RoA set of each controller. If a common state does not exist, or a controller does not have enough time. This chapter considers these issues.

% This could go somewhere 
% Behaviours may also have partial, or incomplete overlap, where some of the states in the goal set exist in the RoA of the next controller, but not all. This can be predicated on terrain, or periodic behaviours. 

    
\begin{figure}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=0.8\columnwidth]{images/ch5/ch5/Fig1.png}
\hfill
\caption{A Setup Policy allows the robot to transition from the trajectory of policy $i$ to the trajectory of the Target Policy $j$.}
\label{fig:cha4_setup_fig1}
% \vspace{-3mm}
\end{figure}


This chapter further explores research question 2, learning how to reliably switch behaviours, and investigates scenarios when a switch location cannot be reached (research question 3). Presented is a method that simultaneously learns when to switch to a target behaviour, while moving the robot into the RoA for this controller. Figure \ref{fig:cha4_setup_fig1} highlights the primary problem investigated in this chapter. The trajectory of one behaviour does not intersect the trajectory of the behaviour that is needed to complete the obstacle. Setup Policies are trained to transition between behaviours by preparing the robot for the upcoming obstacle, and switching when in a state optimised for success. Figure \ref{fig:cha4_setup_fig2} shows the modular system. Figure \ref{fig:cha4_setup_fig2}a) shows the pipeline from robot state and perception input to joint torque using any number of terrain behaviours. Figure \ref{fig:cha4_setup_fig2}b) shows the separate modules containing both the Setup Policy, a switch bit that determines when to switch, and the Target Policy. The contributions to research question 2 include a switch mechanism that is trained simultaneously with a transition policy. Research question 3 is explored by learning how to transition to a behaviour such that safe switching can occur.
% This is how we answer RQ2 and 3. 
\section{Method}
\label{sec:method}

In this section we describe the problem we are solving and our method for training setup policies. 

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\subfloat[]{\includegraphics[width=\columnwidth]{images/ch5/Fig2.png}}
\hfill
\subfloat[]{\includegraphics[width=\columnwidth]{images/ch5/Fig3.png}}
% \hfill
\caption{a) shows the modular pipeline. A terrain classifier selects which module should be utilised, and the torque from the output of the selected module is applied to the robot, returning robot state and depth image. b) Each module is pre-trained on a single terrain type. The Target Policy has been designed to traverse a specific terrain condition. The Setup Policy guides the trajectory of the robot from a default walking controller to the Target Policy, also learning when to switch to the Target Policy.}
\label{fig:ch5_fig2}
% \vspace{-3mm}
\end{figure}

\subsection{Problem Description}
\label{sec:problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We investigate composing controllers for a dynamic platform with little or no state overlap between adjacent behaviours. An example of where this occurs when a bipedal robot performs a jump over a large block. In this scenario, the robot walks up to the block using a walking policy and then performs a jump with a terrain-specific Target Policy, where the behaviour involves jumping with both feet. Fig~\ref{fig:ch5_fig1} shows that the trajectory of the walk policy does not intersect with the trajectory of the Target Policy, therefore we require an intermediate policy. While it may be possible to improve the robustness of the target policies after they have been trained (i.e. to include states visited by the walk policy), we consider the case where target behaviours and value functions are provided as a black box and are therefore immutable. Our agent has 12 torque controlled actuators, simulated in Pybullet~\cite{coumans_pybullet_2020}.

We select which terrain module to employ using an oracle terrain classifier (Fig~\ref{fig:ch5_fig2}a). From a default walking policy, we utilise a Setup Policy that prepares the robot for the Target Policy (Fig~\ref{fig:ch5_fig2}b)). When to switch from the Setup Policy to the Target Policy is also a learned output of the Setup Policy. We first study the traversal of a single difficult terrain artifact that requires walking on a flat surface and performing a jump. We then consider several diverse terrain types (gaps, hurdles, stairs, and steps). The state provided to each policy is $s_t=[rs_t, I_t]$, where $rs_{t}$ is the robot state and $I_t$ is the perception input at time $t$. 

\noindent\textbf{Robot state}: $rs_t=[J_t, Jv_t, c_t, c_{t-1}, v_{CoM,t}, \omega_{CoM,t}, \\ \theta_{CoM,t}, \phi_{CoM,t}, h_{CoM,t}, s_{right}, s_{left} ]$, where $J_t$ are the joint positions in radians, $Jv_t$ are the joint velocities in rad/s, $c_t$ and $c_{t-1}$ are the current and previous contact information of each foot, respectively (four Boolean contact points per foot), $v_{CoM,t}$ and $\omega_{CoM,t}$ are the linear and angular velocities of the body Centre of Mass (CoM), $\theta_{CoM,t}$ and $\phi_{CoM,t}$ are the pitch and roll angles of the CoM and $h_{CoM,t}$ is the height of the robot from the walking surface. $s_{right}$ and $s_{left}$ are Boolean indicators of which foot is in the swing phase, and is updated when the current swing foot makes contact with the ground. All angles except joint angles are represented in the world coordinate frame. In total there are $51$ elements to the robot state, which is normalised by subtracting the mean and dividing by the standard deviation for each variable (statistics are collected as an aggregate during training).

\noindent\textbf{Perception}: Perception is a depth sensor mounted to the robot base, with a resolution of $[48,48,1]$. Each pixel is a continuous value scaled between $0-1$, measuring a distance between 0.25 and $\SI{2}{\metre}$ from the robot base. The sensor moves with the body in translation and yaw, we provide an artificial gimbal to keep the sensor fixed in roll and pitch. The sensor is pointed at the robot's feet (the feet are visible) and covers at least two steps in front of the robot~\cite{zaytsev_two_2015}. We reduce the sampling rate of the perception to $\SI{20}{\hertz}$ (reducing computational complexity), where the simulator operates at $\SI{120}{\hertz}$.

\subsection{Deep Reinforcement Learning for Continuous Control}
\label{sec:ppo}
 
We consider our task to be a Markov Decision Process $\text{MDP}$, defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. 

The goal of reinforcement learning is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is provided by the environment at time $t$. Actions are sampled from a deep neural network policy $a_t\sim\pi_\theta(s_t)$, where $a_t$ is a torque applied to each joint. Each policy is trained with Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}. We use the implementation of PPO from OpenAI Baselines~\cite{dhariwal_openai_2017}.

% We predict the value of being in each state $V(s_t) = r_t + \gamma V(s_{t+1})$, which is an estimate of the sum of future rewards $R$. We calculate an advantage from this prediction $A(s_t) = r_t + \gamma V(s_{t+1}) - V(s_t)$ that provides an estimate of how much better or worse action $a_t$ performed compared to what we expected. 

% We update the policy $\pi(a_t|s_t)$ by scaling the log probability of taking action $a_t$ by the advantage $A(s_t)$ according to the loss function: $L(\theta) = \mathbb{E}[-\log\pi_\theta(a|s)A(s)]$, where $\theta$ is the policy weights. Intuitively, if we did better than expected we want to increase the probability of performing that action next time, and if we did worse reduce its probability.

% In practice this loss can be noisy, and result in large updates to the policy. Insteasd we use Proximal Policy Optimisation~\cite{schulman_proximal_2017}, which uses a surrogate loss that is clipped, preventing policy updates that are too large. We also use Generalised Advantage Estimation (GAE) as a low variance estimate of $A$~\cite{schulman_high-dimensional_2018}. 


\subsection{Training Setup Policies}
\label{sec:setup}

For each target terrain type we train a Setup Policy with the purpose of bridging the trajectories of a default walking policy and the policy for the upcoming terrain condition. The algorithm for training each Setup Policy is shown in Algorithm~\ref{alg:setup}. 

\textbf{Default Policy}: 
The Default Policy is a pre-trained policy designed to walk on a flat surface. When training a Setup Policy we always begin with the Default Policy until the terrain artifact is detected by an oracle. Once the terrain has been traversed, we switch back to the Default Policy when a termination criteria is reached ($\tau_\theta$, defined below). We initialise the Setup Policy from the default walking policy such that the robot continues to walk towards the obstacle while learning how to prepare for the Target Policy.

\textbf{Setup Policy}: 
When terrain type $i$ is detected, we switch immediately from the Default Policy to the Setup Policy for terrain type $i$, denoted as $\pi_\phi^i$. While training we are given access to an oracle terrain detector that indicates when the robot is a fixed distance from the terrain artifact. The Setup Policy outputs joint torques $a_i$, and switch condition $\tau_\phi$. If the switch condition is met, we immediately switch to the Target Policy.

\textbf{Target Policy}: 
The Target Policy for terrain type $i$, denoted as $\pi_\theta^i$, is trained with curriculum learning following the method outlined in our previous work~\cite{tidd_guided_2020}. We also define a termination condition $\tau_\theta$ that denotes switching from the Target Policy back to the Default Policy. For the the termination condition to be reached the robot must be have successfully traversed the terrain artifact, have both feet in contact with the ground plane, and a positive forward velocity $vx$. This condition is the same for all artifact types.

\textbf{Setup Policy Reward}: 
We design a reward function to motivate the Setup Policy to transition the robot from states visited by the Default Policy to states required by the Target Policy. We note the value function of the Target Policy, $\hat{V}(s_t) = \sum_{t=0}^{T}\gamma^tr_t$, (where $r_t$ is the original reward afforded by the environment for the Target Policy), provides an estimate of what return we can expect if we run the Target Policy from $s_t$. However, value functions are notoriously over optimistic for states that have not been visited~\cite{haarnoja_soft_2018} (such as those we might experience by running the Default Policy).

The advantage is a zero centered estimate of the effect of running action $a_t\sim\pi_\theta^i (s_t)$, given by the advantage for the Target Policy:

\begin{equation}
    \hat{A}(s_t, a_t) = r_t + \gamma\hat{V}(s_{t+1)} - \hat{V}(s_t)
\end{equation}

where $r_t$ is the Target Policy reward. (details can be found in our previous work~\cite{tidd_guided_2020}).

Using advantage $\hat{A}(s_t, a_t)$ as a confidence for the accuracy of $\hat{V}(s_t)$, we define the reward from the \textbf{Advantage Weighted Target Value}:
\begin{equation}
    \hat{r}_t = ( 1 - \text{min}(\alpha\hat{A}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}(s_t)
\end{equation}

Where $\alpha$ and $\beta$ are scaling factors are tuned empirically (set to 0.15 and 0.01 respectively). 

The Target Policy value function $\hat{V}(s_t)$ has learned the value for states where the Target Policy has collected experience. Outside of these states, for example when the robot is activating a different policy, we expect the reward provided by the environment $r_t$, and the next state $s_{t+1}$ will not be consistent with what is expected by the Target Policy value function. Therefore, the advantage $\hat{A}(s_t, a_t)$ will not be close to zero, and $\hat{r}_t$ becomes small. Intuitively, for states where the Target Policy value function $\hat{V}(s_t)$ is accurate, the Target Policy advantage $\hat{A}$ will be close to zero, thus the Setup Policy will learn to maximise $\hat{V}$. States where $\hat{A}$ is far from zero will reduce the effect of an overconfident $\hat{V}$. 

\textbf{Extended Reward}: 
One issue with training Setup Policies is the delayed effect of actions, where once switched to the Target policy, the Setup Policy is no longer acting on the environment or receiving a reward. Once the Setup Policy has transitioned to the Target Policy, we must provide the Setup Policy with information regarding the performance of the robot since switching. Our method for solving this problem is to provide the additional reward obtained \textit{after} switching, by including an extended reward in the rollout buffer of the Setup Policy. We add this extended reward to the last element of the Setup Policy buffer: 
\begin{equation}
    % \text{Buffer}[\hat{r}][-1] \mathrel{+}= \hat{r}_t    
    \hat{r}_{final} = \hat{r}_{final} + \hat{r}_t 
\end{equation}
where $\hat{r}_{final}$ is the final reward entry received by the Setup Policy, and $\hat{r_t}$ is the reward received at time $t$, after the Setup Policy has transitioned to the Target Policy. For algorithmic stability, we clear all but the last entry of the buffer after each training update. The procedure for training Setup Policies is provided in Algorithm~\ref{alg:setup}. Note that the termination variable $\tau_t$ (line 7) is either $\tau_\phi$ if the Current Policy is the Setup Policy, or $\tau_\theta$ if the Current Policy is the Target Policy.

\begin{algorithm}
	\caption{Setup Before Switching} 
	\begin{algorithmic}[1]
      \State Load Target Policy. Load Default Policy
      \State Initialise Setup Policy from Default Policy
      \State Initialise Buffer
        \State Current Policy $\gets$ Default Policy
		\For {$iteration=1,2,\ldots$}
		    \While {not $done$}
    		    \State $a_t, \tau_t \sim $ Current Policy$(s_t)$ 
    		  %  \State ($\tau_t = \tau_\theta || \tau_\phi$)
    		    %\Comment{$\tau_\theta$ if Current Policy == }
    		    \State $s_{t+1}, r_t, done = env.step(a_t)$
    		    \If{Terrain detected}
    	            \State $\hat{A}(s_t, a_t) = r_t + \gamma\hat{V}(s_{t+1}) - \hat{V}(s_t)$
        		    \State $\hat{r}_t = (1 - \alpha\hat{A}(s_t, a_t)^2)\cdot \beta\hat{V}(s_t)$
        		    \If{Current Policy == Default Policy}
        		        \State Current Policy $\gets$ Setup Policy 
            		\ElsIf{Current Policy == Setup Policy}
        		        \State Store $s_t$, $a_t$, $\hat{r}_t$, $\tau_\phi$ into Buffer
                        \If{Buffer Full}
                            \State PPO Training Update
                            \State Clear buffer (except last entry)
                        \EndIf
            		    \If {$\tau_\phi$}
            		        \State Current Policy $\gets$ Target Policy 
            		    \EndIf
        			\ElsIf{$\tau_\theta$}
        			    \State Current Policy $\gets$ Default Policy
        		    \EndIf
        		    \If{Current Policy != Setup Policy}
        			 %   \State Buffer$[\hat{r}][-1] \mathrel{+}= \hat{r}_t$
        			    \State $\hat{r}_{final} = \hat{r}_{final} + \hat{r}_t$ 
        			\EndIf
        		\EndIf
        		\State $s_t = s_{t+1}$
        	\EndWhile
		\EndFor
	\end{algorithmic} 
\label{alg:setup}
\end{algorithm}

% \subsection{Terrain Classification}
% \label{sec:classifier}

% Classifier Network \textbf{TBD}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

We evaluate our method with a biped in simulation. Initial evaluations are performed with a single difficult terrain (Sec~\ref{sec:ablation}, Sec~\ref{sec:reward_choice}, Sec~\ref{sec:comparisons}), before adding more behaviours in Sec~\ref{sec:multi_terrain}. The difficult terrain is a sample of flat terrain with a single block 70cm high, and 30cm in length (in the forward direction of the robot), an example is shown in Fig.~\ref{fig:ch5_fig1}. We perform training and evaluation on a single terrain sample, starting the robot from a random $x$ (forward direction) uniformly sampled from $(0.0, 2.2)\si{\meter}$ before the terrain artifact, $y$ (strafe) uniformly sampled from $(-0.6, 0.6)\si{\meter}$, and heading (yaw) uniformly sampled from $(-0.3, 0.3)\si{\radian}$. All experiments are evaluated by pausing training and performing 100 evaluation runs, and recording both the Success percentage and Distance percentage. Success \% is defined as the average success rate to reach a goal location several meters past the terrain artifact. Distance \% is the percentage of total distance the agent successfully traversed of the terrain.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effect of Using Initialisation and Extended Reward}
\label{sec:ablation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We perform an ablation to study the effect of initialising the Setup Policy from the walking policy, and the effect of extending the reward after the Setup Policy has transitioned to the Target Policy. In all experiments the Default Policy is used until the terrain is detected, then the Setup Policy is activated until the termination signal $\tau_\phi$ indicates switching to the Target Policy, and $\tau_\theta$ then results in switching back to the Default Policy.

\begin{itemize}[leftmargin=*]

\item\textbf{Without Initialisation:} We evaluate our method without initialising the Setup Policy from the Default Walk Policy, i.e. the Setup Policy is randomly initialised.

\item\textbf{Without Extended Reward:} We evaluate our method without including the reward after the Setup Policy has switched to the Target Policy. 

\item\textbf{Full Method:} Our method uses a Setup Policy initialised from the Default Walk Policy, and receives reward signal after the Setup Policy has transitioned to the Target Policy. 

\end{itemize}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Initialisation        & 38.8      & 73.2  \\
        Without Extended Reward       & 12.3      & 58.3  \\
        Full Method                          & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study for Initialising from Walk Policy and Extended Rewards, when switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:ch5_results}
\end{table}

We can see that initialising the Setup Policy with the default walking policy and extending the reward improves learning outcomes as shown in Table~\ref{tab:ch5_results}, where our method achieves 82.2\% success compared to 38.8\% (without initialisation from the default walking policy) and 12.3\% (without extended reward). 
% It is worth noting that training without initialisation from the walking policy required many more training steps to reach an asymptotic result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setup Policy Reward Choice}
\label{sec:reward_choice}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For training the setup policy, we investigate several options for the reward provided at each timestep. For each reward type we evaluate with three different random seeds, results are shown in Fig~\ref{fig:ch5_results}.

\begin{figure}[tb!]
% \vspace{2mm}
\centering
\includegraphics[width=\columnwidth]{images/ch5/results.png}
\hfill
\caption{We investigate several options for the reward function used by the Setup Policy on the difficult jump terrain. We show the percentage of successful runs (robot reaches several meters after the jump) from three different random seeds.}
\label{fig:ch5_results}
% \vspace{-3mm}
\end{figure}

\begin{itemize}[leftmargin=*]
\item\textbf{Original:} The reward afforded by the environment that is used to train the Target Policy: the reward encourages following an expert motion (See~\cite{tidd_guided_2020} for details of the reward function). 

\item\textbf{Constant:} At each timestep a constant reward of 1.5 is given.

\item\textbf{Target Torque:} We match the output of the Target Policy torque by minimising the error between the Setup Policy and the Target Policy: $\exp[-2.0\cdot (\pi_\phi(s_t) - \pi_\theta(s_t))^2]$.

\item\textbf{Target Value:} We evaluate the effect of using the Target Policy value function as the reward for the Setup Policy. This is not the same as the original reward, as it is not provided by the environment, but by $\beta\hat{V}(s_t)$, where $\beta$ is scaling factor 0.01.
%  maximising the Target Policy value function 

\item\textbf{Advantage Weighted Target Value:} We evaluate the reward based on the Target Policy advantage $\hat{A}$ and value function $\hat{V}$: $( 1 - \text{min}(\alpha\hat{A}(s_t, a_t)^2,1) ) \cdot \beta\hat{V}(s_t)$, where $\alpha$ and $\beta$ are scaling factors 0.15 and 0.01 respectively.

\end{itemize}

It can be seen from Fig~\ref{fig:ch5_results} that a reward using \textbf{Advantage Weighted Target Value} performs better than other reward choices, achieving the highest average success rate (78.7\%). Using the Target Value reaches a success rate of 63.9\%. This disparity, and the large variation in the Target Value (green line), shows the effect of over estimation bias often seen with value functions, validating our idea that weighting the value by the advantage reduces the effect of this bias when training Setup Policies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparisons}
\label{sec:comparisons}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We compare our method with several others, including end to end methods, without using Setup Policies, and a method that uses proximity prediction to train a Transition Policy~\cite{lee_composing_2019}.

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.8\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success\% & Distance\% \\
       \hline
        Single Policy                 & 0.0           & 11.3  \\
        Single Policy With Curriculum & 0.0           &  3.8 \\
        No Setup Policy               & 1.5           & 51.3 \\
        Learn When to Switch          & 0.0           & 44.2  \\
        Proximity Prediction         & 51.3           & 82.4 \\
        Setup Policy (Ours)         & \textbf{82.2} & \textbf{96.1}\\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success and average distance covered when switching from a walking policy to a jump policy on a single terrain sample.}
    \label{tab:ch5_results_compare}
\end{table}

\begin{itemize}[leftmargin=*]

\begin{figure*}[tb!]
% \vspace{2mm}
\centering
% \includegraphics[width=\columnwidth]{images/ch5/Fig1_2.png}
\includegraphics[width=\textwidth]{images/ch5/all.png}
\hfill
\caption{Setup policies allow us to transition between behaviours to traverse several complex terrains.}
\label{fig:ch5_multi}
% \vspace{-3mm}
\end{figure*}

\item\textbf{Single Policy:} We train a single end to end policy on the terrain sample.

\item\textbf{Single Policy With Curriculum:} We utilise curriculum learning to train a single end to end policy on the terrain sample (using the method defined in~\cite{tidd_guided_2020}).

\item\textbf{No Setup Policy:} We switch to the Target Policy from the Default Policy as soon as the terrain oracle detects the next terrain.

\item\textbf{Learn When to Switch:} We collect data by switching from the Default Policy to the Target Policy at random distances from the Jump. We use supervised learning to learn when the robot is in an suitable state to switch. Details of this method is found in our previous work~\cite{tidd_learning_2021}.

\item\textbf{Proximity Prediction:} We follow the method defined by Lee et al~\cite{lee_composing_2019} to train Transition Policies (one for each behaviour) using a proximity predictor function $P(s_t)$. $P(s_t)$ outputs a continuous value that indicates how close the agent is to a configuration that resulted in successful traversal. $P_(s_t)$ is trained using supervised learning from success and failure buffers. The reward used to train the Transition Policy is the dense reward created by  $P(s_{t+1}) - P(s_{t})$, encouraging the agent to move closer to a successful switching configuration. For accurate comparison we initialise the transition policy with weights from the walk policy, and utilise the terrain oracle for policy selection (the paper refers to a rule-based meta-policy in place of a terrain oracle~\cite{lee_composing_2019}).

\item\textbf{Setup Policy (Ours):} We follow Algorithm~\ref{alg:setup} to train Setup Policies. 

\end{itemize}

We can see from Table~\ref{tab:ch5_results_compare} that our method for developing Setup Policies performs the best (82.2\% success rate), compared to other methods. A single policy was unable to traverse the difficult jump terrain, even after an extended learning time and with curriculum learning. We show that Setup Policies are necessary for this problem, with \textbf{No Setup Policy} unable to successfully traverse the terrain (1.5\% success). \textbf{Learning When to Switch} also performed poorly as there are very few states that overlap between the Default Policy and the Target Policy for the switch estimator to learn. The \textbf{Proximity Prediction} method was able to successfully traverse the jump 51.3\% of the time. It is worth noting that this method required approximately three times more training episodes than our method to reach the provided results, despite also being initialised from the Default Policy.

These experiments show that for the difficult jump terrain, we require a specialised Target Policy dedicated to learning the complex jumping behaviour. We show that this specialised policy has a trajectory that does not overlap with the Default Policy, and thus Setup Policies are required. Our method for learning a Setup Policy method achieves the highest performance on this difficult task.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Multiple Terrain Types}
\label{sec:multi_terrain}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


For our final experiment we train Setup Policies for several additional terrain types. In total we now have modules for jumps, gaps, hurdles, stairs, and steps. Fig~\ref{fig:ch5_multi} shows a sequence with each terrain type. We follow the pipeline shown in Fig~\ref{fig:ch5_fig2}a), where a terrain oracle determines which module should be selected. On selection, the Setup Policy is employed until it determines when to switch to the Target Policy.
Termination criteria $\tau_\theta$ (introduced in Sec~\ref{sec:method}) determines when to switch back to the Default Policy for the Jump Policy only. All other policies resemble the behaviour of the Default Policy on flat terrain, i.e. we continue using the Target Policy after the terrain has been traversed for Gaps, Hurdles, Stairs, and Steps, until the oracle determines the terrain has changed.

We evaluate with 7 randomly selected terrains types in sequence. We perform 1000 runs, with a total of 7000 various terrain types to be traversed. In Table~\ref{tab:ch5_multi_results} we show the percentage of total distance travelled and success rate with and without using Setup Policies. A successful run in this scenario is defined as traversing the last terrain in the sequence. Table~\ref{tab:ch5_multi_breakdown} shows the failure count for each terrain type.
% Table~\ref{tab:ch5_multi_breakdown} shows the individual performance of the agent for each terrain type (number of successful traversals / total traversals).

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    % \begin{tabular}{c|c|c|c|c|c}
    % \begin{adjustbox}{max width=1.0\columnwidth}
    \begin{adjustbox}{min width=0.71\columnwidth}
    \begin{tabular}{cccccc}
        % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                      & Success \% & Distance \% \\
       \hline
        Without Setup Policies        & 6.8      & 37.1  \\
        With Setup Policies       & \textbf{26.4}      & \textbf{53.2}  \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Success rate and percent total distance travelled for 1000 episodes of 7 randomly selected terrain types.}
    \label{tab:ch5_multi_results}
\end{table}

\begin{table}[h!]
    \vspace{-2mm}
    \centering
    \begin{adjustbox}{min width=0.95\columnwidth}
    \begin{tabular}{cccccc}
                                      & Jump & Gap & Hurdle & Stairs & Steps \\
      \hline
        Without Setup Policies       & 710      & 90  & \textbf{43} &  \textbf{20} & \textbf{90}  \\
        With Setup Policies        & \textbf{420}      & \textbf{70}  & 73 & 36 & 144 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Number of failures by terrain type from 1000 episodes of 7 randomly selected terrain types.}
    \label{tab:ch5_multi_breakdown}
\end{table}

We can see from Table~\ref{tab:ch5_multi_results} that Setup Policies improve the success rate compared to switching policies without the intermediate policy (26.4\% success compared to 6.8\%). Table~\ref{tab:ch5_multi_breakdown} provides a breakdown of the number of times the robot failed on each terrain. From Table~\ref{tab:ch5_multi_breakdown} we can see that Setup Policies are most critical for traversing the difficult jump terrain (reducing the failures from 710 to 420), though we also see improvements for gap terrain. These results show the highest failure rate on the multi terrain setup is on the jump terrain, and that there is clear room for improvement on this terrain. While the results show that without setup policies the hurdle, stairs, and steps terrain appear to have less failures than running setup policies, we note that these terrains are visited far less times when running without setup policies due to significant failure with the jumps terrain.

Despite the clear need for Setup Policies, we attribute the relatively low success rate (26.4\%) to out of distribution states, i.e. the robot visits states in the terrain sequence that it does not experience when training the Setup Policy. For example, if the robot was on a gap, and using the gaps behaviour, then switches to the jumps Setup Policy to prepare for an upcoming jump, it will not necessarily be in a state that has been seen during training. Training Setup Policies for wider range of states will be investigated in future work. 



This chapter explored answers to research question 2 and 3. A switch mechanism was learned in conjunction with a Setup Policy that greatly improved the reliability of switching between complex behaviours. Setup Policies are suited for composing behaviour sets where a reliable switch state may not exist between sequential controllers. The contributions of this chapter are listed below. 
\begin{itemize}
    % \item We develop a Setup Policy that significantly improves the success rate from transitioning from a default walking policy to a Target Policy (from 1.5\% success rate without Setup Policies to 82\% for a difficult 70cm jump). The setup policy also learns when to switch to the target policy
    % \item We introduce a novel reward, called Advantage Weighted Target Value, based on the performance of the Target Policy
    % \item We show that we can use our Setup Policies with several difficult  terrain types, allowing for a modular control suite by combining policies that have been trained separately
    \item Setup Policies were developed that demonstrated great improvement in the reliability of transitioning between sequential behaviours, particularly for controllers with incomplete or no RoA overlap
    \item A reward signal was designed for guiding the robot towards a target behaviour for Setup Policies training. By weighting the target policy value function by its advantage, this reward minimised over estimation bias, resulting in the better learning outcomes of transition policies compared to several alternatives
\end{itemize}


“Learning Setup Policies: Reliable Transition Between Locomotion Behaviours” is
under review for the IEEE Robotics and Automation Letters (RA-L). 
\newpage
\newpage


==> old/Ch6.tex <==
% ch6.tex
\chapter[Passing Through Narrow Gaps with Deep Reinforcement Learning]{Passing Through Narrow Gaps with Deep Reinforcement Learning}
\label{cha:ch6}
% Motivation/contribution/abstract -----------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    The DARPA subterranean challenge requires teams of robots to traverse difficult and diverse underground environments. Traversing small gaps is one of the challenging scenarios that robots encounter. Imperfect sensor information makes it difficult for classical navigation methods, where behaviours require significant manual fine tuning. In this paper we present a deep reinforcement learning method for autonomously navigating through small gaps, where contact between the robot and the gap may be required. We first learn a gap behaviour policy to get through small gaps (only centimeters wider than the robot). We then learn a goal-conditioned behaviour selection policy that determines when to activate the gap behaviour policy. We train our policies in simulation and demonstrate their effectiveness with a large tracked robot in simulation and on the real platform. In simulation experiments, our approach achieves 93\% success rate when the gap behaviour is activated manually by an operator, and 67\% with autonomous activation using the behaviour selection policy. In real robot experiments, our approach achieves a success rate of 73\% with manual activation, and 40\% with autonomous behaviour selection. While we show the feasibility of our approach in simulation, the difference in performance between simulated and real world scenarios highlight the difficulty of direct sim-to-real transfer for deep reinforcement learning policies. In both the simulated and real world environments alternative methods were unable to traverse the gap. 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \section{Introduction}
    \label{sec:introduction}
    
    Navigation over various difficult terrain situations requires robust robotic platforms. The DARPA subterranean challenge (SubT)~\cite{darpa_darpa_2021} highlights the need for such platforms in unstructured underground circuits from tunnel, urban, and cave domains. Tracked robotic platforms are capable of navigating rough terrain and are well suited for subterranean search and rescue tasks, particularly where contact with the environment may be required. A number of the SubT scenarios requires the robots to navigate in human environments including small passages and doorways, where significant portions of the course may be obstructed by a narrow bottleneck. Fig.~\ref{fig:fig1} shows examples of narrow gaps which is only centimeters wider than the OzBot BIA5 ATR robot~\cite{bia5_robotic_2021}, which is a large tracked robot. With teleoperation, a strategy often employed for doorways is to approach the gap on a slight angle, making contact with one side of the door, and then turn while pushing through. For autonomous operation, such a behaviour is difficult to derive manually, particularly for robots with imperfect velocity tracking, noisy perception systems and without sensors that can sense contact.
    
    In this paper, we propose a deep reinforcement learning approach to pass through narrow gaps, which is intended to be integrated with a classical behaviour stack. Reinforcement learning methods has lately been used to develop complex navigation behaviours and has improved the performance of navigation robots compared with classically designed controllers~\cite{rana_multiplicative_2020}. Our gap behaviour policy assumes that it is already facing a gap, however, it is also important to know when to activate the gap behaviour, especially when other behaviours (e.g. path following) are used the majority of the time. Integration of a behaviour within a behaviour stack is necessary, though reinforcement learning methods typically act as a black box, with no way to know when a behaviour should be active. Learning when to use the gap behaviour so that it is autonomously activated is an important part of the problem.
    
    % \begin{figure}[tb!]
    % % \vspace{2mm}
    % \centering
    % \includegraphics[width=0.95\columnwidth]{images/ch6/doors2.png}
    % %\hfill
    % \caption{We study the problem of traversing narrow gaps with a mobile robot.}
    % \label{fig:fig1}
    % % \vspace{-3mm}
    % \end{figure}
    
    \begin{figure}[t!]
        % \vspace{2mm}
        \captionsetup[subfigure]{labelformat=empty}
        \centering
        \subfloat[]{\includegraphics[trim=1cm 1cm 1cm 2cm, clip,width=0.45\columnwidth]{images/ch6/real_door4.png}}
        \hfil
        \subfloat[]{\includegraphics[trim=5.0cm 0.0cm 0.2cm 15.3cm, clip, width=0.5\columnwidth]{images/ch6/real_door2.jpg}}
        \hfil
        \vspace*{-3mm}
        % \hfill
        \caption{We study the problem of traversing narrow gaps with a mobile robot.}
        \label{fig:fig1}
        %\vspace{-3mm}
    \end{figure}
    
    Our contributions as follows:
    \begin{itemize}
        \item A gap behaviour policy using deep reinforcement learning for controlling a mobile robot through small gaps
        \item A method to learn when to autonomously activate the gap behaviour policy
        \item Proof-of-concept demonstration of the effectiveness of the approach in simulation and in the real world, using a policy trained only in simulation
    \end{itemize}
    
    
    % Our method has a better success rate than the current behaviour stack. We show that only using our controller can we successfully go through small gaps, minimising manual intervention by the operator
    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \section{Related Work}
    \label{sec:related_work}
    
    
    Designing an autonomous navigation system to handle difficult terrain scenarios is challenging. Often a collection of behaviours are required, where each behaviour has been designed for a unique situation~\cite{arkin_behavior-based_1998, hines_virtual_2021}. 
    
    \subsection{Classical Methods for Robot Navigation}
    
    Artificial potential fields (APF)~\cite{khatib_real-time_1986} is a widely used algorithm for navigation, where the robot is attracted to goal locations, and repelled from obstacles. Bug algorithms have also been used extensively~\cite{mcguire_comparative_2019}. The robot moves toward a goal unless an obstacle is encountered, then the robot moves along the boundary of the obstacle until it can once again move toward the goal. Small gaps is a limitation for each of these methods. Local minima with narrow gaps causes oscillations when the attractive and repelling forces are balanced~\cite{koren_potential_1991}. Probabilistic planners like Probabilistic Roadmap (PRM) and Rapidly-exploring Random Tree (RRT) also have difficulty with narrow spaces. Sun et al~\cite{zheng_sun_narrow_2005} introduce a bridge test to detect narrow passages for use with PRM planning.
    
    Navigating through narrow gaps is challenging. Mujahed et al~\cite{mujahed_admissible_2018} propose an admissibility gap: a virtual gap that satisfies the kinematic constraints of the vehicle to plan through tight spaces. In urban environments, Rusu et al ~\cite{rusu_laser-based_2009} design a geometric door detection method using 3D point cloud information, provided the door is within a set of specifications. A PR2 robot is able to detect a door and its handles~\cite{meeussen_autonomous_2010}, and negotiate the open or closed configuration to get through~\cite{chitta_planning_2010}. Cosgun~\cite{cosgun_context_2018} detects doors from door signs, and direct a robot through with pointing gestures.
    
    Hines et al~\cite{hines_virtual_2021} design a behaviour stack where each behaviour has a priority, and an admissibility criteria. A behaviour becomes active if it has a higher priority than the current behaviour, and is admissible. Admissibility criteria, and the behaviours themselves, are manually designed. The primary path follow method uses Hybrid A*~\cite{dolgov_path_2010} to plan a path through a costmap to a goal, considering the vehicle constraints. 
    
    In each of these approaches, the robot does not make contact with the environment. Therefore gaps that are less than the robot footprint are not considered for traversal, even though the robot may be able to get through. Sensory errors and coarse perception maps contribute to the failure of these methods. Furthermore, classical navigation methods often rely on manual tuning of parameters~\cite{khatib_real-time_1986, hines_virtual_2021, mcguire_comparative_2019}. Next, we review learning methods for navigation, aimed to eliminate such manual tuning.
    
    \subsection{Learning Methods for Robot Navigation}
    
    Learning methods used for navigation have shown promising results for robot navigation in human domains~\cite{rana_multiplicative_2020,bansal_combining_2019,kumar_learning_2019,moreno_automatic_2020,gupta_cognitive_2019} and in the field~\cite{kahn_badgr_2020}. 
    
    Rana et al~\cite{rana_multiplicative_2020} efficiently learn a navigation policy from an APF prior controller while also learning a confidence for when the learned behaviour should be active, or when the robot should use the prior controller. 
    
    With learning methods it is possible to navigate on various surfaces~\cite{kahn_badgr_2020}, and through narrow gaps~\cite{bansal_combining_2019} from RGB images. BADGR by Kahn et al~\cite{kahn_badgr_2020} learn a navigation policy directly from images with a self supervised approach that not only learns to navigate to a waypoint, but also to favour traversing a concrete path over grass. Bansal et al~\cite{bansal_combining_2019} learn to navigate through narrow doorways to get to a specified goal location using a monocular camera mounted to a robot.
    
    Other learning approaches map and plan~\cite{gupta_cognitive_2019}, generate waypoints~\cite{kumar_learning_2019}, or use motion primitives~\cite{moreno_automatic_2020}. Gupta et al~\cite{gupta_cognitive_2019} learn a map and how to plan to a goal from egocentric map with end-to-end reinforcement learning. Kumar et al~\cite{kumar_learning_2019} learn to plan at a high level of abstraction (turn left, turn right) from video data. Moreno et al~\cite{moreno_automatic_2020} generate auxiliary waypoint locations (critical navigation points) at problematic narrow regions.
    
    With the exception of Rana et al~\cite{rana_multiplicative_2020}, learning methods are do not typically integrate with classical methods. In our previous work we introduce the idea of developing behaviours separately~\cite{tidd_guided_2020}, then learning when they should be used, either with a supervised approach~\cite{tidd_learning_2020}, or through reinforcement learning~\cite{tidd_learning_2021}. For our problem we require a behaviour that can learn to perform complex maneuvers (such as make contact with a door), and can be integrated into an existing behaviour stack. 
    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \section{Robotic Platform}
    \label{sec:robotic_platform}
    The `Titan' all terrain robot (ATR) from BIA5~\cite{bia5_robotic_2021} is a 90Kg tracked vehicle, with a length of 1.4m and a width of 0.78m. It is the primary autonomous platform in a heterogeneous fleet of robots (tracked, legged, aerial) used by team CSIRO Data61's~\cite{hudson_heterogeneous_2021} entry in the SubT challenge systems track~\cite{darpa_darpa_2021}. The Titan moves with nonholonomic motion following forward and heading velocity commands, and can turn on the spot (skid-steer).
    
    \textbf{Perception Stack:}
    Like all robots in team CSIRO Data61, the Titan has a `Catpack' perception system equipped with a tilted spinning Velodyne Lidar, Inertial Measurement Unit (IMU), 4 RGB cameras, and 3 thermal cameras. Each robot performs Simultaneous Localisation and Mapping (SLAM) onboard, providing a occupancy map to local navigation behaviours for fully autonomous navigation. Goals are provided by a higher level planner, encouraging thorough exploration in the search for artifacts (the full specifications of the Catpack and system solution can be found in~\cite{hudson_heterogeneous_2021} and ~\cite{hines_virtual_2021}). 
    
    \textbf{Behaviour Stack:}
    Among several manual defined controllers, the primary navigation behaviour is a \textit{path follow} behaviour that takes a goal point and calculates a safe path using hybrid A* search that associates a continuous state with each grid cell (in opposed to discrete cell center in standard A* search), allowing the path to consider vehicle kinematic constraints~\cite{dolgov_path_2010, hines_virtual_2021}. An \textit{orientation correction} behaviour recovers the robot to a level position in the case of extreme roll or pitch, and a \textit{decollide} behaviour will perform a maneuver into a safe location when there is fatal cost within the robot footprint. There is also a teleoperation behaviour (\textit{Joy}) for situations the operator can manually control a robot (when the robot is within communication with the ground control station). Each behaviour is ranked in order of priority (shown in Fig.~\ref{fig:fig2}, behaviour stack), where the admissible behaviour with the highest priority is activated. Each behaviour is responsible for detecting its own admissibility.
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \section{Method}
    \label{sec:method}
    
    \begin{figure}[tb!]
    % \vspace{2mm}
    \centering
    \includegraphics[width=\columnwidth]{images/ch6/Fig2.png}
    %\hfill
    \caption{We learn a gap behaviour and a behaviour selection policy using an occupancy map. The behaviour selection policy determines when the gap behaviour should be active based on a goal location, or when we should rely on a manually designed behaviour stack~\cite{hudson_heterogeneous_2021}.}
    \label{fig:fig2}
    % \vspace{-3mm}
    \end{figure}
    
    %Despite a sophisticated perception stack and a well-tuned navigation stack, identifying and traversing narrow gaps remains a challenge. 
    
    Figure~\ref{fig:fig2} outlines our system. The gap behaviour policy receives $s_t = [rs_t, I_t]$ (defined below), and outputs action $a_t$, consisting of forward and angular velocity about the $z$ axis (heading). The behaviour selection policy is also provided with $s_t$, as well as a goal location, and outputs switching parameter $\tau$. The gap behaviour should be activated by the behaviour selection policy when a goal is located behind a small gap, otherwise the behaviour stack should be active.
    
    \subsection{Problem Description}
    \label{sec:problem}
    
    Traversing small gaps is important for underground search and rescue scenarios, such as those found in the SubT challenge~\cite{darpa_darpa_2021}. The SubT challenge involves detecting and localising artifacts (survivors, backpacks, helmets) in underground environments (mine, urban, cave), where large portions of the course may only be accessible after a narrow constriction. Due to the large scale of the scenarios encountered, teams of robots are required to enter the underground environment, with the imposed limitation that there can only be a single human operator. The human operator can command the robots through any method, though communications to robots are severely limited. Furthermore, coordinating multiple robots while reporting artifact detections in a timed competition (1 hour) presents a significant load on the operator. The robots must be as autonomous as possible. In these search and rescue scenarios the robot is allowed to make contact with the environment, but not intentionally damage it. In this paper we target traversing small doorways.
    
    
    \subsection{Reinforcement Learning}
    \label{sec:rl}
    
    We consider our problem to be a Markov Decision Process $\text{MDP}$, where each state contains all relevant information to make a decision. An MDP is defined by tuple $\{\mathcal{S},\mathcal{A}, R, \mathcal{P}, \gamma\}$ where $s_t \in \mathcal{S}$, $a_t \in \mathcal{A}$, $r_t \in R$ are state, action and reward observed at time $t$, $\mathcal{P}$ is an unknown transition probability from $s_t$ to $s_{t+1}$ taking action $a_t$, and applying discount factor $\gamma$. 
    
    With reinforcement learning, the goal is to maximise the sum of future rewards $R = \sum_{t=0}^{T}\gamma^tr_t$, where $r_t$ is the reward at time $t$. Actions are continuous values, sampled from a deep neural network ($a_t\sim\pi_\theta(s_t)$ for the gap behaviour policy, $\tau_t\sim\pi_\phi(s_t, goal)$ for the behaviour selection policy), and $s_t$ includes the robot state $rs_t$ and occupancy map $I_t$ (introduced below). We update each policy with Proximal Policy Optimisation (PPO)~\cite{schulman_proximal_2017}, using the implementation by OpenAI~\cite{dhariwal_openai_2017}.
    
    %  where $a_t = \hat{v}_x, \hat{v}_\omega$ is the linear and angular velocity sent to the robot 
     
    \textbf{Robot State $rs_t$:} The robot state is a vector of 7 numbers containing the heading velocity $v_x$, and the angular position and velocities: $roll, pitch, yaw, v_{roll}, v_{pitch}, v_{yaw}$. Velocity terms are calculated with clipped finite differences. These terms inform the policies when the robot has made contact with the wall.
    
    \textbf{Occupancy Map $I_t$:} A binary occupancy map with dimensions $[80,80,1]$ and resolution of 0.1m is provided from the high density point cloud (details are provided in~\cite{hudson_heterogeneous_2021}), where a value of 0 indicates a known and unoccupied cell, and a value of 1 indicates an unknown or occupied cell. The occupancy map moves with the $x$, $y$ translation and $yaw$ rotation of the robot, with the center of the robot located at the centre of the occupancy map. 
    
    \begin{figure}[tb!]
    % \vspace{2mm}
    \centering
    \subfloat[Gap Behaviour]{\includegraphics[trim=1.8cm 3.6cm 1.8cm 3cm, clip, width=0.45\linewidth]{images/ch6/door1.png}}
    \hspace{0.3cm}
    \subfloat[Behaviour Selection]{\includegraphics[trim=4.2cm 4.4cm 4cm 3.7cm, clip, width=0.41\linewidth]{images/ch6/door2.png}}
    
    \caption{A simulation of a narrow door. The circular markers represent reward targets. a) The two doorway points are used by the gap behaviour policy. b) Behaviour selection policy uses two pairs of markers.}
    \label{fig:doors}
    \end{figure}
    
    We train a gap behaviour policy to go through small gaps, and a behaviour selection policy that activates the gap behaviour when a goal appears behind a gap. The training setup is show in Fig.~\ref{fig:doors}. Fig.~\ref{fig:doors}a is used to train the gap behaviour policy, markers depict the entrance and exit to a gap ($m_1,m_2$). Fig.~\ref{fig:doors}b shows the setup for training the behaviour selection policy where additional markers show the goal points provided to behaviour selection ($m_1, m_4$).
    
    \subsection{Gap Behaviour Policy}
    \label{sec:behaviour}
    The gap behaviour receives a stacked robot state message from the previous 5 timesteps: $[rs_t, rs_{t-1}, rs_{t-2}, rs_{t-3}, rs_{t-4}]$. The robot starts from a random initial position in front of a doorway, where the initial position is uniformly selected from a circle 1.5m back from the first marker $m_1$, with a radius of 1.5m. We also randomise the heading of the robot, choosing uniformly between -1.5 and 1.5 radians from the heading perpendicular to the gap. The target marker is set to the initial marker at the entrance to the gap $m_1$.
    
    \textbf{Reward:} The reward terms encourage forward progress towards the target marker. Once the robot is within 0.5m of the target marker (initially set to marker $m_1$), the marker through the gap becomes the new target ($m_2$). This encourages the robot to approach the gap with the correct heading to make it through. The reward is defined as:
    \[r_t = 1.5 r_{\dot{v}_x} - 0.1r_\theta - 0.05r_a - 0.75r_{\phi} - 0.001r_{s} - 0.25r_{v_{-x}}\]
    
    where $r_{\dot{v}_x}$ is the velocity towards the target marker, $r_\theta$ is the error in heading between the robot and the target marker, $r_a$ is a penalty on angular velocity, $r_{\phi}$ is a penalty on roll and pitch angles, $r_{s}$ is a smoothing cost (previous actions should be close to the current actions), and $r_{v_{-x}}$ is a penalty for going backward.
    
    We train for 1000 episodes, where episodes are a fixed length of 180 steps (with a timestep of 0.1s), and the policy is updated at the end of an episode. 16 workers (CPU's) run in parallel, performing synchronised policy updates. Each robot is randomly inserted at the beginning of each episode, choosing between 98 different doorways (small variations in gap width, variations to door position). An episode is considered successful if the robot reaches $m_2$, the marker after the door.
    
    % Titan is allowed to make contact with the door
    
    \subsection{Behaviour Selection Policy}
    \label{sec:behaviour_selection_method}
    
    % During the SubT challenge there is a single human supervisor for a fleet of 5 or more robots. Autonomy is paramount for success. 
    While part of the problem we are considering involves controlling the robot through a narrow gap, to integrate the behaviour into the SubT behaviour stack, we must also know when the gap behaviour should be activated.
    
    We once again use reinforcement learning to train an admissibility prediction that detects when the gap behaviour should be run, and when we should default to the behaviour stack (introduced in Sec:\ref{sec:robotic_platform}). The behaviour selection policy receives the robot state message $rs_t$, occupancy map $I_t$, and a goal location (distance and angle in the robot frame).
    
    As we should only traverse a gap if there is a goal on the other side of the gap, we condition behaviour selection on having a goal. If the goal is on the same side of the gap as the robot, we do not want to activate the gap behaviour, but if is on the the other side we do. We have four markers $[m_1, m_2, m_3, m_4]$, shown in Fig.~\ref{fig:doors}b). Markers 1 and 4 are considered goals, and are provided to the behaviour selection policy. These goals would be provided by a higher level exploration planner. Markers 2 and 3 are the same as for the gap behaviour (entrance and exit of the gap) and are used design the reward.
    
    We start the robot from a random position sampled uniformly from a circle 4.5m before the door marker $m_2$ with a radius of 1.5m. $m_1$ and $m_4$ are also randomly selected from a uniform distribution, $m_1$ is located 1.5m \textit{before} $m_2$, and $m_4$ is located 1.5m \textit{after} $m_3$. The robot heading is randomly sampled from $(-\pi, \pi)$. This heading range is larger than the range used to train the gap behaviour, allowing the behaviour selection policy to be robust to any robot heading, where the gap behaviour is only expected to operate when the gap is in front of the robot.
    
    \textbf{Reward:}
    The reward term for behaviour selection is dependent on the current target marker. Once the robot is within 0.5m of a marker, we update the target marker to the next marker in the sequence. The robot should activate the behaviour stack (path follow behaviour) if it has not yet reached $m_1$, or has reached $m_3$. If the robot has reached $m_1$, but has not yet reached $m_3$, it should use the gap behaviour. The reward for behaviour selection is defined as:
    \begin{equation}
    \label{sup_reward}
        r_t = 
    \begin{cases}
        1 - (\tau_t - 0.0)^2,& \text{if the target is } m_1 \text{ or } m_4 \\
        1 - (\tau_t - 1.0)^2,& \text{if the target is } m_2 \text{ or } m_3
    \end{cases}
    \end{equation}
    
    Where $\tau$, a binary variable, is the output of the behaviour selection policy at time $t$. $\tau$ of 1.0 indicates activating the gap behaviour, and 0.0 the behaviour stack.
    
    % ~\textbf{Path Follow Behaviour} is a proportional controller that minimise the angular position error of the robot and the goal point, and the distance to the goal. Starting the robot from a random position in front of the point, we run the policy determined by the gap detector.  
    
    \textbf{Auxiliary task:} Learning an auxiliary task can help with the learning of visual features~\cite{jaderberg_reinforcement_2016}. We learn an auxiliary task with the behaviour selection policy. As shown in Fig.~\ref{fig:fig2}, the auxiliary task shares the convolution layers with behaviour selection, but has two separate fully connected layers. The auxiliary task uses a supervised learning loss to learn the gap width, and location of the gap markers. The auxiliary output is a vector of 5 terms: 
    \[aux = [w, m_{2_{dist}}, m_{2_{angle}}, m_{3_{dist}}, m_{3_{angle}}] \]
    
    Where $w$ is gap width, $dist$ and $angle$ are polar coordinates from the respective gap marker ($m_2, m_3$) to the robot ($dist$ is the distance to the robot, $angle$ is the heading error). We train the auxiliary term with mean squared error loss from the ground truth provided by the simulation. Learning the location of the gap has the additional benefit of providing visual information to the operator. If the gap behaviour is activated, the operator can clearly see the gap.
    
    % We train the behaviour selection for 200 updates with 16 workers, randomly choosing between 98 different doorways. Episode lengths are fixed at 300 timesteps.
    
    The gap behaviour policy and the behaviour selection policy are trained in simulation using the Gazebo simulator. We insert blocks into the simulator so the robot must drive through gaps (sampled uniformly from $0.8 - 0.85$m). We also add blocks to to resemble doors in various open configurations. Due to the computational demands of running the full perception stack on a single computer while running multiple agents, during policy training the occupancy map is generated by inserting blocks into known locations in a global occupancy map, then sampling a robot-centric map using the robot pose ($x,y,yaw$). For testing, we rely on the occupancy map generated by the perception stack, both in simulation and on the real robot (Sec.~\ref{sec:experiments}.B and Sec.~\ref{sec:experiments}.C).
    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \section{Experiments}
    \label{sec:experiments}
    
    \begin{figure}[t!]
        \vspace{-5mm}
        \centering
        % \subfloat[Gap behaviour policy]{\includegraphics[trim=1cm 0.5cm 1cm 2cm, clip, width=0.5\columnwidth]{images/ch6/results0.png}}
        \subfloat[Gap behaviour policy]{\includegraphics[trim=0cm 0.0cm 0cm 0cm, clip, width=0.5\columnwidth]{images/ch6/results0.png}}
        \hfil
        % \subfloat[Behaviour selection policy]{\includegraphics[trim=1cm 1cm 1cm 2cm, clip,width=0.45\columnwidth]{images/ch6/results1.png}}
        \subfloat[Behaviour selection policy]{\includegraphics[trim=0cm 0cm 0cm 0cm, clip,width=0.5\columnwidth]{images/ch6/results1.png}}
        \hfil
        % \hfill
        \caption{Success rates during training for the gap behaviour policy and the behaviour selection policy.}
        \label{fig:learning_curves}
        %\vspace{-3mm}
    \end{figure}
    
    % \begin{figure}[tb!]
    % % \vspace{2mm}
    % \centering
    % \includegraphics[width=0.65\columnwidth]{images/ch6/selector.png}
    % % \includegraphics[width=\columnwidth]{images/ch6/selector.png}
    % % \includegraphics[width=\wIII cm, height=\hII cm]{images/ch6/selector.png}
    % \hfill
    % \caption{We compare training the behaviour selector using a supervised learning approach and a reinforcement learning method, trained with an identical setup for 3 random seeds.}
    % \label{fig:results_selector}
    % % \vspace{-3mm}
    % \end{figure}
    
    We first show the results of training our policies (Sec.~\ref{sec:training}). Sec.~\ref{sec:simulation} shows the results in simulation using the perception stack (introduced in ~\ref{sec:problem}), and the real robot results are shown in Sec.~\ref{sec:real}. Fig~\ref{fig:modes}.a and b) show the setup for the simulated and real doors.
    
    \subsection{Training Results}
    \label{sec:training}
    
    The \textbf{gaps behaviour policy} achieves a success rate of 93.8\% on the simulated environment (98 gaps of random width and door type). The success rate while training is shown in Fig.~\ref{fig:learning_curves}.a). The behaviour performs several complex maneuvers that would be difficult to encode manually. These maneuvers include approaching the gap with one corner and making contact with the door, reversing and re-approaching when the robot pitches, and `wiggling' when the robot is part way through but not making progress.
    
    Once the gap behaviour policy is trained, we train the \textbf{behaviour selection policy} with the method from Sec\ref{sec:behaviour_selection_method}. The results shown in Fig~\ref{fig:learning_curves}.b), display the success rate for behaviour selection training. We compare using a supervised loss to using our reinforcement learning method for learning behaviour selection:
    
    ~\textbf{Supervised Learning:} Behaviour selection could be considered a supervised learning problem where robot state with occupancy map at each timestep are taken as input, and are given a label. We use labels of 0 if the target marker is $m_1$ or $m_4$, and 1 if the target marker is $m_2$ or $m_3$. We update network weights using mean squared error loss.
    
    ~\textbf{Reinforcement Learning:}
    We train the behaviour selection policy using the reinforcement learning approach introduced in Sec~\ref{sec:behaviour_selection_method}, where we use a reinforcement learning update with the reward from Equation~\ref{sup_reward}.
    
    In both examples we also predict the auxiliary terms, which include door size, and marker locations relative to the robot. As can be seen in Fig.~\ref{fig:learning_curves}, the reinforcement learning approach achieves more successful door traversals, with an asymptotic success rate of 88.7\%, compared to 75.8\% with the supervised learning approach. We attribute the difference between the methods on the reinforcement learning approach considering the sum of future behaviour selections, whereas the supervised approach only considers the current timestep. We found that excluding the auxiliary terms from training had very little effect on success rate. We also tested various additional parameters in the reward function but found almost no effect on success rate. We have omitted these results from Fig.~\ref{fig:learning_curves}b) for clarity.
    
    % ~\textbf{Additional Reward Terms:}
    % We train with additional reward terms.
    
    % ~\textbf{Supervised Reward with Reinforcement Learning:}
    % We use a supervised reward from equation ~\ref{sup_reward}, using reinforcement loss from PPO~\cite{schulman_proximal_2017}.
    
    % ~\textbf{Supervised Reward with Auxiliary Terms:}
    % We train a reinforcement learning network to also predict the auxiliary terms, which include door size, and marker locations relative to the robot.
    
    
    \subsection{Simulation Results}
    \label{sec:simulation}
    
    We test our gap behaviour and behaviour selection policies in simulation on an unseen test world, using the SubT perception stack (Lidar scans are used to produce the occupancy map). The test world has gaps uniformly sampled from $0.8-0.85$m, with random door types. We compare several modes of operation including using the behaviour stack without the gap behaviour, manually activating the gap behaviour, and using the behaviour selection policy to autonomously activate the gap behaviour.
    
    ~\textbf{Behaviour Stack:} The current navigation stack used by the Titan platform uses several behaviours described in Sec~\ref{sec:problem}: path follow, orientation correction and decollide. Path follow is the dominant behaviour where hybrid A* search is used to find a path to a local goal. For more details about the behaviour stack see~\cite{hines_virtual_2021} and~\cite{hudson_heterogeneous_2021}. For these experiments the operator inserts a waypoint on the opposite side of a gap.
    
    ~\textbf{Manual Gap Behaviour Selection:} The operator can manually call the gap behaviour from a GUI. The operator must first insert a waypoint so the robot approaches the gap (running the behaviour stack), then activate the gap behaviour, and when the robot is through the gap once again activate the behaviour stack to get the robot to the waypoint after the door.
    
    ~\textbf{Autonomous Gap Behaviour Selection:} The gap behaviour is autonomously selected when the conditions are met (there is a goal behind a small gap). The operator can place a waypoint on the other side of a door and behaviour selection will activate the behaviour stack or the gap behaviour autonomously. 
    
    
    \begin{table}[h!]
        %\vspace{-2mm}
        \centering
        % \begin{tabular}{c|c|c|c|c|c}
        % \begin{adjustbox}{max width=1.0\columnwidth}
        % \begin{adjustbox}{min width=0.75\columnwidth}
        \begin{adjustbox}{max width=1.0\columnwidth}
        \begin{tabular}{cccccc}
            % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                          & Success \% & Time(s) & Operator Actions \\
           \hline
            Behaviour Stack      & 0.0            &  50.2 &    1  \\
            Manual Gap Behaviour Selection        & 93.3          &  29.7 &    3  \\
            Auto Gap Behaviour Selection  & 66.7          &  45.3 &    1 \\
        \hline
        \end{tabular}
        \end{adjustbox}
        \caption{Simulation results for passing through a narrow gap (15 trials)}
        \label{tab:sim_results}
    \end{table}
    
    % Fig~\ref{fig:modes}.c to e) show the three modes of operation. In Fig~\ref{fig:modes}.c) the behaviour stack reaches a timeout for all small gaps. Fig~\ref{fig:modes}.d) shows the additional operator load for running the gap behaviour manually, and Fig~\ref{fig:modes}.e) shows behaviour selection including the auxiliary reward marking the gap position.
    
    We perform 15 trials and present results in Table~\ref{tab:sim_results}. We show the average success rate, time until the final waypoint, and the number of operator actions. We can see that the behaviour stack cannot traverse the gap and reaches a timeout (no progress after 30 seconds). Manually activating the gap behaviour has a high success rate (93\%), and autonomously selecting behaviours has a reasonable success rate of 66.7\%. Of the failure cases of the behaviour selection, one was a result of the behaviour selector not recognising the gap, 2 were due to the gap behaviour failing, and 2 were a result of the decollide behaviour causing a timeout on the waypoint when switching between the behaviour stack. Where decollide did not activate (behaviour selection did not switch back to the behaviour stack midway through the gap), the average time through the gap was 17.3 seconds, suggesting behaviour selection is a viable method, however requires further investigation to ensure robustness.
    
    \begin{figure}[t!]
        % \vspace{2mm}
        \centering
        \subfloat[Gazebo Simulator]{\includegraphics[trim=3cm 7cm 3cm 6cm, clip, width=0.5\linewidth]{images/ch6/gazebo.png}}
        \hspace{0.3cm}
        \subfloat[Real Robot]{\includegraphics[trim=3cm 4cm 0cm 12.2cm, clip, width=0.4\linewidth]{images/ch6/real_door.jpg}}
        \caption{Experimental setup in simulation and with the real robot.}
        \label{fig:modes}
    \end{figure}
    
    \subsection{Real Robot Results}
    \label{sec:real}
    
    % \begin{figure}[tb!]
    %     % \vspace{2mm}
    %     \centering
    %     \subfloat[Real Door]{\includegraphics[width=\w cm, height=\h cm]{images/ch6/real_door.jpg}}
    %     \hfil
    %     \subfloat[Robot tries to reach goal]{\includegraphics[width=\w cm, height=\h cm]{images/ch6/waypoint1.png}}
    %     \hfil
    %     \subfloat[Goal timesout]{\includegraphics[width=\w cm, height=\h cm]{images/ch6/Fig5.png}}
    %     % \hfill
    %     \caption{Real door, waypoint, behaviour, selection.}
    %     \label{fig:real}
    %     \vspace{-3mm}
    % \end{figure}
    
    \begin{table}[h!]
        \vspace{-2mm}
        \centering
        % \begin{tabular}{c|c|c|c|c|c}
        % \begin{adjustbox}{max width=1.0\columnwidth}
        \begin{adjustbox}{max width=1.0\columnwidth}
        \begin{tabular}{cccccc}
            % \multicolumn{1}{l}{\textbf{Less Difficult}} & Flat & Gap & Hurdle & Stairs & Steps \\ 
                                          & Success \% & Time(s) & Operator Actions \\
           \hline
            Behaviour Stack              & 0.0           &  44.6 &    1  \\
            Manual Gap Behaviour Selection               & 73.3          &  24.1 &    3  \\
            Auto Gap Behaviour Selection         & 40.0          &  30.9 &    1 \\
        \hline
        \end{tabular}
        \end{adjustbox}
        \caption{Real robot results for passing through a narrow gap (15 trials).}
        \label{tab:real_results}
    \end{table}
    
    Table~\ref{tab:real_results} show our final experiments applied in a door scenario on a real robot. We use a constructed wooden door rather than a real door as the gap behaviour is allowed to contact the door, which can result in the robot damaging the environment. The constructed door shown in Fig~\ref{fig:modes}.b).
    
    We run 15 trials for all experiments, results are shown in Table~\ref{tab:real_results}. We confirm our behaviour succeeds in more than 70\% of trials, where the current behaviour stack cannot traverse the gap, timing out after 30 seconds. The behaviour selection method is successful 40\% of the time. Both manually evoking the gap behaviour, and relying on autonomous behaviour selection had the same failure case: the edge of the robot would grab the protrusion of the door and the tracks would spin on the slippery surface. This was not seen as in the simulation trials as track slippage is not modeled in simulation. While this situation may not occur regularly with real doors, future policies will be trained with examples of gaps with small protruding edges. 
    
    Autonomous behaviour selection had a much lower success rate than manually activating the gap behaviour. This is due to the late switching from the behaviour stack to the gap behaviour, and the limitation of our test door (protruding edges). With late switching, the gap behaviour was more likely to get the robot caught on the outer wooden structure of the door. Future behaviour selection models would encourage switching to the gap behaviour earlier, allowing more time to align with the door.
    
    In one case with behaviour selection, the robot was mostly through the gap when the behaviour switched back to the behaviour stack, triggering a decollide behaviour and causing the robot to go in and out of the gap. Training the behaviour selection policy with the marker after the door ($m_3$) further back should result in the gap behaviour being active until after the robot has cleared the door.
    
    While these limitations must be addressed before the behaviour can be properly integrated into the behaviour stack for autonomous operation, the manual activation of the gap behaviour policy has been utilised in a SubT 1 hour test run with 5 different robots (3 Titan's, 1 Ghost Vision60 quadruped, and a drone). A small gap was identified when the behaviour stack timed out at a constriction in the tunnel. The operator manually intervened to execute the gap behaviour policy, resulting in the robot successfully going through the gap.
    
    % shown in Fig~\ref{fig:modes}.f),
    
    % \begin{figure}[tb!]
    % % \vspace{2mm}
    % \centering
    % % width=\w cm, height=\h cm
    % % \includegraphics[width=\columnwidth]{images/ch6/Fig5.png}
    % \includegraphics[width=\w cm, height=\h cm]{images/ch6/Fig5.png}
    % \hfill
    % \caption{A real use case of the gaps behaviour in a SubT test run. Magenta blocks indicate fatal cost.}
    % \label{fig:fig5}
    % % \vspace{-3mm}
    % \end{figure}
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \section{Conclusion}
    \label{sec:conclusion}
    
    We present a reinforcement learning approach to develop a gap behaviour policy to traverse small gaps. We also learn a behaviour selection policy that determines when to autonomously activate the gaps behaviour (when a goal is through a small gap). We show that our gap behaviour policy is more reliable than the current stack of tuned behaviours, both in simulation (93\% compared to 0\%) and on a real robot (73\% compared to 0\%), though we recognise that work is too be done to make autonomous behaviour selection more robust (success rates of 67\% in simulation and 40\% in real trials). Future work will look at improving the reliability of the system for a wider range of gap scenarios. 
    
    A significant limitation of our method occurs when gaps are smaller than the robot. It is likely in these situations the gap behaviour policy will still be selected for operation and try to traverse the gap. Methods to handle these scenarios will be considered in future work. 
    
    
    
    

==> old/Ch7.tex <==
% Ch6.tex
\chapter[Obstacle Classification]{Obstacle Classification}
\label{cha:ch7}


% Integrating
% behaviours into pre-existing libraries was shown by training switch mechanisms: with access
% to other behaviours; separately by learning reliable switch states for individual behaviours; and
% concurrently with intermediate policies that move the robot towards suitable switch locations.

% for learning methods  Learning how to traverse these environments is an exciting avenue for designing complex behaviours over labour intensive manually designed controllers, however sample inefficiency prevents use.

% research questions pertaining to traversing difficult obstacles. 

% The objective of this thesis has been to investigate deep learning algorithms to enable robots to learn visuo-motor policies through trial and error in simulation for real-world manipulation tasks. To achieve the goal, we have evaluated the feasibility of deep reinforcement learning for robotic reaching, and proposed modular DQNs and adversarial discriminative transfer for sim-to-real transfer of visuo-motor policies. This chapter summarizes the contributions made in this thesis and discusses potential improvement and directions in the future work.

    % It was shown that classical control methods and na\"ive learning approaches were inefficient at solving these tasks. 
    
    % for difficult scenarios,
    % For complex terrains, the guided curriculum learning approach was able to learn complex behaviours that were difficult to achieve with other methods. F
    % What are the key takeaways / why does Juxi care
    % The methods developed from these contributions provide steps towards answering the research question: \textit{How can complex visuo-motor locomotion behaviours be learned efficiently?} Behaviours developed from these methods were used in the remaining contributions.
% \item


    % Conclude, complete, finalise.
    
    % for situations where a reliable switch location did not occur between sequential behaviours
    
    % Using a reward developed from key waypoint locations, this policy determined if a goal location was through a small gap.
    
    % \item The effect of state overlap on safe policy switching was investigated by training diverse policies with common initial conditions. The results showed that state overlap was crucial for switching between behaviours
    % \item A policy switching network was designed to estimate the likelihood of success for switching policies in a given state, improving the reliability of traversing a sequence of obstacles
% \end{itemize}



% Three separate approaches for determining a safe switch state were explored: training a high level policy to learned when to switch behaviours, training a switch estimator to learn the likelihood of success Behaviours that have a RoA overlap, predicting the switch state was shown to increase reliability. Finally, training a switch mechanism concurrently with a separate task is an efficient method for learning when to switch. 

% RoA overlap is key for developing reliable switching methods.

% What did we learn about switching? It needs to happen during RoA overlap. 


% Methods were presented for reliable behaviour switching in chapters \ref{cha:ch3b}, \ref{cha:ch4}, and \ref{cha:ch5}. These chapters contribute to the answer of the research question: \textit{How can a safe switch location be determined to facilitate the reliable switching of sequential behaviours?}.  
% \item

% \textbf{Improving switching among unreliable switch locations}
    % \begin{itemize}[label={}]
        % \item Setup Policies were developed that demonstrated improved reliability of transitioning between sequential behaviours, particularly for controllers with partial or no RoA overlap
        % \item A reward signal was designed for guiding the robot towards a target behaviour for Setup Policies training. By weighting the target policy value function by its advantage, this reward minimised over estimation bias, resulting in better learning outcomes of transition policies compared to several alternatives
        
        
     % as the reward reward guided the robot towards a target behaviour. By weighting the target policy value function by its advantage, this reward minimised over estimation bias. 
        
        % Context, For this to work xxx yyy zzz was done/investigated/developed/deployed….”
    % \end{itemize}
    % Policies were initialised from a walking policy and required an extended reward to provide experience to the policy after the transition was complete.
    
    
    % How can an agent prepare for an upcoming behaviour such that safe switching can occur?
    
    % This occurs between complex behaviours that perform specialist actions, an example is a bipedal jump behaviour that requires the robot to push off the ground with both feet. This work explored a solution to this scenario, producing a policy for preparing the robot for an upcoming behaviour to safely switch.
    
    % Research question 3: \textit{How can an agent prepare for an upcoming behaviour such that safe switching can occur?} was investigated in chapter \ref{cha:ch5}. This chapter explored complex behaviours with the simulated biped, particularly a jump behaviour that required the robot to jump with both feet together. This controller did not present with reliable switch locations for other controllers required to traverse a sequence of obstacles. Setup Policies improved the reliability of switching. 
    
    % We investigate two principle components for reliable behaviour switching: when is the robot in a suitable state to switch to a desired controller, and how can we move the robot into a reliable state to safely switch. With these contributions we answer the question: ``How can we reliably learn how to transition between behaviours." The combination of behaviours and switching mechanisms allowed our simulated biped to traverse a sequence of complex obstacles. For the tracked platform, we were able to switch between a pre-existing Behaviour Stack and a learned Gap Behaviour.
% \item
%     \textbf{Autonomous traversal of narrow gaps}
%     \begin{itemize}
%         \item In Chapter \ref{cha:ch5} we showed that a Gap Behaviour and a Behaviour Selection policy were able to autonomously command a large tracked platform through small gaps
%         \item We identified some of the challenges of simulation to real transfer and ways we could improve robustness and reliability in future work 
%     \end{itemize}
%     We successfully implemented policies trained in simulation onto a real robotic platform to maneuver through a difficult obstacle, answering the question ``How can we learn to autonomously traverse narrow gaps." We identified some of the challenges of training behaviours in simulation for real world applications. We discussed the source of disparity between the results achieved in the simulation and those demonstrated on the real agent.
% \end{enumerate}


% \section[Discussion]{Discussion}
% \label{cha:discussion}
% Behaviours are important

==> old/classical_notes.tex <==
Note from the memmo workshop on classical control of bipeds.
\begin{itemize}
    \item Planning is hard, high dimensional, most are uninteresting 
    \item contact choices are important
    \item highly non-linear
    \item too hard to be tackled as it is. We need to cheat, this has a cost
    \item probability of sampling a valid configuration in contact is equal to zero.
    \item loco3d
    \item important to have good models
    \item have to use heuristics to combine parts of the problem.
    \item 
\end{itemize}

\begin{enumerate}
    \item Global path planner
    \item contact planner
    \item CoM + whole body motion
\end{enumerate}



\begin{enumerate}
    \item Pinocchio (simulator?)
    \begin{itemize}
        \item Not a solver, not an application, 
        \item urdf parser
        \item forward kinematics and jacobians
        \item forward and inverse dynamics
        \item display
        \item collision detection HPP-FCL (Humanoid path planner)
        \item derivatives of kinematics and dynamics
        \item type templatization and code generalisation
    \end{itemize}
    \item Task Space Inverse Dynamics (TSID) - Balance after pushes
    \begin{itemize}
        \item Inverse dynamics
        \item formulation of tasks
        \item contact solvers
        \item QP solver 
    \end{itemize}
    \item Crocoddyl
    \begin{itemize}
        \item optimal control
        \item DDP optimizer
        \item task/cost formulation
    \end{itemize}
\end{enumerate}


\begin{itemize}
    

\item the recursive Newton-Euler algorithm (RNEA) computes the inverse dynamics
\item the articulated rigid body algorithm (ABA) computes the direct dynamics
\item the composite rigid body algorithm (CRBA) computes the mass matrix. The 3 algorithms can be directly called by their names in Pinocchio.
\end{itemize}

\begin{itemize}
    \item
\end{itemize}



\begin{itemize}
    \item
\end{itemize}

\begin{itemize}
    \item
\end{itemize}

\begin{itemize}
    \item
\end{itemize}

==> old/nomenclature_examples.tex <==
% nomenclature

%\newenvironment{nomenc}{\prefacesection{Nomenclature}}{}

%\chapter*{Nomenclature}
%\addcontentsline{toc}{chapter}{Nomenclature}

%\begin{nomenc}
{
\renewcommand{\arraystretch}{1.2} 
\begin{longtable}{llr}
\multicolumn{3}{l}{\textbf{Abbreviations}\hspace{0.4\textwidth}~~}\\
CAN & Controller Area Network\\
DM & Deadline-Monotonic (Scheduling) \\
EDF & Earliest-Deadline-First (Scheduling)\\
FP & Fixed Priority\\
IAE & Integral of Absolute Error\\
IP & Internet Protocol\\
ITAE & Integral of Time Absolute Error\\
LCT & Least-Compute-Time (Scheduling)\\
%MTBE & Methyl \textit{tert}-buty ether\\
QoC & Quality of Control\\
QoS & Quality of Service\\
PD & \multicolumn{2}{l}{Proportional plus derivative (Control/Controller)}\\
PD2 & \multicolumn{2}{l}{Proportional plus up to the Second-Order Derivative (Compensation)}\\
PD3 & \multicolumn{2}{l}{Proportional plus up to the Third-Order Derivative (Compensation)}\\
PI &\multicolumn{2}{l}{ Proportional-Integral (Control/Controller)}\\
PID & \multicolumn{2}{l}{Proportional-Integral-Derivative (Control/Controller)}\\
RM & Rate-Monotonic (Scheduling)\\
NCS & Networked Control System/s\\
SSE & Sum of Square Error\\
TCP & Transport Control Protocol\\
WCCD & Worst-Case Communication Delay\\
\\
\multicolumn{2}{l}{\textbf{Symbols}} \hspace{0.4\textwidth}~& {\bf Chapter}\\
A1 $\sim$ Am & Smart actuators & Ch8,9\\
C1 $\sim$ C5 & Control computers & Ch8,9\\
{$c$}  & {Worst case computation time} & Ch5,6,7\\
{$d$}  & Deadline & Ch5,6,7\\
$e$ & Control error, $e = r - y_d$ & Ch1\\
$f(\cdot)$ & Function & Ch10\\
$G$ & Controller or its transfer function & Ch6,7\\
{$G_c$} & {Controller or its transfer function}& Ch3,4,10\\
{$G_L$} & {Process transfer function in disturbance path}& Ch3,4\\
{$G_p$} & {Process transfer function in manipulation path}& Ch3,4,10\\
$K$ & Gain & Ch6,7\\
$K_c$ & Controller gain & Ch3,4,10\\
$K_p$ & Process gain & Ch3,4,10\\
{$k$} & {Present sampling instant}& Ch3,4\\
      & Integer & Ch8\\
      & Integer representing the $k$th control period & Ch10\\
$lr$ & Loss rate & Ch10\\
M1 $\sim$ M5 & Management computers & Ch8,9\\
$m$ & Integer variable, or the number of smart actuators & Ch8,9\\
$N$ & Number of requests for scaling down periods & Ch6,7\\  
$n$ & Total number of tasks & Ch5,6,7\\
    & The number of data, or the number of smart sensors & Ch8,9\\
    & Integer & Ch10\\
$p$ & Period & Ch5,6,7\\
$Q_1$ & Queue to store one control packet & Ch9,10,11\\
$Q_2$ & First-in-first-out (FIFO) queue of past control packets & Ch9,10\\
{$R$} & {Set-point}& Ch3,4\\
$r$ & Set-point of the plant output & Ch1\\
{$r_1 \sim r_3$} & {Parameters for prediction of the controlled variable}& Ch3,4\\
S1 $\sim$ Sn & Smart sensors & Ch8,9\\
$s$ & Laplace transform operator & 6,7,10\\
{$T  $} & {Process time constant}& Ch3,4\\
			  & Task & Ch5,6,7\\
			  & Control period & Ch9,10,11\\
$T_C$ & Time instant to deal with control packet dropout & Ch9,11\\
$T_c$ & Control integral time & Ch6,7\\
$T_D$ & Time instant to dequeue $Q_1$ & Ch9,10,11\\
$T_E$ & Earliest time instant to receive control packet & Ch9\\
{$T_i$} & {Controller integral time (min)}& Ch3,4,10\\
$T_O$ & Time instant at which a control period commences & Ch9\\
$T_L$ & Latest time instant to accept control packet & Ch9,10\\
$T_p$ & Time constant for plant & Ch6,7,10\\
{$T_s$} & {Sampling period (min)}& Ch3,4\\
$T_t$ & Time series & Ch8\\
$t$ & Integer, $t=1, 2, \cdots, N$ & Ch8\\
    & Time variable & Ch10\\
$t_{ca}$ & Controller-to-actuator delay & Ch9\\
$t_{ctr}$ & Control computation time & Ch9\\
$t_j$ & \multicolumn{2}{l}{Sum of sensor-to-controller-to-actuator jitters \hfill Ch9}\\
$t_{sc}$ & Sensor-to-controller delay & Ch9\\
$U$ & CPU utilization & Ch5,6,7\\
$U^I$ & Workload of the subtask $T^I$ & Ch6,7\\
$U^{II}$ & workload of the subtask $T^{II}$ & Ch6,7\\
{$u$} & {Manipulated variable }& Ch1,3,4,10\\
			& Integer & Ch8\\
$\hat{u}$ & The estimate of the control signal $u$ & Ch10\\		
$u_d$ & The digitised form of $u$ & Ch1\\
$wrt$ & Worst response time & Ch5\\
{$y$} & {Controlled variable (e.g., stage 7 temperature)}& Ch1,3,4,6,7,10\\
{$\hat{y}$} & {$d$ steps ahead prediction of $y$}& Ch3,4\\
$\tilde{y}$ & Control error & Ch6,7\\
$y_m$& Measurement of the plant output $y$ & Ch1\\
$y_d$ & The digitised form of the measurement $y_m$ & Ch1\\
$y_r$ & Set-point of the controlled variable $y$ & Ch10\\
\\
\multicolumn{2}{l}{\textbf{Greek Letters}} & \\
%{$\alpha$} & {Design parameter in $S_2$} & Ch3,4\\
{$\beta_i$} & {Degree of fulfilment for the \textit{i}th rule}& Ch3,4\\
$\Delta_H$ & QoC upper bound & Ch6,7\\
$\Delta_L$ & Dead zone around $\delta\tilde{y}$. $\Delta_L < \Delta_H$ & Ch6,7\\
$\Delta y_j$ & Control error $(= y_r - y_j)$ & Ch10\\
{$\Delta \hat{y}$} & {$d\/$ steps ahead prediction of the $y\/$ deviation}& Ch3,4\\
$\delta\tilde{y}$ & One-step difference of $tilde{y}$ & Ch6,7\\
{$\epsilon$} & {Small and positive threshold in $S_2$}& Ch3,4\\
					   & Forgetting factor & Ch6,7\\
					   & Side length of a non-empty box & Ch8\\
{$\mu$} & {Membership function}& Ch3,4\\
        & A measure on interval $[0, 1]$ & Ch8\\
$\tau$ & Time delay & Ch6,7\\
       & Scaling exponent & Ch8\\
$\tau_c$ & \multicolumn{2}{l}{Sum of network delay and control computation delay \hfill Ch10}\\
$\tau_p$ & Process time delay & Ch10\\
{$\theta$} & {Process time delay (min)}& Ch3,4\\
\\
\multicolumn{2}{l}{\textbf{Superscripts}}\\
(i) & \multicolumn{2}{l}{The first-, second, or third-order derivative ($i=1, 2$, or $3$) \hfill Ch10}\\
$max$ & Maximum value or upper bound (for $p$, $p_i$ and $N$) & Ch6,7\\
$min$ & Minimum value or lower bound (for $p$ and $p_i$) & Ch6,7\\
\\
\multicolumn{3}{l}{\textbf{Subscripts}}\\
$c$ & Controller & Ch6,7\\
$i$ & \multicolumn{2}{l}{The first or sole subscript to some variables ($c$, $d$, $O$, $p$, $T$, $wrt$)}\\
    & ~~~~~~to indicate  the $i$th task & Ch5,6,7\\
$j$ & \multicolumn{2}{l}{The second subscript to some variables ($c$, $d$, $O$, $T$, $wrt$)}\\
    & ~~~~~~to indicate the $j$th subtask decomposed from a task & Ch5,6,7\\ 
 & Integers representing the $j$th control period & Ch10\\
$k$  & Integers representing the $k$th control period & Ch10\\
$p$ & Plant & Ch6,7\\
$rq$ & Requests (for $N$) & Ch6,7\\
$sp$ & Set-point for $U$ and $y$ & Ch6,7\\
\end{longtable}
}

%\end{nomenc}


==> scratch.tex <==


Introduction:
        
        % Experiments to answer this question are conducted with a simulated biped crossing obstacles such as gaps, hurdles, steps, and stairs, and with a large tracked robot required to pass through small gaps in a real world scenario.
        
        % Dynamic agent and obstacles.. 
        
        % For robots where dynamic stability is less of a concern, complex behaviours may emerge from situations where sensor information is limited. For these problems, the question extends to include behaviour design where coarse costmaps make planning through small passageways difficult. Can complex behaviours be learned, for example without the explicit ability to detect contact with the environment. Finally, learned behaviours can cause damage to hardware and the environment if trained on real platforms. We would verify that a method trained in simulation is compatible with an agent in the real world, and investigate any disparity in results. 
        

        % needed by an agent to traverse obstacles such as stairs, gaps, hurdles, jumps, and steps. 
         
        % Navigation through small gaps is a challenging problem. Standard navigation methods such as artificial potential fields (APF) [\cite{khatib_real-time_1986}], or path planners that perform grid search over an occupancy map [\cite{dolgov_path_2010}] struggle to traverse narrow spaces. Reactive methods fall into oscillatory behaviour when a local minima occurs between attractive and repulsive forces. Grid search methods that incorporate robot kinematics into path planning fail to generate a path when the robot footprint appears larger than the gap in the costmap. Methods to alleviate these pain points utilise higher resolution local sensors or computational expensive search algorithms. A human that is teleoperating a mobile robot may solve this problem by making contact with the gap. One such strategy is to angle one of the leading corners of the robot into the narrow space, then turning the robot while making contact with the wall in order to align with the gap. This method ensures the robot is as far against one surface as possible. Such a complex controller is difficult to hand design. In addition, the decision to activate a gaps behaviour must also occur autonomously, where the robot would employ a traditional path follow behaviour when it is not required to go through a narrow space. We will investigate how we can learn a behaviour for traversing a narrow gap, then learn when to activate this behaviour. Finally, learned behaviours can cause damage to hardware and the environment if trained on real platforms. We would verify that a method trained in simulation is compatible with an agent in the real world, and investigate any disparity in results.
 
        
        % We also hope to answer the question of can complex behaviours emerge without the ability to explicitly detect contact with the environment? For example a behaviour to wiggle through tight spaces.

        % Complex terrain obstacles such as stairs, gaps, hurdles, jumps, and steps require the robot to perceive the environment. Legged platforms typically plan for footstep placement and body pose when approaching an obstacle. There are many examples of learning controllers for autonomous agents that require perception. However, utilising expert knowledge as a way of providing insight to the learning agent has not been investigated well for high degree of freedom agents over difficult terrain. Curriculum learning (CL) has been shown to improve learning outcomes for a range of tasks, though has not yet been used efficiently for robot control over difficult terrain. 
        
    % \item How can complex visuo-motor locomotion behaviours be learned efficiently, without knowing exactly how an expert would perform the action?
    % - Titan    
    % - Biped curriculum learning
        
    % \item How can we reliably transition between behaviours? \\
    % \item How can a suitable switch location be determined to safely switch between behaviours?
    
    % This question is of particular importance for dynamic controllers where a stable switch point may not exist
    
    % Terrain conditions must be considered.
    
    % This ensures the current behaviour will guide the robot to a state within the RoA of the next controller, and allow for reliable switching. If no suitable overlap exists the robot will not be able to safely switch at any time. In the case where there is a narrow overlap, the  the robot may not have time in a perodic walk cycle to reach the RoA of the target controller
    
    % It is also possible that a complex obstacle prevents a 
    
    
    % However,if there is no state where an overlap occurs, the robot will be unable to safely switch to the target behaviour. Furthermore, complex obstacles may prevent the robot from reaching  goal set before switching is required, terrain conditions must be considered. The final research question explored in this thesis is how the robot can be controlled to prepare for an upcoming behaviour such that safe switching can occur. This question is of particular importance for dynamic controllers where a stable switch point may not exist.
    
    % and allows complex behaviours to be joined sequentially without explicit
    
 
    % \item How can we learn to autonomously traverse narrow gaps?
    
    %     Navigation through small gaps is a challenging problem. Standard navigation methods such as artificial potential fields (APF) [\cite{khatib_real-time_1986}], or path planners that perform grid search over an occupancy map [\cite{dolgov_path_2010}] struggle to traverse narrow spaces. Reactive methods fall into oscillatory behaviour when a local minima occurs between attractive and repulsive forces. Grid search methods that incorporate robot kinematics into path planning fail to generate a path when the robot footprint appears larger than the gap in the costmap. Methods to alleviate these pain points utilise higher resolution local sensors or computational expensive search algorithms. A human that is teleoperating a mobile robot may solve this problem by making contact with the gap. One such strategy is to angle one of the leading corners of the robot into the narrow space, then turning the robot while making contact with the wall in order to align with the gap. This method ensures the robot is as far against one surface as possible. Such a complex controller is difficult to hand design. In addition, the decision to activate a gaps behaviour must also occur autonomously, where the robot would employ a traditional path follow behaviour when it is not required to go through a narrow space. We will investigate how we can learn a behaviour for traversing a narrow gap, then learn when to activate this behaviour. Finally, learned behaviours can cause damage to hardware and the environment if trained on real platforms. We would verify that a method trained in simulation is compatible with an agent in the real world, and investigate any disparity in results.



    % \item What are some of the challenges of training behaviours in simulation for real world applications? \\
        
    %     While behaviours that are developed with DRL methods can perform impressive tasks, they require trial and error interaction with the environment. This exploration behaviour can be destructive to the robot and the environment. Many works look at how we can transfer behaviours trained in simulation to real world tasks. We are interested in learning about the challenges of incorporating a DRL behaviour into a pre-existing behaviour stack for use on a real platform. 
    
        % Learning controllers are good, but require trial and error interaction with the environment, at the motor control level. This means destruction of the robot and the world. Training in simulation allows the flexibility of behaviour design, however sim-to-real disparity limits the direct transfer of behaviours developed in simulation to the real robot. For mobile robots traversing complex terrains we need to know how effective they can be, and what are the sources of failure/improvements that need to be made.
    
        
        % particularly if the robot is highly dynamic.
        
        % Studies are also necessary to investigate methods for incorporating black box behaviours into a pre-existing behaviour stack, 
    
        % For scalable control suites to operate in open set conditions, where controllers can be added as they become available, multiple behaviours are required. However, selecting the correct behaviour to activate in a particular state requires care. For highly dynamic robots such as bipeds, switching to a behaviour at the wrong time can result in instability. Furthermore, for complex behaviours an overlap might not exist between the states that two behaviours operate safely within, meaning a stable switch point may not exist. Studies are also necessary to investigate methods for incorporating obstacle specific learned behaviours into a more broad, manually designed, behaviour stack. 
 
 

While behaviours that learn from experience have great potential for performing complex actions, DRL policies are typically a black box, with no indication of when the behaviour should or should not be used. For robots to replicate human capabilities, locomotion must be considered an open set problem. As such, a control suite needs to be modular, requiring many behaviours, with the ability to include or update any single behaviour without heavy retraining of the complete stack.

For dynamic robots such as bipeds, controllers cannot be switched unless the target controller can accommodate the current state of the robot. Ensuring the the robot is in an suitable state, or transitioning to a suitable state, must occur before switching to an adjacent controller. For robots that have integration with other types of controllers (for example a combination of manually designed, and learned controllers), it is also important to switch at appropriate times to allow controllers time to perform their designated task.


% =========================================

As robots become increasingly ubiquitous they are required to operate over an ever increasing range of terrain conditions. In lieu of a single monolithic controller, separate behaviours can be designed to traverse difficult obstacles. A design paradigm that utilises separate behaviours draws benefit from expert knowledge and allows for controller development (for example in robots that require harnesses and support). 


Learning locomotion behaviours for traversing difficulty obstacles. 

Our work looks at how we can design locomotion behaviours using reinforcement learning

Break the world into pieces -> behaviour per section, 


\textbf{Illustration of papers / story!!}



Difficult obstacles require perception, 


Mobile robots that have their center of gravity within the support of the ground contact throughout locomotion are considered to be statically stable. Examples of static mobile robots include most wheeled and tracked platforms, and some legged robots that are typically slower moving with a limited range of motion. Robots that are not always in balance, where the center of gravity leaves the support for part of locomotion, are considered dynamic. Dynamic walking requires the robot to undergo a periods of controlled falling throughout its step cycle. Through this falling period, the robot does not have control authority over the contact with the ground, as such is considered underactuated~\cite{http://underactuated.mit.edu/intro.html}. Common examples of dynamic platforms include legged robots such as bipeds. Dynamic walking is found very abundantly in nature~\cite{https://en.wikibooks.org/wiki/Robotics/Types_of_Robots/Walkers#Dynamic_v._Static}.

Underactated: when the robot does not have enough controllable degrees of freedom compared to degrees of freedom it can move.



Reasons we love PPO - on-policy: good for curriculum / when the mdp changes, still widely used for legged robots / navigation robots, simplicity: especially when training many separate policies.


why do I care about this thesis? What are you trying to do, and why.

To operate in humancentric environments, general purpose robots must be able to perform a many tasks. To perform many tasks, they must have many controllers. To operate in humancentric environments, legged robots have several advantages to other types of robots (


Legged robots will have a great role to play as we develop general purpose robots to operate in humancentric environments.

A general purpose platform must be modular, as there is no way to know a priori every condition the robot must operate. Legged platforms are often dynamic, requiring constant control input. For a modular control suite for a dynamic robot, we must be able to seamlessly select and transition between controllers without compromising dynamic stability. 

Deep reinforcement learning is an appealing control method for platforms that rely on perception input, however DRL policies typically behave as a black-box, providing little insight into stability or admissibility.

Where is DRL for legged/dynamic robots at, what is missing from what we need. What do we need?


Why will legged robots have a great role to play? Define humancentric. Dynamic, vs static, vs quasidynamic

Main points:
Dynamic robots - important for general purpose robots i.e. legged robots.
Deep reinforcement learning - important alternative to to manually designing controllers 
- because we want to develop lots of controllers
- because controllers are complex
- because we need perception integrated with the control
General purpose robots
Modular control suite - must be able to add to the control suite without retraining low level controllers
- We don't want to retrain low level controllers because often they require fine tuning in constrained conditions (harnesses and treadmill)
- And because we hope we can scale to many controllers, want to be able to 'plug and play' with new controllers.

% Motivation -----------------------------
Designing a controller for a dynamic legged robot is a difficult task. Robust control over a variety of terrain types 



% Each of these questions has progress from the development of individual behaviours, to how can behaviours be used together, and finally what are the challenges of developing behaviours in simulation for deployment on a real agent.


% Included is the motivation for each question, some of the expected challenges, and sub-questions that aim to answer underlying elements of each problem.

% Learning Behaviours 
%     Guided curriculum learning, \cite{tidd_guided_2020}
    
%     Passing through gaps \cite{tidd_passing_2021}

% Transitioning between Behaviours:
%     Learning when to switch \cite{tidd_learning_2021}

%     Setup policies for switching \cite{tidd_learning_2021-1}

%     Passing through gaps \cite{tidd_passing_2021}

% Obstacle detection
%     Passing through gaps \cite{tidd_passing_2021}

%     Spot the stairs %\cite{tidd_spot_2021}


  
        % The disparity from policies trained in simulation and applied to the real world is an active area of research, particularly where perception is a vital component.
        
        % For high degree of freedom dynamic legged robots, traversing complex obstacles is a difficult control problem. While there are many examples of learning for traversing various terrains, utilising expert knowledge about the task can reduce the complexity. Curriculum learning (CL) can    
        
        % Embedding Prior controller terrains learning behaviours for traversing complex obstacles
        % with minimal priors, learn to traverse complex terrain obstacles with a dynamic robot such as a biped. 
        
        % However, studies are necessary..
        
        % Techniques such as Curriculum Learning (CL) have been unde
        
        % \begin{itemize}
        %     \item How can we utilise expert knowledge to improve learning outcomes for mobile robots traversing difficult obstacles?
        % \end{itemize}
        
        % Expert controllers, expert knowledge in reward design (following expert controller, and heading towards expert markers), curriculum learning. 
        
        % \begin{itemize}
        %     \item What are some of the simulation to real disparities?
        % \end{itemize}
        
        % A common pitfall of learning methods is they require large amounts of training, where training requires online interactions with the robot acting in the world. It is often practical to learn behaviours in simulation where there is no risk of damage to hardware or the environment as policies explore the action space of the robot. 
        
            
    
    % \item How can we detect upcoming obstacles? \\
        
    %     Terrain detection is an important component of creating a modular control suite. Understanding 
    
        % \begin{itemize}
        %     \item How can reinforcement learning be used to detect upcoming terrain obstacles?
        % \end{itemize}
        
        % \begin{itemize}
        %     \item How can we use terrain detection as part of a much wider autonomy stack?
        % \end{itemize}
    
    
    
        % The choice of perception depends on many factors, including what is available to the robot. 
        % \begin{itemize}
        %     \item What forms of perception are available to mobile robots that can be utilised by a behaviour learning system? 
        % \end{itemize}
        
        % Common perception modalities include a depth map from a body mounted camera, an occupancy map generated using simultaneous localisation and mapping (SLAM) from a Velodyne LiDAR, and surfel (3D locations of laser points on a surface) points relative to the robot. While classical search methods are limited to occupancy maps, learning approaches can couple salient information from perception and the controller.
        
%     \item How can we identify when we do not have a controller available for a given terrain scenario? \\
    
%     All terrain conditions may not be available while behaviours are developed. Robots that must operate in open world conditions will encounter obstacles it does not have a behaviour to traverse. For each behaviour, the robot must learn when it should activate the behaviour, even when obstacles  Furthermore, when no suitable behaviour exists for an upcoming obstacle, the robot must act safely.
    
%   \begin{itemize}
%         \item How can we learn which behaviour to use without experiencing training data from all obstacles?
%     \end{itemize}
   
%     \begin{itemize}
%         \item Can we operate safely when the robot encounters obstacles it does not have a controller for?
%     \end{itemize}
    
            % \begin{itemize}
        %     \item How can we learn when we can safely switch between policies?
        %     % \item Assuming there exists a region of attraction overlap between policies.
        % \end{itemize}
   
        % \begin{itemize}
        %     \item How can we learn to bridge the trajectories from one policy to another to allow a dynamic robot to transition between behaviours?
        %     % \item Given that we have small or no overlap between adjacent policies.
        % \end{itemize}
        
        % \begin{itemize}
        %     \item How can we integrate a learned behaviour with a classical navigation control stack?
        % \end{itemize}
        




\chapter[Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts]{Learning When to Switch: Composing Controllers to Traverse a Sequence of Terrain Artifacts}
\label{cha:ch4}


% Motivation/contribution/abstract -----------------------
Armed with a set of policies, we now need a way to combine them. The idea of combining controllers to move through a state and accomplish a task is a well studied problem in control literature. Here we will introduce the idea of a region of attraction of a controller.

We first define the concept of a goal set. This is a set of states that a controller is designed to operate. For some controllers, like an inverted pendulum, the goal set is a single point, i.e. when the pendulum is 0 degrees from the upright position. For periodic controllers, such as those used for walking the goal set is every state a system visits as it executes a walking command. 

The region of attraction is any state where the system will converge to the goal set using a given controller. Like the goal set, the region of attraction is a set of states. The goal set is included in the region of attraction. If we start our walking robot in any arbitrary state and execute a walking command, if over time the robot walks, then every state from the initial state is in the region of attraction of the walking controller. the region of attraction is a Boolean set, either the state is in the region of attraction or the system will diverge.

Provided the goal set, and the region of attraction of a set of controllers, it is possible to 
use this information to move through the state by selecting the appropriate controllers to guide the robot to a desire goal. The notion of using several controllers to move from one goal state to another is known as sequential composition. Sequential composition is famously depicted as a set of funnels, guiding an agent to the centre of each funnel to the outer portion of funnel representing the next controller.

Sequential composition:
Start in a state.
Select a controller of which the state lies in its region of attraction, with a goal set in the region of attraction of the next controller. 
repeat until goal set.

In this section we consider the region of attraction for our reinforcement learning policies from the previous section. It is now that we highlight that we have been discussing the state of the system. For a complex dynamic biped, the state includes environment configurations as well as configurations of the robot. Thus we highlight that the region of attraction of a visuomotor policy depends not only on the proprioceptive state of the robot, but also where it is relative to artifacts that it will interact with in upcoming steps. It is difficult to quantify a goal set for a reinforcement learning policy for a high dimensional robot, it is much more difficult when we consider a policy that has been trained to overcome steps of random size.

Notation explanation:
% \begin{equation} <x>_{n}=\frac{1}{n}\sum_{i=1}^{n}x_i \end{equation}
Deterministic discrete time dynamics system
\begin{equation} 
    \bold{x}_{t+1} = f(\bold{x}_t, \bold{u}_t ) = h(\bold{x}_t, \bold{u}_t ) + g(\bold{x}_t, \bold{u}_t ), 
\end{equation}

$\bold{x} \in \mathcal{X} \subset \mathbb{R}^q$, $\bold{u} \in \mathcal{U} \subset \mathbb{R}^p$, $f : \mathcal{X} \times \mathcal{U} \xrightarrow{} \mathcal{X}$

Lipschitz continuous: 
If your function is differentiable, Lipschitz continuity just says that the function has bounded derivative. I think of this as a "wiggling" and "stretching" bound.https://math.stackexchange.com/questions/2374289/understanding-lipschitz-continuity
If the constant M<1, a function is said to be a contraction which has many nice properties as well.
It's just a bound on the derivative, the function can't change too rapidly, the minimum bound is the Lipshictz constant.
$https://en.wikipedia.org/wiki/Lipschitz_continuity$
\begin{equation} 
    d_Y(f(x_1),f(x_2))\leq Kd_X(x_1,x_2) \text{ and } |f(x_1) - f(x_2)| \leq K|x_1-x_2|
\end{equation}

Level set: When you set a function to a constant, i.e. a contour map with a constant height for each line.

\begin{equation}
    v : X → R ≥0 with v(0) = 0 and v(x) > 0 for all x ∈ X \ {0}.
\end{equation}

Lyapunov functions $v(\bold{x_t})$:
we require a tool to determine whether individual states and actions are safe, In control theory, this safety is defined through the region of attraction, which can be computed for a fixed policy using Lyapunov functions [4].
Lyapunov functions are continuously differentiable functions
In our experiments, we exploit the fact that value functions in
RL are Lyapunov functions if the costs are strictly positive away from the origin.~\cite{berkenkamp_safe_2017}
v(x) = r(x, π(x)) + v(f (x, π(x)) ≤ v(f (x, π(x)))

in a discontinuous system even a slight change in the control policy can lead to drastically
different behavior~\cite{berkenkamp_safe_2017}

% \mathcal{H}
Discrete MDP "All these methods require an accurate probabilistic model of the system." ~\cite{berkenkamp_safe_2017}

There is work in this space with learning based controllers. Though it is difficult to define a goal set for a complex controller, where 

Terms:
agent, system, robot
policy, controller, control policy, behaviour
state vs observation
visuomotor


Most hierarchical methods rely on learning the primitive policies either concurrently ~\cite{} or 


Selection criteria:
\begin{itemize}
    \item Of the admissible policies, which is likely to give the best reward on the current task?
\end{itemize}

Which means we have a task (i.e go forward, stop, jump? etc), and a list of policies. The first step is to know if a policy will work. If it will, what is the task it is trained for, is it the best available policy to do the task.
    
We are going to do 2 things: learning to add lots of policies together. We are going to compare with training a dqn.

Task policies. Transition policies. Recovery policies.

Policy list:
\begin{itemize}
    \item stairs
    \item No velocity
    \item walk
    \item run
    \item slow turn
    \item walk turn
    \item run turn
    \item jump
\end{itemize}

\section{Introduction}
\section{Related Work}
\section{Background}
\section{Method}
\section{Results}
\section{Discussion}
